OneQ: A Compilation Framework for Photonic One-Way Quantum Computation

In this paper, we propose OneQ, the first optimizing compilation framework for one-way quantum computation towards realistic photonic quantum architectures. Unlike previous compilation efforts for solid-state qubit technologies, our innovative framework addresses a unique set of challenges in photonic quantum computing. Specifically, this includes the dynamic generation of qubits over time, the need to perform all computation through measurements instead of relying on 1-qubit and 2-qubit gates, and the fact that photons are instantaneously destroyed after measurements. As pioneers in this field, we demonstrate the vast optimization potential of photonic one-way quantum computing, showcasing the remarkable ability of OneQ to reduce computing resource requirements by orders of magnitude.

==> 02_introduction0724.tex <==
\section{Introduction}

Quantum computing (QC) is promising in its potential of providing significant speedup to many problems, such as large-number
factorization with an exponential speedup \cite{shor1999polynomial} and unordered
database search with a quadratic speedup\cite{grover1996fast}. From the hardware side, a list of computing technologies have achieved promising progresses toward physical
realization at both research lab settings and industrial production levels, including superconducting~\cite{}, ion trap~\cite{}, neutral atoms~\cite{}, and photonics~\cite{}. There is not yet a clear winner and it is anticipated that multiple technologies will develop together and serve different mission needs and application requirements. 

Computer scientists, especially experts from the field of high-performance computer architecture and compiler have been actively participated in the development of both software and architecture support for quantum computing~\cite{}, leading to a great open-source field for exploiting and pushing the development of quantum hardware towards practical usage. Yet, most of the efforts are focusing on the superconducting technologies, with a few on ion trap and neutral atoms


PsiQuantum~\cite{} announces world’s first manufacturing milestone in photonic quantum computing: Quantum photonic and electronic chips being manufactured using the advanced semiconductor tools.

Among various quantum hardware technologies\cite{hareware1,hardware2,hardware3,hardware4}, photonic quantum computing can potentially stand out for its unique features. First, it can potentially work in an atmospheric environment at room temperature due to their weaker decoherence, in comparison with other systems whose fragile quantum states have to be maintained in vacuum or extremely low temperature[?]. Second, it can be easily integrated with quantum communication, considering the wide use of photonic approaches in quantum communication~\cite{OBrien2009,Bogdanov:17}\HS{perhaps these two refs cover both aspects room temp and distributed computing}. 

Along with those unique advantages come intrinsic challenges of implementation in traditional circuit based model. First, photons are flying qubits 
and applying quantum gates on them
requires sending them through some optical devices. 
This requirement implies that a direct implementation of quantum circuits for photons involves design and fabrication of a chip with a specific (non-reconfigurable) pattern of optical devices for every given circuit. Such a process is clearly not scalable, since we need a new chip for every computation task.
\textcolor{orange}{@Hassan: Why is sending them through optical devices a challenge?}
% Second, the weak interaction between photons make it difficult to implement arbitrary entangling gates. %Second, phonotic quantum computers rely on hardware reconfiguration to implement different circuits[?], which compromises their programmability and results in overhead.
\HS{How about now?}
Second, measurements on photons are destructive, which means that the photons will vanish once they are measured and new qubits need to be generated to replace them.  \textcolor{orange}{Great to mention the non-reconfigurable circuits. But not clear about what it has to do with the above challenges.} Fortunately, these challenges can be overcome in a one-way quantum computing scheme, a different computation model from the circuit model. %\textcolor{yellow}{and continuous variable?}
This scheme is particularly designed for systems where reconfigurable single-qubit gates are available as opposed to two-qubit gates.
In the one-way approach, an entangled resource state (the so-called graph state or cluster state) is prepared using a fixed pattern of devices necessary to generate two-qubit entangling gates and then
various tasks can be performed by a series of single-qubit projective measurements on the resource state. In photonic systems, single-qubit measurements in arbitrary bases can be implemented on a single \emph{universal} chip
by combining reconfigurable single-qubit gates and photon detectors. %called cluster state
Furthermore, during the computation in the one-way approach, each qubit is measured only once, which is why it is called "one-way" model, and is then free to detach from the computing system or even disappear. This low depth of operation on each qubit reduces the requirement for coherence time.
\textcolor{orange}{@Hassan: Please add to either this or next paragraph some explanation about the difference between doing entangled gates in photonics and generating entanglements for computation to avoid confusion, i.e. why is doing entangled gates hard but generating entangled states easier?}\HS{I made some changes. Let me know if it is unclear. I also rewrote the next paragraph.}


% One-way quantum computing, also known as measurement based quantum computing (MBQC)~\cite{} is a more favorable computational model for photonic QC than the circuit model~\cite{} because it eliminates the requirements of implementing entangled gates which are hard for photonic QC due to the weak interaction between photons, and is compatible with the destructive manner~ \cite{} that photons disappear after measurements. \todo{turn this into several sentences, with each sentence focusing on only one key point.}

Large-scale one-way quantum computing requires a large entangled state to be prepared as a resource. This is a challenging task because weak interaction between photons makes it difficult to entangle them. There are two approaches to entangle photonic qubits. One way is to use linear optical devices and photon detectors to realize quantum gates \emph{probabilistically}. The other way is to send photons through nonlinear optical devices which induce interactions between photons and effectively lead to a \emph{deterministic} quantum gate. Both approaches have their benefits and shortcomings. First approach is readily CMOS compatible and easy to scale; however, it is not deterministic and implies a large overhead if we require a near unity success probability.
The second approach solves the finite success probability issue by being deterministic; nevertheless, such nonlinear systems are difficult to scale.
% to generate (due to weak interaction between photons) and maintain (due to photon loss). 
% \todo{a logic gap between the entangle gate in previous paragraph and the entangle state here. You shall be more accurate about what you want to say here} 
Therefore, it is more realistic to take advantages of both methods and reduce their shortcomings by combining them in the following way: A bunch of small entangled states can be generated (almost) deterministically at first and then can be \emph{fused} to construct a large static entangled state. %in a separate stage of generating all the entanglements before the stage of computation.
\todo{not even clear why we need a more promising methods. It is important to thoroughly elaborate the challenges and the drawbacks of existing methods before even talking about your solution} \todo{one or even several paragraph(s) here about the drawbacks of existing methods. Your setting or the problem you want to solve is more important than your solution for  writing the introduction section. Each of your proposed methods shall have a corresponding challenge here. This part shall be understandable even to a outsider.} 

In this paper, we envision a fusion-based implementation of the one-way model, where we develop a compiler for generating on-demand graph states by fusing the output of an array of small-resource-state generators...\HS{I added this (optional) opening... I think we should start with the general and setup and then go into details}


We foresee a more promising solution by incorporating dynamism, i.e. generating a dynamic structure of entanglements, and coarse-grained pipelining, i.e. consuming the entanglements while more are being produced, so that we can accommodate input adaptivity and hide latency. However, those capabilities are not low hanging fruits, but with the following obstacles.
First, a scheme of simultaneous consumer and producer requires careful analysis of dependency among operations, including the dependency emerging from the pattern of measurements as well as a type of dependency we recognize that is induced by the fusion operation. Second, the simple fixed structure in the small entangled states limits the degree of each qubit, and hence prevents a direct synthesis of the high-degree vertices in the graph that represents the measurement pattern. Third, a real-world compiler also needs to take into account the limitations of hardware, eg. constraints on temporal and spatial connectivity between the small entangled states.

We propose the first compilation framework for a dynamic pipelining one-way QC by overcoming the above challenges in three phases: dynamic scheduling, adaptive synthesis and planarized mapping. 

\textit{Dynamic scheduling} outputs a set of executable qubits in each round, with each qubit assigned a choice of operation from measurement, synthesis, and refresh. The insight is that not all dependency blocks the measurements, with some only affecting the interpretation of the measurement outcomes. Meanwhile, we recognize a new type of dependency induced by fusion operations which motivates an lookahead synthesis of the qubits to be executed next round. Moreover, the possible long wait resulting from the dependency block requires a mechanism of refreshing qubits when its lifetime approaches to the limit. 

\textit{Adaptive synthesis} gives a fusion scheme between small entangled states to generate all entanglements required by the scheduled commands of the input program. The insight is that a large-degree qubit can be synthesized by a proper pattern of fusion between low-degree qubits. By matching the graph representation of the input program with some basic fusion patterns, an arbitrary entanglement structure can be synthesized to accommodate the input adaptivity.

\textit{Planar mapping} finds a layout of the small entangled states on a layer of available hardware resource per clock cycle to enable the fusion scheme under the hardware constraints. The insight is that fusion operations between non-connective small entangled states on the hardware can be achieved by a path through connected ones. But each small entangled states can be used by one (or few) paths due to the size limit of the small entangled states, which requires a planar embedding for those paths with an optimization on the total length.



Our contributions in this paper are summarized as follows:
\begin{itemize}
    \item We enable a coarse-grained pipelining compilation with the entanglements consumed as more are being produced by deriving the rules of scheduling the commands.
    \item We enable a dynamic compilation that accommodates the adaptivity of input programs by synthesize the entanglement structure according to the measurement pattern.
    \item We enable a realistic implementation of one-way quantum computing by mapping the computational resource onto hardware under reasonable constraints.
    
    % \item We systematically formulate the problem of compiling a program under the scheme of one-way quantum computing to operations on resource states of a small size of entanglement.
    % \item We propose the first adaptive framework that synthesis graph state according to the given program, addressing the aforementioned challenges in its three stages.
    % \item Our evaluation demonstrates ...
\end{itemize}

We evaluated our framework by comparing it with a baseline that generates a static large entangled state before the computation. The results show that...


==> 03_background.tex <==
\vspace{0.3em}
\section{Background and Related Work}\label{sect:background}
We start with the necessary background about measurement-base quantum computing (MBQC) paradigm.
The basic quantum computing concepts and the circuit model are not covered, we recommend~\cite{nielsen2002quantum} for more details.

\vspace{0.3em}

\subsection{Programming Paradigm of MBQC}
MBQC is a universal but conceptually distinct computational model from the circuit model. In this model, computation is driven by a pattern of single-qubit projective measurements on an initialized entangled state as a resource.

\vspace{0.3em}
\subsubsection{MBQC Basics}
The computing resource in the MBQC model is a specific form of entangled states called the \emph{graph state}, which is a pure quantum state of qubits located on a graph $G=(V,E)$, formally defined as the eigenstates of operator\[s=X_i \bigotimes_{j\in n_i} Z_j, \quad\forall i\in V\] where $n_i$ stands for the set of qubits on the neighboring vertices of qubit $i\in V$. It can be generated by preparing all qubits in $\ket{+}$ and applying a CZ gate on each pair of qubits connected by an edge $e\in E$.

On this graph state, \emph{equatorial measurements} $E(\alpha)$, i.e., measurements in the bases on the equatorial plane of Bloch sphere at an angle $\alpha$, are applied to drive the computation. Due to the non-determinism of quantum measurement, Pauli X- or Z-corrections may be applied to the unmeasured qubits depending on the outcomes of the measured qubits.
% dependent X- or Z-corrections to remaining qubits are needed after measurement outcomes are obtained. 
During the implementation, those corrections can be postponed to the end of the computation by allowing \emph{adaptive measurements}, i.e., by changing the measurement bases of the following qubits according to the previous measurement outcomes.
% measurements whose bases are dependent on outcomes of previous measurements. 
In particular, an $X^s Z^t$-correction where $s,t\in\{0,1\}$ on a qubit $i$ can be postponed by adjusting its measurement angle from $\alpha$ to $(-1)^s\alpha+t\pi$ because $E(\alpha)X^s Z^t = E((-1)^s\alpha+t\pi)$. These adaptive measurements induce a \emph{measurement dependency}, with the dependencies in $s$ and $t$ called X- and Z-dependency respectively. The graph state geometry and the adaptive measurements are together called a \emph{measurement pattern}.

% the angle $\alpha$ of an equatorial measurement on an $X^s Z^t$-corrected qubit $i$ should be adjusted to $(-1)^s\alpha+t\pi$ because $E_i(\alpha)X^s Z^t = E_i((-1)^s\alpha+t\pi)$, where $s$ and $t$ are called X- and Z-dependency respectively. The graph state geometry and the adaptive measurements together form a \emph{measurement pattern}.

% Different quantum programs require different geometries of graph states and lead to different measurement patterns.
There is a direct translation from a circuit in the universal gate set $\{J(\alpha), \mathrm{CZ}\}$ into a measurement pattern, because a measurement $E(\alpha)$ yielding a value $m$ is equivalent to a $J(\alpha)$ operator followed by a Z-measurement $M_z$ yielding the same value, i.e., $E(\alpha)\ket{\psi}=m$~corresponds to $M_z J(\alpha)\ket{\psi}=m$ where $m=0$ or 1 and
\begin{align}
J(\alpha)=
\begin{bmatrix}
1 & \mathrm{e}^{\mathrm{i} \alpha}\\
1 & -\mathrm{e}^{\mathrm{i} \alpha}
\end{bmatrix}   
\end{align}
% An arbitrary single-qubit gate $U$ can be decomposed into $U = \mathrm{e}^{\mathrm{i} \theta} J(\alpha)J(\beta)J(\gamma)$.
We refer to \cite{translation} for the concrete algorithm and hereby only demonstrate it with an example (Figure~\ref{fig:circuit_translation}(a) to Figure~\ref{fig:circuit_translation}(b)).
% Here we demonstrate the translation with an example (Figure~\ref{fig:circuit_translation}(a) to Figure~\ref{fig:circuit_translation}(b)) and refer to \cite{translation} for the concrete algorithm.
In Figure~\ref{fig:circuit_translation},
node $a$ in ~\ref{fig:circuit_translation}(b) corresponds to qubit A in~\ref{fig:circuit_translation}(a).
It connects to three nodes as there are three $\rm CZ$ gates connecting qubit A to qubit B, C, and D respectively. Single-qubit J gates on qubit B are represented by nodes $b_1,b_2,b_3$ (similarly for qubit C and D).
There would be a measurement dependency when the $J$ gates are non-Clifford and we use directed edges to represent it.
For example, the edge $b_1\rightarrow b_2$ indicates that the measurement basis of $b_2$ may need to be adjusted according to the measurement outcome of $b_1$.

\begin{figure}[h!]
    \centering
     \vspace{-5pt}
    \includegraphics[width=0.9\linewidth]{fig/translation.pdf}\\
    \hspace{0pt}(a)\hspace{100pt}(b)
    % \vspace{-15pt}
    \caption{Translation from a circuit (a) to a graph state (b), with the measurement bases labeled on qubits. Logical qubit $A$ corresponds to physical qubit
    $a$ and $B,C,D$ correspond to  $\left\{b_1,b_2,b_3\right\}, \left\{c_1,c_2,c_3\right\}$ and $\left\{d_1,d_2,d_3\right\}$. Qubits in (b) with `in',`out' or `in/out' are input or output qubits. Arrows on edges indicate the dependency between qubit measurements.}
    \vspace{-5pt}
    \label{fig:circuit_translation}
\end{figure}

\vspace{0.3em}
\subsubsection{MBQC Interpreter}
It is not yet known how we can efficiently compile a graph state measurement pattern onto a practical MBQC machine that generates small resource states with a set of hardware constraints. Previous work on gate implementation on the \emph{cluster state}, i.e. graph state in lattice geometry, can provide a basic interpreter. Although it is far from an efficient compiler, we give a brief introduction to it since it is used as the baseline in our evaluation.

An arbitrary single-qubit gate can be implemented by single-qubit measurements on a line of qubits in the cluster state.
% A single-qubit measurement along arbitrary basis can be implemented by a single-qubit gate and a normal Z basis measurement Figure~\ref{} 
% For example, in Figure~\ref{fig:circuit_simulation}, the xx gate on qubit xx is implemented by 
For example, the Hadamard gate and the $R(\xi,\eta,\zeta)$ gate in Figure~\ref{fig:circuit_simulation}(a) can be implemented by measurement patterns in the red circles of Figure~\ref{fig:circuit_simulation}(b), where the $X,Y$ labels stand for X-, Y-basis respectively, and $\xi,\eta,\zeta$ stand for the angles of general equatorial measurements.
% measurement bases on the $xy$ plane of the Bloch sphere.
Two-qubit gates can also be implemented by single-qubit measurements on the cluster state.
For example, the CNOT gates in Figure~\ref{fig:circuit_simulation}(a) are implemented by the measurement patterns in the green circles of Figure~\ref{fig:circuit_simulation}(b), with the two connected strips of physical qubits in the cluster state corresponding to the two logical qubits in the circuit. 
Measurement bases except X, Y and Z are adaptive to the outcomes of previous measurements (e.g., from $\xi$ to $-\xi$) and thus can induce dependency. But those adaptive measurements only arise in the measurement patterns of non-Clifford gates. Namely, all Clifford gates can be conducted simultaneously on the cluster state even if they are dependent in the circuit model.
For more details about measurement patterns of different gates, please refer to \cite{mbqc2009}.

\begin{figure}[h!]
    \centering
    \vspace{-5pt}
    \includegraphics[width=\linewidth]{fig/circuit_simulation_colored.pdf}\\
    \hspace{-50pt}(a) \hspace{120pt} (b) 
    \caption{From a circuit (a) to a MBQC measurement pattern (b), with the measurement bases labeled on qubits. Patterns in red correspond to single qubit gates, patterns in green correspond to CNOT gates. Two adjacent X-measurements can play the role of a wire as marked in yellow. Shaded qubits are removed by Z-measurements.}
    \vspace{-5pt}
    \label{fig:circuit_simulation}
\end{figure}



A naive interpreter from the circuit model to MBQC can be constructed by simply joining the inputs and outputs of those measurement patterns according to the gates in the circuit, as shown in Figure~\ref{fig:circuit_simulation}. Those measurement patterns can be aligned up by inserting identity gates implemented by two adjacent X-measurements, as shown by the yellow wires in Figure~\ref{fig:circuit_simulation}(b). The qubits not used by measurement patterns of any gates are redundant to the computation, and can be removed by measurements in Z-basis (shaded qubits in Figure~\ref{fig:circuit_simulation}(b)).
% Redundant qubits (shaded qubits in Figure~\ref{fig:circuit_simulation}(b)) can be removed by measurements in Z-basis. 
Similar to the circuit compilation~\cite{sabre}, CNOT gates on non-neighboring qubit strips can be implemented by inserting measurement patterns of SWAP gates whenever necessary. In this way, we can implement any quantum circuit in an MBQC manner, thus it serves as a basic MBQC interpreter and is regarded as the baseline in our evaluation.
This interpreter greatly simplifies the mapping from qubits and gates in the cirucit to the measurements on the cluster state. However, it is inefficient in the utilization of computing resources. Specifically, it makes many qubits redundant for computation and consumes their entanglements trivially by Z-measurements, without any regard for the huge overhead of generating those redundant entanglements on a practical MBQC machine.
% . Moreover, the generation of those redundant entanglements on practical MBQC machines would incur a huge overhead.

% many redundant entanglements are created and then consumed trivially by Z-measurements.

% This approach simplifies the mapping from the qubits and gates in the circuit to the measurement operations on cluster state while it comes with great overhead when deploying the cluster state onto a realistic MBQC device. Many redundant entanglements are created and then consumed trivially by Z-measurements (shaded qubits in Figure~\ref{fig:circuit_simulation}(b)). The two-qubit gates can be implemented on two adjacently logical qubit strips easily but are much more expensive when applied on logical qubit strips that not adjacent. Moreover, on a realistic MBQC device like a photonics quantum computer introduced later in this section, the hardware only generates small sparse cluster states.

\vspace{0.3em}
\subsection{MBQC on Photonic Platforms}
Photonic quantum computing is highly scalable with its ability to constantly generate a large number of photons. Moreover, it does not require an extremely low temperature compared with other quantum hardware technologies\cite{hareware1,hardware2,hardware3}. These advantages make it a promising candidate among various platforms for quantum computing. Here we give a brief introduction to photonic quantum devices and their support for MBQC paradigm.

% the qubit of choice is usually taken to be a single photon that has the choice of two different modes. This is called a dual-rail qubit.When the two modes represent the internal polarization degree of freedom of the photon, we speak of a polarization qubit.

In photonic quantum computing, a qubit is usually implemented by representing the two basis states $\ket{0}_L$ and $\ket{1}_L$ with two optical modes of a single photon. The optical modes can be either two spatial modes ($\ket{0}_L = \ket{1} \otimes \ket{0}$ and $\ket{1}_L = \ket{0} \otimes \ket{1}$, where $\ket{0}$ and $\ket{1}$ are the two basis states of a spatial mode), referred as `dual-rail qubits', or two polarization modes ($\ket{0}_L = \ket{H}$ and $\ket{1}_L = \ket{V}$, where $\ket{H}$ and $\ket{V}$ represent the horizontal and vertical polarization of the photon), referred to as `polarization qubits'. 
These two representations are mathematically equivalent and can be physically switched to each other using polarizing beam
splitters~\cite{photonics_review}. 

Large-scale MBQC requires the generation of large-scale entanglements between photonic qubits. On practical hardware, this is scaled up by generating small-size resource states and cascading them via fusion~\cite{GHZcluster, photonics_review}.
% With a practical hardware capable of generating small-size resource states, this can be made scalable via fusion~\cite{GHZcluster, photonics_review}. 
Fusion is a native operation in linear optics that projects two-qubit states to an entangled state through joint measurements on the two qubits (e.g., joint measurements in XX- and ZZ-basis is a projection to the Bell basis). If not otherwise specified, the joint measurements we use in this paper are in XZ- and ZX-basis, which merge two graph states to another graph state. As depicted in Figure~\ref{fig:fusion_XZ_ZX}, the 3-qubit graph states $ABC$ and $DEF$ can be merged into a 4-qubit graph state $ABEF$ via a fusion on qubits $C$ and $D$. The cost of each fusion is losing the two measured photons (qubit $C$ and $D$ in Fig.~\ref{fig:fusion_XZ_ZX}), so in general the fusion between an $m$-qubit graph state and an n-qubit graph state generates an $(m+n-2)$-qubit graph state, which is larger than the original ones when $m,n>2$.

\begin{figure}[h!]
    \centering
    \vspace{-5pt}
    \includegraphics[width=0.8\linewidth]{fig/three_qubit_fusion.pdf}
    \caption{A fusion between graph states $ABC$ and $DEF$. After the fusion between $C$ and $D$, qubit $C$ and $D$ vanish while qubit $A,B,C$ and $D$ form a new graph state.}
    % \vspace{-5pt}
    \label{fig:fusion_XZ_ZX}
\end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\linewidth]{fig/fusion_XZ_ZX.pdf}
%     % \vspace{-5pt}
%     \caption{A fusion between graph states $AC$ and $BD$. After the fusion (joint XZ-,ZX-measurements on $C$ and $D$), qubit $C$ and $D$ vanish while qubit $A$ and $B$ form a new graph state.}
%     \vspace{-5pt}
%     \label{fig:fusion_XZ_ZX}
% \end{figure}

Despite its facilitation to scalability, fusions bring an overhead of losing two qubits each time, and are the lowest-fidelity operations in the computation. Therefore, one of the goals of our compiler is to minimize the number of fusions, similar to the goal of minimizing the number of CNOT gates for compilers in the circuit model. Under this goal, it is inefficient to generate a cluster state in which lots of entanglements are redundant. Hence our compiler makes a choice of starting from the more general graph state representation, which only contains the necessary entanglement structure derived from the input circuit.



==> 03_background_0731.tex <==
\section{Background and Related Work}
We start with the necessary background about measure-base quantum computing (MBQC) paradigm.
The basic quantum computing concepts (e.g., qubit, gate, linear operator, circuit) are not covered and we recommend~\cite{nielsen2010quantum} for more details.
\newline


\subsection{Programming Paradigm and Compilation in MBQC}
%Compare with the quantum circuit model, the MBQC~\cite{} is a also universal while its formulation and properties are quite different. 
Previous works have proved that MBQC is also universal by studying how to theoretically convert a quantum circuit in the circuit model to operations in the MBQC paradigm~\cite{}.
These works can be considered as basic and preliminary compilation to execute a quantum circuit on an MBQC machine.
They can be categorized into two types and are briefly introduced in the following.
%We first introduce the computation resource and then show how to implement the functions of quantum gates in using measurement sequence in the MBQC

\vspace{0.5em}
\subsubsection{Mapping onto Regular Lattice First}\label{sect:baseline}

%\textbf{Computational Resource Initialization}
The computational resource in MBQC is the so-called cluster state~\cite{mbqc2009}, which consists of an array of qubits initialized and coupled together with some specific structure.
This `Mapping onto Regular Lattice First' approach will first assume that the qubits in the cluster state is in a common regular structure like a 2D grid~\cite{mbqc2009}.
%A common structure is the 2D grid yet other coupling structures are also feasible.
With the qubits in a 2D grid cluster state, we can find directly mapping from the logical qubits and gates in a quantum circuit to the operations on the cluster state.
After initializing the clustered state, all remaining operations are measurement along different basis. 
No more two-qubit gates are required.
%on the braids of single-qubit measurement sequences on the cluster state and 
As shown in Fig.~\ref{fig:circuit_simulation}, a circuit on the left can be translated to a pattern of single-qubit measurement on the right, with the measurement bases marked on corresponding qubits. 


%\todo{universal. 1 qubit 2 qubit --> new dependence }
\textbf{Single-Qubit Gate}
Arbitrary single-qubit gate can be implemented with single-qubit measurements along different measurement basis on at most four qubits in the logical qubit braid.
% A single-qubit measurement along arbitrary basis can be implemented by a single-qubit gate and a normal Z basis measurement Figure~\ref{} 
% For example, in Figure~\ref{fig:circuit_simulation}, the xx gate on qubit xx is implemented by 
For example, the Hadamard gate and the $R(\xi,\eta,\zeta)$ gate can be implemented by a pattern of measurements in the red circles, while an identity gate can be implemented by inserting two adjacent X-measurements, which can be used to align the patterns of different gates.

Note that for Clifford gates like the Hadamard gate (Fig.~\ref{fig:circuit_simulation}(a)), the measurement sequence does not have a dependency on the measurement outcomes of any other qubit. That is, all X-, Y-basis measurements can be done simultaneously even though their corresponding gates are at the end of the circuit.
But for non-Clifford single-qubit gates, the measurement basis on one qubit may depend on the measurement outcomes on previous qubits.
For example, in the measurement pattern of $R(\xi,\eta,\zeta)$, the angles of measurement basis in the red circle may need to be adjusted according previous measurement outcomes (eg.from $\xi$ to $\pm\xi$).




%MBQC is a universal computing model because each gate in circuit model can be simulated by a pattern of single-qubit measurements on a specific form of entangled state called \emph{cluster state}. As shown in Fig.\ref{fig:single_qubit_gate_simulation}, an arbitrary single-qubit gate, eg. general rotation, z-rotation, Hadamard gate and $\frac{\pi}{2}$-phase gate, can be simulated by a sequence of measurements on at most 5 linearly entangled qubits, with the leftmost one being input and the rightmost being output. Moreover, adjacent pairs of X-measured cluster qubits act the same as wires and thus can be added or removed as needed. In the figure, qubits are entangled with their neighbors, with the basis of each measurement denoted on the corresponding qubit. $X,Y$ stand for measurements on $X,Y$ bases, $\xi,\eta,\zeta$ indicate the angles of equatorial measurements on the Bloch sphere, which is determined by the rotation angle of the gate since  $R(\xi,\eta,\zeta)=Z(\xi)X(\eta)Z(\zeta)$. Due to the non-determinism of quantum measurements, the angles need to be adjusted, eg. from $\xi$ to $\pm\xi$, according to the outcomes of previous measurements, inducing a dependency relation between the measurements. For example, in the figure the measurement of each qubit relies on the outcome of the qubit to its left, with the exception that measurements in $X,Y,Z$ bases do not reply on other measurements. 

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/single_qubit_gate_simulation.png}
%     \caption{A placeholder}
%     \label{fig:single_qubit_gate_simulation}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/circuit_simulation.pdf}
%     \caption{A placeholder}
%     \label{fig:circuit_simulation}
% \end{figure}
\begin{figure}[h!]
    \centering
    \vspace{-5pt}
    \includegraphics[width=\linewidth]{fig/circuit_simulation_colored.pdf}\\
    \hspace{-50pt}(a) \hspace{120pt} (b) 
    \caption{A placeholder}
    \vspace{-5pt}
    \label{fig:circuit_simulation}
\end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/circuit_simulation_draw.pdf}
%     \caption{A placeholder}
%     \label{fig:circuit_simulation}
% \end{figure}

\textbf{Two-Qubit Gate}
A two-qubit gate applied on two logical qubits are also implemented by single-qubit measurement sequences while a key difference is that there will be measurement patterns to connected those two logical qubits.
For example in Figure~\ref{fig:circuit_simulation}, the CNOT gate applied on $q_0$ and $q_1$ is implemented by the measurement pattern in the green circle on the right and the measurements need to connect the two braids corresponding to the two logical qubits. CNOT on non-neighboring qubits can be implemented by inserting a measurement pattern of SWAP gate (up to a $\pi$ phase) as shown in Fig.~\ref{fig:non-neighboring}(a). For example, Fig.~\ref{fig:non-neighboring}(b) shows a measurement pattern of implementing a CNON gate between the top and bottom logic qubits.


The compilation framework in this paper focuses on the topological constraints when deploying a quantum program onto a MBQC device.
For more details about the specific measurement patterns for different gates, please refer to \cite{mbqc2009}.

\textbf{Drawbacks}
The approach simplifies the mapping from the qubits and gates in the circuit to the measurement operations on cluster state while it comes with great overhead when deploying the regular 2D cluster state onto a realistic MBQC device.
Many qubits are initialized in the cluster state and then disregarded by Z measurement immediately (shaded qubits in Figure~\ref{fig:circuit_simulation}(b)). 
The two-qubit gates can be implemented on two adjacently logical qubit braids easily but are much more expensive when applied on logical qubit braids that not adjacent. As shown in Fig.~\ref{fig:non-neighboring}(b), the spacing between logical qubit braids need to be doubled compared to Fig.~\ref{fig:circuit_simulation} in order to maintain a fixed width of pattern. On a 3D grid of cluster state with one of its dimension playing the role of time axis (Fig.~\ref{fig:3d_simulation}(a)), the active qubits, i.e. those not removed by Z-measurements, on each layer of the cluster state would be sparse. Fig.~\ref{fig:3d_simulation}(b) shows an example, with the small squares representing the active physical qubits whose measurements are not in Z-basis.
% (xx times qubit resourse consumption) on two non-neighboring logical qubit braids that are not adjacent~\cite{}.
Moreover, on a realistic MBQC device like a photonics quantum computer introduced later in this section, the hardware only generate small sparse cluster states.
% A lot of redundancies are introduced when translating a quantum circuit through a 2D regular cluster state.



%A CNOT gate can be simulated by a pattern as shown in Fig.\ref{fig:CNOT_simulation}. Qubits located at the spaces need not be removed physically, although a cluster state forms a grid where each qubit is entangled with all its neighbors.Instead, they can be effectively removed by implementing a Z-measurement on each of them. Measurements for Clifford gates including CNOT can be implemented simultaneously, because dependent measurements appear only in patterns of non-Clifford gates. Therefore the dependency in MBQC can be quite different from the circuit it simulates. CNOT gates between two distant logical qubits can be achieved by inserting SWAP gates as can be realized by patterns in Fig.\ref{fig:swap_gate_pattern}. This requires leaving enough spaces between logical qubits on the cluster, as shown in Fig.\ref{fig:spaces_between_logical_qubits}, to avoid a linear growth of the width with the separation of the two logical qubits. For a 3-dimensional cluster state, a measurement pattern can be implemented as shown in Fig.~\ref{fig:3d_simulation}, which is usually sparse on each layer of 2d grid.
% In the one-way model, computing is driven by a pattern of single-qubit measurements on qubits in an entangled state, called a \textit{measurement pattern}. This can be realized by simulating each quantum gate in a quantum circuit on a universal computing resource called a \textit{cluster state}, which leads to a direct correspondence between circuits and measurement patters. Due to the non-determinism of quantum measurements, the bases of some measurements need to be adjusted according to the outcomes of previous measurements, inducing a dependency relation between the measurements. For example, Fig.\ref{fig:gate_patterns} shows the patterns of implementing CNOT gate, general rotation, z-rotation, Hadamard gate and $\frac{\pi}{2}$-phase gate, where $X,Y$ stand for measurements on $X,Y$ bases, $\ksi,\eta,\zeta$ indicate the angles of the bases of dependent measurements. It is worth mentioning that those dependent measurements appear only in simulations of non-Clifford gates. CNOT gates between two distant logical qubits can be achieved by inserting SWAP gates as can be realized by patterns in Fig.\ref{fig:swap_gate_pattern}. This requires leaving enough spaces between input qubits on the cluster, as shown in Fig.\ref{fig:spaces_between_logical_qubits}, to avoid a linear growth of the width with the separation of the two logical qubits. All the qubits at the locations of the spaces can be removed by measurements in Z-basis. For a 3-dimensional cluster state, a measurement pattern can be implement as shown in Fig.~\ref{fig:3d_simulation}, which is usually sparse on each layer of 2d grid.


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.8\linewidth]{fig/CNOT_simulation.png}
%     \caption{A placeholder}
%     \label{fig:CNOT_simulation}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/swap_gate_pattern.png}
%     \caption{A placeholder}
%     \label{fig:swap_gate_pattern}
% \end{figure}


\begin{figure}[h]
    \newcommand{\fhe}{0.25}
    \centering
        \includegraphics[height=\fhe\textwidth]{fig/non-nei.pdf}
        \\
    (a)\hspace{90pt}(b)
        % \hphantom{} \hspace{58pt}(a) \hspace{105pt} (b) 
        % \vspace{-5pt}
        \caption{(a) Measurement pattern of a SWAP gate up to a phase of $\pi$. (b) Implementing a CNOT between the top and bottom qubits by inserting SWAP patterns in (a).
                 }
        \label{fig:non-neighboring}
\end{figure}
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/space_between_logical_qubits.png}
%     \caption{A placeholder}
%     \label{fig:spaces_between_logical_qubits}
% \end{figure}


\begin{figure}[h!]
    \centering
    \vspace{-10pt}
    \includegraphics[width=0.8\linewidth]{fig/3d_simulation_1.pdf}
    \vspace{-5pt}
    \caption{A 3D cluster state with one of its dimension playing the role of time axis. Each layer along the time axis is a 2D cluster state as Fig.~\ref{fig:circuit_simulation}. Small squares represent the qubits whose measurements are not in the Z-basis, which are usually sparse on each 2D layer.}
    \label{fig:3d_simulation}
\end{figure}

\subsubsection{Converting to Graph State First}
% \todo{Highlight that a graph doesn't have to be translated from a circuit, but can also be designed natively in MBQC. In this case, the simulational compiler would not work.}
%\textbf{Circuit Translation}
Instead of embedding the gates into the grid of cluster state, the second approach is to
convert the input circuit into a graph state~\cite{translation}, which also can naturally show the measurement sequence required to execute the input circuit in MBQC but do not demand the 2D grid structure as the cluster state.
To turn a circuit into its corresponding graph state, it is first compiled to a universal gate set $\left\{J(\theta), CZ\right\}$~\cite{translation}. 
\iffalse
To turn a circuit into its corresponding graph state, it is first compiled to a universal gate set $\left\{J(\theta), CZ\right\}$, where the $J$ gate is defined as:
%simulate the gates is to implement the measurement pattern on a \emph{graph state} whose geometry is determined by the circuit[?]. Similar to cluster states, graph states can also be generated by implementing CZ gates among a bunch of qubits in $\ket{+}$ state. The difference is that it forms only necessary edges in the geometry, instead of a grid with neighboring connectivity. According to the rules in \cite{translation}, a circuit decomposed to the universal gate set $\left\{J(\theta), CZ\right\}$ can be translated to a graph as shown in Fig.~\ref{fig:circuit_translation}, where $J$ gate is defined as
\begin{align}
J(\alpha)=
\begin{bmatrix}
1 & \mathrm{e}^{\mathrm{i} \alpha}\\
1 & \mathrm{e}^{-\mathrm{i} \alpha}
\end{bmatrix}   
\end{align}
\fi
%with the decomposition of an arbitrary single-qubit gates as 
Note that an arbitrary single-qubit gate $U$ can be decomposed into $
U = \mathrm{e}^{\mathrm{i} \theta} J(\alpha)J(\beta)J(\gamma).
$

Figure~\ref{fig:circuit_translation} shows an example of this approach.
On the left is the input circuit and its generated graph state is on the right.
The node $a$ corresponds to the qubit A.
It connects to three nodes as there are three $\rm CZ$ gates connection the qubit A to qubit B, C, and D.
$CZ$ is a Clifford gate so there is no dependency regarding the measurements on node $a$ and node $b_2$, $c_2$, and $c_2$.
There are also single-qubit J gates on qubits and they are represented by nodes $b_1,b_2,b_3$
There will be a measurement order requirement when the $J(\theta)$ gate is non-Clifford and we use directed edges to represent such dependency.
For example, the edge $b_1\rightarrow b_2$ indicates that the measurement basis of $b_2$ may need to be adjusted according the measurement outcome of $b_1$. In the following sections, we will omit the arrows as they can always be derived from the graph state \cite{translation}.

\textbf{Drawbacks}
The generated graph state contains the necessary coupling structure so that the qubits and coupling requirements are much smaller compared with the first `Mapping onto Regular Lattice First' which are purely derived from the input circuit.
It is not yet known how we can efficiently map the graph state onto an MBQC machine, which usually generate the cluster states on physical qubits with hardware constraints.

%It can be observed that the generated graph state

%In the figure, each vertex represents a physical, each edge is generated by applying a CZ between its corresponding vertices. $X$ indicates a $X$-measurement, while $\alpha,\beta,\gamma$, etc. indicate the angles of the equatorial measurements on the qubits, which may also be adaptive according previous measurement outcomes. For example, a circuit as simple as three CNOTs can be translated to a graph as showns in Fig.~\ref{fig:circuit_translation}(a), with a rough correspondence between A and a, B and $b_1,b_2,b_3$, C and $c_1,c_2,c_3$ as well as between D and $d_1,d_2,d_3$. The complex structure in a circuit may result in high-degree vertices in the graph, eg.$a,b_2,c_2,d_2$, leading to a difficult for implementation. Since all gates are Clifford gates, the measurements in the graph does not have dependencies between each other. Adding non-Clifford J gates would induce dependency as shown in Fig.~\ref{fig:circuit_translation}, where we use arrows $q_1\rightarrow q_2$ to indicate that the measurement basis of qubit $q_2$ depends on the measurement outcome of qubit $q_1$. The depedency orders in a general graph can be derived from the \emph{flow} of the graph [?]. 



% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/circuit_translation.pdf}
%     \caption{A placeholder}
%     \label{fig:circuit_translation}
% \end{figure}

\begin{figure}[h!]
    \centering
     \vspace{-5pt}
    \includegraphics[width=\linewidth]{fig/translation.pdf}
    \vspace{-15pt}
    \caption{A placeholder}
    \vspace{-5pt}
    \label{fig:circuit_translation}
\end{figure}

\subsection{MBQC on Photonics Quantum Hardware}
This paper focuses on the linear optical quantum computing technology. 
We will introduce the basics as well as the key architectural constraints that need to be considered in the compilation optimization. 
For more details about linear photonics, we recommend ~\cite{photonics_review}.

\textbf{Photonic qubits}
In linear optical quantum computing, a qubit is usually implemented by representing $\ket{0}$ and $\ket{1}$ with two optical modes, either two spatial modes, referred as `dual-rail qubits', or two polarization modes, of a single qubit, referred to as `polarization qubits'. 
%Those two representations are mathematically equivalent and can be physically switched to each other using polarizing beam
%splitters~\cite{photonics_review}. 
Photonic quantum computing does not require an extremely low temperature compared with other quantum hardware technologies\cite{hareware1,hardware2,hardware3,hardware4}, and is potentially highly scalable with the ability of constantly generating a large amount of photons. 
This is especially advantageous for MBQC as each qubit in MBQC is measured only once and then thrown away or initialized again. Compared to solid state qubits such as superconducting qubits, phontoics qubits naturally favors MBQC for mainly three reasons. First, the weak interactions between photons make it hard to directly implement multi-qubit gates on arbitrary qubit states, while in MBQC the only thing needed is single-qubit measurements with a fixed, initialized cluster states or graph states.
Second, measurements on photons are destructive, meaning that photons will disappear after measurements, however in MBQC, each qubit is measured only once, and is then free to detach from the computing system or even disappear. Third, the low depth of operation (measured only once) on each qubit reduces the requirement for coherence time.


\textbf{Generating Cluster State}
Large-scale one-way quantum computing requires a large cluster state to be prepared as a resource.
%This is a challenging task because weak interaction between photons makes it difficult to entangle them. 
There are two approaches to entangle photonic qubits and create cluster state upon them. 
One approach is to directly created entangled photons through nonlinear optical devices which induce interactions between photons and effectively lead to a deterministic cluster state generation.
However, such nonlinear systems are difficult to scale\cite{\todo{?}}. 
%One way is to send photons through nonlinear optical devices which induce interactions between photons and effectively lead to a deterministic quantum gate, however such linear nonlinear \todo{what is this linear nonlinear system?} systems are difficult to scale\cite{}. 
%, with a typical size of $O(10)$ qubits~\.
The second approach is to use linear optical devices and photon detectors to realize a special operation, namely fusion, which can merge two cluster states to construct a larger cluster state.
This approach is readily CMOS compatible and easy to scale; nevertheless, it is at the cost of consuming two qubits in the two cluster states to be merged and is not deterministic.
Significantly overhead is required if we need to construct a large cluster state with a high probability.
%implies a large overhead if we require a near unity success probability. 
Thus, recent efforts~\cite{GHZcluster,psiquantum-fbqc} are to take advantages of both methods and reduce their shortcomings by combining them in the following way: A bunch of small entangled states can be generated deterministically using the first approach and then can be fused to construct a large cluster state.

%The other way is to use linear optical devices and photon detectors to realize quantum gates, eg., fusion gates[?], probabilistically. This fusion operation can This approach is readily CMOS compatible and easy to scale; nevertheless, it is not deterministic and implies a large overhead if we require a near unity success probability. 
%Therefore, it is more realistic to take advantages of both methods and reduce their shortcomings by combining them in the following way: A bunch of small entangled states can be generated (almost) deterministically at first and then can be fused to construct a large static entangled state.

\textbf{Fusion}
%Small entangled states can be expanded to large states via fusion gates, which effectively acts as a joint measurement on two qubits. 
% \todo{fusion term: gate or operation;}
The fusion operation is a native gate on photonic device that can merge two cluster state through two joint measurement operaions on two qubits from the two cluster states.
For example, a joint measurement in the basis of $XX,ZZ$ projects a state to the Bell basis, which creates entanglement between the qubits. The joint measurement we use in this paper is in $XZ,ZX$ basis, which entangles two cluster states into a larger one at the cost of losing two photons. 
For example, in Figure~\ref{fig:fusion_XZ_ZX} we use fusion operation to merge two two-qubit cluster states.\todo{update figure}
After the two joint measurements on qubit x and x, the two measured qubits are lost and the rest qubits are now merged to one cluster state, which is a new two-qubit cluster state. 
In general, when we merge two cluster states with $m$ and $n$ qubits, the final cluster state after fusion will have $m+n-2$ qubits.
Since fusion operations succeeds probablistically and has the overhead of losing two qubits per fusion, one of the goals in our compiler is to minimize the number of fusion operations. However it is worth mentioning that although fusions are probabilistic, they are heralded \cite{GHZcluster} and can be handled by error corrections along with other errors as claimed by \cite{psiquantum-fbqc}. As an initial research towards the compilation onto photonics MBQC,  %compilation framework, 
error correction design is not taken into account and can be left to the future work.

\iffalse
For illustration, let's consider the fusion between two two-qubit cluster states~\cite{}. The state of a two-qubit cluster state can be written as $\ket{\psi}=\ket{0+}+\ket{1-}$, since a cluster state can be created by applying CZ gates on a bunch of qubits in $\ket{+}$ state. Implementing a $XZ,ZX$ measurement on two qubits with each qubit from one of them projects the state into a basis of 
\begin{align*}
    &XZ=1,ZX=1: &\ket{0}_2\otimes\ket{+}_3+\ket{1}_2\otimes\ket{-}_3\\ 
    &XZ=1, ZX=-1: &\ket{0}_2\otimes\ket{+}_3-\ket{1}_2\otimes\ket{-}_3\\
    &XZ=-1,ZX=1: &\ket{0}_2\otimes\ket{-}_3+\ket{1}_2\otimes\ket{+}_3\\
    &XZ=-1,ZX=-1: &\ket{0}_2\otimes\ket{-}_3-\ket{1}_2\otimes\ket{+}_3
\end{align*}
determined by the measurement outcome. With qubit 2 and qubit 3 lost after the fusion, qubit 1 and qubit 4 forms a state
% \begin{align*}
%     &\ket{0}_1\otimes\ket{+}_4+\ket{1}_1\otimes\ket{-}_4\\ 
%     &\ket{0}_1\otimes\ket{+}_4-\ket{1}_1\otimes\ket{-}_4\\
%     &\ket{0}_1\otimes\ket{-}_4+\ket{1}_1\otimes\ket{+}_4\\
%     &\ket{0}_1\otimes\ket{-}_4-\ket{1}_1\otimes\ket{+}_4,
% \end{align*}
that is equivalent to $\ket{\psi}$ up to a local $X$ or $Z$ correction.
\fi
%When the initial cluster states are longer than 2, this constructs a larger cluster state of $m+n-2$ qubit, as shown in Fig.~\ref{fig:fusion_XZ_ZX} with $m,n$ being the number of qubits in the small cluster states. Since fusion operations succeeds probablistically and has the over head of losing two qubits per fusion, one of the goals in our compiler is to minimize the number of fusion operations. However it is worth mentioning that although fusions are probabilistic, they are heralded and can be handled by error corrections along with other errors as claimed by [?]. As an initial research towards the compilation onto photonics MBQC,  %compilation framework, 
%error correction design is not taken into account and can be left in the future work.


\iffalse

\textbf{Hardware Architecture} % and Constraints}
This paper adopts the hardware architecture from PsiQuantum~\cite{psiquantum-fbqc}, a leading industry in the area of photonic quantum computing, as shown in Fig.~\ref{fig:device2d}.
This architecture consists of resource state generators (RSG), routers and measurement device. 
A RSG repeatedly produces a copy of small cluster state (e.g., a three-qubit GHZ state~\cite{}) every clock cycle. Without loss of generality, the rest of the paper uses GHZ as the basic RSG state unless otherwise stated.
%, which is called a \textit{resource state}.
%We adopt a hardware model recently proposed by [?], which consists of resource state generators (RSG), routers and measurement device, as shown in Fig.~\ref{fig:device2d}. 
Those small cluster states %  resource states 
are channelled to different measurement locations by the routers. The routing includes spatial routing as well as temporal routing in the form of delay lines.
The spatial routing allows a small cluster state to be fused with cluster states generated by other RSGs.
The temporal routing delay the arrival of photons by some clock cycles so that they can be fused with photons generated later by the same RSG. 
%, which delay the arrival of photons by some clock cycles so that they can be fused with photons generated later by the same RSG. 
% The size of the resource states is typically considered as $\mathit{O}(10)$ since generating large resource states is  exponentially hard.
%\textbf{Architectural Constraints} %However,
%It is conceivable that a global spatial connectivity is hard to realize due to difficulty of hardware routing as the number of RSGs scales up. 
%Therefore, in this paper, we consider that the RSGs formulate a 2D array and each RSG has spatial connection to its neighbors.
%For the temporal routing, note that photons suffer more from the photon loss error as the photon stays longer in the delay line.
%In this paper, we assume a certain temporal distance is constraint, that is, the photons can only stay in the delay line for at most a specific number of cycles.
%Moreover, photons should not be stored in the delay line for too long as it increases the loss rate of photons. In the near-term, it is reasonable to target at realizing adjacent spatial connectivity, and a temporal connectivity between photons routed to the same delay line within a certain temporal distance. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/device2d.jpg}
    \caption{screenshot, \textcolor{red}{to be modified} \yuke{Add the "Note that ``RSG'' means XXX, ``F'' means XXX"} \todo{Yufei: can remove this figure if space is limited}}
    \label{fig:device2d}
\end{figure}
\fi




 
% Large-scale one-way quantum computing requires a large entangled state to be prepared as a resource. However the non-linearity effects required for deterministically generating entanglements between photons make it difficult to scale. Instead, it is more realistic to generate a bunch of small entangled states (almost) deterministically and construct a large entangled state via \emph{fusion} operations in linear optics. A fusion operation is a two-qubit joint measurement that succeeds probablistically with a herald if it fails. On success, a fusion entangles two small cluster states into a larger one at the cost of losing two qubits, as shown in Fig.~\ref{fig:fusion_XZ_ZX}. Due to the non-determinism of fusion operations, we want to minimize the number of fusion operations. However it is worth mentioning that although fusions are probabilistic, they can be handled by error corrections along with other errors as claimed by [?]. As the first compilation framework, we do not take error correction design into account in this paper.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{fig/fusion_XZ_ZX.pdf}
    \caption{A placeholder}
    \label{fig:fusion_XZ_ZX}
\end{figure}




==> 03_background_10-06.tex <==
\subsection{Programming Paradigm of MBQC}
\fix{There are several competing models of quantum computing which are equivalent in computational terms, but which are conceptually quite distinct.}

\vspace{-10pt}\fix{\subsubsection{Cluster State and MBQC Universality}}\label{sect:baseline}
As a quantum computational model, MBQC is universal and equivalent to the circuit model in the sense that any program in the circuit model can be realized in MBQC as well. This is proved~\cite{mbqc2009} by transforming arbitrary quantum gates in the circuit model to measurement patterns in MBQC and joining those measurement patterns according to the circuit on a specific form of entangled state called cluster state.

\fix{\textbf{Cluster State} Cluster states are pure quantum states of qubits located on a subset of a simple cubic lattice $\mathbb{Z}^d$ in $d\ge1$ dimensions, as depicted in Figure~\ref{fig:circuit_simulation}(b).
It is defined as the eigenstate of operator\[s=X_i \bigotimes_{j\in n_i} Z_j\]
for all qubit $i$ where $n_i$ stands for the set of qubits on the neighboring lattice sites of qubit $i$. A cluster state can be generated by first preparing all qubits in $\ket{+}$ and then applying a CZ gate on each pair of qubits connected by an edge in the cluster.}

%\todo{universal. 1 qubit 2 qubit --> new dependence }
\textbf{Gate Implementation}
An arbitrary single-qubit gate can be implemented by single-qubit measurements on a line of qubits in the cluster state.
% A single-qubit measurement along arbitrary basis can be implemented by a single-qubit gate and a normal Z basis measurement Figure~\ref{} 
% For example, in Figure~\ref{fig:circuit_simulation}, the xx gate on qubit xx is implemented by 
For example, the Hadamard gate and the $R(\xi,\eta,\zeta)$ gate in Figure~\ref{fig:circuit_simulation}(a) can be implemented by measurement patterns in the red circles of Figure~\ref{fig:circuit_simulation}(b), where the $X,Y$ labels stand for X-, Y-bases respectively, and $\xi,\eta,\zeta$ stand for the angles of measurement bases on the $xy$ plane of the Bloch sphere.
Two-qubit gates can also be achieved by single-qubit measurement sequences on the cluster state.
For example, the CNOT gates in Figure~\ref{fig:circuit_simulation}(a) are implemented by the measurement patterns in the green circles of Figure~\ref{fig:circuit_simulation}(b), with the two connected braids of physical qubits in the cluster state corresponding to the two logical qubits in the circuit. 
Measurement bases except X, Y and Z are adaptive to the outcomes of previous measurements (e.g., from $\xi$ to $-\xi$) and thus can induce dependency. But adaptive bases only arise in the measurement patterns of non-Clifford gates. Namely, all Clifford gates can be conducted simultaneously on the cluster state even if they are dependent in the circuit model.
For more details about the specific measurement patterns for different gates, please refer to \cite{mbqc2009}.
% while an identity gate can be implemented by inserting two adjacent X-measurements, which can be used to align the patterns of different gates.

% Note that for Clifford gates like the Hadamard gate (Fig.~\ref{fig:circuit_simulation}(a)), the measurement sequence does not have a dependency on the measurement outcomes of any other qubit. That is, all X-, Y-basis measurements can be done simultaneously even if their corresponding gates are at the end of the circuit.
% But for non-Clifford single-qubit gates, the measurement basis on one qubit may depend on the measurement outcomes of previous qubits.
% For example, in the measurement pattern of $R(\xi,\eta,\zeta)$, the angles of measurement basis in the red circle may need to be adjusted according previous measurement outcomes (e.g., from $\xi$ to $\pm\xi$).




%MBQC is a universal computing model because each gate in circuit model can be simulated by a pattern of single-qubit measurements on a specific form of entangled state called \emph{cluster state}. As shown in Fig.\ref{fig:single_qubit_gate_simulation}, an arbitrary single-qubit gate, eg. general rotation, z-rotation, Hadamard gate and $\frac{\pi}{2}$-phase gate, can be simulated by a sequence of measurements on at most 5 linearly entangled qubits, with the leftmost one being input and the rightmost being output. Moreover, adjacent pairs of X-measured cluster qubits act the same as wires and thus can be added or removed as needed. In the figure, qubits are entangled with their neighbors, with the basis of each measurement denoted on the corresponding qubit. $X,Y$ stand for measurements on $X,Y$ bases, $\xi,\eta,\zeta$ indicate the angles of equatorial measurements on the Bloch sphere, which is determined by the rotation angle of the gate since  $R(\xi,\eta,\zeta)=Z(\xi)X(\eta)Z(\zeta)$. Due to the non-determinism of quantum measurements, the angles need to be adjusted, eg. from $\xi$ to $\pm\xi$, according to the outcomes of previous measurements, inducing a dependency relation between the measurements. For example, in the figure the measurement of each qubit relies on the outcome of the qubit to its left, with the exception that measurements in $X,Y,Z$ bases do not reply on other measurements. 

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/single_qubit_gate_simulation.png}
%     \caption{A placeholder}
%     \label{fig:single_qubit_gate_simulation}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/circuit_simulation.pdf}
%     \caption{A placeholder}
%     \label{fig:circuit_simulation}
% \end{figure}
\begin{figure}[h!]
    \centering
    \vspace{-5pt}
    \includegraphics[width=\linewidth]{fig/circuit_simulation_colored.pdf}\\
    \hspace{-50pt}(a) \hspace{120pt} (b) 
    \caption{From a circuit (a) to a MBQC measurement pattern (b), with the measurement bases labeled on qubits. Patterns in red correspond to single qubit gates, patterns in green correspond to CNOT gates. Two adjacent X-measurements can play the role of a wire as marked in yellow. Shaded qubits are removed by Z-measurements.}
    \vspace{-5pt}
    \label{fig:circuit_simulation}
\end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/circuit_simulation_draw.pdf}
%     \caption{A placeholder}
%     \label{fig:circuit_simulation}
% \end{figure}

% \textbf{Two-Qubit Gate}
% Two-qubit gates applied on two logical qubits are also implemented by single-qubit measurement sequences, with a key difference that there will be measurement patterns to connect those two logical qubits. For example, in Figure~\ref{fig:circuit_simulation}, the CNOT gates are implemented by the measurement patterns in the green circles on the right and the measurements need to connect the two braids corresponding to the two logical qubits. For more details about the specific measurement patterns for different gates, please refer to \cite{mbqc2009}.

\fix{\textbf{MBQC Interpreter} 
A naive interpreter from the circuit model to MBQC can be constructed by simply joining the inputs and outputs of those measurement patterns according to the gates in the circuit, as shown in Figure~\ref{fig:circuit_simulation}. Those measurement patterns can be aligned up by inserting dentity gates implemented by two adjacent X-measurements, as shown by the yellow wires in Figure~\ref{fig:circuit_simulation}(b).
Similar to that in the circuit model~\cite{sabre}, CNOT gates on non-neighboring qubits can be implemented by inserting measurement patterns of SWAP gates whenever necessary. Redundant qubits (shaded qubits in Figure~\ref{fig:circuit_simulation}(b)) can be removed by measurements in Z-basis. In this way we can simulate any circuit in MBQC and we treat this naive interpreter as a baseline of our work.} However, this simulational interpreter is far from efficient since many redundant entanglements are created and then consumed trivially by Z-measurements.


%The compilation framework in this paper focuses on the topological constraints when deploying a quantum program onto a MBQC device.


% \textbf{Drawbacks} This simulational interpreter on the cluster state simplifies the mapping from qubits and gates in a circuit to measurements on a cluster state while it comes with great overhead when deploying the regular 3D cluster state onto a realistic MBQC device. Many qubits are initialized in the cluster state and then disregarded by Z measurement immediately (shaded qubits in Figure~\ref{fig:circuit_simulation}(b)). The two-qubit gates can be implemented on two adjacently logical qubit braids easily but are much more expensive when applied on logical qubit braids that not adjacent. 
%On a 3D grid of cluster state with one of its dimension playing the role of time axis (Fig.~\ref{fig:3d_simulation}(a)), the active qubits, i.e. those not removed by Z-measurements, on each layer of the cluster state would be sparse. Fig.~\ref{fig:3d_simulation}(b) shows an example, with the small squares representing the active physical qubits whose measurements are not in Z-basis.
% (xx times qubit resourse consumption) on two non-neighboring logical qubit braids that are not adjacent~\cite{}.
% Moreover, on a realistic MBQC device like a photonics quantum computer introduced later in this section, the hardware only generates small sparse cluster states.
% A lot of redundancies are introduced when translating a quantum circuit through a 2D regular cluster state.



%A CNOT gate can be simulated by a pattern as shown in Fig.\ref{fig:CNOT_simulation}. Qubits located at the spaces need not be removed physically, although a cluster state forms a grid where each qubit is entangled with all its neighbors.Instead, they can be effectively removed by implementing a Z-measurement on each of them. Measurements for Clifford gates including CNOT can be implemented simultaneously, because dependent measurements appear only in patterns of non-Clifford gates. Therefore the dependency in MBQC can be quite different from the circuit it simulates. CNOT gates between two distant logical qubits can be achieved by inserting SWAP gates as can be realized by patterns in Fig.\ref{fig:swap_gate_pattern}. This requires leaving enough spaces between logical qubits on the cluster, as shown in Fig.\ref{fig:spaces_between_logical_qubits}, to avoid a linear growth of the width with the separation of the two logical qubits. For a 3-dimensional cluster state, a measurement pattern can be implemented as shown in Fig.~\ref{fig:3d_simulation}, which is usually sparse on each layer of 2d grid.
% In the one-way model, computing is driven by a pattern of single-qubit measurements on qubits in an entangled state, called a \textit{measurement pattern}. This can be realized by simulating each quantum gate in a quantum circuit on a universal computing resource called a \textit{cluster state}, which leads to a direct correspondence between circuits and measurement patters. Due to the non-determinism of quantum measurements, the bases of some measurements need to be adjusted according to the outcomes of previous measurements, inducing a dependency relation between the measurements. For example, Fig.\ref{fig:gate_patterns} shows the patterns of implementing CNOT gate, general rotation, z-rotation, Hadamard gate and $\frac{\pi}{2}$-phase gate, where $X,Y$ stand for measurements on $X,Y$ bases, $\ksi,\eta,\zeta$ indicate the angles of the bases of dependent measurements. It is worth mentioning that those dependent measurements appear only in simulations of non-Clifford gates. CNOT gates between two distant logical qubits can be achieved by inserting SWAP gates as can be realized by patterns in Fig.\ref{fig:swap_gate_pattern}. This requires leaving enough spaces between input qubits on the cluster, as shown in Fig.\ref{fig:spaces_between_logical_qubits}, to avoid a linear growth of the width with the separation of the two logical qubits. All the qubits at the locations of the spaces can be removed by measurements in Z-basis. For a 3-dimensional cluster state, a measurement pattern can be implement as shown in Fig.~\ref{fig:3d_simulation}, which is usually sparse on each layer of 2d grid.


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.8\linewidth]{fig/CNOT_simulation.png}
%     \caption{A placeholder}
%     \label{fig:CNOT_simulation}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/swap_gate_pattern.png}
%     \caption{A placeholder}
%     \label{fig:swap_gate_pattern}
% \end{figure}


% \begin{figure}[h]
%     \newcommand{\fhe}{0.25}
%     \centering
%         \includegraphics[height=\fhe\textwidth]{fig/non-nei.pdf}
%         \\
%     (a)\hspace{90pt}(b)
%         % \hphantom{} \hspace{58pt}(a) \hspace{105pt} (b) 
%         % \vspace{-5pt}
%         \caption{(a) Measurement pattern of a SWAP gate up to a phase of $\pi$. (b) Implementing a CNOT between the top and bottom qubits by inserting SWAP patterns in (a).
%                  }
%         \label{fig:non-neighboring}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/space_between_logical_qubits.png}
%     \caption{A placeholder}
%     \label{fig:spaces_between_logical_qubits}
% \end{figure}


% \begin{figure}[h!]
%     \centering
%     \vspace{-10pt}
%     \includegraphics[width=0.8\linewidth]{fig/corrected_3d.pdf}
%     \vspace{-5pt}
%     \caption{A 3D cluster state with one of its dimension playing the role of time axis. Each layer along the time axis is a 2D cluster state as Fig.~\ref{fig:circuit_simulation}. Small squares represent the qubits whose measurements are not in the Z-basis, which are usually sparse on each 2D layer.}
%     \label{fig:3d_simulation}
% \end{figure}
\vspace{0.3em}
\subsubsection{Graph State Representation}
% \todo{Highlight that a graph doesn't have to be translated from a circuit, but can also be designed natively in MBQC. In this case, the simulational compiler would not work.}
%\textbf{Circuit Translation}
A more general representation of a MBQC measurement pattern is the graph state representation~\cite{translation}, which is a generalization of the cluster state from lattice geometry to arbitrary graph geometry, with the edges of the graph indicating necessary entanglements to be prepared.

\fix{\textbf{Graph State} Graph states are pure quantum states of qubits located on a graph $G$, defined as the eigenstate of operator\[s=X_i \bigotimes_{j\in n_i} Z_j\]
for all qubit $i$ where $n_i$ stands for the set of qubits on the neighboring vertices of qubit $i$ in $G$. }

\fix{\textbf{Native Operator Set} An \emph{equatorial measurement} $E(\alpha)$, i.e., a measurement in a basis on the equatorial plane of the Bloch sphere at an angle $\alpha$, that yields a value $m$ is equivalent to a $J(\alpha)$ operator followed by a Z-measurement $M_z$ yielding the same value, i.e., $E(\alpha)\ket{\psi}=m$~corresponds to $M_z J(\alpha)\ket{\psi}=m$ where $m=0$ or 1 and
\begin{align}
J(\alpha)=
\begin{bmatrix}
1 & \mathrm{e}^{\mathrm{i} \alpha}\\
1 & \fix{-\mathrm{e}^{\mathrm{i} \alpha}}
\end{bmatrix}   
\end{align}
An arbitrary single-qubit gate $U$ can be decomposed into $
U = \mathrm{e}^{\mathrm{i} \theta} J(\alpha)J(\beta)J(\gamma)
$.
Considering that a graph state can be generated by preparing all qubits in $\ket{+}$ and applying a CZ gate on each pair of qubits connected by an edge in the graph, a suitable native operator set is $\left\{J(\theta), \mathrm{CZ}\right\}$. }

\fix{\textbf{Circuit Translation}} \cite{translation} introduces a multi-step algorithm of translating a circuit to a graph state. Here we only demonstrate it with an example.
Figure~\ref{fig:circuit_translation}(a) is a circuit and Figure~\ref{fig:circuit_translation}(b) is the generated graph state.
The node $a$ corresponds to the qubit A.
It connects to three nodes as there are three $\rm CZ$ gates connection the qubit A to qubit B, C, and D.
$\mathrm{CZ}$ is a Clifford gate so there is no dependency regarding the measurements on node $a$ and node $b_2$, $c_2$, and $c_2$.
There are also single-qubit J gates on qubits and they are represented by nodes $b_1,b_2,b_3$
There will be a measurement order requirement when the $J(\theta)$ gate is non-Clifford and we use directed edges to represent such dependency.
For example, the edge $b_1\rightarrow b_2$ indicates that the measurement basis of $b_2$ may need to be adjusted according to the measurement outcome of $b_1$.
We remark that the generated graph state only contains the necessary coupling structure that is purely derived from the input circuit, so that the qubits and coupling requirements are potentially much smaller that of cluster states.
%In the following sections, we often omit the arrows and explicit measurement bases when not important for our optimization techniques, and they can always be derived from the graph state \cite{translation}.
Unfortunately, it is not yet known how we can efficiently map the graph state onto an MBQC machine which generates small entangled states with a set of other hardware constraints.


% \textbf{Drawbacks} Unfortunately, it is not yet known how we can efficiently map the graph state onto an MBQC machine, which usually generate small cluster states on physical qubits with a set of other hardware constraints. There is neither any prior work discussing possible graph transformations that could potentially enabling us to resolve the mismatch between the topology of arbitrary graph states with the fixed topology of the underlying hardware. To this end, our work gives an in-depth analysis of the challenges here and build up the first modular compiler to automate the mapping. 


%It can be observed that the generated graph state

%In the figure, each vertex represents a physical, each edge is generated by applying a CZ between its corresponding vertices. $X$ indicates a $X$-measurement, while $\alpha,\beta,\gamma$, etc. indicate the angles of the equatorial measurements on the qubits, which may also be adaptive according previous measurement outcomes. For example, a circuit as simple as three CNOTs can be translated to a graph as showns in Fig.~\ref{fig:circuit_translation}(a), with a rough correspondence between A and a, B and $b_1,b_2,b_3$, C and $c_1,c_2,c_3$ as well as between D and $d_1,d_2,d_3$. The complex structure in a circuit may result in high-degree vertices in the graph, eg.$a,b_2,c_2,d_2$, leading to a difficult for implementation. Since all gates are Clifford gates, the measurements in the graph does not have dependencies between each other. Adding non-Clifford J gates would induce dependency as shown in Fig.~\ref{fig:circuit_translation}, where we use arrows $q_1\rightarrow q_2$ to indicate that the measurement basis of qubit $q_2$ depends on the measurement outcome of qubit $q_1$. The depedency orders in a general graph can be derived from the \emph{flow} of the graph [?]. 



% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/circuit_translation.pdf}
%     \caption{A placeholder}
%     \label{fig:circuit_translation}
% \end{figure}

\begin{figure}[h!]
    \centering
     \vspace{-5pt}
    \includegraphics[width=0.9\linewidth]{fig/translation.pdf}\\
    \hspace{0pt}(a)\hspace{120pt}(b)
    % \vspace{-15pt}
    \caption{Translation from a circuit (a) to a graph state (b), with the measurement bases labeled on qubits. Logical qubit $A$ corresponds to physical qubit
    $a$ and $B,C,D$ correspond to  $\left\{b_1,b_2,b_3\right\}, \left\{c_1,c_2,c_3\right\}$ and $\left\{d_1,d_2,d_3\right\}$. Qubits in (b) with `in',`out' or `in/out' are input or output qubits. Arrows on edges indicate the dependency between qubit measurements.}
    \vspace{-5pt}
    \label{fig:circuit_translation}
\end{figure}

\vspace{0.3em}
\subsection{MBQC on Photonic Platforms}
%This paper focuses on the linear optical quantum computing technology. 
% We will introduce some basics about the linear optical quantum computing and the key architectural constraints that need to be considered in the compilation optimization. For more details about linear photonics, we recommend~\cite{photonics_review}.
We introduce some basics about photonic quantum computing and its support for MBQC. For more detailed knowledge, we recommend~\cite{photonics_review}.

% \textbf{Photonic qubits}
% In linear optical quantum computing, a qubit is usually implemented by representing the two basis states $\ket{0}_L$ and $\ket{1}_L$ with two optical modes of a fixed photon number. The optical modes can be either two spatial modes ($\ket{0}_L = \ket{1} \otimes \ket{0}$ and $\ket{1}_L = \ket{0} \otimes \ket{1}$, where $\ket{0}$ and $\ket{1}$ are the two basis states in one optical mode), referred as `dual-rail qubits', or two polarization modes of a single qubit ($\ket{0}_L = \ket{H}$ and $\ket{1}_L = \ket{V}$, where $\ket{H}$ and $\ket{V}$ represent the horizontal and vertical polarization of one photon), referred to as `polarization qubits'. Those two representations are mathematically equivalent and can be physically switched to each other using polarizing beam splitters~\cite{photonics_review}. Photonic quantum computing does not require an extremely low temperature compared with other quantum hardware technologies\cite{hareware1,hardware2,hardware3,hardware4}, and is potentially highly scalable with the ability of constantly generating a large number of photons.


%\todo{rephrase the picture here}
\iffalse
This is especially advantageous for MBQC as each qubit in MBQC is measured only once and then thrown away or initialized again. Compared to solid state qubits such as superconducting qubits, phontoics qubits naturally favors MBQC for mainly three reasons. First, the weak interactions between photons make it hard to directly implement multi-qubit gates on arbitrary qubit states, while in MBQC the only thing needed is single-qubit measurements with a fixed, initialized cluster states or graph states.
Second, measurements on photons are destructive, meaning that photons will disappear after measurements, however in MBQC, each qubit is measured only once, and is then free to detach from the computing system or even disappear. Third, the low depth of operation (measured only once) on each qubit reduces the requirement for coherence time.
\fi

\fix{\textbf{Photonic Platforms} Photonic quantum computing relies on either the generation, entanglement and detection of individual photons or the generation of squeezed states of light. These intrinsically different hardware approaches are suitable for conceptually distinct computation model as well, with the former particularly suitable for the MBQC model (discrete variable) and the latter more suitable for the continuous variable model. Both of these two approaches are being actively explored by leading companies in industry such as PsiQuantum~\cite{psiquantum-fbqc} (discrete) and Xanadu~\cite{Xanadu} (continuous). The rest of the paper targets the single-photon approach if not otherwise specified.  This approach does not require an extremely low temperature compared with solid-state quantum hardware technologies\cite{hareware1,hardware2,hardware3,hardware4}, and is potentially highly scalable with the ability of constantly generating a large number of photons. But applying two-qubit gates on those individual photons are much harder than that on solid-state platforms, and measurements on photons would cause them to vanish.}

\fix{\textbf{Scalability \todo{ToDo}}} Large-scale MBQC runs on large entangled resource states. Directly creating such large-scale entanglement deterministically through nonlinear optical devices is exponentially hard as the size increases. \fix{An alternative approach is to merge small resource states via the so-called fusion operations~\cite{photonics_review} using linear optical devices and photon detectors so that programs can run on a large amount of small resource states. This approach is readily CMOS compatible and easy to scale;} nevertheless, it is at the cost of consuming two qubits in each merge and is not deterministic. \fix{This brings significant overhead and harms the overall fidelity if we need to construct a large entangled state from small resource states~\cite{GHZcluster}.
%implies a large overhead if we require a near unity success probability. 
Thus, it is of vital importance to minimize the number of fusions required by the program execution.}

% Large-scale one-way quantum computing requires a large cluster state to be prepared as a resource. There are two approaches to entangle photonic qubits and create cluster state upon them. One approach is to directly create entangled photons through nonlinear optical devices which induce interactions between photons and effectively lead to a deterministic cluster state generation. However, such nonlinear systems are difficult to scale\cite{photonics_review,GHZcluster}. The second approach is to use linear optical devices and photon detectors to realize a special operation, namely fusion, which can merge two cluster states to construct a larger cluster state. This approach is readily CMOS compatible and easy to scale; nevertheless, it is at the cost of consuming two qubits in the two cluster states to be merged and is not deterministic. Significantly overhead is required if we need to construct a large cluster state with a high probability. Thus, recent efforts~\cite{GHZcluster,psiquantum-fbqc} are to take advantages of both methods and reduce their shortcomings by combining them in the following way: A bunch of small entangled states can be generated deterministically using the first approach and then can be fused to construct a large cluster state.

%The other way is to use linear optical devices and photon detectors to realize quantum gates, eg., fusion gates[?], probabilistically. This fusion operation can This approach is readily CMOS compatible and easy to scale; nevertheless, it is not deterministic and implies a large overhead if we require a near unity success probability. 
%Therefore, it is more realistic to take advantages of both methods and reduce their shortcomings by combining them in the following way: A bunch of small entangled states can be generated (almost) deterministically at first and then can be fused to construct a large static entangled state.

\textbf{Fusion}
%Small entangled states can be expanded to large states via fusion gates, which effectively acts as a joint measurement on two qubits. 
% \todo{fusion term: gate or operation;}
The fusion operation~\cite{psiquantum-fbqc, browne2005resource, photonics_review} is a native operation on photonic device that can merge two cluster states through two joint measurement operations on two qubits from the two cluster states.
For example, a joint measurement in the basis of $XX,ZZ$ projects a state to the Bell basis, which creates entanglement between the qubits. The joint measurement we use in this paper is in $XZ,ZX$ basis, which entangles two cluster states into a larger one at the cost of losing two photons. 
In Figure~\ref{fig:fusion_XZ_ZX}, we use fusion operation to merge two two-qubit cluster states $AC$ and $BD$.
After the two joint measurements on qubits $C$ and $D$ are implemented, the two measured qubits are destroyed and the rest qubits $A$ and $B$ are now merged to one cluster state, which is a new two-qubit cluster state. 
In general, when we merge two cluster states with $m$ and $n$ qubits, the final cluster state after fusion will have $m+n-2$ qubits.
Since fusion operations themselves are very costly~\cite{psiquantum-fbqc, browne2005resource} and have the overhead of losing two qubits per fusion, one of the goals in our compiler is to minimize the number of fusion operations. 
\iffalse
Since fusion operations succeeds probablistically and has the overhead of losing two qubits per fusion, one of the goals in our compiler is to minimize the number of fusion operations.
However it is worth mentioning that although fusions are probabilistic, they are heralded \cite{GHZcluster} and can be handled by error corrections along with other errors as claimed by \cite{psiquantum-fbqc}. As an initial research towards the compilation onto photonics MBQC,  %compilation framework, 
error correction design is not taken into account and can be left to the future work.
\fi
\iffalse
For illustration, let's consider the fusion between two two-qubit cluster states~\cite{}. The state of a two-qubit cluster state can be written as $\ket{\psi}=\ket{0+}+\ket{1-}$, since a cluster state can be created by applying CZ gates on a bunch of qubits in $\ket{+}$ state. Implementing a $XZ,ZX$ measurement on two qubits with each qubit from one of them projects the state into a basis of 
\begin{align*}
    &XZ=1,ZX=1: &\ket{0}_2\otimes\ket{+}_3+\ket{1}_2\otimes\ket{-}_3\\ 
    &XZ=1, ZX=-1: &\ket{0}_2\otimes\ket{+}_3-\ket{1}_2\otimes\ket{-}_3\\
    &XZ=-1,ZX=1: &\ket{0}_2\otimes\ket{-}_3+\ket{1}_2\otimes\ket{+}_3\\
    &XZ=-1,ZX=-1: &\ket{0}_2\otimes\ket{-}_3-\ket{1}_2\otimes\ket{+}_3
\end{align*}
determined by the measurement outcome. With qubit 2 and qubit 3 lost after the fusion, qubit 1 and qubit 4 forms a state
% \begin{align*}
%     &\ket{0}_1\otimes\ket{+}_4+\ket{1}_1\otimes\ket{-}_4\\ 
%     &\ket{0}_1\otimes\ket{+}_4-\ket{1}_1\otimes\ket{-}_4\\
%     &\ket{0}_1\otimes\ket{-}_4+\ket{1}_1\otimes\ket{+}_4\\
%     &\ket{0}_1\otimes\ket{-}_4-\ket{1}_1\otimes\ket{+}_4,
% \end{align*}
that is equivalent to $\ket{\psi}$ up to a local $X$ or $Z$ correction.
\fi
%When the initial cluster states are longer than 2, this constructs a larger cluster state of $m+n-2$ qubit, as shown in Fig.~\ref{fig:fusion_XZ_ZX} with $m,n$ being the number of qubits in the small cluster states. Since fusion operations succeeds probablistically and has the over head of losing two qubits per fusion, one of the goals in our compiler is to minimize the number of fusion operations. However it is worth mentioning that although fusions are probabilistic, they are heralded and can be handled by error corrections along with other errors as claimed by [?]. As an initial research towards the compilation onto photonics MBQC,  %compilation framework, 
%error correction design is not taken into account and can be left in the future work.


\iffalse

\textbf{Hardware Architecture} % and Constraints}
This paper adopts the hardware architecture from PsiQuantum~\cite{psiquantum-fbqc}, a leading industry in the area of photonic quantum computing, as shown in Fig.~\ref{fig:device2d}.
This architecture consists of resource state generators (RSG), routers and measurement device. 
A RSG repeatedly produces a copy of small cluster state (e.g., a three-qubit GHZ state~\cite{}) every clock cycle. Without loss of generality, the rest of the paper uses GHZ as the basic RSG state unless otherwise stated.
%, which is called a \textit{resource state}.
%We adopt a hardware model recently proposed by [?], which consists of resource state generators (RSG), routers and measurement device, as shown in Fig.~\ref{fig:device2d}. 
Those small cluster states %  resource states 
are channelled to different measurement locations by the routers. The routing includes spatial routing as well as temporal routing in the form of delay lines.
The spatial routing allows a small cluster state to be fused with cluster states generated by other RSGs.
The temporal routing delay the arrival of photons by some clock cycles so that they can be fused with photons generated later by the same RSG. 
%, which delay the arrival of photons by some clock cycles so that they can be fused with photons generated later by the same RSG. 
% The size of the resource states is typically considered as $\mathit{O}(10)$ since generating large resource states is  exponentially hard.
%\textbf{Architectural Constraints} %However,
%It is conceivable that a global spatial connectivity is hard to realize due to difficulty of hardware routing as the number of RSGs scales up. 
%Therefore, in this paper, we consider that the RSGs formulate a 2D array and each RSG has spatial connection to its neighbors.
%For the temporal routing, note that photons suffer more from the photon loss error as the photon stays longer in the delay line.
%In this paper, we assume a certain temporal distance is constraint, that is, the photons can only stay in the delay line for at most a specific number of cycles.
%Moreover, photons should not be stored in the delay line for too long as it increases the loss rate of photons. In the near-term, it is reasonable to target at realizing adjacent spatial connectivity, and a temporal connectivity between photons routed to the same delay line within a certain temporal distance. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/device2d.jpg}
    \caption{screenshot, \textcolor{red}{to be modified} \yuke{Add the "Note that ``RSG'' means XXX, ``F'' means XXX"} \todo{Yufei: can remove this figure if space is limited}}
    \label{fig:device2d}
\end{figure}
\fi




 
% Large-scale one-way quantum computing requires a large entangled state to be prepared as a resource. However the non-linearity effects required for deterministically generating entanglements between photons make it difficult to scale. Instead, it is more realistic to generate a bunch of small entangled states (almost) deterministically and construct a large entangled state via \emph{fusion} operations in linear optics. A fusion operation is a two-qubit joint measurement that succeeds probablistically with a herald if it fails. On success, a fusion entangles two small cluster states into a larger one at the cost of losing two qubits, as shown in Fig.~\ref{fig:fusion_XZ_ZX}. Due to the non-determinism of fusion operations, we want to minimize the number of fusion operations. However it is worth mentioning that although fusions are probabilistic, they can be handled by error corrections along with other errors as claimed by [?]. As the first compilation framework, we do not take error correction design into account in this paper.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.6\linewidth]{fig/fusion_XZ_ZX.pdf}
    \caption{A fusion between cluster states $AC$ and $BD$. After the fusion (a $XZ,ZX$ measurement on $C,D$), qubit $C,D$ vanish and qubit $A,B$ form a new cluster state.}
    \label{fig:fusion_XZ_ZX}
\end{figure}




==> 03_background_unrevised.tex <==
\vspace{0.3em}
\section{Background and Related Work}\label{sect:background}
We start with the necessary background about measurement-base quantum computing (MBQC) paradigm.
The basic quantum computing concepts (e.g., qubit, gate, linear operator, circuit) are not covered and we recommend~\cite{nielsen2002quantum} for more details.

\vspace{0.3em}
\subsection{Programming Paradigm and Compilation in MBQC}
%Compare with the quantum circuit model, the MBQC~\cite{} is a also universal while its formulation and properties are quite different. 
Previous works have proved that MBQC is a universal computing paradigm by studying how to theoretically convert a quantum circuit in the circuit model to operations in the MBQC paradigm~\cite{mbqc2009}.
These works can be considered as basic and preliminary compilation to execute a quantum circuit on an MBQC machine.
They can be categorized into two types and are briefly introduced here.

%in the following.
%We first introduce the computation resource and then show how to implement the functions of quantum gates in using measurement sequence in the MBQC

\vspace{0.5em}
\subsubsection{Mapping onto Regular Lattice First}\label{sect:baseline}
The `Mapping onto Regular Lattice First' approach could translate a circuit in  Fig.~\ref{fig:circuit_simulation} (a) to a pattern of single-qubit measurement as shown in Fig.~\ref{fig:circuit_simulation} (b), with the measurement basis marked on the corresponding qubits. 
The general computational resource in MBQC is the so-called cluster state~\cite{mbqc2009}, which consists of an array of qubits initialized and entangled together with some specific structure. This `Mapping onto Regular Lattice will first assume that the qubits in the cluster state is coupled in a special regular structure, a 3D lattice~\cite{mbqc2009}.
With the qubits in a 3D cluster state, there would be a direct mapping from the logical qubits and gates in a quantum circuit to the operations on the cluster state.
We next give some details about the mapping of single-qubit and two-qubit gates. 
%With such a paradigm, after preparing the clustered state, all remaining operations are measurement along different basis. No more two-qubit gates are required.

\iffalse
%\textbf{Computational Resource Initialization}
The computational resource in MBQC is the so-called cluster state~\cite{mbqc2009}, which consists of an array of qubits initialized and entangled together with some specific structure.
This `Mapping onto Regular Lattice First' approach will first assume that the qubits in the cluster state is coupled in a common regular structure like a 2D grid~\cite{mbqc2009}.
%A common structure is the 2D grid yet other coupling structures are also feasible.
With the qubits in a 2D grid cluster state, we can find directly mapping from the logical qubits and gates in a quantum circuit to the operations on the cluster state.
After preparing the clustered state, all remaining operations are measurement along different basis. 
No more two-qubit gates are required.
%on the braids of single-qubit measurement sequences on the cluster state and 
As shown in Fig.~\ref{fig:circuit_simulation}, a circuit on the left can be translated to a pattern of single-qubit measurement on the right, with the measurement bases marked on corresponding qubits. 
\fi

%\todo{universal. 1 qubit 2 qubit --> new dependence }
\textbf{Single-Qubit Gate}
An arbitrary single-qubit gate can be implemented with single-qubit measurements along different measurement basis on at most four qubits in the logical qubit braid.
% A single-qubit measurement along arbitrary basis can be implemented by a single-qubit gate and a normal Z basis measurement Figure~\ref{} 
% For example, in Figure~\ref{fig:circuit_simulation}, the xx gate on qubit xx is implemented by 
For example, the Hadamard gate and the $R(\xi,\eta,\zeta)$ gate can be implemented by a pattern of measurements in the red circles, while an identity gate can be implemented by inserting two adjacent X-measurements, which can be used to align the patterns of different gates.

Note that for Clifford gates like the Hadamard gate (Fig.~\ref{fig:circuit_simulation}(a)), the measurement sequence does not have a dependency on the measurement outcomes of any other qubit. That is, all X-, Y-basis measurements can be done simultaneously even if their corresponding gates are at the end of the circuit.
But for non-Clifford single-qubit gates, the measurement basis on one qubit may depend on the measurement outcomes of previous qubits.
For example, in the measurement pattern of $R(\xi,\eta,\zeta)$, the angles of measurement basis in the red circle may need to be adjusted according previous measurement outcomes (e.g., from $\xi$ to $\pm\xi$).




%MBQC is a universal computing model because each gate in circuit model can be simulated by a pattern of single-qubit measurements on a specific form of entangled state called \emph{cluster state}. As shown in Fig.\ref{fig:single_qubit_gate_simulation}, an arbitrary single-qubit gate, eg. general rotation, z-rotation, Hadamard gate and $\frac{\pi}{2}$-phase gate, can be simulated by a sequence of measurements on at most 5 linearly entangled qubits, with the leftmost one being input and the rightmost being output. Moreover, adjacent pairs of X-measured cluster qubits act the same as wires and thus can be added or removed as needed. In the figure, qubits are entangled with their neighbors, with the basis of each measurement denoted on the corresponding qubit. $X,Y$ stand for measurements on $X,Y$ bases, $\xi,\eta,\zeta$ indicate the angles of equatorial measurements on the Bloch sphere, which is determined by the rotation angle of the gate since  $R(\xi,\eta,\zeta)=Z(\xi)X(\eta)Z(\zeta)$. Due to the non-determinism of quantum measurements, the angles need to be adjusted, eg. from $\xi$ to $\pm\xi$, according to the outcomes of previous measurements, inducing a dependency relation between the measurements. For example, in the figure the measurement of each qubit relies on the outcome of the qubit to its left, with the exception that measurements in $X,Y,Z$ bases do not reply on other measurements. 

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/single_qubit_gate_simulation.png}
%     \caption{A placeholder}
%     \label{fig:single_qubit_gate_simulation}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/circuit_simulation.pdf}
%     \caption{A placeholder}
%     \label{fig:circuit_simulation}
% \end{figure}
\begin{figure}[h!]
    \centering
    \vspace{-5pt}
    \includegraphics[width=\linewidth]{fig/circuit_simulation_colored.pdf}\\
    \hspace{-50pt}(a) \hspace{120pt} (b) 
    \caption{From a circuit (a) to its MBQC measurement pattern (b), with the measurement bases labeled on the qubits (e.g., X means measuring in X-basis). Patterns in red correspond to the single qubit gates, patterns in green correspond to the CNOT gates. Two adjacent X-measurement can play the role of a wire to align up the patterns, as marked in yellow. Shaded qubits are the ones removed by measurements in Z-basis.}
    \vspace{-5pt}
    \label{fig:circuit_simulation}
\end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/circuit_simulation_draw.pdf}
%     \caption{A placeholder}
%     \label{fig:circuit_simulation}
% \end{figure}

\textbf{Two-Qubit Gate}
Two-qubit gates applied on two logical qubits are also implemented by single-qubit measurement sequences, with a key difference that there will be measurement patterns to connect those two logical qubits.
For example, in Figure~\ref{fig:circuit_simulation}, the CNOT gates are implemented by the measurement patterns in the green circles on the right and the measurements need to connect the two braids corresponding to the two logical qubits. Similar to the circuit model, CNOT gates on non-neighboring qubits in MBQC can be implemented by inserting measurement patterns of SWAP gates whenever necessary. Redundant qubits (shaded qubits in Figure~\ref{fig:circuit_simulation}) can be removed by being measured in Z-basis.
For more details about the specific measurement patterns for different gates, please refer to \cite{mbqc2009}.

%The compilation framework in this paper focuses on the topological constraints when deploying a quantum program onto a MBQC device.


\textbf{Drawbacks}
The approach simplifies the mapping from qubits and gates in a circuit to measurement operations on a cluster state while it comes with great overhead when deploying the regular 3D cluster state onto a realistic MBQC device.
Many qubits are initialized in the cluster state and then disregarded by Z measurement immediately (shaded qubits in Figure~\ref{fig:circuit_simulation}(b)). 
The two-qubit gates can be implemented on two adjacently logical qubit braids easily but are much more expensive when applied on logical qubit braids that not adjacent. 
%On a 3D grid of cluster state with one of its dimension playing the role of time axis (Fig.~\ref{fig:3d_simulation}(a)), the active qubits, i.e. those not removed by Z-measurements, on each layer of the cluster state would be sparse. Fig.~\ref{fig:3d_simulation}(b) shows an example, with the small squares representing the active physical qubits whose measurements are not in Z-basis.
% (xx times qubit resourse consumption) on two non-neighboring logical qubit braids that are not adjacent~\cite{}.
Moreover, on a realistic MBQC device like a photonics quantum computer introduced later in this section, the hardware only generates small sparse cluster states.
% A lot of redundancies are introduced when translating a quantum circuit through a 2D regular cluster state.



%A CNOT gate can be simulated by a pattern as shown in Fig.\ref{fig:CNOT_simulation}. Qubits located at the spaces need not be removed physically, although a cluster state forms a grid where each qubit is entangled with all its neighbors.Instead, they can be effectively removed by implementing a Z-measurement on each of them. Measurements for Clifford gates including CNOT can be implemented simultaneously, because dependent measurements appear only in patterns of non-Clifford gates. Therefore the dependency in MBQC can be quite different from the circuit it simulates. CNOT gates between two distant logical qubits can be achieved by inserting SWAP gates as can be realized by patterns in Fig.\ref{fig:swap_gate_pattern}. This requires leaving enough spaces between logical qubits on the cluster, as shown in Fig.\ref{fig:spaces_between_logical_qubits}, to avoid a linear growth of the width with the separation of the two logical qubits. For a 3-dimensional cluster state, a measurement pattern can be implemented as shown in Fig.~\ref{fig:3d_simulation}, which is usually sparse on each layer of 2d grid.
% In the one-way model, computing is driven by a pattern of single-qubit measurements on qubits in an entangled state, called a \textit{measurement pattern}. This can be realized by simulating each quantum gate in a quantum circuit on a universal computing resource called a \textit{cluster state}, which leads to a direct correspondence between circuits and measurement patters. Due to the non-determinism of quantum measurements, the bases of some measurements need to be adjusted according to the outcomes of previous measurements, inducing a dependency relation between the measurements. For example, Fig.\ref{fig:gate_patterns} shows the patterns of implementing CNOT gate, general rotation, z-rotation, Hadamard gate and $\frac{\pi}{2}$-phase gate, where $X,Y$ stand for measurements on $X,Y$ bases, $\ksi,\eta,\zeta$ indicate the angles of the bases of dependent measurements. It is worth mentioning that those dependent measurements appear only in simulations of non-Clifford gates. CNOT gates between two distant logical qubits can be achieved by inserting SWAP gates as can be realized by patterns in Fig.\ref{fig:swap_gate_pattern}. This requires leaving enough spaces between input qubits on the cluster, as shown in Fig.\ref{fig:spaces_between_logical_qubits}, to avoid a linear growth of the width with the separation of the two logical qubits. All the qubits at the locations of the spaces can be removed by measurements in Z-basis. For a 3-dimensional cluster state, a measurement pattern can be implement as shown in Fig.~\ref{fig:3d_simulation}, which is usually sparse on each layer of 2d grid.


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.8\linewidth]{fig/CNOT_simulation.png}
%     \caption{A placeholder}
%     \label{fig:CNOT_simulation}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/swap_gate_pattern.png}
%     \caption{A placeholder}
%     \label{fig:swap_gate_pattern}
% \end{figure}


% \begin{figure}[h]
%     \newcommand{\fhe}{0.25}
%     \centering
%         \includegraphics[height=\fhe\textwidth]{fig/non-nei.pdf}
%         \\
%     (a)\hspace{90pt}(b)
%         % \hphantom{} \hspace{58pt}(a) \hspace{105pt} (b) 
%         % \vspace{-5pt}
%         \caption{(a) Measurement pattern of a SWAP gate up to a phase of $\pi$. (b) Implementing a CNOT between the top and bottom qubits by inserting SWAP patterns in (a).
%                  }
%         \label{fig:non-neighboring}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/space_between_logical_qubits.png}
%     \caption{A placeholder}
%     \label{fig:spaces_between_logical_qubits}
% \end{figure}


% \begin{figure}[h!]
%     \centering
%     \vspace{-10pt}
%     \includegraphics[width=0.8\linewidth]{fig/corrected_3d.pdf}
%     \vspace{-5pt}
%     \caption{A 3D cluster state with one of its dimension playing the role of time axis. Each layer along the time axis is a 2D cluster state as Fig.~\ref{fig:circuit_simulation}. Small squares represent the qubits whose measurements are not in the Z-basis, which are usually sparse on each 2D layer.}
%     \label{fig:3d_simulation}
% \end{figure}

\subsubsection{Converting to Graph State First}
% \todo{Highlight that a graph doesn't have to be translated from a circuit, but can also be designed natively in MBQC. In this case, the simulational compiler would not work.}
%\textbf{Circuit Translation}
Instead of embedding the gates into the grid of cluster state, the second approach is to
convert the input circuit into a graph state~\cite{translation} which also can show the measurement sequence required to execute the input circuit in MBQC but do not demand the 3D lattice structure in the cluster state.
To turn a circuit into its corresponding graph state, it is first compiled to a universal gate set $\left\{J(\theta), CZ\right\}$~\cite{translation}, where $J$ gate is defined as
\begin{align}
J(\alpha)=
\begin{bmatrix}
1 & \mathrm{e}^{\mathrm{i} \alpha}\\
1 & \fix{-\mathrm{e}^{\mathrm{i} \alpha}}
\end{bmatrix}   
\end{align}
\iffalse
To turn a circuit into its corresponding graph state, it is first compiled to a universal gate set $\left\{J(\theta), CZ\right\}$, where the $J$ gate is defined as:
%simulate the gates is to implement the measurement pattern on a \emph{graph state} whose geometry is determined by the circuit[?]. Similar to cluster states, graph states can also be generated by implementing CZ gates among a bunch of qubits in $\ket{+}$ state. The difference is that it forms only necessary edges in the geometry, instead of a grid with neighboring connectivity. According to the rules in \cite{translation}, a circuit decomposed to the universal gate set $\left\{J(\theta), CZ\right\}$ can be translated to a graph as shown in Fig.~\ref{fig:circuit_translation}, where $J$ gate is defined as
\begin{align}
J(\alpha)=
\begin{bmatrix}
1 & \mathrm{e}^{\mathrm{i} \alpha}\\
1 & \mathrm{e}^{-\mathrm{i} \alpha}
\end{bmatrix}   
\end{align}
\fi
%with the decomposition of an arbitrary single-qubit gates as 
Note that an arbitrary single-qubit gate $U$ can be decomposed into $
U = \mathrm{e}^{\mathrm{i} \theta} J(\alpha)J(\beta)J(\gamma).
$

Figure~\ref{fig:circuit_translation} shows an example of this approach.
On the left is the input circuit and its generated graph state is on the right.
The node $a$ corresponds to the qubit A.
It connects to three nodes as there are three $\rm CZ$ gates connection the qubit A to qubit B, C, and D.
$CZ$ is a Clifford gate so there is no dependency regarding the measurements on node $a$ and node $b_2$, $c_2$, and $c_2$.
There are also single-qubit J gates on qubits and they are represented by nodes $b_1,b_2,b_3$
There will be a measurement order requirement when the $J(\theta)$ gate is non-Clifford and we use directed edges to represent such dependency.
For example, the edge $b_1\rightarrow b_2$ indicates that the measurement basis of $b_2$ may need to be adjusted according to the measurement outcome of $b_1$.
We remark that the generated graph state only contains the necessary coupling structure that is purely derived from the input circuit, so that the qubits and coupling requirements are much smaller compared with the first `Mapping onto Regular Lattice First'.
%In the following sections, we often omit the arrows and explicit measurement bases when not important for our optimization techniques, and they can always be derived from the graph state \cite{translation}.


\textbf{Drawbacks}
Unfortunately, it is not yet known how we can efficiently map the graph state onto an MBQC machine, which usually generate small cluster states on physical qubits with a set of other hardware constraints. There is neither any prior work discussing possible graph transformations that could potentially enabling us to resolve the mismatch between the topology of arbitrary graph states with the fixed topology of the underlying hardware. To this end, our work gives an in-depth analysis of the challenges here and build up the first modular compiler to automate the mapping. 


%It can be observed that the generated graph state

%In the figure, each vertex represents a physical, each edge is generated by applying a CZ between its corresponding vertices. $X$ indicates a $X$-measurement, while $\alpha,\beta,\gamma$, etc. indicate the angles of the equatorial measurements on the qubits, which may also be adaptive according previous measurement outcomes. For example, a circuit as simple as three CNOTs can be translated to a graph as showns in Fig.~\ref{fig:circuit_translation}(a), with a rough correspondence between A and a, B and $b_1,b_2,b_3$, C and $c_1,c_2,c_3$ as well as between D and $d_1,d_2,d_3$. The complex structure in a circuit may result in high-degree vertices in the graph, eg.$a,b_2,c_2,d_2$, leading to a difficult for implementation. Since all gates are Clifford gates, the measurements in the graph does not have dependencies between each other. Adding non-Clifford J gates would induce dependency as shown in Fig.~\ref{fig:circuit_translation}, where we use arrows $q_1\rightarrow q_2$ to indicate that the measurement basis of qubit $q_2$ depends on the measurement outcome of qubit $q_1$. The depedency orders in a general graph can be derived from the \emph{flow} of the graph [?]. 



% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/circuit_translation.pdf}
%     \caption{A placeholder}
%     \label{fig:circuit_translation}
% \end{figure}

\begin{figure}[h!]
    \centering
     \vspace{-5pt}
    \includegraphics[width=\linewidth]{fig/translation.pdf}\\
    \hspace{0pt}(a)\hspace{120pt}(b)
    % \vspace{-15pt}
    \caption{Translation from a circuit (a) to its graph state (b), with the measurement bases labeled on the qubits in (b). The logical quit $A$ corresponds to physical qubit
    a and $B,C,D$ correspond to  $\left\{b_1,b_2,b_3\right\}, \left\{c_1,c_2,c_3\right\}$ and $\left\{d_1,d_2,d_3\right\}$, respectively. Qubits in (b) with `in',`out' or `in/out' are input or output qubits. Arrows such as $b_1\rightarrow b_2$ indicate that the measurements of some qubits depend on the measurement outcomes of other qubits (e.g., $b_2$ depends on $b_1$).}
    \vspace{-5pt}
    \label{fig:circuit_translation}
\end{figure}

\vspace{0.3em}
\subsection{MBQC on Photonics Quantum Hardware}
%This paper focuses on the linear optical quantum computing technology. 
We will introduce some basics about the linear optical quantum computing and the key architectural constraints that need to be considered in the compilation optimization. 
For more details about linear photonics, we recommend~\cite{photonics_review}.

\textbf{Photonic qubits}
In linear optical quantum computing, a qubit is usually implemented by representing the two basis states $\ket{0}_L$ and $\ket{1}_L$ with two optical modes of a fixed photon number. The optical modes can be either two spatial modes ($\ket{0}_L = \ket{1} \otimes \ket{0}$ and $\ket{1}_L = \ket{0} \otimes \ket{1}$, where $\ket{0}$ and $\ket{1}$ are the two basis states in one optical mode), referred as `dual-rail qubits', or two polarization modes of a single qubit ($\ket{0}_L = \ket{H}$ and $\ket{1}_L = \ket{V}$, where $\ket{H}$ and $\ket{V}$ represent the horizontal and vertical polarization of one photon), referred to as `polarization qubits'. 
Those two representations are mathematically equivalent and can be physically switched to each other using polarizing beam
splitters~\cite{photonics_review}. 
Photonic quantum computing does not require an extremely low temperature compared with other quantum hardware technologies\cite{hareware1,hardware2,hardware3,hardware4}, and is potentially highly scalable with the ability of constantly generating a large number of photons.


%\todo{rephrase the picture here}
\iffalse
This is especially advantageous for MBQC as each qubit in MBQC is measured only once and then thrown away or initialized again. Compared to solid state qubits such as superconducting qubits, phontoics qubits naturally favors MBQC for mainly three reasons. First, the weak interactions between photons make it hard to directly implement multi-qubit gates on arbitrary qubit states, while in MBQC the only thing needed is single-qubit measurements with a fixed, initialized cluster states or graph states.
Second, measurements on photons are destructive, meaning that photons will disappear after measurements, however in MBQC, each qubit is measured only once, and is then free to detach from the computing system or even disappear. Third, the low depth of operation (measured only once) on each qubit reduces the requirement for coherence time.
\fi


\textbf{Generating Cluster State}
Large-scale one-way quantum computing requires a large cluster state to be prepared as a resource.
%This is a challenging task because weak interaction between photons makes it difficult to entangle them. 
There are two approaches to entangle photonic qubits and create cluster state upon them. 
One approach is to directly create entangled photons through nonlinear optical devices which induce interactions between photons and effectively lead to a deterministic cluster state generation.
However, such nonlinear systems are difficult to scale\cite{photonics_review,GHZcluster}. 
%One way is to send photons through nonlinear optical devices which induce interactions between photons and effectively lead to a deterministic quantum gate, however such linear nonlinear \todo{what is this linear nonlinear system?} systems are difficult to scale\cite{}. 
%, with a typical size of $O(10)$ qubits~\.
The second approach is to use linear optical devices and photon detectors to realize a special operation, namely fusion, which can merge two cluster states to construct a larger cluster state.
This approach is readily CMOS compatible and easy to scale; nevertheless, it is at the cost of consuming two qubits in the two cluster states to be merged and is not deterministic.
Significantly overhead is required if we need to construct a large cluster state with a high probability.
%implies a large overhead if we require a near unity success probability. 
Thus, recent efforts~\cite{GHZcluster,psiquantum-fbqc} are to take advantages of both methods and reduce their shortcomings by combining them in the following way: A bunch of small entangled states can be generated deterministically using the first approach and then can be fused to construct a large cluster state.

%The other way is to use linear optical devices and photon detectors to realize quantum gates, eg., fusion gates[?], probabilistically. This fusion operation can This approach is readily CMOS compatible and easy to scale; nevertheless, it is not deterministic and implies a large overhead if we require a near unity success probability. 
%Therefore, it is more realistic to take advantages of both methods and reduce their shortcomings by combining them in the following way: A bunch of small entangled states can be generated (almost) deterministically at first and then can be fused to construct a large static entangled state.

\textbf{Fusion}
%Small entangled states can be expanded to large states via fusion gates, which effectively acts as a joint measurement on two qubits. 
% \todo{fusion term: gate or operation;}
The fusion operation~\cite{psiquantum-fbqc, browne2005resource, photonics_review} is a native gate on photonic device that can merge two cluster states through two joint measurement operations on two qubits from the two cluster states.
For example, a joint measurement in the basis of $XX,ZZ$ projects a state to the Bell basis, which creates entanglement between the qubits. The joint measurement we use in this paper is in $XZ,ZX$ basis, which entangles two cluster states into a larger one at the cost of losing two photons. 
In Figure~\ref{fig:fusion_XZ_ZX}, we use fusion operation to merge two two-qubit cluster states $AC$ and $BD$.
After the two joint measurements on qubits $C$ and $D$ are implemented, the two measured qubits are destroyed and the rest qubits $A$ and $B$ are now merged to one cluster state, which is a new two-qubit cluster state. 
In general, when we merge two cluster states with $m$ and $n$ qubits, the final cluster state after fusion will have $m+n-2$ qubits.
Since fusion operations themselves are very costly~\cite{psiquantum-fbqc, browne2005resource} and have the overhead of losing two qubits per fusion, one of the goals in our compiler is to minimize the number of fusion operations. 
\iffalse
Since fusion operations succeeds probablistically and has the overhead of losing two qubits per fusion, one of the goals in our compiler is to minimize the number of fusion operations.
However it is worth mentioning that although fusions are probabilistic, they are heralded \cite{GHZcluster} and can be handled by error corrections along with other errors as claimed by \cite{psiquantum-fbqc}. As an initial research towards the compilation onto photonics MBQC,  %compilation framework, 
error correction design is not taken into account and can be left to the future work.
\fi
\iffalse
For illustration, let's consider the fusion between two two-qubit cluster states~\cite{}. The state of a two-qubit cluster state can be written as $\ket{\psi}=\ket{0+}+\ket{1-}$, since a cluster state can be created by applying CZ gates on a bunch of qubits in $\ket{+}$ state. Implementing a $XZ,ZX$ measurement on two qubits with each qubit from one of them projects the state into a basis of 
\begin{align*}
    &XZ=1,ZX=1: &\ket{0}_2\otimes\ket{+}_3+\ket{1}_2\otimes\ket{-}_3\\ 
    &XZ=1, ZX=-1: &\ket{0}_2\otimes\ket{+}_3-\ket{1}_2\otimes\ket{-}_3\\
    &XZ=-1,ZX=1: &\ket{0}_2\otimes\ket{-}_3+\ket{1}_2\otimes\ket{+}_3\\
    &XZ=-1,ZX=-1: &\ket{0}_2\otimes\ket{-}_3-\ket{1}_2\otimes\ket{+}_3
\end{align*}
determined by the measurement outcome. With qubit 2 and qubit 3 lost after the fusion, qubit 1 and qubit 4 forms a state
% \begin{align*}
%     &\ket{0}_1\otimes\ket{+}_4+\ket{1}_1\otimes\ket{-}_4\\ 
%     &\ket{0}_1\otimes\ket{+}_4-\ket{1}_1\otimes\ket{-}_4\\
%     &\ket{0}_1\otimes\ket{-}_4+\ket{1}_1\otimes\ket{+}_4\\
%     &\ket{0}_1\otimes\ket{-}_4-\ket{1}_1\otimes\ket{+}_4,
% \end{align*}
that is equivalent to $\ket{\psi}$ up to a local $X$ or $Z$ correction.
\fi
%When the initial cluster states are longer than 2, this constructs a larger cluster state of $m+n-2$ qubit, as shown in Fig.~\ref{fig:fusion_XZ_ZX} with $m,n$ being the number of qubits in the small cluster states. Since fusion operations succeeds probablistically and has the over head of losing two qubits per fusion, one of the goals in our compiler is to minimize the number of fusion operations. However it is worth mentioning that although fusions are probabilistic, they are heralded and can be handled by error corrections along with other errors as claimed by [?]. As an initial research towards the compilation onto photonics MBQC,  %compilation framework, 
%error correction design is not taken into account and can be left in the future work.


\iffalse

\textbf{Hardware Architecture} % and Constraints}
This paper adopts the hardware architecture from PsiQuantum~\cite{psiquantum-fbqc}, a leading industry in the area of photonic quantum computing, as shown in Fig.~\ref{fig:device2d}.
This architecture consists of resource state generators (RSG), routers and measurement device. 
A RSG repeatedly produces a copy of small cluster state (e.g., a three-qubit GHZ state~\cite{}) every clock cycle. Without loss of generality, the rest of the paper uses GHZ as the basic RSG state unless otherwise stated.
%, which is called a \textit{resource state}.
%We adopt a hardware model recently proposed by [?], which consists of resource state generators (RSG), routers and measurement device, as shown in Fig.~\ref{fig:device2d}. 
Those small cluster states %  resource states 
are channelled to different measurement locations by the routers. The routing includes spatial routing as well as temporal routing in the form of delay lines.
The spatial routing allows a small cluster state to be fused with cluster states generated by other RSGs.
The temporal routing delay the arrival of photons by some clock cycles so that they can be fused with photons generated later by the same RSG. 
%, which delay the arrival of photons by some clock cycles so that they can be fused with photons generated later by the same RSG. 
% The size of the resource states is typically considered as $\mathit{O}(10)$ since generating large resource states is  exponentially hard.
%\textbf{Architectural Constraints} %However,
%It is conceivable that a global spatial connectivity is hard to realize due to difficulty of hardware routing as the number of RSGs scales up. 
%Therefore, in this paper, we consider that the RSGs formulate a 2D array and each RSG has spatial connection to its neighbors.
%For the temporal routing, note that photons suffer more from the photon loss error as the photon stays longer in the delay line.
%In this paper, we assume a certain temporal distance is constraint, that is, the photons can only stay in the delay line for at most a specific number of cycles.
%Moreover, photons should not be stored in the delay line for too long as it increases the loss rate of photons. In the near-term, it is reasonable to target at realizing adjacent spatial connectivity, and a temporal connectivity between photons routed to the same delay line within a certain temporal distance. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/device2d.jpg}
    \caption{screenshot, \textcolor{red}{to be modified} \yuke{Add the "Note that ``RSG'' means XXX, ``F'' means XXX"} \todo{Yufei: can remove this figure if space is limited}}
    \label{fig:device2d}
\end{figure}
\fi




 
% Large-scale one-way quantum computing requires a large entangled state to be prepared as a resource. However the non-linearity effects required for deterministically generating entanglements between photons make it difficult to scale. Instead, it is more realistic to generate a bunch of small entangled states (almost) deterministically and construct a large entangled state via \emph{fusion} operations in linear optics. A fusion operation is a two-qubit joint measurement that succeeds probablistically with a herald if it fails. On success, a fusion entangles two small cluster states into a larger one at the cost of losing two qubits, as shown in Fig.~\ref{fig:fusion_XZ_ZX}. Due to the non-determinism of fusion operations, we want to minimize the number of fusion operations. However it is worth mentioning that although fusions are probabilistic, they can be handled by error corrections along with other errors as claimed by [?]. As the first compilation framework, we do not take error correction design into account in this paper.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.6\linewidth]{fig/fusion_XZ_ZX.pdf}
    \caption{A fusion between cluster states $AC$ and $BD$. After the fusion (a $XZ,ZX$ measurement on $C,D$), qubit $C,D$ vanish and qubit $A,B$ form a new cluster state.}
    \label{fig:fusion_XZ_ZX}
\end{figure}




==> 03_background_v0.tex <==
\section{Background}
\subsection{Photonic Quantum Computing}
\paragraph{Qubit in Linear Optics} A classical bit is the basic unit of information in classical computing whose value is either `0' or `1'. In quantum computing, a quantum bit or qubit is an analog of the classical bit whose state can be a superposition of two basic states $\ket{0}$ and $\ket{1}$, represented by $\ket{\Psi}=\alpha\ket{0}+\beta\ket{1}$ where $\alpha,\beta\in \mathbb{C}$ and $\norm{\alpha}^2+\norm{\beta}^2=1$. We say two qubits are entangled if their states $\ket{\Psi}=\alpha_{00}\ket{00}+\alpha_{01}\ket{01}+\alpha_{10}\ket{10}+\alpha_{11}\ket{11}$ where $\ket{ab}=\ket{a}\otimes\ket{b}$ can not be decomposed to a tensor product of two single-qubit states $\ket{\psi_1}\otimes \ket{\psi_2}$. In linear optical quantum computing, a qubit is usually implemented by representing $\ket{0}$ and $\ket{1}$ with two optical modes, either two spatial modes or two polarization modes, of a single qubit. We refer to the qubits represented by spatial modes as `dual-rail qubits', and the ones represented by polarization modes as `polarization qubits'. Those two representations are mathematically equivalent and can be physically switched to each other using polarizing beam splitters~\cite{photonics_review}.

\paragraph{Fusion in Linear Optics}
 As mentioned earlier, we use fusion-based approach to generate arbitrary graph states. A fusion gate acts on two qubits and  project them onto a \emph{symmetric} Bell state, i.e., $\ket{00}\pm \ket{11}$. We use a slightly different Bell basis $\ket{+0}\pm \ket{-1}$ which corresponds to measuring the stabilizers $X_1Z_2$ and $Z_1X_2$ and can be obtained by applying a Hadamard gate to one the qubits prior to a symmetric Bell state measurement.  \textcolor{orange}{@Hassan: The fusion operation we use in this paper is XZ,ZX measurement, not Bell measurement XX, ZZ.}\HS{fixed.}
The general idea here is to stitch together two smaller graph states (i.e., entangle them) by performing fusion gates on two qubits one from each graph.
In the dual-rail encoding, fusion gates can be realized by two beam splitters, and the projected state is determined by the pattern in the measurement outcome. Such fusion gates in linear optics are non-deterministic and has a success probability of $50\%$, which can be improved by including ancilla Bell pairs or concatenating with a quantum code such as $[[4,1,2]]$ code (a.k.a.~$(2,2)$-Shor code). 
Quantum error correcting codes may be developed to account for unsuccessful fusion events~\cite{psiquantum-fbqc}.
However, in this work we neglect the probabilistic nature of these gates for simplicity and postpone it to a future work.

\subsection{One-Way Quantum Computing}
%https://arxiv.org/pdf/0704.1736.pdf: Note that since classical computation is cheaper than quantum computation, one might consider MBQC as a favourable ultimate architecture for a quantum computer as it keeps the quantum and classical depth separate \yuke{this paragraph looks strange, why need this paragraph, also MBQC is undefined.}


\paragraph{One-Way Model}
The one-way measurement model is a framework for universal quantum computation, first proposed by [?][?], in which algorithms are partially described by a graph G of entanglements on a collection of qubits. Transformations of quantum states in the one-way measurement model are essentially described by a sequence of single-qubit measurements performed on the entangled system, which is called a \textit{graph state}. An \textit{open graph state} includes \textit{input qubits} $\mathit{I}$ and a collection of auxiliary qubits prepared in the $\ket{+}=\ket{0}+\ket{1}$ state. Those are operated on by a collection of entangling operations, described by a graph G. After the sequence of measurements, any qubits left unmeasured are interpreted as \textit{output qubits} $\mathit{O}$.


\paragraph{Graph State}
A \textit{graph state} $\ket{\phi\left\{\kappa\right\}}_G$ of a graph $G(V,E)$ is defined by a set of eigenvalue equations \[
\sigma_x^{(a)}\bigotimes_{b\in V}\left(\sigma_z^{(b)}\right)^{\Gamma_{ab}}\ket{\phi\left\{\kappa\right\}}_G = (-1)^{\kappa_a}\ket{\phi\left\{\kappa\right\}}_G
\] where $\Gamma_{ab}=1$ if $a$ and $b$ \yuke{what is a and b?} are connected via and edge $e\in E$, and $\Gamma_{ab}=0$ otherwise. If the graph $G$ is a square lattice in 2D or a simple cubic lattice in 3D, then the particular graph state described by $G$ is referred to as a \textit{cluster state}. If the graph state contains two possibly overlapping subsets $I$ and $O$ which are specified as inputs and outputs, then the graph state is called an \textit{open} graph state. A graph state with all $\kappa_a=0$ can be generated as follows.
\begin{enumerate}
    \item Prepare all the vertices in $\ket{+}$ state, except the input qubits as $\ket{\psi}$
    \item For each qubit, entangle it with all its neighbors via controlled-Z operator
\end{enumerate}
As graph states with different eigenvalues are orthogonal, a graph state can be uniquely represented by its eigenvalue. It is worth mentioning that all $\phi\left\{\kappa\right\}$ are equally good for computation $\left\{\kappa\right\}$...We can remove a vertex from the graph by measuring the corresponding qubit in the $Z$ basis. Although the randomness in the measurement outcome may change the eigenvalue set, it is equivalent to the target graph state up to a local unitary, which can be absorbed to the basis change of qubit measurements.

\paragraph{Measurement Pattern} In one-way model, computations are presented as \textit{measurement patterns}, which are sequences of commands acting on the qubits in the patter. %A \textit{measurement pattern} is defined by the choice of $\mathit{V}$ a finite set of qubits, two possibly overlapping subsets $I$ and $O$ determining the pattern inputs and outputs, and a finite sequence of commands acting on $V$. 
The command are of four types i) 1-qubit preparations $N_i^\alpha$ which prepares qubit $i$ in state $\ket{+_\alpha}:=\ket{0}\pm\mathrm{e}^{i\alpha}\ket{1}$, ii) 2-qubit entanglement operators $E_{ij}:=\land Z_{ij}$ (controlled-Z) on qubit $i,j$, iii) 1-qubit measurement $M_i^\alpha := \ket{\pm_\alpha}\bra{\pm_\alpha}$ on qubit $i$ where $\alpha\in[0,2\pi)$ and iv) 1-qubit Pauli corrections $X_i, Z_i$ on qubit $i$ which are usually propagated to the end and applied only on output qubits. In order to obtain universality, there is a classical control mechanism, called \textit{feed-forward}, that allows measurement and correction commands to depend on the results of previous measurements. %If the commands are in the order of preparation, entanglement, measurement and correction, 
If all the preparation $N_i$ and entanglement operators $E_{ij}$ appear first in its command sequence, followed by measurements and finally corrections, then the pattern it is called a \textit{standard} pattern, otherwise it is called a \textit{wild} pattern. Any wild pattern can be \textit{standardized} to a unique standard form [?calculus] by applying \textit{rewrite rules} for each qubit, noting that measurements, corrections and entanglement commands on disjoint sets of qubits commute pairwise.


\paragraph{Measurement Dependency}
A quantum circuit can be translated to a measurement pattern with \textit{flow} using the rules in \cite{translation}. A flow $(f, \preceq)$ for a geometry $(G,I,O)$ consists of a map $f:O^c\rightarrow I^c$ and a partial order $\preceq$ over $V$ \textcolor{red}{(def)} such that $\forall x\in O^c$:
\begin{align*}
    &(i)x\sim f(x);\\
    &(ii)x\preceq f(x);\\
    &(iii) y\sim f(x), x\preceq y
\end{align*}
where $\sim$ denotes that $x,y$ are neighbors in $G$, and $\preceq$ is called a \textit{dependency order} induced by $f$. In such a pattern, when qubit $i$ is measured, $f(i)$ receives a $X_{f(i)}^{s_i}$ correction, while all the neighbors $k$ of $f(i)$ except $i$ receive a $Z_k^{s_i}$ correction. Formally, if a geometry $(G,I,O)$ has a flow, then the pattern\[
\mathcal{P}_{f,G,\vec\alpha} := {\prod_{i\in O^c}}^\preceq \left(X_f(i)^{s_i}\prod_{\stackrel{k\sim f(i)}{ k\neq i}} Z_k^{s_i}M_i^{\alpha_i}\right)E_G
\]
deterministically realizes the unitary embedding\[
U_{G,I,O,\vec\alpha} := 2^{|O^c|/2}\left(\prod_{i\in O^c} \bra{+_{\alpha_i}}_i\right)E_G
\] 
It is worthing mentioning that measurements in $X$ or $Z$ basis are not affected by those corrections...





==> 03_related_work.tex <==

\section{Background} 
%\label{sect: Related Works}

%\todo{Gushu: please add a sentence and reference for quantum basics}
\iffalse
\subsection{Quantum Error Correction}
%The quantum computers work in an analog manner and are fragile without error correction.
The quantum computers are fragile without error correction.
The information stored in qubits can be easily distorted due to the interaction with the environment~\cite{}. 
The imprecise quantum operation~\cite{} and erroneous quantum measurement~\cite{} further worsen the situation. 
To enable the fault-tolerant quantum computation, various Quantum Error Correction (QEC) codes~\cite{} are proposed.
In general, QEC codes use redundant physical qubits to create a code space where encoded quantum states or logical qubits are protected with redundant information. 
More redundancy will increase the error tolerance and result in a larger code distance.
The state of all physical qubits are divided into two orthogonal subspaces, \todo{the
Once the qubits state is in the wrong subspace due to any error, a measurement (a.k.a. syndrome measurement) in the QEC protocol} would either project the state back to the correct subspace or detect the error so that follow-up correction operations can be applied.
%Like in classical error correction, 
%The subspace $H_L$ of encoded logical qubits is orthogonal to the subspace $H_R$ of redundant information and these two subspace together constitute the whole code space defined by physical qubits.
% error state will have components in both subspace and can be detected immediately.
%Corrupted logical states that deviate from logical subspace $H_L$ can be immediately detected and corrected with redundant information in $H_R$.
%Corrupted logical states have non-zero projection in $H_R$ and thus can be detected upon measurement and then corrected immediately.

%\subsection{Fault-tolerant Quantum Computation}

%The unit of information in quantum computation is a qubit. The quantum
%state of a qubit is a probabilistic superposition of basis states $|0\rangle$ and $|1\rangle$.
%The state of a qubit can be manipulated by quantum gates or unitary operators. Single-qubit Pauli operators $\{X, Y, Z\}$ are among the most commonly used unitary operators. Pauli operators on $n$ qubits, e.g. $\otimes_{i=1}^n X_i$, are constructed by taking the tensor product of single-qubit Pauli operators. We often omit the tensor product operator in $n$-qubit Pauli operators for simplicity. Pauli operators can describe not only quantum operations but also quantum measurement. For example, a $Z$-type quantum measurement projects the state of a qubit into $|0\rangle$ or $|1\rangle$, which are both eigenstates of Pauli $Z$ operator.

% TODO:
% Pauli operators;
% Logical qubit in Hilbert space;
% Stabilizer;
% Code distance;

%Quantum computation is fragile without error correction. Information in qubits can be easily distorted by the interaction with the environment. The imprecise quantum operation and erroneous quantum measurement further worsen the situation. To ensure the fault-tolerant quantum computation, various QEC codes are proposed.
%QEC codes use redundant physical qubits to create a code space where encoded quantum states or logical qubits are protected with redundant information. More redundancy will increase the error tolerance and result in a larger code distance $d$.
%Like in classical error correction, the subspace $H_L$ of encoded logical qubits is orthogonal to the subspace $H_R$ of redundant information and these two subspace together constitute the whole code space defined by physical qubits.
% error state will have components in both subspace and can be detected immediately.
%Corrupted logical states that deviate from logical subspace $H_L$ can be immediately detected and corrected with redundant information in $H_R$.
%Corrupted logical states have non-zero projection in $H_R$ and thus can be detected and corrected immediately.


% \textbf{Stabilizer formalism}: the stabilizer of a quantum error correction code.
% The basic idea of the stabilizer formalism is that many quantum states can be more easily described by working with the operators that stabilize them than by working explicitly with the state itself.
% In QEC code, quantum states of data qubits are better described by stabilizers rather than the state-vector.
\fi
%\label{sect: surface code basics}
% TODO: why choose surface code? surface code is good
% TODO list
% 1. data qubit and measurement qubit
% 2. stabilizer and its measurement
%In this paper, we will focus on the surface quantum error correction code~\cite{} as surface code family provides one of the highest error tolerance threshold~\cite{} and is relatively hardware-friendly~\cite{}.
%Surface code family provides one of the highest error tolerance threshold~\cite{} and is relatively hardware-friendly~\cite{}. 
In this section, we introduce some key concepts for understanding the implementation requirements of surface code~\cite{bravyi1998quantum,dennis2002topological,barends2014superconducting}. 
%In this section, we introduce the necessary background %about quantum error correction, especially the
%surface code and the related hardware constraints on superconducting quantum circuit technology. 
We do not cover the basics of quantum computing and recommend~\cite{nielsen2002quantum} for reference.


\begin{figure}[ht]
% \vspace{-5pt}
    \centering
    \includegraphics[width=\linewidth]{fig/surfgrid1.pdf}
    \caption{Common components of surface codes. (a) Surface code lattice with data qubits represented by blue circles and syndrome qubits by red circles. (b) Z-type syndrome extraction circuit. (c) X-type syndrome extraction.}
    \label{fig:surf_grid}
% \vspace{-8pt}
\end{figure}

\textbf{Data and syndrome qubits:}
Surface codes encode logical qubit information in a two-dimensional lattice of physical qubits, as shown in Figure~\ref{fig:surf_grid}(a). Physical qubits in the code lattice can be divided into two types: data qubits and syndrome qubits (represented as blue and red circles respectively, see Figure~\ref{fig:surf_grid}(a)).
The information is encoded in the data qubits while the syndrome qubit will extract error information from their neighboring data qubits. % with syndrome extraction circuits.


\textbf{Pauli Operator and Stabilizer:} In stabilizer codes, one uses products of Pauli operators to represent the correlations among data qubits that are measured using the syndrome qubits. 
For the surface code, and avoiding boundary considerations, each correlation operator is the product of four Pauli operators $X$ or $Z$ and this is visualized in Figure~\ref{fig:surf_grid}(a) by labeling the edge connecting a syndrome qubit to its relevant data qubits with either $X$ or $Z$.
There are two patterns of connections between syndrome and data qubits.
The first one (Z-type) is shown in Figure~\ref{fig:surf_grid}(b). The connections between the center syndrome qubit and the four data qubits are all labeled by the $Z$ operators and represented by the Pauli string $Z_aZ_bZ_cZ_d$.
The second one (X-type) in Figure~\ref{fig:surf_grid}(c) is similar but all connections are labeled by the $X$ operators and represented by the Pauli string $X_aX_bX_cX_d$.
For these two different patterns, we will have corresponding syndrome measurement circuits to detect errors in the data qubits (shown on the right of Figure~\ref{fig:surf_grid}(b) and (c)).
Basically the syndrome extraction circuits project the state of data qubits $\{a,b,c,d\}$ into the eigenstates of the corresponding Pauli strings.
In the context of QEC, the specific Pauli strings that one measures are called \textit{stabilizers}~\cite{gottesman1996class} and the syndrome extraction circuits are also known as \textit{stabilizer measurements} ~\cite{ calderbank1997quantum}.
Without ambiguity, we use the stabilizer notation to represent a syndrome extraction. And we denote the stabilizer $Z_aZ_bZ_cZ_d$ ($X_aX_bX_cX_d$) with $Z_{abcd}$ (respectively $X_{abcd}$) for simplicity.


\textbf{Error Detection:} Surface code can detect Pauli X- and Z-errors on data qubits by using Z- and X-type stabilizer measurement circuits, respectively. 
\iffalse
To give a concrete example for illustration, we assume the state of all data qubits is initialized into the simultaneous +1 eigenstate of all stabilizers, i.e., for the quantum state $|\phi_{abcd}\rangle$ of data qubits $\{a,b,c,d\}$, $Z_{abcd}|\phi_{abcd}\rangle = X_{abcd}|\phi_{abcd}\rangle = |\phi_{abcd}\rangle$. If an Pauli $X$ error happens on data qubit $a$, the error state $X_{a}|\phi_{abcd}\rangle$ will become a -1 eigenstate of $Z_{abcd}$ since $Z_{abcd}X_{a}|\phi_{abcd}\rangle = -X_{a}Z_{abcd}|\phi_{abcd}\rangle = -X_{a}|\phi_{abcd}\rangle$. As a result, the measurement of $Z_{abcd}$ will return -1, contrasting to +1. Similarly, a Pauli Z error on data qubit $a$ will flip the measurement result of $X_{abcd}$. 
\fi
By gathering all such stabilizer measurement results, a surface code error detector can infer which errors occurred in the lattice and consequently apply the corresponding correction. Further details of surface code error detection and correction can be found in \cite{fowler2012surface}.


\begin{figure}[ht]
% \vspace{-5pt}
    \centering
    \includegraphics[width=\linewidth]{fig/surflogi2.pdf}
    \caption{Code distance and compact lattice. (a)  Surface code logical operations with distance 3. (b) Inside the rotated rectangle (dashed brown line) is a compact surface code lattice with same code distance.}
    \label{fig:surf_logi}
% \vspace{-8pt}
\end{figure}

\textbf{Code Distance:} The error correction ability of QEC codes is measured by their code distance~\cite{knill2000theory,calderbank1996good}. The code distance is defined to be the minimum number of physical qubits in the support of logical X or Z operations on the encoded qubit
(denoted by $X_L$ or $Z_L$ in Figure~\ref{fig:surf_logi}). 
Figure~\ref{fig:surf_logi} (a) shows logical operations in a distance-3 surface code. It is possible to obtain a more compact surface code lattice without changing the code distance, as shown in Figure~\ref{fig:surf_logi}(b).
Code distance is an important property since it relates to the number of one-qubit errors that can be corrected. It provides a good quantity to express the expected performance of the surface codes we synthesize for superconducting devices in later sections.

%ly quantum operations but also quantum measurement. For example, a $Z$-type quantum measurement projects the state of a qubit into $|0\rangle$ or $|1\rangle$, which are both eigenstates of Pauli $Z$ operator.



%Data qubits encode logical qubits while syndrome qubits extract error syndromes from their neighboring data qubits with Z- and X-type syndrome extraction circuits. 
%Figure~\ref{fig:surf_grid}(b) and (c) give examples about Z- and X-type syndrome extraction circuits with four data qubits. Syndrome extraction circuits on the boundaries of the code lattice can be depicted in the same way but only with three data qubits.

%The state of a qubit can be manipulated by quantum gates or unitary operators. Single-qubit Pauli operators $\{X, Y, Z\}$ are among the most commonly used unitary operators. Pauli operators on $n$ qubits, e.g. $\otimes_{i=1}^n X_i$, are constructed by taking the tensor product of single-qubit Pauli operators. We often omit the tensor product operator in $n$-qubit Pauli operators for simplicity. Pauli operators can describe not only quantum operations but also quantum measurement. For example, a $Z$-type quantum measurement projects the state of a qubit into $|0\rangle$ or $|1\rangle$, which are both eigenstates of Pauli $Z$ operator.

%Among various quantum error correction codes, surface code family provides one of the highest error tolerance threshold and has been widely utilized and studied. 
%Surface codes encode logical qubit information in a two-dimensional lattice of physical qubits, as shown in Figure~\ref{fig:surf_grid}(a). Physical qubits in the code lattice can be divided into two types: data qubits (blank circles in Figure~\ref{fig:surf_grid}(a)) and syndrome qubits (solid circles). Data qubits encode logical qubits while syndrome qubits extract error syndromes from their neighboring data qubits with Z- and X-type syndrome extraction circuits. Figure~\ref{fig:surf_grid}(b) and (c) gives examples about Z- and X-type syndrome extraction circuits with four data qubits. Syndrome extraction circuits on the boundaries of the code lattice can be depicted in the same way but only with three data qubits.
%Specifically, Z-type measurement qubits (surrounded by `Z' in Figure~\ref{fig:surf_grid}(a)) and X-type measurement qubits (surrounded by `X') are used to extract Pauli X errors and Pauli Z errors,  respectively.

% why this paragraph is necessary
% \textbf{Stabilizers of surface codes}: 
% Measurements in Z- and X-type syndrome extraction circuits project the state of data qubits $\{a,b,c,d\}$ into the eigenstate of Pauli operators $Z_aZ_bZ_cZ_d$ and $X_aX_bX_cX_d$, respectively. Such Pauli operators are termed `stabilizers' in  literature. 
%All measurements in the lattice collectively stabilize the state of all data qubits in a simultaneous eigenstate of corresponding stabilizers. 
% Due to the connection between syndrome extraction circuits and stabilizers, syndrome extraction is also called stabilizer measurement. To measure a stabilizer, we first need to construct the syndrome extraction circuit and then execute it. The measurement outcome of a stabilizer usually refers to the measurement outcome of the syndrome qubit in the corresponding syndrome extraction circuit. In following sections, we use the stabilizer notation to represent a syndrome extraction. And we denote the stabilizer $Z_aZ_bZ_cZ_d$ ($X_aX_bX_cX_d$) with $Z_{abcd}$ (resp. $X_{abcd}$) for simplicity.


% For simplicity, we denote the stabilizer $Z_aZ_bZ_cZ_d$ ($X_aX_bX_cX_d$) with $Z_{abcd}$ (resp. $X_{abcd}$), and say that the syndrome extraction circuit in Figure~\ref{fig:surf_grid}(b) (resp. (c)) measures $Z_{abcd}$ (resp. $X_{abcd}$). Stabilizer measurement is also called syndrome extraction in literature.

% error detection introduction
% stress the meaning of stabilizer measurement
%Surface code can detect Pauli X- and Z-errors on data qubits by using Z- and X-type syndrome circuits, respectively. To show in detail, we assume the state of all data qubits is initialized into the +1 eigenstate of all stabilizers, i.e., for the quantum state $|\phi_{abcd}\rangle$ of data qubits $\{a,b,c,d\}$, $Z_{abcd}|\phi_{abcd}\rangle = X_{abcd}|\phi_{abcd}\rangle = |\phi_{abcd}\rangle$. If an Pauli $X$ error happens on data qubit $a$, the error state $X_{a}|\phi_{abcd}\rangle$ will become a -1 eigenstate of $Z_{abcd}$ since $Z_{abcd}X_{a}|\phi_{abcd}\rangle = -X_{a}Z_{abcd}|\phi_{abcd}\rangle = -X_{a}|\phi_{abcd}\rangle$. As a result, the measurement of $Z_{abcd}$ will return -1, contrasting to +1. Similarly, a Pauli Z error on data qubit $a$ will flip the measurement result of $X_{abcd}$. By gathering all such stabilizer measurement results, a surface code error detector can locate errors occurred in the lattice, and correct them correspondingly. Further details of surface code error detection and correction can be found in \cite{}.

% define code distance
%The error correction ability of a surface code is measured by its code distance~\cite{}. The code distance is defined to be the minimum number of data qubits for defining logical $X_L$ or $Z_L$. However, definitions of logical operations vary with surface codes. Figure~\ref{fig:surf_logi} (a) and (b) show logical operations on a planar surface code and a double-defect surface code. Planar surface code uses the whole lattice to encode a single logical qubit while double-defect surface code create logical qubits by introducing holes (or `defects') in the lattice. Both Surface codes in Figure~\ref{fig:surf_logi} are of distance-3. % meaningless statement
%Code distance is an important property of surface codes, and is used for measuring the quality of the synthesized surface code on superconducting devices in later sections.

% code distance --> boundary --> logical operation --> figure
% code distance
% a quick statement of double defect code;



% introduce details up to stabilizer circuit.
% Intuitively, surface codes are so fault tolerant because they employ a “soft decoding” scheme in which error syndromes are measured and recorded over an extended time period, and then a minimum-weight perfect-matching algorithm [25] is used to identify errors after the fact (and then the errors are post-corrected due to commutativity of the correction operations).

% TODO: introduce the distance concept

% drawing graphs for surface code.

%As discussed previously, detecting bit-flips and phase-flips is sufficient to correct arbitrary qubit errors. Therefore, ancillas are alternately designated as those that measure bit-flip syndromes and those that measure phase-flip syndromes from their surrounding data (shown as orange and blue interactions in Figure 1). By recording a history of syndrome measurements, we are able to detect (in classical software) anomalous syndromes and trace their cause to specific qubit corruptions.
\iffalse
\subsection{Superconducting Technology}
% todo: emphasize we cannot create the 2d grid as in surface code;
\todo{add a connectivity constraint figure}

% second paragraph: superconducting for fault tolerant
The low error rates and fast operation speed of superconducting qubits make it an ideal platform for implementing surface codes that require high-fidelity quantum operations and short stabilizer measurement latency to detect data qubit errors in time. 
\textbf{However, the surface code lattice and stabilizer measurement circuits cannot be mapped to superconducting devices directly due to the connectivity constraints of such devices.} 
% provide some evidence for constraints; stress we mainly use connectivity constraints; reference: ibm device, hexagon architecture, ...., 
\iffalse
\begin{figure}[ht!]
    \centering
    \includegraphics[width=\linewidth]{fig/datalayout_0.pdf}
    \caption{ Device coupling graph of IBM's superconducting devices: graph nodes represents qubits, and edges denotes the physical connections between qubits.}
    \label{fig:ibm_devices}
\end{figure}
\fi


Figure~\ref{} shows us two IBM superconducting devices. Each qubit in such superconducting devices can only connect to its neighboring qubits due to the routing constraints of planar superconducting devices. For example, as shown in Figure~\ref{fig:ibm_devices}(a), qubit $Q_0$ is connected to $Q_1$ and $Q_5$ but not to $Q_{10}$, which means the CNOT gate cannot be directly applied on the qubit pair $\{Q_0, Q_{10}\}$ as on $\{Q_0, Q_1\}$ and $\{Q_0, Q_5\}$. The average degree of IBM device coupling graph is usually kept low ($< 4$) to 
avoid frequency collision and 
reduce the effect of the crosstalk error~\cite{}.

The limited connectivity in superconducting devices complicates the mapping of surface code lattice in Figure~\ref{fig:surf_grid}. On many superconducting devices, we do not have enough four degree nodes (qubits) to map the syndrome qubit which connects to four data qubits. In such cases, extra work is required to map the stabilizer measurement circuit of surface code lattice.

% On the other hand, with the crosstalk error, it's unlikely that a physical qubit connects to many other qubits. Thus, extra work is required to map a stabilizer circuit, in which the measurement qubit interacts with 4 data qubits, to a superconducting device when we cannot find more than 4-degree qubits in the device coupling graph. We will discuss this problem further in Section xxx.
% \todo{frequency collision, crosstalk, }

%In this work, we focus on superconducting technology, and propose a general framework to synthesize surface code on superconducting devices.

% benefits:
% 1. the ability to easily address and control the system’s many qubits
% 2. operations with high fidelity
% 3. accommodate large numbers of stable qubits
\fi

==> 04_motivation_0723.tex <==


\section{Problem Formulation}



In this section, we first formulate the hardware abstraction of a linear photonics quantum computer and then introduce the compilation challenges that will be tackled in this paper.
%the the problem of synthesizing graph states with small cluster states \textcolor{red}{(def)}, and then discuss the challenges in it.


\subsection{Hardware Abstraction}

%We create for the first time
We first create a formal hardware model abstraction for photonics based quantum devices []. We name it Temporal-spatial hierarchy coupling graph, as shown in Figure~\ref{}.




It can be regarded as an extension of the coupling group abstraction [] prevailing used for today’s superconducting and ion trap hardware architectures. 
This abstraction also helps us to relate the quantum compilation intensively studied recently [] with many new problems studied in the photonics context. 




%+ also highlight different physical layer here. 

Despite the similarity with the quantum hardware coupling graph, we still emphasize on their differences and our high level insights behind such an extended, more complex abstraction.
\begin{enumerate}
    \item First, we turn 3D temporal-spatial 3D -> 2D
Delay line → active layers simulatousy → containsts in the mapping. 
First, the 3D structure is composed of a series of 2D physical layers coming out constantly in the time axis. The photons in the physical layers can live in the delay line for an amount of time before they disappear. However due to the limit of the length of delay lines, only a limited number of physical layers can be active simultaneously, leading to a hardware constraint on the mapping.
\item Hierarchical coupling: within each RSG it is determined by the the RSG generator. Among RSG node it is determined by the the fusion device; GHZ line , RSG
Within each physical layer, the resource states are generated by resource state generators (RSG) sitting on fixed locations. Resource states generated from different RSGs can be routed to fusion devices by routers, whose structure determines the spatial connectivity. Resource states generated by the same RSG but at different times also have connections, because early resource states can be delayed before being routed to fusion devices.
\item We remark that different levels of coupling are not independent of each other, and actually their inteplay could create some additional constraints. For example, suppose we have a GHZ state (three qubits) as the our RSG state, then even when the fusion device allows a RSG to maximally connect to 6 other RSGs (4 spatial neighbors (up, down, left, right) + 2 temporal neighbors (future, previous)), only 3 of them can be simultaneously activated. 
\item To distinguish between different coupling edges, we thus often draw the coupling among qubtis within a RSG with a solid edge (suggest: flattened edge), while those connected by fusion with a blurred, flattened edge (suggest: solid edge) when they are activated.
\end{enumerate}

%1) First, we turn 3D temporal-spatial 3D -> 2D
%Delay line → active layers simulatousy → containsts in the mapping. 
%First, the 3D structure is composed of a series of 2D physical layers coming out constantly in the time axis. The photons in the physical layers can live in the delay line for an amount of time before they disappear. However due to the limit of the length of delay lines, only a limited number of physical layers can be active simultaneously, leading to a hardware constraint on the mapping.

%2) Hierarchical coupling: within each RSG it is determined by the the RSG generator. Among RSG node it is determined by the the fusion device; GHZ line , RSG
%Within each physical layer, the resource states are generated by resource state generators (RSG) sitting on fixed locations. Resource states generated from different RSGs can be routed to fusion devices by routers, whose structure determines the spatial connectivity. Resource states generated by the same RSG but at different times also have connections, because early resource states can be delayed before being routed to fusion devices.

%3) We remark that different levels of coupling are not independent of each other, and actually their inteplay could create some additional constraints. For example, suppose we have a GHZ state (three qubits) as the our RSG state, then even when the fusion device allows a RSG to maximally connect to 6 other RSGs (4 spatial neighbors (up, down, left, right) + 2 temporal neighbors (future, previous)), only 3 of them can be simultaneously activated. 
%4) To distinguish between different coupling edges, we thus often draw the coupling among qubtis within a RSG with a solid edge (suggest: flattened edge), while those connected by fusion with a blurred, flattened edge (suggest: solid edge) when they are activated.

In this work, we focus on GHZ based RSG as it represents our state-of-art (not sure) hardware development. but our optimization are largely general and can be extended to other general cluster states if produced by RSG.




%We create for the first time a formal hardware model abstraction for photonics based quantum devices []. We name it Temporal-spatial Hierarchy Coupling Graph (TSHGraph) (as shown in Fig.~\ref{fig:connectivity2d}). It can be regarded as an extension of the coupling group abstraction [] prevailing used for today’s superconducting and ion trap hardware architectures. This abstraction also helps us to relate what we have intensively studied in the last few years [] with many new problems studied in the photonics context. We also remark that TSHGraph features several unique properties that is missing in standard quantum coupling graph. We next highlight our key insights behind such an extended, more complex abstraction.

%First, 


\subsection{Problem Formulation}
\yuke{usually start with ``In this section, we formulate the problem XXX as XXX''}A 2d-array of RSGs generates a 3d-grid of resource states with time being the third dimension. The combination of spatial and temporal routing enables the connectivity between any resource state and all its neighbors. To look at it in a low dimension, an equivalent way to represent the connectivity is by having a 2d-grid of resource states with adjacent connectivity as well as some long range connectivity, which we refer to as a \textit{connectivity graph}. 

As shown in Fig.~\ref{fig:connectivity2d}. Each red box stands for a resource state, with the time and RSG from which it is generated marked inside. In this example, the six RSGs form a 2x3 array. During each clock cycle, eg. $t_0, t_1$ or $t_2$, the RSGs generate a layer of resource states, which we refer to as a \textit{physical layer}. Note that physical layer $t_1$ is in a reverse order of physical layer $t_0$. The reason we arrange them in this way is to make every resource state connected to all its neighbors in the representation so that we do not need to consider the boundary effect\yuke{Add more detailed explaination to this effect or add citation or reference}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/connectivity2d.pdf}
    \caption{2d connectivity graph \yuke{I suggest using different color for different RSG while circling out the group of RSG by time steps}}
    \label{fig:connectivity2d}
\end{figure} 

With this representation, the compilation problem is then formulated as assigning each qubit of each resource state an operation, either measure, fusion, delay or throw away, according to the connectivity structure so that i) the qubits assigned `measure' operation form the graph state \textcolor{red}{(more clear?)} through fusion and ii) the time order of the qubits assigned `measure' operation satisfy their dependency relation.

\subsection{Challenges}
With the compilation problem formulated, we then talk about the challenges of resolving it.

\textit{Operation Order:}
%\textcolor{red}{i)  A-B, C-D: B-C fusion (A-D entanglement) commute with A measurement?} \textcolor{red}{ii) fusion: adjust basis according to collapsed state?} \textcolor{red}{iii)How many layers in advance?}
In one-way quantum computing, dependent corrections resulting from the non-determinism in quantum measurements play a key role in ensuring universality. %While in a standard pattern, dependency comes only from the non-determinism of single-qubit measurements, in the scheme of real-time synthesis, the fusion operations add a new type of dependency between single-qubit measurements and fusions.
In the scheme of real-time synthesis, the non-determinism in fusion outcomes adds more complexity.
Because now we need to consider not only the dependency between single-qubit measurements, but also the dependency between single-qubit measurements and fusion operations. As an example, Fig.~\ref{fig:fusion_dependency} shows a simple pattern on a 4-qubit linear graph state\yuke{explain the meaning of A ,B, C, D}. As shown in Fig.~\ref{fig:fusion_dependency}(a), if we implement it in a standard form, i.e. first prepare all qubits and entangle them and then do the measurements, then the measurement outcome of $M_\alpha$ leads to a correction on qubit $B$, and the measurement outcome of $M_\gamma$ leads to a correction on qubit $C$, resulting a dependency $A\rightarrow B\rightarrow C \rightarrow D$. However, if the graph state needs to be generated from two GHZ states as shown in Fig.~\ref{fig:fusion_dependency}(b), then the outcome of fusion between qubit $F_1$ and qubit $F_2$ also leads to corrections on both qubit $B$ and qubit $C$, resulting in another dependency $F\rightarrow \left\{B,D\right\}$. %Therefore, when scheduling the execution of a pattern, we need to take care of the dependency to make sure that a qubit should be measured only if all the single-qubit measurements and fusions that it depends on are completed.
That means measurements on qubits in the ${i+1}^\mathrm{th}$ dependency layer depends not only on the $i^\mathrm{th}$ layer\yuke{explain the meaning of layer here}, but also on the fusion between the $i^\mathrm{th}$ and $i+1^\mathrm{th}$ layers, while the $i^\mathrm{th}$ layer depends on the fusion as well. Meanwhile, the dependency may result in a long waiting period for some qubits. Since there is a limit for the delay time, we have to refresh those qubits before they expire.
%which causes more complexity in scheduling, especially when two neighboring qubits are in the $i^\mathrm{th}$ and $i+n^\mathrm{th}$ dependency layers where $n>1$.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{fig/dependency.pdf}
    \caption{Fusion dependency}
    \label{fig:fusion_dependency}
\end{figure} 

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/fusion_dependency.pdf}
%     \caption{Fusion dependency}
%     \label{fig:fusion_dependency}
% \end{figure} 



%We need to consider the order of operations in two folds. First, due to the non-determinism in the measurement pattern, the measurement bases of some qubits in the graph state have to be adjusted according to the measurement outcomes of other qubits. Since measurements of the same physical layer are implement at the same time, those dependent qubits have to be measured in a later physical layer than the qubits they depend on. Second, as photons would vanish once measured, we have to make sure that their computational information is kept by the remaining qubits after they vanish. That requires each qubit to be entangled to some other qubits before it is measured. In particular, for each dependency layer, its computational information needs to be transferred to to the next layer when new physical layers are generated. That requires each dependency layer to be entangled to some qubits which will be stored in the delay line before the layer it is measured up.

\textit{Adaptive Fusion Decomposition:}
When computing with a graph state instead of a 2d-grid cluster state, the structure of the graph varies from program to program. However, the resource states are not only small, preventing them to be born with a complex structure, but also in a fixed state. For example, in a GHZ state, each qubit have only one or two neighbors entangled with it. But in a sub-graph of the graph state which is scheduled to be implemented, the nodes may live in a complex neighborhood. For example, in the graph shown in Fig.~\ref{fig:high_degree_decomposition}, the graph on the right is translated from a circuit on the left. As node A,B,C,D,E,F all have a degree of 3, and node G has a degree of 6, it means they cannot be assigned to any single qubit in the resource states. Instead, it has to be synthesized by multiple resource states with the help of a proper pattern of fusion operations.
%Therefore, to implement a sub-graph of the graph state in a certain physical layer, we have to decompose the formation of the sub-graph to a set of fusion operations. For example, 

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/high_degree_synthesis.pdf}
    \caption{Decomposition Graph}
    \label{fig:high_degree_decomposition}
\end{figure}


\subsection{Overview of Our Planar-centric Compiler}
We propose an end-to-end, planar-centric compilation framework that supports the mapping of any regular circuit program (e.g., program in Figure~\ref{} (a)) to its execution pattern on our hardware model (final mapping in Figure~\ref{} (d)). Our framework consists of three major optimization passes, ~\textit{Fusion Graph Generation} (section~\ref{}), ~\textit{2D-Lattice Mapping and Routing} (section~\ref{}), and ~\textit{Large-scope Graph Partition and Scheduling} (section~\ref{}). We also remark that the planar graph theory~\cite{} plays an important role in our compiler design, and this is why we name it planar-centric compilation framework. 

In this section, we will use motivating examples to give some high-level ideas about the key challenges being addressed by these three passes and the highlights of our technical contributions. We have attempted to maximize simplicity and easy understanding, while perhaps sacrificing
some rigor. Formal and Detailed description of these techniques can be found in section~\ref{}.

\paragraph{Fusion Graph Generation} This step focuses on transforming a regular graph based on the input quantum circuits to a low-degree \text{Fusion Graph} abstraction (from Figure~\ref{} (b) to Figure~\ref{} (c)).  

\paragraph{2D-Lattice Mapping and
Routing} In this step we map such processed low-degree graph to a 2D lattice layout for the actual execution on hardware.
Our compiler is set towards two key optimization goals. 

\paragraph{Large-scope Graph Partition and Scheduling}





\yuke{Add the challenges based on Fig.~\ref{fig:high_degree_decomposition}. 1) Low-degree nodes, 2) Path Directions in 2D Space, 3) Large graph,} 
%
\fix{The overall flow starts from the regular graph based on the input quantum circuits to a low-degree graph abstraction. Then we map such processed low-degree graph to a 2D lattice layout for the actual execution on hardware.
%
Specifically, the first major constraints is the \textit{circuit-graph node degree} constraint. This is mainly because of the limitation of hardware that cannot support high-degree inter-connections among individual nodes, as discussed in Section~\ref{}. Therefore, a set of node-level graph transformation (e.g., node split or duplication) is in demand for satisfying such constraint.
%
The second major limitation is the \textit{direction of circuit-graph edge expansion.}
The major insight is that despite the freedom of the initial quantum circuit graphs, the final hardware mapping has to strictly follow the hardware-level propertities, such as the 2D lattices layout as illustrated in Figure~\ref{fig:high_degree_decomposition}, where the connections has to be either straight up/down or horizontal. Therefore, a set of edge-level graph transformation (e.g., alternating edge direction) is required before the hardware mapping.
%
The third challenge is the \textit{scale of input circuits}. This is because in many real-world settings , graphs are usually huge in terms of its number of nodes and edges (i.e., significantly larger than our example graph in Figure~\ref{fig:high_degree_decomposition}). In order to accommodate such large quantum circuit graph on hardware, a careful scheduling is thus in demands for decomposing the large input circuit recursively into small pieces and scheduling those processed small graphs on hardware by following the hardware constraints. 
%
The last challenge is the \textit{planar graph structure} constraint, which prohibits any edge crossovers that cannot be accommodated on the existing quantum hardware during the mapping. Such a complexity can be either directly introduced due to the non-planar input graphs or indirectly raised during the optimization or decomposition of the original input graphs.
}


\textit{Qubit Mapping:}
After decomposing the graph synthesis into fusions, mapping those required resource states onto RSGs on the device is also challenging. First, the neighboring constraint of spatial connectivity may prevent a direct one-to-one mapping. For example, in the case shown in Fig.~\ref{fig:detour} where the fusions between resource states A, B and C form a cycle, if we map B and C to the neighboring resource states of A, then B and C cannot be neighbors to each other. To resolve the conflicts, we need to make a detour, eg. through location \textcolor{red}{(def?)} D, with the qubit in blue removed by a $Z$-measurement \textcolor{red}{(background)}. A good mapping should find a trajectory for the pair of qubits in each fusion while making those trajectories as short as possible. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/detour.pdf}
    \caption{Connectivity Conflicts}
    \label{fig:detour}
\end{figure}
Second, as the number of qubits in each resource state is limited, each location cannot be passed by too many trajectories. In the specific case of resource states being GHZ states, each location can be passed by only one trajectory. However, some patterns can be intrinsically non-planar, such as shown in Fig~\ref{fig:k33}. For those patterns, it is impossible to embed them into a layer of resource states with all trajectories being disjoint, thus multiple layers may be required even for a small sub-graph. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.65\linewidth]{fig/k33.pdf}
    \caption{Non-planar Graph}
    \label{fig:k33}
\end{figure}
Third, the increase in the number of required physical layers may cause the qubits in delay lines to expire due to the limit of delay time. This in turn affects the scheduling and decomposition of the pattern.

%After decomposing the graph synthesis into fusions, we need to map it to the physical resource states under the connectivity constraints. For example, the fusion decomposition in Fig.~\ref{fig:high_degree_decomposition} can be mapped to a layout of resource states in Fig.~\ref{fig:high_degree_mapping}. But there are some cases where a direct one-to-one mapping does not exist. The first reason is that for each physical layer, the initial mapping of some resource states are already determined by the previous physical layer since they need to fuse with the delayed qubits from the previous layer.
%The second reason is that the decomposition graph \textcolor{red}{(def)} can contain some cycles \textcolor{red}{(no conflicts in tree?)} that conflict with the connectivity constraints. In those cases, auxiliary resource states are needed. For example, as shown in Fig.~\ref{fig:detour}, the fusions between resource states A, B and C form a cycle. If we map B and C to the neighboring resource states of A, then B and C cannot be neighbors to each other. To resolve the conflicts, we can make a detour, eg. through location \textcolor{red}{(define something like generation location)} D. Since only two qubits of resource state D is needed to connect B and C, the qubit in blue will be assigned a `measure in Z' \textcolor{red}{(explain in background)} operation to detach from the resource state. %The second reason is that for each physical layer, the initial mapping of some resource states are already determined by the previous physical layer since they need to fuse with the delayed qubits from the previous layer. In this case we also need auxiliary resource states as in Fig.~\ref{fig:detour}.


\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/high_degree_mapping.pdf}
    \caption{High degree node mapping}
    \label{fig:high_degree_mapping}
\end{figure}










==> 04_motivation_rebuttal.tex <==

\vspace{0.3em}
\section{Problem Formulation}



In this section, we first formulate the hardware abstraction of a photonic quantum computer and its compilation challenges.
Then we provide an overview of our proposed framework.
%\newline
%the the problem of synthesizing graph states with small cluster states \textcolor{red}{(def)}, and then discuss the challenges in it.

\iffalse
This paper adopts the hardware architecture from PsiQuantum~\cite{psiquantum-fbqc}, a leading industry in the area of photonic quantum computing, as shown in Fig.~\ref{fig:device2d}.
This architecture consists of resource state generators (RSG), routers and measurement device. 
A RSG repeatedly produces a copy of small cluster state (e.g., a three-qubit GHZ state~\cite{}) every clock cycle. Without loss of generality, the rest of the paper uses GHZ as the basic RSG state unless otherwise stated.
%, which is called a \textit{resource state}.
%We adopt a hardware model recently proposed by [?], which consists of resource state generators (RSG), routers and measurement device, as shown in Fig.~\ref{fig:device2d}. 
Those small cluster states %  resource states 
are channelled to different measurement locations by the routers. The routing includes spatial routing as well as temporal routing in the form of delay lines.
The spatial routing allows a small cluster state to be fused with cluster states generated by other RSGs.
The temporal routing delay the arrival of photons by some clock cycles so that they can be fused with photons generated later by the same RSG. 
\fi

\vspace{0.3em}
\subsection{Hardware Abstraction}
% \todo{Hezi, fix me}
\label{sect:hardware_model}
%We create for the first time
We formulate a hardware model abstraction, namely the \textit{\archName}, for a photonics based quantum computer, as shown in Fig.~\ref{fig:archoverview}. 
This abstraction follows the hardware architecture from PsiQuantum~\cite{psiquantum-fbqc}, a leading industry in the area of photonic quantum computing. 
There are three levels of coupling in this graph and they are introduced as follows.

\textbf{Coupling in the resource state} 
The first level of coupling comes from qubits in the same \emph{resource state}, i.e. the small cluster state generated by a resource state generator (RSG). Each node in Fig.~\ref{fig:archoverview} represents a resource state, which contains a few entangled qubits.
% (e.g., a three-qubit GHZ state~\cite{GHZcluster}).
% unless otherwise stated.
Each RSG can repeatedly generate resource states at a constant rate, with each unit time interval called a \emph{clock cycle}. \fix{Without loss of generality, the rest of the paper uses three-qubit GHZ states as the basic resource states generated by RSGs for illustration. Our proposed optimizations are general and can be applied to hardware with different basic types of resource states.} 
 %every clock cycle. 

\textbf{Coupling within a clock cycle}
The second level of coupling comes from the resource states generated within the same clock cycle, which together form a layer of qubits referred to as a \emph{physical layer}.
As shown in Fig.~\ref{fig:archoverview}, the nodes in the physical layer at $t_0$ (or $t_1,t_2$) are connected into a 2D lattice structure.
Such connections within a clock cycle represent the spatial connections supported directly by the hardware.
That is, a resource state generated by an RSG can conduct a fusion with resource states generated at the same clock cycle by its neighboring RSGs.

% the hardware RSGs a small cluster state can be routed to make a fusion with the small cluster states generated at the same clock cycle by its neighboring RSGs.

\textbf{Coupling across time frames}
The third level of coupling is that a resource state can make a fusion with another resource state generated in a different clock cycle by the same RSG with the help of \fix{\emph{delay lines} that delay the photons' arrival at the measurement devices}, as shown by the red and grey vertical lines in Fig.~\ref{fig:archoverview}(a) (connections of distance larger than one are omitted).
Note that we should avoid using too long-range temporal connections because photons suffer more from the loss error as they stay longer in the delay lines. The 3D structure of the connectivity as shown in Fig.~\ref{fig:archoverview}(a) can be transformed to a \archName~as shown in Fig.~\ref{fig:archoverview}(b), with every other physical layer (e.g., the physical layer at $t_1$) being flipped in the horizontal direction. To keep the figure clear, some temporal connections are omitted in Fig.~\ref{fig:archoverview}(b)  (preserving only the first row). Using this coupling graph, we can define an \emph{extended physical layer} by combining multiple physical layers and ignoring some temporal connections (preserving only the red ones on the boundaries).
% Multiple physical layers can be combined to an \emph{extended physical layer} by ignoring temporal connections except for some connections on the boundary.
For example, in Figure~\ref{fig:archoverview}, physical layers at $t_0,t_1$ and $t_2$ form an extended physical layer when preserving the spatial connections and the temporal connections in red.
% Therefore, a cluster state cannot be directly coupled another cluster state that is generated too late.

%Temporal routing connects nodes that represent the same RSG at different clock cycles (e.g., the RSG 0 at $t_0$ connects to the RSG 0 at $t_1$ and $t_2$ in Fig.~\ref{fig:archoverview}), with the maximum distance between the time frames determined by the length of delay lines.
%This represents that a small cluster state can be routed to make a fusion with the small cluster states generated later by the same RSG.



\begin{figure}[h!]
    \centering
    % \vspace{-5pt}
    \includegraphics[width=\linewidth]{fig/flattened_hardware_model_bold.pdf}\\
    \vspace{-5pt}
    (a)\hspace{110pt}(b)
    % \vspace{-5pt}
    \caption{3D structure of hardware connectivity (a) and its \archName~(b). The physical layer $t_1$ in (b) is flipped in the horizontal direction so that physical layers $t_0,t_1$ and $t_2$ form an extended physical layer by preserving all the spatial connections and only the temporal connections in red. To keep the figure clear, temporal connections of distance larger than 1 are omitted, some temporal connections of distance 1 are omitted in (b) as well (except for the first row).}
    % \caption{Example of the \archName. The nodes are labeled with different RSG indices represent the cluster states generated by the corresponding RSGs. Fusion operations are directly supported between the cluster  states of two connected nodes. For simplicity, connections across different time frames are omitted except for RSG0.}
    \vspace{-10pt}
    \label{fig:archoverview}
\end{figure}

%This \archName can be regarded as a counterpart of the coupling graph abstraction~\cite{sabre} prevailing used for today’s superconducting and ion trap hardware architectures. 
%This abstraction also helps us to relate the quantum compilation intensively studied recently [\todo{?}] with many new problems studied in the photonics context \todo{Hezi: what does it mean here?}. 
Despite the similarity to the quantum hardware coupling graph~\cite{sabre} prevailing used for today’s superconducting and ion trap hardware architectures, we emphasize on their differences and our high-level insights behind such an abstraction.

%\begin{enumerate}
 %   \item 
%First, we turn 3D temporal-spatial 3D -> 2D
%Delay line -> active layers simulatousy -> containsts in the mapping. 
1) The 3D connectivity structure is flattened into a series of 2D physical layers along the time dimension, with each layer consisting of the resource states generated at a specific clock cycle. Successive layers can be chosen to form \emph{extended physical layers} by preserving spatial connections within the layers and some of the temporal connection across the layer on the boundaries (red lines in Fig.~\ref{fig:archoverview}).
%We refer to the physical layers that can be accommodated by the delay lines as \emph{active} physical layers.
 Within an extended physical layer, the time dimension is treated the same as a spatial dimension to enable the accommodation of larger size programs.
 This greatly simplifies the follow-up compilation optimization algorithm designs
%  (i.e., the program synthesis, mapping, routing, and scheduling) 
 since the properties of planar graphs can be leveraged.
% \todo{active physics layers include this keyword}
%The photons in the physical layers can live in the delay line for an amount of time before they disappear. However due to the limit of the length of delay lines, only a limited number of physical layers can be active simultaneously, leading to a hardware constraint on the mapping.
%\item %Hierarchical coupling: 
%within each RSG it is determined by the the RSG generator. Among RSG node it is determined by the the fusion device; GHZ line , RSG
%Within each physical layer, the resource states are generated by resource state generators (RSG) sitting on fixed locations. Resource states generated from different RSGs can be routed to fusion devices by routers, whose structure determines the spatial connectivity. Resource states generated by the same RSG but at different times also have connections, because early resource states can be delayed before being routed to fusion devices.

2) We remark that different levels of coupling are not independent, and actually their interplay could create some additional constraints. For example, suppose the resource states generated by RSGs are 3-qubit GHZ states, then although the fusion device allows a RSG to maximally connect to 4 spatial neighbors (up, down, left, right) and previous or future resource states generated by the same RSG within the range of delay lines, only up to 3 of them can be activated.
%\item To distinguish betwe\ten different coupling edges, we thus often draw the coupling among qubtis within a RSG with a solid edge (suggest: flattened edge), while those connected by fusion with a blurred, flattened edge (suggest: solid edge) when they are activated. \todo{consider this when drawing the figure}
%\end{enumerate}




\iffalse

This architecture consists of \emph{resource state generators} (RSG), routers and measurement device. 
A RSG repeatedly produces a copy of small cluster state referred to as \emph{resource states} (e.g., a three-qubit GHZ state~\cite{GHZcluster}) every clock cycle. Without loss of generality, the rest of the paper uses GHZ as the basic RSG state unless otherwise stated.


In our \archName~(Fig.~\ref{fig:archoverview}), each node represents a small cluster state generated by an RSG at a specific clock cycle.
Those small cluster states %  resource states 
are channelled to different measurement locations by the routers. The routing includes spatial routing as well as temporal routing in the form of delay lines.
Connections between the nodes represent the allowed routing for the small cluster states generated by the RSGs at the same clock cycle (e.g., RSGs in the $t_0$ cycle have 2D lattice connections in Fig.~\ref{fig:archoverview}).
Spatial routing connections exist among the RSG nodes from the same clock cycle and they formulate a 2D array structure.
That is, a small cluster state can be routed to make a fusion with the small cluster states generated at the same clock cycle by its neighboring RSGs.
Temporal routing connects nodes that represent the same RSG at different clock cycles (e.g., the RSG 0 at $t_0$ connects to the RSG 0 at $t_1$ and $t_2$ in Fig.~\ref{fig:archoverview}), with the maximum distance between the time frames determined by the length of delay lines.
This represents that a small cluster state can be routed to make a fusion with the small cluster states generated later by the same RSG.
% the same RSG in the next time frame using a delay line.
%Note that photons suffer more from the photon loss error as the photon stays longer in the delay line.
%Therefore, we define an active layer in our model. 
%This active layer contains nodes from a specific number of consecutive time frames as we assume that the photons can only stay in the delay line for at most a specific number of cycles. \todo{rephrase the active layer description}


%A 2d-array of RSGs generates a 3d-grid of resource states with time being the third dimension. The combination of spatial and temporal routing enables the connectivity between any resource state and all its neighbors. To look at it in a low dimension, an equivalent way to represent the connectivity is by having a 2d-grid of resource states with adjacent connectivity as well as some long range connectivity, which we refer to as a \textit{connectivity graph}. 

%As shown in Fig.~\ref{fig:connectivity2d}. Each red box stands for a resource state, with the time and RSG from which it is generated marked inside. In this example, the six RSGs form a 2x3 array. During each clock cycle, eg. $t_0, t_1$ or $t_2$, the RSGs generate a layer of resource states, which we refer to as a \textit{physical layer}. Note that physical layer $t_1$ is in a reverse order of physical layer $t_0$. The reason we arrange them in this way is to make every resource state connected to all its neighbors in the representation so that we do not need to consider the boundary effect\yuke{Add more detailed explaination to this effect or add citation or reference}.


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/archoverview.jpeg}
%     \caption{A placeholder: \todo{wrong order!}}
%     \label{fig:archoverview}
% \end{figure}


This \archName~can be regarded as a counterpart of the coupling graph abstraction~\cite{sabre} prevailingly used for today’s superconducting and ion trap hardware architectures. 
%This abstraction also helps us to relate the quantum compilation intensively studied recently [\todo{?}] with many new problems studied in the photonics context \todo{Hezi: what does it mean here?}. 
Despite the similarity with the quantum hardware coupling graph, we still emphasize on their differences and our high level insights behind such an extended, more complex abstraction.
\begin{enumerate}
    \item 
%First, we turn 3D temporal-spatial 3D -> 2D
%Delay line -> active layers simulatousy -> containsts in the mapping. 
The 3D routing structure is flattened into a series of 2D \emph{physical layers} coming out constantly in the time axis, with each layer consisting of the resource states generated at a specific clock cycle. Together those layers can form an extended 2D plane of resource states by ignoring the some of the temporal connections as shown by the grey lines in Fig.~\ref{fig:archoverview}. We refer to the physical layers that can be accommodated by the delay lines as \emph{active} physical layers. This greatly simplifies the follow-up compilation optimization algorithm designs (i.e., the program synthesis, mapping, routing, and scheduling) since the properties of planar graphs can be leveraged. 
The time dimension is also treated as a spatial dimension, enabling the accommodation of larger size programs.
% \todo{active physics layers include this keyword}
%The photons in the physical layers can live in the delay line for an amount of time before they disappear. However due to the limit of the length of delay lines, only a limited number of physical layers can be active simultaneously, leading to a hardware constraint on the mapping.
%\item %Hierarchical coupling: 
%within each RSG it is determined by the the RSG generator. Among RSG node it is determined by the the fusion device; GHZ line , RSG
Within each physical layer, the resource states are generated by resource state generators (RSG) sitting on fixed locations. Resource states generated from different RSGs can be routed to fusion devices by routers, whose structure determines the spatial connectivity. Resource states generated by the same RSG but at different times also have connections, because early resource states can be delayed before being routed to fusion devices.
\item We remark that different levels of coupling are not independent of each other, and actually their inteplay could create some additional constraints. For example, suppose we have a 3-qubit GHZ state as the our RSG state, then even when the fusion device allows a RSG to maximally connect to 4 spatial neighbors (up, down, left, right) and previous or future resource states generated by the same RSG within the range of delay lines, only up to 3 of them can be activated.
%\item To distinguish betwe\ten different coupling edges, we thus often draw the coupling among qubtis within a RSG with a solid edge (suggest: flattened edge), while those connected by fusion with a blurred, flattened edge (suggest: solid edge) when they are activated. \todo{consider this when drawing the figure}
\end{enumerate}
\fi
%1) First, we turn 3D temporal-spatial 3D -> 2D
%Delay line → active layers simulatousy → containsts in the mapping. 
%First, the 3D structure is composed of a series of 2D physical layers coming out constantly in the time axis. The photons in the physical layers can live in the delay line for an amount of time before they disappear. However due to the limit of the length of delay lines, only a limited number of physical layers can be active simultaneously, leading to a hardware constraint on the mapping.

%2) Hierarchical coupling: within each RSG it is determined by the the RSG generator. Among RSG node it is determined by the the fusion device; GHZ line , RSG
%Within each physical layer, the resource states are generated by resource state generators (RSG) sitting on fixed locations. Resource states generated from different RSGs can be routed to fusion devices by routers, whose structure determines the spatial connectivity. Resource states generated by the same RSG but at different times also have connections, because early resource states can be delayed before being routed to fusion devices.

%3) We remark that different levels of coupling are not independent of each other, and actually their inteplay could create some additional constraints. For example, suppose we have a GHZ state (three qubits) as the our RSG state, then even when the fusion device allows a RSG to maximally connect to 6 other RSGs (4 spatial neighbors (up, down, left, right) + 2 temporal neighbors (future, previous)), only 3 of them can be simultaneously activated. 
%4) To distinguish between different coupling edges, we thus often draw the coupling among qubtis within a RSG with a solid edge (suggest: flattened edge), while those connected by fusion with a blurred, flattened edge (suggest: solid edge) when they are activated.


%In this work, we focus on GHZ based RSG as it represents our state-of-art (not sure) hardware development. but our optimization are largely general and can be extended to other general cluster states if produced by RSG.




%We create for the first time a formal hardware model abstraction for photonics based quantum devices []. We name it Temporal-spatial Hierarchy Coupling Graph (TSHGraph) (as shown in Fig.~\ref{fig:connectivity2d}). It can be regarded as an extension of the coupling group abstraction [] prevailing used for today’s superconducting and ion trap hardware architectures. This abstraction also helps us to relate what we have intensively studied in the last few years [] with many new problems studied in the photonics context. We also remark that TSHGraph features several unique properties that is missing in standard quantum coupling graph. We next highlight our key insights behind such an extended, more complex abstraction.

%First, 

\iffalse

\subsection{Problem Formulation}
\yuke{usually start with ``In this section, we formulate the problem XXX as XXX''}A 2d-array of RSGs generates a 3d-grid of resource states with time being the third dimension. The combination of spatial and temporal routing enables the connectivity between any resource state and all its neighbors. To look at it in a low dimension, an equivalent way to represent the connectivity is by having a 2d-grid of resource states with adjacent connectivity as well as some long range connectivity, which we refer to as a \textit{connectivity graph}. 

As shown in Fig.~\ref{fig:connectivity2d}. Each red box stands for a resource state, with the time and RSG from which it is generated marked inside. In this example, the six RSGs form a 2x3 array. During each clock cycle, e.g., $t_0, t_1$ or $t_2$, the RSGs generate a layer of resource states, which we refer to as a \textit{physical layer}. Note that physical layer $t_1$ is in a reverse order of physical layer $t_0$. The reason we arrange them in this way is to make every resource state connected to all its neighbors in the representation so that we do not need to consider the boundary effect\yuke{Add more detailed explaination to this effect or add citation or reference}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/connectivity2d.pdf}
    \caption{2d connectivity graph \yuke{I suggest using different color for different RSG while circling out the group of RSG by time steps}}
    \label{fig:connectivity2d}
\end{figure} 

With this representation, the compilation problem is then formulated as assigning each qubit of each resource state an operation, either measure, fusion, delay or throw away, according to the connectivity structure so that i) the qubits assigned `measure' operation form the graph state \textcolor{red}{(more clear?)} through fusion and ii) the time order of the qubits assigned `measure' operation satisfy their dependency relation.

\subsection{Challenges}
With the compilation problem formulated, we then talk about the challenges of resolving it.

\textit{Operation Order:}
%\textcolor{red}{i)  A-B, C-D: B-C fusion (A-D entanglement) commute with A measurement?} \textcolor{red}{ii) fusion: adjust basis according to collapsed state?} \textcolor{red}{iii)How many layers in advance?}
In one-way quantum computing, dependent corrections resulting from the non-determinism in quantum measurements play a key role in ensuring universality. %While in a standard pattern, dependency comes only from the non-determinism of single-qubit measurements, in the scheme of real-time synthesis, the fusion operations add a new type of dependency between single-qubit measurements and fusions.
In the scheme of real-time synthesis, the non-determinism in fusion outcomes adds more complexity.
Because now we need to consider not only the dependency between single-qubit measurements, but also the dependency between single-qubit measurements and fusion operations. As an example, Fig.~\ref{fig:fusion_dependency} shows a simple pattern on a 4-qubit linear graph state\yuke{explain the meaning of A ,B, C, D}. As shown in Fig.~\ref{fig:fusion_dependency}(a), if we implement it in a standard form, i.e. first prepare all qubits and entangle them and then do the measurements, then the measurement outcome of $M_\alpha$ leads to a correction on qubit $B$, and the measurement outcome of $M_\gamma$ leads to a correction on qubit $C$, resulting a dependency $A\rightarrow B\rightarrow C \rightarrow D$. However, if the graph state needs to be generated from two GHZ states as shown in Fig.~\ref{fig:fusion_dependency}(b), then the outcome of fusion between qubit $F_1$ and qubit $F_2$ also leads to corrections on both qubit $B$ and qubit $C$, resulting in another dependency $F\rightarrow \left\{B,D\right\}$. %Therefore, when scheduling the execution of a pattern, we need to take care of the dependency to make sure that a qubit should be measured only if all the single-qubit measurements and fusions that it depends on are completed.
That means measurements on qubits in the ${i+1}^\mathrm{th}$ dependency layer depends not only on the $i^\mathrm{th}$ layer\yuke{explain the meaning of layer here}, but also on the fusion between the $i^\mathrm{th}$ and $i+1^\mathrm{th}$ layers, while the $i^\mathrm{th}$ layer depends on the fusion as well. Meanwhile, the dependency may result in a long waiting period for some qubits. Since there is a limit for the delay time, we have to refresh those qubits before they expire.
%which causes more complexity in scheduling, especially when two neighboring qubits are in the $i^\mathrm{th}$ and $i+n^\mathrm{th}$ dependency layers where $n>1$.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{fig/dependency.pdf}
    \caption{Fusion dependency}
    \label{fig:fusion_dependency}
\end{figure} 

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/fusion_dependency.pdf}
%     \caption{Fusion dependency}
%     \label{fig:fusion_dependency}
% \end{figure} 



%We need to consider the order of operations in two folds. First, due to the non-determinism in the measurement pattern, the measurement bases of some qubits in the graph state have to be adjusted according to the measurement outcomes of other qubits. Since measurements of the same physical layer are implement at the same time, those dependent qubits have to be measured in a later physical layer than the qubits they depend on. Second, as photons would vanish once measured, we have to make sure that their computational information is kept by the remaining qubits after they vanish. That requires each qubit to be entangled to some other qubits before it is measured. In particular, for each dependency layer, its computational information needs to be transferred to to the next layer when new physical layers are generated. That requires each dependency layer to be entangled to some qubits which will be stored in the delay line before the layer it is measured up.

\textit{Adaptive Fusion Decomposition:}
When computing with a graph state instead of a 2d-grid cluster state, the structure of the graph varies from program to program. However, the resource states are not only small, preventing them to be born with a complex structure, but also in a fixed state. For example, in a GHZ state, each qubit have only one or two neighbors entangled with it. But in a sub-graph of the graph state which is scheduled to be implemented, the nodes may live in a complex neighborhood. For example, in the graph shown in Fig.~\ref{fig:high_degree_decomposition}, the graph on the right is translated from a circuit on the left. As node A,B,C,D,E,F all have a degree of 3, and node G has a degree of 6, it means they cannot be assigned to any single qubit in the resource states. Instead, it has to be synthesized by multiple resource states with the help of a proper pattern of fusion operations.

%Therefore, to implement a sub-graph of the graph state in a certain physical layer, we have to decompose the formation of the sub-graph to a set of fusion operations. For example, 

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/high_degree_synthesis.pdf}
%     \caption{Decomposition Graph}
%     \label{fig:high_degree_decomposition}
% \end{figure}

\fi


%\vspace{0.3em}
\subsection{Overview of \frameworkname}\label{sect:overview}
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/procedure-2.pdf}\\
    % \vspace{-5pt}
    \hspace{-25pt}
    (a)\hspace{120pt}(b)\hspace{120pt}(c)\hspace{150pt}(d)
    \caption{Compilation flow. (a) Quantum circuit. (b) Graph state. (c) Fusion graph generation. (d) Fusion mapping and routing.
    }
    % \vspace{-15pt}
    \label{fig:procedure}
\end{figure*}

\iffalse
Upon the abstracted linear photonic quantum hardware model above, 
we propose an end-to-end, planar-centric compilation framework that supports the mapping of any MBQC program to its execution pattern on our hardware model. 
By identifying the compilation challenges in this compilation flow, our framework consists of three major optimization modules, \textit{Fusion Graph Generation} (Section~\ref{sect:module1}), \textit{Fusion Mapping and Routing} (Section~\ref{sect:module2}), and \textit{Graph Partition and Scheduling} (Section~\ref{sect:module3}). 
We also remark that the planar graph theory ~\cite{PQtree,min_edge_NPhard} 
plays an important role in our compiler design, and this is why we name it planar-centric compilation framework. 
\vspace{0.3em}
\fi

\paragraph{Objectives}
As the first end-to-end compiler for MBQC, it is important to figure out a set of meaningful optimization goals. Our investigation on photonic one-way computing and realistic photonic quantum device development suggests the following two key optimization objectives.
%\begin{enumerate}
    %\item 
    \textbf{1) Minimizing the physical depth}. The physical depth is defined as the number of physical layers consumed in the computation, which represents the time of executing the compiled program.
    %\item 
    \textbf{ 2) Reducing the number of fusions}. Fusions are often the most low-fidelity and costly operations incurred in such an MBQC photonic quantum computer.
%\end{enumerate}
%is to reduce the \emph{physical depth} (the number of physical layers) of the mapping.  2) The second is to minimize the number of fusion operations in the compiled program as fusion operation is often is most low-fidelity and costly operations.
%These two metrics on high level are analogous to the circuit depth, and the number of CNOT gates for gate-model based quantum compiler optimization.  

% \vspace{0.3em}
\paragraph{Compiler Modules}
In the rest of this section, we use a motivating example (shown in Figure~\ref{fig:procedure}) to give some high-level ideas about the key challenges being addressed by these three modules and the highlights of our technical contributions. We have attempted to maximize simplicity and ease of understanding, while possibly sacrificing
some rigor. We often omit the dependency arrows and explicit measurement bases when they are not important for our optimization techniques, and they can always be derived from the graph state \cite{translation}.
%Formal and detailed descriptions of these techniques can be found in section~\ref{sect:module1},\ref{sect:module2},\ref{sect:module3}.

\vspace{0.3em}
\textbf{Module 1: Fusion Graph Generation} This module focuses on strategies of synthesizing a graph state representing any input quantum circuit from resource states, as shown in Figure~\ref{fig:procedure}(b) and (c), which can be further abstracted to \textit{fusion graphs} that indicate necessary fusions at the granularity of resource states (e.g. Fig.~\ref{fig:linear_fusion}(c),~\ref{fig:vertex_split}(d)).
% An example is shown in Figure~\ref{fig:procedure} (b) and (c). 
It mainly tackles the constraints from the \textit{limited inter-connections among individual photonic qubits in resource states}. 
This is important as a qubit conducting many two-qubit gates with other qubits (e.g. node $G$ in Figure~\ref{fig:procedure}(a)) would naturally result in a high-degree qubit node in the graph state
% representation converted from the input circuit
(e.g., node $G$ in Figure~\ref{fig:procedure}(b)) and this could prevent us from executing the program on real hardware where only limited connections among qubits are provided. 
Our key insight is that those high-degree qubit nodes can be synthesized by a proper strategy of fusions between low-degree qubits in resource states (e.g., node $A$ to the shaded area in Figure~\ref{fig:procedure}(c), and node $G$ to the area around $G$ in the central part of Figure~\ref{fig:procedure}(c)). 
By matching
% the graph representation of the input program 
with some basic fusion patterns, arbitrary high-degree input graph states (Figure~\ref{fig:procedure}(b)) can be synthesized to accommodate input adaptivity.
% with the fusions between the resource states forming a fusion Graph (Figure~\ref{fig:procedure} (c)). 
% Meanwhile, we recognize a new type of dependency induced by fusion operations. 
Section~\ref{sect:module1} gives detailed schemes for the generation of fusion graphs representing those synthesis strategies. % \fix{in an $O(|V|)$ complexity, where $|V|$ is the number of nodes}. 
% and this new dependence required by the the input program. 

% \vspace{0.2em}
\textbf{Module 2: Fusion Mapping and
Routing}
In the next module we transform a fusion graph into a final embedding compatible with the topology of the hardware connectivity, in particular \textit{the orthogonality of 2D lattice for potential fusion operations}. Example is shown in Fig.~\ref{fig:procedure}(c) and (d). 
In Fig.~\ref{fig:procedure}(c), the triangle consisting of resource states $P,Q$ and $R$ (circled part in Fig.~\ref{fig:procedure}(c)) cannot be mapped to an orthogonal grid directly because $R$ can not be adjacent to both $P$ and $Q$ if $P$ and $Q$ are mapped to adjacent RSG locations. Such incompatibility exists widely in a general fusion graph, which prevents a direct mapping from the fusion graph to the underlying hardware topology. Our insight is that such an issue can be resolved by extending some of the edges and winding them along the 2D lattice of individual or extended physical layers, which form paths of consecutive fusions. We refer to this procedure as routing. For example, in Fig.~\ref{fig:procedure}(d), $P,Q$ and $R$ can conduct fusions with each other with an auxiliary resource state $S$. In $S$, two qubits participate in the routing path $RSQ$, with the other qubit (in blue) removed by a Z-measurement. By watching the available adjacent positions of each node on the lattice and penalizing node mapping congestion in a heuristic search, we can maximize the compactness of the layout and thus minimize the overhead from extra fusions. Section~\ref{sect:module2} gives detailed searching schemes to map the edges onto orthogonal paths while minimizing the routing overhead.

% \vspace{0.2em}
%\noindent
\textbf{Module 3: Graph Partition and Scheduling}
The third module addresses the conflict between \emph{the large size of quantum programs and the small size of available resources} in each clock cycle limited by the generation speed and lifetime of resource states. The graphs for real-world quantum programs are too huge (in terms of their number of nodes and edges) to be mapped onto one or a few physical layers. In order to accommodate such large quantum programs on the hardware, careful partition and scheduling schemes are thus in demand for decomposing large input programs into smaller components which can then be synthesized and mapped onto the hardware by the two modules above. Our insight is that both the program dependency and the graph topology should be taken into account to enable a more global optimization within the range of available resources. By balancing the leverage of global structure of the graph and the requirement for long-range temporal connections arising from the dependency relation, we can maximize the parallelism between operations while benefiting the efficiency of resource utilization. Section~\ref{sect:module3} gives detailed schemes of partition and scheduling.
%\fix{that utilizing a flow finding algorithm in complexity $O(|V|^2)$ where $|V|$ is the number of nodes~\cite{}.}


% The third challenge addressed in this module is the \textit{scale of input graph}. 
% The input graphs for real-world quantum programs are too huge (in terms of its number of nodes and edges) %(i.e., significantly larger than our example graph in Figure~\ref{fig: motivating1}) (b) %and thus can not
% to be mapped to one or a few physical layers allowed by our delay line limits. In order to accommodate such large quantum graphs on our hardware, careful partition and scheduling schemes are thus in demand for decomposing the large input circuit into small pieces and scheduling those processed small graphs on hardware. 
% Our insight is that rather a direct one-to-one mapping from dependency layers to physical layers,  a synthetically consideration of both dependency relations and the entire volume of active physical layers can enable a more flexible and adaptive optimization opportunity for maximizing both the parallelism between measurements and resource utilization on the hardware. 
% Meanwhile, we recognize a new type of dependency induced by fusion operations which motivates a look-ahead in the scheduling. 
% Moreover, the possible long wait resulting from the dependency block requires a mechanism of refreshing qubits when its lifetime approaches to the limit of the system. 
% Section~\ref{sect:module3} gives a detailed scheme of partition and scheduling as well as the new type of dependency.
%which includes analysis of both types of dependencies and the implementation of refreshing.

%Our insight is that a synthetical consideration of both dependency relations and graph topology can enable an optimization opportunity as global for maximizing the parallelism between measurements as allowed by the entire volume of active physical layers. By considering the program dependency and a new type of dependency we recognized in the existence of fusion gates, as well as the hardware constraints, we can schedule a large graph into multiple executable rounds with the help of a refreshing mechanism. Section ? gives a detailed scheme of partition and scheduling which includes analysis of both types of dependencies and the implementation of refreshing.


%
%By considering the program dependency and a new type of dependency we recognized in the existence of fusion gates, as well as the hardware constrains, we can schedule a large graph into multiple executable rounds with the help of a refreshing mechanism. 
% The insight is that not all dependency blocks the measurements, with some only affecting the interpretation of the measurement outcomes. Meanwhile, we recognize a new type of dependency induced by fusion operations which motivates an lookahead synthesis of the qubits to be executed next round. Moreover, the possible long wait resulting from the dependency block requires a mechanism of refreshing qubits when its lifetime approaches to the limit. 
%v\textit{Dynamic scheduling} outputs a set of executable qubits in each round, with each qubit assigned a choice of operation from measurement, synthesis, and refresh. 

% \vspace{0.2em}
%\noindent 
\textbf{All Modules: Non-Planar Graph  Prohibition}
The last challenge we identify is  \textit{non-planar graph prohibition}, which plays an important role in all three modules. By non-planar graph prohibition, we mean that the graph embedded into each physical layer should be a planar graph~\cite{PQtree}, i.e., a graph that can be drawn on a plane in a way that no edges cross each other.
\iffalse
On one hand, this is because the small size of resource states and the limited physical connections among them prevent the routing paths on the lattice from crossing each other. On the other hand, we find the design philosophy motivated by this requirement powerful in suppressing the optimization space and thus leading to a more efficient heuristic search. 
\fi
%\fix{Such an embedding can be found in $O(|E|)$, where $|E|$ is the number of edges~\cite{}.}
The complexity of graph non-planarity can either arise directly from the input graphs (Figure.~\ref{fig:program_non-planarity}(b)) or indirectly from our optimization steps if not carefully designed (Fig.~\ref{fig:vertex_split}(e)). Our insight is that such a challenge can be tackled by (1) eliminating the non-planarity by decomposing each non-planar component to a set of planar graphs (Fig.~\ref{fig:program_non-planarity}(c)), (2) enforcing our key modules to maintain such a planar property as an optimization. Details are incorporated in each section of the key modules, with the elimination included in Section~\ref{sect:module3} and the enforcement included in Section~\ref{sect:module1},~\ref{sect:module2}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/planar_decomp.png}\\
    \hspace{-10pt}(a)\hspace{70pt}(b)\hspace{100pt}(c)
    \caption{A non-planar graph state (b) translated from a circuit (a), with the measurement basis omitted. The non-planar graph (b) can be broken into two planar sub-graphs in (c).}
    % \vspace{-5pt}
    \label{fig:program_non-planarity}
\end{figure}

%Our insight is that the planarity should be  taken into account as a prerequisite, when e(Figure\ref{} (d）) , with the fusion graph generation maintaining the planarity () and the 2D Lattice Mapping and Routing following the planar embedding.

%By taking this into consideration and prerequisite, we can not only makes our heuristics design in all modules easier and powerful.


% \todo{end of this section}
\iffalse

\yuke{Add the challenges based on Fig.~\ref{fig:high_degree_decomposition}. 1) Low-degree nodes, 2) Path Directions in 2D Space, 3) Large graph,} 
%
\fix{The overall flow starts from the regular graph based on the input quantum circuits to a low-degree graph abstraction. Then we map such processed low-degree graph to a 2D lattice layout for the actual execution on hardware.
%
Specifically, the first major constraints is the \textit{circuit-graph node degree} constraint. This is mainly because of the limitation of hardware that cannot support high-degree inter-connections among individual nodes, as discussed in Section~\ref{}. Therefore, a set of node-level graph transformation (e.g., node split or duplication) is in demand for satisfying such constraint.
%
The second major limitation is the \textit{direction of circuit-graph edge expansion.}
The major insight is that despite the freedom of the initial quantum circuit graphs, the final hardware mapping has to strictly follow the hardware-level propertities, such as the 2D lattices layout as illustrated in Figure~\ref{fig:high_degree_decomposition}, where the connections has to be either straight up/down or horizontal. Therefore, a set of edge-level graph transformation (e.g., alternating edge direction) is required before the hardware mapping.
%
The third challenge is the \textit{scale of input circuits}. This is because in many real-world settings , graphs are usually huge in terms of its number of nodes and edges (i.e., significantly larger than our example graph in Figure~\ref{fig:high_degree_decomposition}). In order to accommodate such large quantum circuit graph on hardware, a careful scheduling is thus in demands for decomposing the large input circuit recursively into small pieces and scheduling those processed small graphs on hardware by following the hardware constraints. 
%
The last challenge is the \textit{planar graph structure} constraint, which prohibits any edge crossovers that cannot be accommodated on the existing quantum hardware during the mapping. Such a complexity can be either directly introduced due to the non-planar input graphs or indirectly raised during the optimization or decomposition of the original input graphs.
}


\textit{Qubit Mapping:}
After decomposing the graph synthesis into fusions, mapping those required resource states onto RSGs on the device is also challenging. First, the neighboring constraint of spatial connectivity may prevent a direct one-to-one mapping. For example, in the case shown in Fig.~\ref{fig:detour} where the fusions between resource states A, B and C form a cycle, if we map B and C to the neighboring resource states of A, then B and C cannot be neighbors to each other. To resolve the conflicts, we need to make a detour, e.g., through location \textcolor{red}{(def?)} D, with the qubit in blue removed by a $Z$-measurement \textcolor{red}{(background)}. A good mapping should find a trajectory for the pair of qubits in each fusion while making those trajectories as short as possible. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/detour.pdf}
    \caption{Connectivity Conflicts}
    \label{fig:detour}
\end{figure}
Second, as the number of qubits in each resource state is limited, each location cannot be passed by too many trajectories. In the specific case of resource states being GHZ states, each location can be passed by only one trajectory. However, some patterns can be intrinsically non-planar, such as shown in Fig~\ref{fig:k33}. For those patterns, it is impossible to embed them into a layer of resource states with all trajectories being disjoint, thus multiple layers may be required even for a small sub-graph. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.65\linewidth]{fig/k33.pdf}
    \caption{Non-planar Graph}
    \label{fig:k33}
\end{figure}
Third, the increase in the number of required physical layers may cause the qubits in delay lines to expire due to the limit of delay time. This in turn affects the scheduling and decomposition of the pattern.

%After decomposing the graph synthesis into fusions, we need to map it to the physical resource states under the connectivity constraints. For example, the fusion decomposition in Fig.~\ref{fig:high_degree_decomposition} can be mapped to a layout of resource states in Fig.~\ref{fig:high_degree_mapping}. But there are some cases where a direct one-to-one mapping does not exist. The first reason is that for each physical layer, the initial mapping of some resource states are already determined by the previous physical layer since they need to fuse with the delayed qubits from the previous layer.
%The second reason is that the decomposition graph \textcolor{red}{(def)} can contain some cycles \textcolor{red}{(no conflicts in tree?)} that conflict with the connectivity constraints. In those cases, auxiliary resource states are needed. For example, as shown in Fig.~\ref{fig:detour}, the fusions between resource states A, B and C form a cycle. If we map B and C to the neighboring resource states of A, then B and C cannot be neighbors to each other. To resolve the conflicts, we can make a detour, eg. through location \textcolor{red}{(define something like generation location)} D. Since only two qubits of resource state D is needed to connect B and C, the qubit in blue will be assigned a `measure in Z' \textcolor{red}{(explain in background)} operation to detach from the resource state. %The second reason is that for each physical layer, the initial mapping of some resource states are already determined by the previous physical layer since they need to fuse with the delayed qubits from the previous layer. In this case we also need auxiliary resource states as in Fig.~\ref{fig:detour}.


\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/high_degree_mapping.pdf}
    \caption{High degree node mapping}
    \label{fig:high_degree_mapping}
\end{figure}
\fi









==> 04_motivation_v1.tex <==
\section{Problem Formulation}
In this section, we first formulate the problem of synthesizing graph states with small cluster states \textcolor{red}{(def)}, and then discuss the challenges in it.

\subsection{Hardware Model}
We adopt a hardware model recently proposed by [?], which consists of resource state generators (RSG), routers and measurement device\yuke{1. explicitly label those items in the figures. 2. clearly describe the role/function of each component in one/two sentence}, as shown in Fig.~\ref{fig:device2d}. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/device2d.jpg}
    \caption{screenshot, \textcolor{red}{to be modified} \yuke{Add the "Note that ``RSG'' means XXX, ``F'' means XXX"}}
    \label{fig:device2d}
\end{figure}

A RSG repeatedly produces a copy of small cluster state every clock cycle, which is called a \textit{resource state}. The size of the resource states is typically considered as $\mathit{O}(10)$ since generating large resource states is  exponentially hard. %For simplicity, we illustrate our framework with generators of three-qubit cluster states, which are the same as GHZ states. 
Those resource states are channelled to different measurement locations by the routers. The routing includes both spatial routing and temporal routing in the form of delay lines, which delay the arrival of photons by some clock cycles so that they can be fused with photons generated later by the same RSG. However, it is conceivable that a global spatial connectivity is hard to realize as the number of RSGs scales up. Moreover, photons should not be stored in the delay line for too long as it increases the loss rate of photons. %For simplicity, we assume that the delay is no more than one clock cycle.
As for measurement device, we only require it to support single-qubit measurements and fusions (two-qubit entangled measurements).

For simplicity, we illustrate our framework assuming that: i) The RSGs form an 2D array, each generating three-qubit cluster states, which are the same as GHZ states, ii) for spatial connectivity, a resource state can only be fused with resource states generated by its neighboring RSGs, iii) for temporal connectivity, the delay is no more than $\tau$ clock cycle.
Despite the assumptions, our framework should adapt to the model with more qubits in the resource states, more cycles of delay or more complex connectivity, except that the concrete implementation becomes more complicated.

It is worth mentioning that although fusions in linear optics are probabilistic, they can be handled by error corrections along with other errors as claimed by [?]. As the first compilation framework, we do not take error correction design into account.%, but consider each qubit as an encoded logical qubit. For example, with a (2,2)-Shor code \textcolor{red}{(explain?)}, an encoded GHZ state is shown as in Fig.~\ref{fig:Shor_encoding}.

\textcolor{orange}{@Hassan: Please modify or rewrite this paragraph. Add more context and argument about fault tolerance, error correction codes to make it reasonable here. Would be great if illustrated with figures.}\HS{Let's just say we neglect the non-deterministic nature. We should also remove the following figure.}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.6\linewidth]{fig/encoding.png}
%     \caption{placeholder, \textcolor{red}{to be modified}}
%     \label{fig:Shor_encoding}
% \end{figure} 

\subsection{Problem Formulation}
\yuke{usually start with ``In this section, we formulate the problem XXX as XXX''}A 2d-array of RSGs generates a 3d-grid of resource states with time being the third dimension. The combination of spatial and temporal routing enables the connectivity between any resource state and all its neighbors. To look at it in a low dimension, an equivalent way to represent the connectivity is by having a 2d-grid of resource states with adjacent connectivity as well as some long range connectivity, which we refer to as a \textit{connectivity graph}. 

As shown in Fig.~\ref{fig:connectivity2d}. Each red box stands for a resource state, with the time and RSG from which it is generated marked inside. In this example, the six RSGs form a 2x3 array. During each clock cycle, eg. $t_0, t_1$ or $t_2$, the RSGs generate a layer of resource states, which we refer to as a \textit{physical layer}. Note that physical layer $t_1$ is in a reverse order of physical layer $t_0$. The reason we arrange them in this way is to make every resource state connected to all its neighbors in the representation so that we do not need to consider the boundary effect\yuke{Add more detailed explaination to this effect or add citation or reference}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/connectivity2d.pdf}
    \caption{2d connectivity graph \yuke{I suggest using different color for different RSG while circling out the group of RSG by time steps}}
    \label{fig:connectivity2d}
\end{figure} 

With this representation, the compilation problem is then formulated as assigning each qubit of each resource state an operation, either measure, fusion, delay or throw away, according to the connectivity structure so that i) the qubits assigned `measure' operation form the graph state \textcolor{red}{(more clear?)} through fusion and ii) the time order of the qubits assigned `measure' operation satisfy their dependency relation.

\subsection{Challenges}
With the compilation problem formulated, we then talk about the challenges of resolving it.

\textit{Operation Order:}
%\textcolor{red}{i)  A-B, C-D: B-C fusion (A-D entanglement) commute with A measurement?} \textcolor{red}{ii) fusion: adjust basis according to collapsed state?} \textcolor{red}{iii)How many layers in advance?}
In one-way quantum computing, dependent corrections resulting from the non-determinism in quantum measurements play a key role in ensuring universality. %While in a standard pattern, dependency comes only from the non-determinism of single-qubit measurements, in the scheme of real-time synthesis, the fusion operations add a new type of dependency between single-qubit measurements and fusions.
In the scheme of real-time synthesis, the non-determinism in fusion outcomes adds more complexity.
Because now we need to consider not only the dependency between single-qubit measurements, but also the dependency between single-qubit measurements and fusion operations. As an example, Fig.~\ref{fig:fusion_dependency} shows a simple pattern on a 4-qubit linear graph state\yuke{explain the meaning of A ,B, C, D}. As shown in Fig.~\ref{fig:fusion_dependency}(a), if we implement it in a standard form, i.e. first prepare all qubits and entangle them and then do the measurements, then the measurement outcome of $M_\alpha$ leads to a correction on qubit $B$, and the measurement outcome of $M_\gamma$ leads to a correction on qubit $C$, resulting a dependency $A\rightarrow B\rightarrow C \rightarrow D$. However, if the graph state needs to be generated from two GHZ states as shown in Fig.~\ref{fig:fusion_dependency}(b), then the outcome of fusion between qubit $F_1$ and qubit $F_2$ also leads to corrections on both qubit $B$ and qubit $C$, resulting in another dependency $F\rightarrow \left\{B,D\right\}$. %Therefore, when scheduling the execution of a pattern, we need to take care of the dependency to make sure that a qubit should be measured only if all the single-qubit measurements and fusions that it depends on are completed.
That means measurements on qubits in the ${i+1}^\mathrm{th}$ dependency layer depends not only on the $i^\mathrm{th}$ layer\yuke{explain the meaning of layer here}, but also on the fusion between the $i^\mathrm{th}$ and $i+1^\mathrm{th}$ layers, while the $i^\mathrm{th}$ layer depends on the fusion as well. Meanwhile, the dependency may result in a long waiting period for some qubits. Since there is a limit for the delay time, we have to refresh those qubits before they expire.
%which causes more complexity in scheduling, especially when two neighboring qubits are in the $i^\mathrm{th}$ and $i+n^\mathrm{th}$ dependency layers where $n>1$.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{fig/dependency.pdf}
    \caption{Fusion dependency}
    \label{fig:fusion_dependency}
\end{figure} 

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/fusion_dependency.pdf}
%     \caption{Fusion dependency}
%     \label{fig:fusion_dependency}
% \end{figure} 



%We need to consider the order of operations in two folds. First, due to the non-determinism in the measurement pattern, the measurement bases of some qubits in the graph state have to be adjusted according to the measurement outcomes of other qubits. Since measurements of the same physical layer are implement at the same time, those dependent qubits have to be measured in a later physical layer than the qubits they depend on. Second, as photons would vanish once measured, we have to make sure that their computational information is kept by the remaining qubits after they vanish. That requires each qubit to be entangled to some other qubits before it is measured. In particular, for each dependency layer, its computational information needs to be transferred to to the next layer when new physical layers are generated. That requires each dependency layer to be entangled to some qubits which will be stored in the delay line before the layer it is measured up.

\textit{Adaptive Fusion Decomposition:}
When computing with a graph state instead of a 2d-grid cluster state, the structure of the graph varies from program to program. However, the resource states are not only small, preventing them to be born with a complex structure, but also in a fixed state. For example, in a GHZ state, each qubit have only one or two neighbors entangled with it. But in a sub-graph of the graph state which is scheduled to be implemented, the nodes may live in a complex neighborhood. For example, in the graph shown in Fig.~\ref{fig:high_degree_decomposition}, the graph on the right is translated from a circuit on the left. As node A,B,C,D,E,F all have a degree of 3, and node G has a degree of 6, it means they cannot be assigned to any single qubit in the resource states. Instead, it has to be synthesized by multiple resource states with the help of a proper pattern of fusion operations.
%Therefore, to implement a sub-graph of the graph state in a certain physical layer, we have to decompose the formation of the sub-graph to a set of fusion operations. For example, 

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/high_degree_synthesis.pdf}
    \caption{Decomposition Graph}
    \label{fig:high_degree_decomposition}
\end{figure}

\textit{Qubit Mapping:}
After decomposing the graph synthesis into fusions, mapping those required resource states onto RSGs on the device is also challenging. First, the neighboring constraint of spatial connectivity may prevent a direct one-to-one mapping. For example, in the case shown in Fig.~\ref{fig:detour} where the fusions between resource states A, B and C form a cycle, if we map B and C to the neighboring resource states of A, then B and C cannot be neighbors to each other. To resolve the conflicts, we need to make a detour, eg. through location \textcolor{red}{(def?)} D, with the qubit in blue removed by a $Z$-measurement \textcolor{red}{(background)}. A good mapping should find a trajectory for the pair of qubits in each fusion while making those trajectories as short as possible. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/detour.pdf}
    \caption{Connectivity Conflicts}
    \label{fig:detour}
\end{figure}
Second, as the number of qubits in each resource state is limited, each location cannot be passed by too many trajectories. In the specific case of resource states being GHZ states, each location can be passed by only one trajectory. However, some patterns can be intrinsically non-planar, such as shown in Fig~\ref{fig:k33}. For those patterns, it is impossible to embed them into a layer of resource states with all trajectories being disjoint, thus multiple layers may be required even for a small sub-graph. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.65\linewidth]{fig/k33.pdf}
    \caption{Non-planar Graph}
    \label{fig:k33}
\end{figure}
Third, the increase in the number of required physical layers may cause the qubits in delay lines to expire due to the limit of delay time. This in turn affects the scheduling and decomposition of the pattern.

%After decomposing the graph synthesis into fusions, we need to map it to the physical resource states under the connectivity constraints. For example, the fusion decomposition in Fig.~\ref{fig:high_degree_decomposition} can be mapped to a layout of resource states in Fig.~\ref{fig:high_degree_mapping}. But there are some cases where a direct one-to-one mapping does not exist. The first reason is that for each physical layer, the initial mapping of some resource states are already determined by the previous physical layer since they need to fuse with the delayed qubits from the previous layer.
%The second reason is that the decomposition graph \textcolor{red}{(def)} can contain some cycles \textcolor{red}{(no conflicts in tree?)} that conflict with the connectivity constraints. In those cases, auxiliary resource states are needed. For example, as shown in Fig.~\ref{fig:detour}, the fusions between resource states A, B and C form a cycle. If we map B and C to the neighboring resource states of A, then B and C cannot be neighbors to each other. To resolve the conflicts, we can make a detour, eg. through location \textcolor{red}{(define something like generation location)} D. Since only two qubits of resource state D is needed to connect B and C, the qubit in blue will be assigned a `measure in Z' \textcolor{red}{(explain in background)} operation to detach from the resource state. %The second reason is that for each physical layer, the initial mapping of some resource states are already determined by the previous physical layer since they need to fuse with the delayed qubits from the previous layer. In this case we also need auxiliary resource states as in Fig.~\ref{fig:detour}.


\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/high_degree_mapping.pdf}
    \caption{High degree node mapping}
    \label{fig:high_degree_mapping}
\end{figure}










==> 04_oneq_overview_rebuttal.tex <==
%\vspace{0.3em}
\subsection{Overview of \frameworkname}\label{sect:overview}
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/procedure-2.pdf}\\
    % \vspace{-5pt}
    \hspace{-25pt}
    (a)\hspace{120pt}(b)\hspace{120pt}(c)\hspace{150pt}(d)
    \caption{Compilation flow. (a) Quantum circuit. (b) Graph state. (c) Fusion graph generation. (d) Fusion mapping and routing.
    }
    % \vspace{-15pt}
    \label{fig:procedure}
\end{figure*}

\iffalse
Upon the abstracted linear photonic quantum hardware model above, 
we propose an end-to-end, planar-centric compilation framework that supports the mapping of any MBQC program to its execution pattern on our hardware model. 
By identifying the compilation challenges in this compilation flow, our framework consists of three major optimization modules, \textit{Fusion Graph Generation} (Section~\ref{sect:module1}), \textit{Fusion Mapping and Routing} (Section~\ref{sect:module2}), and \textit{Graph Partition and Scheduling} (Section~\ref{sect:module3}). 
We also remark that the planar graph theory ~\cite{PQtree,min_edge_NPhard} 
plays an important role in our compiler design, and this is why we name it planar-centric compilation framework. 
\vspace{0.3em}
\fi

\paragraph{Objectives}
As the first end-to-end compiler for MBQC, it is important to figure out a set of meaningful optimization goals. Our investigation on photonic one-way computing and realistic photonic quantum device development suggests the following two key optimization objectives.
%\begin{enumerate}
    %\item 
    \textbf{1) Minimizing the physical depth}. The physical depth is defined as the number of physical layers consumed in the computation, which represents the time of executing the compiled program.
    %\item 
    \textbf{ 2) Reducing the number of fusions}. Fusions are often the most low-fidelity and costly operations incurred in such an MBQC photonic quantum computer.
%\end{enumerate}
%is to reduce the \emph{physical depth} (the number of physical layers) of the mapping.  2) The second is to minimize the number of fusion operations in the compiled program as fusion operation is often is most low-fidelity and costly operations.
%These two metrics on high level are analogous to the circuit depth, and the number of CNOT gates for gate-model based quantum compiler optimization.  

% \vspace{0.3em}
\paragraph{Compiler Modules}
In the rest of this section, we use a motivating example (shown in Figure~\ref{fig:procedure}) to give some high-level ideas about the key challenges being addressed by these three modules and the highlights of our technical contributions. We have attempted to maximize simplicity and ease of understanding, while possibly sacrificing
some rigor. We often omit the dependency arrows and explicit measurement bases when they are not important for our optimization techniques, and they can always be derived from the graph state \cite{translation}.
%Formal and detailed descriptions of these techniques can be found in section~\ref{sect:module1},\ref{sect:module2},\ref{sect:module3}.

% \vspace{0.3em}
\textbf{Module 1: Fusion Graph Generation} This module focuses on strategies of synthesizing a graph state representing any input quantum circuit from resource states, as shown in Figure~\ref{fig:procedure}(b) and (c), which can be further abstracted to \textit{fusion graphs} that indicate necessary fusions at the granularity of resource states (e.g. Fig.~\ref{fig:linear_fusion}(c),~\ref{fig:vertex_split}(d)).
% An example is shown in Figure~\ref{fig:procedure} (b) and (c). 
It mainly tackles the constraints from the \textit{limited inter-connections among individual photonic qubits in resource states}. 
This is important as a qubit conducting many two-qubit gates with other qubits (e.g. node $G$ in Figure~\ref{fig:procedure}(a)) would naturally result in a high-degree qubit node in the graph state
% representation converted from the input circuit
(e.g., node $G$ in Figure~\ref{fig:procedure}(b)) and this could prevent us from executing the program on real hardware where only limited connections among qubits are provided. 
Our key insight is that those high-degree qubit nodes can be synthesized by a proper strategy of fusions between low-degree qubits in resource states (e.g., node $A$ to the shaded area in Figure~\ref{fig:procedure}(c), and node $G$ to the area around $G$ in the central part of Figure~\ref{fig:procedure}(c)). 
By matching
% the graph representation of the input program 
with some basic fusion patterns, arbitrary high-degree input graph states (Figure~\ref{fig:procedure}(b)) can be synthesized to accommodate input adaptivity.
% with the fusions between the resource states forming a fusion Graph (Figure~\ref{fig:procedure} (c)). 
% Meanwhile, we recognize a new type of dependency induced by fusion operations. 
Section~\ref{sect:module1} gives detailed schemes for the generation of fusion graphs representing those synthesis strategies. % \fix{in an $O(|V|)$ complexity, where $|V|$ is the number of nodes}. 
% and this new dependence required by the the input program. 

% \vspace{0.2em}
\textbf{Module 2: Fusion Mapping and
Routing}
In the next module we transform a fusion graph into a final embedding compatible with the topology of the hardware connectivity, in particular \textit{the orthogonality of 2D lattice for potential fusion operations}. Example is shown in Fig.~\ref{fig:procedure}(c) and (d). 
In Fig.~\ref{fig:procedure}(c), the triangle consisting of resource states $P,Q$ and $R$ (circled part in Fig.~\ref{fig:procedure}(c)) cannot be mapped to an orthogonal grid directly because $R$ can not be adjacent to both $P$ and $Q$ if $P$ and $Q$ are mapped to adjacent RSG locations. Such incompatibility exists widely in a general fusion graph, which prevents a direct mapping from the fusion graph to the underlying hardware topology. Our insight is that such an issue can be resolved by extending some of the edges and winding them along the 2D lattice of individual or extended physical layers, which form paths of consecutive fusions. We refer to this procedure as routing. For example, in Fig.~\ref{fig:procedure}(d), $P,Q$ and $R$ can conduct fusions with each other with an auxiliary resource state $S$. In $S$, two qubits participate in the routing path $RSQ$, with the other qubit (in blue) removed by a Z-measurement. By watching the available adjacent positions of each node on the lattice and penalizing node mapping congestion in a heuristic search, we can maximize the compactness of the layout and thus minimize the overhead from extra fusions. Section~\ref{sect:module2} gives detailed searching schemes to map the edges onto orthogonal paths while minimizing the routing overhead.

% \vspace{0.2em}
%\noindent
\textbf{Module 3: Graph Partition and Scheduling}
The third module addresses the conflict between \emph{the large size of quantum programs and the small size of available resources} in each clock cycle limited by the generation speed and lifetime of resource states. The graphs for real-world quantum programs are too huge (in terms of their number of nodes and edges) to be mapped onto one or a few physical layers. In order to accommodate such large quantum programs on the hardware, careful partition and scheduling schemes are thus in demand for decomposing large input programs into smaller components which can then be synthesized and mapped onto the hardware by the two modules above. Our insight is that both the program dependency and the graph topology should be taken into account to enable a more global optimization within the range of available resources. By balancing the leverage of global structure of the graph and the requirement for long-range temporal connections arising from the dependency relation, we can maximize the parallelism between operations while benefiting the efficiency of resource utilization. Section~\ref{sect:module3} gives detailed schemes of partition and scheduling.
%\fix{that utilizing a flow finding algorithm in complexity $O(|V|^2)$ where $|V|$ is the number of nodes~\cite{}.}


% The third challenge addressed in this module is the \textit{scale of input graph}. 
% The input graphs for real-world quantum programs are too huge (in terms of its number of nodes and edges) %(i.e., significantly larger than our example graph in Figure~\ref{fig: motivating1}) (b) %and thus can not
% to be mapped to one or a few physical layers allowed by our delay line limits. In order to accommodate such large quantum graphs on our hardware, careful partition and scheduling schemes are thus in demand for decomposing the large input circuit into small pieces and scheduling those processed small graphs on hardware. 
% Our insight is that rather a direct one-to-one mapping from dependency layers to physical layers,  a synthetically consideration of both dependency relations and the entire volume of active physical layers can enable a more flexible and adaptive optimization opportunity for maximizing both the parallelism between measurements and resource utilization on the hardware. 
% Meanwhile, we recognize a new type of dependency induced by fusion operations which motivates a look-ahead in the scheduling. 
% Moreover, the possible long wait resulting from the dependency block requires a mechanism of refreshing qubits when its lifetime approaches to the limit of the system. 
% Section~\ref{sect:module3} gives a detailed scheme of partition and scheduling as well as the new type of dependency.
%which includes analysis of both types of dependencies and the implementation of refreshing.

%Our insight is that a synthetical consideration of both dependency relations and graph topology can enable an optimization opportunity as global for maximizing the parallelism between measurements as allowed by the entire volume of active physical layers. By considering the program dependency and a new type of dependency we recognized in the existence of fusion gates, as well as the hardware constraints, we can schedule a large graph into multiple executable rounds with the help of a refreshing mechanism. Section ? gives a detailed scheme of partition and scheduling which includes analysis of both types of dependencies and the implementation of refreshing.


%
%By considering the program dependency and a new type of dependency we recognized in the existence of fusion gates, as well as the hardware constrains, we can schedule a large graph into multiple executable rounds with the help of a refreshing mechanism. 
% The insight is that not all dependency blocks the measurements, with some only affecting the interpretation of the measurement outcomes. Meanwhile, we recognize a new type of dependency induced by fusion operations which motivates an lookahead synthesis of the qubits to be executed next round. Moreover, the possible long wait resulting from the dependency block requires a mechanism of refreshing qubits when its lifetime approaches to the limit. 
%v\textit{Dynamic scheduling} outputs a set of executable qubits in each round, with each qubit assigned a choice of operation from measurement, synthesis, and refresh. 

% \vspace{0.2em}
%\noindent 
\textbf{All Modules: Non-Planar Graph  Prohibition}
The last challenge we identify is  \textit{non-planar graph prohibition}, which plays an important role in all three modules. By non-planar graph prohibition, we mean that the graph embedded into each physical layer should be a planar graph~\cite{PQtree}, i.e., a graph that can be drawn on a plane in a way that no edges cross each other.
\iffalse
On one hand, this is because the small size of resource states and the limited physical connections among them prevent the routing paths on the lattice from crossing each other. On the other hand, we find the design philosophy motivated by this requirement powerful in suppressing the optimization space and thus leading to a more efficient heuristic search. 
\fi
%\fix{Such an embedding can be found in $O(|E|)$, where $|E|$ is the number of edges~\cite{}.}
The complexity of graph non-planarity can either arise directly from the input graphs (Figure.~\ref{fig:program_non-planarity}(b)) or indirectly from our optimization steps if not carefully designed (Fig.~\ref{fig:vertex_split}(e)). Our insight is that such a challenge can be tackled by (1) eliminating the non-planarity by decomposing each non-planar component to a set of planar graphs (Fig.~\ref{fig:program_non-planarity}(c)), (2) enforcing our key modules to maintain such a planar property as an optimization. Details are incorporated in each section of the key modules, with the elimination included in Section~\ref{sect:module3} and the enforcement included in Section~\ref{sect:module1},~\ref{sect:module2}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/planar_decomp.png}\\
    \hspace{-10pt}(a)\hspace{70pt}(b)\hspace{100pt}(c)
    \caption{A non-planar graph state (b) translated from a circuit (a), with the measurement basis omitted. The non-planar graph (b) can be broken into two planar sub-graphs in (c).}
    % \vspace{-5pt}
    \label{fig:program_non-planarity}
\end{figure}

%Our insight is that the planarity should be  taken into account as a prerequisite, when e(Figure\ref{} (d）) , with the fusion graph generation maintaining the planarity () and the 2D Lattice Mapping and Routing following the planar embedding.

%By taking this into consideration and prerequisite, we can not only makes our heuristics design in all modules easier and powerful.


% \todo{end of this section}
\iffalse

\yuke{Add the challenges based on Fig.~\ref{fig:high_degree_decomposition}. 1) Low-degree nodes, 2) Path Directions in 2D Space, 3) Large graph,} 
%
\fix{The overall flow starts from the regular graph based on the input quantum circuits to a low-degree graph abstraction. Then we map such processed low-degree graph to a 2D lattice layout for the actual execution on hardware.
%
Specifically, the first major constraints is the \textit{circuit-graph node degree} constraint. This is mainly because of the limitation of hardware that cannot support high-degree inter-connections among individual nodes, as discussed in Section~\ref{}. Therefore, a set of node-level graph transformation (e.g., node split or duplication) is in demand for satisfying such constraint.
%
The second major limitation is the \textit{direction of circuit-graph edge expansion.}
The major insight is that despite the freedom of the initial quantum circuit graphs, the final hardware mapping has to strictly follow the hardware-level propertities, such as the 2D lattices layout as illustrated in Figure~\ref{fig:high_degree_decomposition}, where the connections has to be either straight up/down or horizontal. Therefore, a set of edge-level graph transformation (e.g., alternating edge direction) is required before the hardware mapping.
%
The third challenge is the \textit{scale of input circuits}. This is because in many real-world settings , graphs are usually huge in terms of its number of nodes and edges (i.e., significantly larger than our example graph in Figure~\ref{fig:high_degree_decomposition}). In order to accommodate such large quantum circuit graph on hardware, a careful scheduling is thus in demands for decomposing the large input circuit recursively into small pieces and scheduling those processed small graphs on hardware by following the hardware constraints. 
%
The last challenge is the \textit{planar graph structure} constraint, which prohibits any edge crossovers that cannot be accommodated on the existing quantum hardware during the mapping. Such a complexity can be either directly introduced due to the non-planar input graphs or indirectly raised during the optimization or decomposition of the original input graphs.
}


\textit{Qubit Mapping:}
After decomposing the graph synthesis into fusions, mapping those required resource states onto RSGs on the device is also challenging. First, the neighboring constraint of spatial connectivity may prevent a direct one-to-one mapping. For example, in the case shown in Fig.~\ref{fig:detour} where the fusions between resource states A, B and C form a cycle, if we map B and C to the neighboring resource states of A, then B and C cannot be neighbors to each other. To resolve the conflicts, we need to make a detour, e.g., through location \textcolor{red}{(def?)} D, with the qubit in blue removed by a $Z$-measurement \textcolor{red}{(background)}. A good mapping should find a trajectory for the pair of qubits in each fusion while making those trajectories as short as possible. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/detour.pdf}
    \caption{Connectivity Conflicts}
    \label{fig:detour}
\end{figure}
Second, as the number of qubits in each resource state is limited, each location cannot be passed by too many trajectories. In the specific case of resource states being GHZ states, each location can be passed by only one trajectory. However, some patterns can be intrinsically non-planar, such as shown in Fig~\ref{fig:k33}. For those patterns, it is impossible to embed them into a layer of resource states with all trajectories being disjoint, thus multiple layers may be required even for a small sub-graph. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.65\linewidth]{fig/k33.pdf}
    \caption{Non-planar Graph}
    \label{fig:k33}
\end{figure}
Third, the increase in the number of required physical layers may cause the qubits in delay lines to expire due to the limit of delay time. This in turn affects the scheduling and decomposition of the pattern.

%After decomposing the graph synthesis into fusions, we need to map it to the physical resource states under the connectivity constraints. For example, the fusion decomposition in Fig.~\ref{fig:high_degree_decomposition} can be mapped to a layout of resource states in Fig.~\ref{fig:high_degree_mapping}. But there are some cases where a direct one-to-one mapping does not exist. The first reason is that for each physical layer, the initial mapping of some resource states are already determined by the previous physical layer since they need to fuse with the delayed qubits from the previous layer.
%The second reason is that the decomposition graph \textcolor{red}{(def)} can contain some cycles \textcolor{red}{(no conflicts in tree?)} that conflict with the connectivity constraints. In those cases, auxiliary resource states are needed. For example, as shown in Fig.~\ref{fig:detour}, the fusions between resource states A, B and C form a cycle. If we map B and C to the neighboring resource states of A, then B and C cannot be neighbors to each other. To resolve the conflicts, we can make a detour, eg. through location \textcolor{red}{(define something like generation location)} D. Since only two qubits of resource state D is needed to connect B and C, the qubit in blue will be assigned a `measure in Z' \textcolor{red}{(explain in background)} operation to detach from the resource state. %The second reason is that for each physical layer, the initial mapping of some resource states are already determined by the previous physical layer since they need to fuse with the delayed qubits from the previous layer. In this case we also need auxiliary resource states as in Fig.~\ref{fig:detour}.


\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/high_degree_mapping.pdf}
    \caption{High degree node mapping}
    \label{fig:high_degree_mapping}
\end{figure}
\fi









==> 05_algorithm_design_01.tex <==
% \newpage
% \section{Synthesis Algorithm Design}
% \label{sect:algorithm}
% In this section, we present the three stages of our compilation framework: xxx, xxx and xxx
% \subsection{Graph Scheduling}
% Given a graph state, each vertex in the underlying graph represents a qubit. We refer to them as \textit{computational qubits}, and denote them with capital letters eg. $U,V,W$ etc. In the synthesis of a graph state, we need some extra qubits which do not appear in the graph but necessary for fusion operations. We refer to them as \textit{auxiliary qubits}, and denote them with small letters eg. $u,v,w$ etc. We say a computational qubit $V$ has a \textit{leg} $l_{Vw}$ if an auxiliary qubit $w$ is entangled with $V$. We say a computational vertex $V$ is \textit{synthesized} if it is entangled with all its neighbors in previous and current dependency layers \textcolor{red}{(precedent/subsequent neighbor??)}, and has a leg $l_{Vw}$ for each of its neighbors $W$ in future dependency layers, with the auxiliary qubit $w$ of the leg representing that neighbor $W$. We say a dependency layer is \textit{synthesized} if all computational qubits in the layer are synthesized. For example, suppose we have a measurement pattern as shown in Fig.~\ref{fig:vertex_synthesis}(a), then Fig.~\ref{fig:vertex_synthesis}(b) shows the process of synthesizing $A$ in $t=0$, synthesizing $B,C$ in $t=1$ and synthesizing $D,E$ in $t=2$, with filled dots representing synthesized computational qubits and hollow dots representing the auxiliary qubits in the legs. The auxiliary qubits are pushed into delay lines for use of synthesizing future computational qubtis via fusions.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/vertex_synthesis.pdf}
%     \caption{Vertex Synthesis}
%     \label{fig:vertex_synthesis}
% \end{figure}

% Considering both measurement-measurement corrections and fusion-measurement corrections \textcolor{red}{(define in challenges)}, a computational qubit is executable when all the qubits in its previous dependency layers are measured, and all its neighbors in future layers are synthesized. Thus for a pattern in Fig.~\ref{fig:vertex_synthesis}(a), the graph scheduling \textcolor{red}{(def)} is shown in Fig.~\ref{fig:scheduling}(a). As we can see, although the $i^\mathrm{th}$ dependency layer is synthesized in $t=i$, it is not executable until $t=i+2$ due to the corrections induced by fusions in $t=i+1$ in order to synthesize the ${i+1}^\mathrm{th}$ dependency layers.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.95\linewidth]{fig/scheduling.pdf}
%     \caption{Graph Scheduling}
%     \label{fig:scheduling}
% \end{figure}

% Note that the pattern in Fig.~\ref{fig:vertex_synthesis}(a) is a simple one because each computational qubit in the $i^\mathrm{th}$ dependency layer is entangled with only computational qubits in the ${i-1}^\mathrm{th}$,$i^\mathrm{th}$, or ${i+1}^\mathrm{th}$ dependency layer. However, in a more complex pattern, that is not guaranteed. A computational qubit in the $i^\mathrm{th}$ layer may have a neighbor in ${i+n}^\mathrm{th}$ dependency layer, which requires a \textit{dependency order separation}. That is, for each computational qubit, we split the dependency order $O_\mathrm{dpnd}$ into a \textit{formation order} $O_\mathrm{form}$ and \textit{execution order} $O_\mathrm{exec}$ according to its neighborhood, represented by an \textit{order vector} $( O_\mathrm{form}, O_\mathrm{exec})$. For each computational qubit $V$, its execution order is the same as its dependency order \textcolor{red}{(modify)}, and its formation order is determined by the neighbor with smallest execution order. If the smallest execution order among all its neighbor is $n$, then its formation order is $n+1$ unless it is in layer 0. Namely
% \begin{align*}
%     O_\mathrm{form}(V) &=\min\left\{O_\mathrm{exec}(V), \min_{U\in nghb\{V\}} O_\mathrm{exec}(U)+1\right\}\\
%     O_\mathrm{exec}(V) &=\max\left\{O_\mathrm{dpnd}, O_\mathrm{form}+2\right\}\\
% \end{align*}
% An auxiliary qubit does not have a formation order, while its execution order is equal to the formation order of the computational qubits it represents, i.e. \[
% O_\mathrm{exec}(w) = O_\mathrm{form}(W)
% \]
% For example, in the pattern shown in Fig.~\ref{fig:order_separation}(a), since vertex $E$ in dependency layer 3 is entangled with vertex $A$ in dependency layer 0, its formation order should be $O_\mathrm{form}(E)=O_\mathrm{form}(A)+1=1$, and its execution order should be $O_\mathrm{exec}(E)=O_\mathrm{dpnd}(E)=3$ \textcolor{red}{(def)}, hence its order is $(1,3)$. Thus the synthesis process of the whole graph is as shown in Fig.~\ref{fig:order_separation}(b).

% %However, while scheduling qubits via their $O_\mathrm{form}$ and $O_\mathrm{exec}$, one thing we need to take care of is the limit in the delay time. If the formation time of a computational qubit is too much earlier than its execution time, the qubit may have exceeded the delay limit by the time it is executable. We address that by introducing an \textit{aging mechanism}, i.e., a qubit ages with the time it is stored in the delay line, and should be \textit{refreshed} once it is too old.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/order_separation.pdf}
%     \caption{Order Separation}
%     \label{fig:order_separation}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/scheduling2.pdf}
%     \caption{Graph Scheduling}
%     \label{fig:scheduling2}
% \end{figure}
\subsection{Adaptive Fusion}
high-degree, planarity

\newpage
\subsection{Adaptive Fusion Decomposition}



%With those primitive patterns, we first

Then we introduce an algorithm to synthesize a vertex from resource states. With that algorithm, each component can be synthesized by traversing the computational qubits by a BFS. In a GHZ state, we refer to the qubit which entangles with both the other two qubits as the \textit{interior qubit}, and the other two qubits as \textit{exterior qubits}. To synthesize a computational qubit $V$, we take a resource state assign its interior qubit as $V$. Then we traverse all neighbors of $V$ in the graph. For a neighbor $U$, if it is already synthesized, then we assign an unused exterior qubits as $u$ and do a leg contraction between $U$ and $V$. Otherwise, we assign an unused exterior qubit as $U$ if the degree of $U$ is 1, and assign it as $u$ if the degree is larger than 1. After that, we check the number of remaining neighbors $n$, and increment the degree of $V$ by a vertex contraction if $n\ge 2$. We visit each neighbor in this way until all are visited. If at this point we have any unused qubit in the resource state, we abandon it by assigning it a $Z$-measurement. 

%Then a graph or a sub-graph can be synthesized by traversing the computational qubits by a BFS. \textcolor{red}{(give an example?)}

 We represent the fusion decomposition by a \textit{fusion graph}. Each vertex in the graph represents a resource state, and there is an edge between two vertices if there is a fusion operation between the quits on those two resource states.



 
 As a summary, we write down the algorithm of vertex synthesis in Algorithm~\ref{alg:vertex_synthesis}, and the algorithm of pattern synthesis in Algorithm~\ref{alg:pattern_synthesis}.

 
\begin{algorithm}[t]
\SetAlgoLined
\KwIn{Synthesized sub-graph $H$ of $G$ \newline new vertex $V$}
\KwOut{Synthesized sub-graph $I$ including $V$}

$visited\_neighbors = []$ ; \\
Assign the interior qubit of $R$ as V\\
visited\_unsythesized\_neighbors = 0;\\
\For{nghb in neighbors}{
    \uIf{$nghb\in H$}{
        Allocate a resource state $R$;\\
        Assign an unused exterior qubit $r$ of $R$ as a representation \textcolor{red}{(def)} of $nghb$;\\
        Fuse $nghb$ and $r$; \tcp{leg contraction}
    }
    \Else{
        \uIf{
            $O_\mathrm{exec}(V) - O_\mathrm{form}(V) > \tau$ and visited\_unsythesized\_neighbors $\ge 1$
        }{
            continue;\\
        }
        \Else{
            Assign an unused exterior qubit $r$ of $R$ as a representation of $nghb$;\\
            visited\_unsythesized\_neighbors = visited\_unsythesized\_neighbors + 1;\\
            \uIf{$O_\mathrm{exec}(V) - O_\mathrm{form}(V) \le \tau$ and degree of nghb == 1}{
                Add $nghb$ to $H$;\\
            }
        }
    }
    Mark $nghb$ as vistied;\\
    \If{number of unvisited neighbors $\ge 2$}{
        Take a new resource state $S$;\\
        Fuse $nghb$ and the interior qubit of $S$; \tcp{vertex contraction}
        Let $R\leftarrow S$;\\
    }
}
Remove unused qubits in $R$ by assigning a $Z$-measurement;\\
Add $V$ to $H$;\\

\caption{Vertex synthesis}
\label{alg:vertex_synthesis}
\end{algorithm}

\begin{algorithm}[t]
\SetAlgoLined
\KwIn{Synthesized sub-graph $H$ of $G$ \newline sub-graph $I$ to synthesize}
\KwOut{Synthesized sub-graph $H\cup I$}

\For{Q in delayed\_computational\_qubits}{
    Q.age $\leftarrow$ Q.age + 1;\\
    \If{Q.age$\ge\tau$ and Q.execution\_order > current\_order}{
        Allocate a new resource state $R$;\\
        Contract one of its leg with the leg of $Q$;\\
        Assign $X$-measurements to $Q$ and the interior qubit of $R$;\\
        Q.formation\_order $\leftarrow$ Q.formation\_order + 1;\\
        vertex\_synthesis(H, Q);\\
    }
}
Traverse $P$ in BFS and synthesize every node in $P$;\\


% \Repeat{$bridge\_rect\_tuple$ converges}{
%     \For{$(r_1, r_2, r_3) \in \otimes^3{bridge\_rects}$}{ 
%         \uIf{$r_0, r_1, r_2, r_3$ are mutually compatible}{
%             $potent\_dqbits = $ qubits enclosed by $r_0, r_1, r_2, r_3$; \tcp{potential data area;}
%             \uIf{$potent\_dqbits \ne \emptyset$}{
%          $bridge\_rect\_tuple.append((r_0,r_1,r_2,r_3))$; \\
%                 break\;
%             }
%         }
%     }
%     set $r_0$ to $r_1, r_2, r_3$ in turn to find new tuples of $r_0, r_1, r_2, r_3$ that has non-empty $potent\_dqbits$\;
% }

% $data\_layout = []$\;
% \For{$r_0, r_1, r_2, r_3$ in $bridge\_rect\_tuple$}{
%     $dqb$ = the qubit at the center of $potent\_dqbits$ of $r_0, r_1, r_2, r_3$\;
%     $data\_layout.append(dqb)$\;
% }
\caption{Pattern synthesis}
\label{alg:pattern_synthesis}
\end{algorithm}


\subsection{Mapping}
This step is to map each resource state to a RSG location of a certain physical layer while satisfying the spatial and temporal constraints on connectivity.

\textit{Planarization:} 
%A \textit{planar graph} is a graph that can be embedded in the plane, i.e., it can be drawn on the plane in such a way that no edges cross each other. Such a drawing is called a \textit{planar embedding} of the graph.
The problem of finding the minimum number of edges that have to be removed from a given graph in order to obtain a planar sub-graph is known to be NP-hard\cite{min_edge_NPhard}. Therefore, we consider finding the \textit{maximal planar sub-graph}, which is defined as a planar sub-graph $G'$ of $G$ that the addition of any edge $e\in G-G'$ destroys planarity. 
In each round, before applying any module, we will always first find a maximal planar sub-graph from the remaining parts of fusion graphs that are not mapped yet.
%we find a maximal planar sub-graph of the fusion graph of each non-separable component which are not mapped yet. 
Then, in a descent order of their sizes, we map them them onto a physical layer until we run out of qubits.


\textit{Planar mapping:} Given a non-separable planar subgraph, we can always find a planar embedding using PQ-trees \textcolor{red}{(in $O(n)?$)}. After that, we map the embedding to the RSG grid of a physical layer. When it is impossible to map neighboring vertices in the graph to neighboring locations on the physical layer, we find a detour to connect them as shown in Fig.~\ref{fig:detour} while minimizing the total lengths of the paths.



\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\linewidth]{fig/planar_decomposition.pdf}
    \caption{Planar Decomposition}
    \label{fig:planar_decomposition}
\end{figure}


\newpage


% \newpage
% \subsection{Graph Generation Scheduling (TO BE DELETED)}
% \label{sect:scheduling}
% In photonic QC, measurements on qubits are destructive, meaning that photons would vanish once measured. Therefore, one important thing we need to make sure is that their computational information is kept by the remaining qubits after they vanish. That requires each qubit to be entangled to some other qubits before it is measured, which induces an operational order when it comes to the execution of a real-time graph state generation \textcolor{red}{(def in background)}. 

% In particular, as qubits in a higher dependency layer \textcolor{red}{(define in background)} have to be measured at least one clock time later than those in the previous dependency layer, the computational information of this dependency layer needs to be transferred to the qubits generated in the future. That requires each dependency layer to be entangled to some qubits which will be stored in the delay line before the layer is measured up, which defines an \textit{extended dependency layer}.

% But there is a tradeoff to make when deciding how much we extend each dependency layer. In principle, a sufficient and necessary condition \textcolor{red}{(modify)} is that each \textit{interface qubit} in the dependency layer, defined as the qubits connected with future dependency layers, is entangled with one other qubit before it is measured. But when an interface qubit is connected to multiple qubits of future dependency layers, generating more of its neighbors with the set of resource states available in this clock time, which we refer to as a \textit{physical layer}, may help reduce the workload of the next physical layer. Considering the varying size of dependency layers and the fix size of physical layers, we may want to generate more or less neighbors for those interface qubits depending on how many qubits are consumed.
% %when we have enough qubits, we always want to generate as many useful neighbors as possible, whereas when the qubits are not abundant, we only want to generate the necessary neighbors.

% However, it is hard to estimate the number of required quits for a given dependency layer because the qubit consumption is significantly affected by the topology \textcolor{red}{(geometry)} of the graph. Since the connectivity between different resource states provided by the fusion operations is at the price of losing two qubits for each fusion, %unlike in the circuit based model, 
% there is not a one-to-one mapping between the qubits in the measurement pattern and the physical qubits as in the circuit based model. 

% To address this problem, we define an \textit{elastic extension} of a dependency layer consisting of a \textit{mandatory extension} which must be generated and a \textit{optional extension} which should be generated as much as possible when having enough physical qubits in the current physical layer. The final extended dependency layer will be optimized by a one-layer lookahead \textcolor{red}{(multi-layer in discussion)}. That is, part of the optional extension may be removed if they turn out to be unhelpful to the implementation of the next dependency layer, as shown in...\textcolor{red}{(add a figure)}

% We introduce the algorithm for elastic extension by first summarize the following observations:
% \begin{enumerate}
%     \item It is necessary to generate at least one neighbor for each interface qubit.
%     \item It is more helpful to generate common neighbors to multiple interface qubits.
%     \item It is less helpful to generate tree-like neighbors.
%     \item It is generally not helpful to consider the interface qubits' connections to dependency layers of distance larger than 1.
% \end{enumerate}


% Non-determinism --> correction --> basis changes --> dependency

% Resource states small --> transfer to future states --> cannot measurement all of them --> must generate more than measured

% The size of each dependency layer varies --> number of cluster state generated in each clock time is fixed --> executing on dependency layer may consume multiple clock times --> fusion acts as glue to connect different resource states, but the price is to lose two photons for each fusion --> unlike in circuit based model, it is hard to estimate how much resources we consume beforehand because we don't have a one-to-one mapping between qubits in the graph state and the physical qubits in the resource states --> we want to consume any few as clock times, but want to use those necessary clock times to generate as much structure as possible --> we address this by finding the set of bonds which are necessary to be generated by executing next dependency layer, and the set of bonds which are not mandatory but can be helpful to next layer if generated --> fully utilize the resource states at hand while leaving optimization opportunities for the stages followed according to the real consumption of resource states.



==> 05_algorithm_design_0724.tex <==
\section{Our Compiler Design}
\label{sect:algorithm}
In this section, we present the three stages of our compilation framework: xxx, xxx and xxx
\subsection{Graph Scheduling}
In this section, we construct a scheduler by analyzing the dependency among operations and taking care of the hardware constraints. Given a measurement pattern in form of a graph, the scheduler finds the executable operations as well as the necessary operations to execute in order to comply with the constraint on delay time.

One-way quantum computing behaves differently with circuit model in its dependency among commands. As an example, all Clifford gates can be executed simultaneously regardless of its position in the corresponding circuit. One type of dependency, which has been well studied, arises from the non-determinism of single-qubit measurements. The other type, which is specific for our setting, comes from the non-determinism of fusion measurements. In the following paragraphs, we rephrase the first type of dependency, specify the second type of dependency, and show how to resolve both types of dependencies jointly.

As introduced in [introsection], 
%a measurement $M_i^\alpha$ on qubit $i$ under $\ket{\pm_\alpha}$ basis induces an operator $X^m J(\alpha)$ with $m$ being the measurement outcome, and any single qubit gate $U$ can be decomposed as $U = e^{i\alpha}J(0)J(\beta)J(\gamma)J(\delta)$.
a dependent measurement \[
_t[M_i^\alpha]^s=M_i^\alpha X_i^s Z_i^t = M_i^{(-1)^s\alpha+t\pi}
\] on qubit $i$ under $\ket{\pm_\alpha}$ basis can be implemented by adjusting the measurement angle from $\alpha$ to $(-1)^s\alpha+t\pi$, where we refer to $s$ as $X$-dependency and $t$ as $Z$-dependency. Note that changing the angle from $\alpha$ to $\alpha+\pi$ only changes $\ket{\pm_\alpha}$ to $\ket{\mp_\alpha}$, i.e., the eigenvalues are interchanged, but the eigenbasis they form remains unchanged. Therefore we do not really need to change the angle but only need to flip the measurement outcome, i.e. interchanging 0 with 1. Namely, the $Z$-dependency only affects the interpretation of the outcome, but does not necessarily leads to an adjustment of measurement basis. We rephrase the rule as following.

\begin{lemma}
\textit{A measurement on a qubit in the graph is executable if all its $X$-dependent qubits are measured and all the $Z$-dependent qubits of each of its $X$-dependent qubits are measured}
\label{lemma:executable_rule}
\end{lemma}

In our fusion-based setting, similar dependency exists due to the non-determinism in fusion operations. 

\begin{lemma}
Let $\ket{\phi},\ket{\psi}$ be arbitrary states. Suppose the original state of $q_1,q_2$ is $E_{12}(\ket{\phi}_1\otimes\ket{+}_2)$, and the original state of $q_3,q_4$ is $E_{12}(\ket{+}_3\otimes\ket{\psi}_4)$. If upon applying a fusion operator on $q_3,q_4$, the outcome is $Z_2X_3=m_{1},X_2Z_3=m_{2}$, then the state of $q_1,q_4$ collapses to\[
\ket{\Psi}=Z_1^{m_{1}}Z_4^{m_{2}}E_{ij}(\ket{\phi}_1\otimes\ket{\psi}_4)
\]
\label{lemma:fusion_Z_correction}
\end{lemma}

Namely, a fusion operator on two qubits induces possible $Z$-corrections on their neighbors, which is illustrated with Fig.~\ref{fig:fusion_Z_correction}. Suppose that in the measurement pattern, $q_4$ is $X$-dependent on $q_1$, then according to Lemma~\ref{lemma:executable_rule}, $q_4$ is executable only after the measurement on $q_1$ and the fusion on $q_2,q_3$ are both completed in the past time cycles.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.3\linewidth]{fig/fusion_Z_correction.pdf}
    \caption{Fusion Z-correction}
    \label{fig:fusion_Z_correction}
\end{figure} 

Let $H$ be a subgraph of $G$, let $H'$ be the graph formed by adding to $H$ all the edges of $G$ with one end in $H$ and the other end in $G-H$. Those edges are called \textit{virtual edges}, and their ends in $G-H$ are called virtual vertices. The virtual vertices are labeled as their counterparts in $G$ but kept separable, i.e. there may be many virtual vertices with the same label, each with exactly one entering edge. We say a vertex is \textit{synthesized} if all its virtual edges, if exist, are added to the subgraph with the help of fusion. The virtual vertices are then stored into delay lines for use of synthesizing future vertices. For example, suppose we have a measurement pattern as shown in Fig.~\ref{fig:graph_synthesis}(a), then Fig.~\ref{fig:graph_synthesis}(b) shows the process of synthesizing $\{A,B,C\}$ in $t=0$, synthesizing $\{D\}$ in $t=1$, $\{E\}$ in $t=2$, etc., with filled dots standing for synthesized vertices, hollow dots standing for the virtual vertices. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/graph_synthesis.pdf}
    \caption{Graph Synthesis}
    \label{fig:graph_synthesis}
\end{figure} From Lemma~\ref{lemma:executable_rule} and Lemma~\ref{lemma:fusion_Z_correction}, each vertex has to be synthesized at least one clock cycle prior to its execution so that is has time to adjust the measurement basis accordingly. In Fig.~\ref{fig:graph_synthesis}, measurable vertices are marked by yellow dots. However, synthesizing the vertices too early bring a risk of qubit expiration due to the limit in delay time, as a result we adopt the one-step lookahead for synthesizing vertices. That is, we find the vertices that can be unblocked by the measurements of this cycle, and synthesize them in this time cycle so that they can be measured in the next time cycle.

Note that in Fig.~\ref{fig:graph_synthesis}, qubit $A$ is born in $t=0$ but need to wait for fusion in the delay line until $t=3$. In a more complex pattern, this waiting period can exceed the limit of delay time. Therefore we need to introduce a refresh mechanism to prevent it from being expired. (more details...)


\begin{lemma}
The scheduler follows the following rules to schedule operations in each round
\begin{itemize}
    \item `measure' to the qubits in the front layer
    \item `synthesize' to the qubits in the next layer
    \item `delay' to all virtual qubits
    \item `refresh' the qubits whose...
\end{itemize}
\end{lemma}

The output of the scheduler is a subgraph with virtual vertices, with some vertices assigned a `measurement' operation, some vertices assigned a `synthesis' operation, all the newly created virtual vertices assigned a `delay' operation, and some of the old vertices assigned a `refresh' operation.

==> 05_algorithm_module0.tex <==
\paragraph{Planarization} 
We first decompose the graph into a set of non-separable sub-graphs by finding all its cut vertices, because those components can be joined easily once we find the fusion decomposition for each of them. A vertex $v$ in a connected graph $G$ is called a \textit{cut vertex} if deleting $v$ and its edges results in disconnected components. A graph is said to be \textit{non-separable} if it is a connected graph of at least two vertices that contains no cut vertices. By splitting the cut vertices, the graph can be decomposed multiple disconnected components. For example, in Fig.~\ref{fig:cut_vertex}, the black dot is a cut vertex whose split results in the sub-graphs in red, blue and green. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/cut_vertex.pdf}
    \caption{Component Decomposition}
    \label{fig:cut_vertex}
\end{figure}



Then, we break the underlying graph of a given measurement pattern into multiple planar graphs in order to allow a pipelining synthesis.  A \textit{planar graph} is a graph that can be drawn on a plane with no edges crossing each other. Such a drawing is called a \textit{planar embedding} of the graph. This is necessary for our pipelining design because only one physical layer \textcolor{red}{(def)} is available at each clock cycle, where each resource state on the physical layer can be passed through by only one (or few) trajectory due to its small size. The planar decomposition ensures that for each subgraph there exists a fusion strategy that can be embedded on the physical layer. For example, suppose that we want to synthesize a graph as shown in Fig.~\ref{fig:planar_decomposition}(a), there is no way to realize that in a single physical layer as the graph itself is non-planar. Instead, we decompose it into 2 planar subgraphs as shown in Fig.~\ref{fig:planar_decomposition}(b) and realize each subgraph in a physical layer.
% each RSG generates only one resource state, together forming a layer of resource states which we refer to as a \textit{physical layer}.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/planar_decomposition.pdf}
    \caption{Decompose a non-planar graph in into  two planar subgraphs, with hollowed dots representing virtual vertices}
    \label{fig:planar_decomposition}
\end{figure}



\textit{Planarization:} 
%A \textit{planar graph} is a graph that can be embedded in the plane, i.e., it can be drawn on the plane in such a way that no edges cross each other. Such a drawing is called a \textit{planar embedding} of the graph.
The problem of finding the minimum number of edges that have to be removed from a given graph in order to obtain a planar sub-graph is known to be NP-hard\cite{min_edge_NPhard}. Therefore, we consider finding the \textit{maximal planar sub-graph}, which is defined as a planar sub-graph $G'$ of $G$ that the addition of any edge $e\in G-G'$ destroys planarity. 
In each round, before applying any module, we will always first find a maximal planar sub-graph from the remaining parts of fusion graphs that are not mapped yet.
%we find a maximal planar sub-graph of the fusion graph of each non-separable component which are not mapped yet. 
Then, in a descent order of their sizes, we map them them onto a physical layer until we run out of qubits.


\textit{Planar mapping:} Given a non-separable planar subgraph, we can always find a planar embedding using PQ-trees \textcolor{red}{(in $O(n)?$)}. After that, we map the embedding to the RSG grid of a physical layer. When it is impossible to map neighboring vertices in the graph to neighboring locations on the physical layer, we find a detour to connect them as shown in Fig.~\ref{fig:detour} while minimizing the total lengths of the paths.



\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\linewidth]{fig/planar_decomposition.pdf}
    \caption{Planar Decomposition}
    \label{fig:planar_decomposition}
\end{figure}


\newpage


% \newpage
% \subsection{Graph Generation Scheduling (TO BE DELETED)}
% \label{sect:scheduling}
% In photonic QC, measurements on qubits are destructive, meaning that photons would vanish once measured. Therefore, one important thing we need to make sure is that their computational information is kept by the remaining qubits after they vanish. That requires each qubit to be entangled to some other qubits before it is measured, which induces an operational order when it comes to the execution of a real-time graph state generation \textcolor{red}{(def in background)}. 

% In particular, as qubits in a higher dependency layer \textcolor{red}{(define in background)} have to be measured at least one clock time later than those in the previous dependency layer, the computational information of this dependency layer needs to be transferred to the qubits generated in the future. That requires each dependency layer to be entangled to some qubits which will be stored in the delay line before the layer is measured up, which defines an \textit{extended dependency layer}.

% But there is a tradeoff to make when deciding how much we extend each dependency layer. In principle, a sufficient and necessary condition \textcolor{red}{(modify)} is that each \textit{interface qubit} in the dependency layer, defined as the qubits connected with future dependency layers, is entangled with one other qubit before it is measured. But when an interface qubit is connected to multiple qubits of future dependency layers, generating more of its neighbors with the set of resource states available in this clock time, which we refer to as a \textit{physical layer}, may help reduce the workload of the next physical layer. Considering the varying size of dependency layers and the fix size of physical layers, we may want to generate more or less neighbors for those interface qubits depending on how many qubits are consumed.
% %when we have enough qubits, we always want to generate as many useful neighbors as possible, whereas when the qubits are not abundant, we only want to generate the necessary neighbors.

% However, it is hard to estimate the number of required quits for a given dependency layer because the qubit consumption is significantly affected by the topology \textcolor{red}{(geometry)} of the graph. Since the connectivity between different resource states provided by the fusion operations is at the price of losing two qubits for each fusion, %unlike in the circuit based model, 
% there is not a one-to-one mapping between the qubits in the measurement pattern and the physical qubits as in the circuit based model. 

% To address this problem, we define an \textit{elastic extension} of a dependency layer consisting of a \textit{mandatory extension} which must be generated and a \textit{optional extension} which should be generated as much as possible when having enough physical qubits in the current physical layer. The final extended dependency layer will be optimized by a one-layer lookahead \textcolor{red}{(multi-layer in discussion)}. That is, part of the optional extension may be removed if they turn out to be unhelpful to the implementation of the next dependency layer, as shown in...\textcolor{red}{(add a figure)}

% We introduce the algorithm for elastic extension by first summarize the following observations:
% \begin{enumerate}
%     \item It is necessary to generate at least one neighbor for each interface qubit.
%     \item It is more helpful to generate common neighbors to multiple interface qubits.
%     \item It is less helpful to generate tree-like neighbors.
%     \item It is generally not helpful to consider the interface qubits' connections to dependency layers of distance larger than 1.
% \end{enumerate}


% Non-determinism --> correction --> basis changes --> dependency

% Resource states small --> transfer to future states --> cannot measurement all of them --> must generate more than measured

% The size of each dependency layer varies --> number of cluster state generated in each clock time is fixed --> executing on dependency layer may consume multiple clock times --> fusion acts as glue to connect different resource states, but the price is to lose two photons for each fusion --> unlike in circuit based model, it is hard to estimate how much resources we consume beforehand because we don't have a one-to-one mapping between qubits in the graph state and the physical qubits in the resource states --> we want to consume any few as clock times, but want to use those necessary clock times to generate as much structure as possible --> we address this by finding the set of bonds which are necessary to be generated by executing next dependency layer, and the set of bonds which are not mandatory but can be helpful to next layer if generated --> fully utilize the resource states at hand while leaving optimization opportunities for the stages followed according to the real consumption of resource states.



==> 05_algorithm_module1.tex <==
\subsection{Fusion Graph Generation}
\label{sect:module1}


\paragraph{High-degree node synthesis}
Then, we define a basic fusion pattern to synthesize high degree nodes given the fact that each qubit in a single GHZ resource state has a degree of at most 2. We adopt a simplest linear pattern despite that there exist multiple options. The comparison between those patterns can be left to future work.
% As shown in Fig.~\ref{fig:primitives}, fusing a vertex with the qubit in a GHZ state of degree 2 increases its degree by one, while fusing it with the qubit of degree 1 extends the edge.
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.75\linewidth]{fig/primitives.pdf}
%     \caption{Primitive Patterns}
%     \label{fig:primitives}
% \end{figure}Therefore, w
We can synthesize a high degree vertex by repeatedly fusing a low degree vertex with the qubits of degree 2 in the resource states until enough degree is obtained, as shown in Fig.~\ref{fig:linear_fusion}(a)(b). Because fusing a vertex with the qubit in a GHZ state of degree 2 increases its degree by one, while fusing it with a qubit of degree 1 extends the edge. In this way, a vertex of degree $n$ can be synthesized with $n-1$ resource states. We can represent a fusion pattern with a \textit{fusion graph} representation, where each node stands for a resource state, and each edge stands for a fusion operation between qubits on two nodes. In this way our basic fusion pattern can be represented by Fig.~\ref{fig:linear_fusion}(c).


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.65\linewidth]{fig/linear_fusion.pdf}
    \caption{Synthesize a high degree vertex in (a) by a basic fusion pattern in (b). Represent the fusion pattern by a fusion graph in (c), with each node representing a resource state, each edge representing a fusion operation}
    \label{fig:linear_fusion}
\end{figure}




\paragraph{Planar graph synthesis}
Last, we produce a fusion graph for the whole planar subgraph using the basic pattern of node synthesis while maintaining the planarity.This can be done by first finding a planar embedding for the planar subgraph, and then replacing each $n$-degree node with their fusion graphs. During the replacement, we join each node of a fusion graph with its neighbors while keeping the clockwise (counter clockwise) order of the neighbors. For example, in the planar graph shown in Fig.~\ref{fig:vertex_split}(a), the 4-degree node $O$ has neighbors $B,A,C,D$ in a counter clockwise order, so we replace $O$ with a fusion graph component of 3 nodes, and join the nodes with $B,A,C,D$ in a counter clockwise order. Note that the last node joins with both $D$ and $B$. For the 3-degree node $A$ (similarly for $B,C,D$) with counter clockwise neighbors $B,C,O$, we replace it with a component of 2 nodes, and join the nodes with $B,C,O$ in an counter clockwise order.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/planar_fusion.jpg}
    \caption{Transform a planar graph (a) into a fusion graph while (b) maintaining the planarity (c) or not. Each vertex in (a) is synthesized by nodes in the same shaded area in (b) and (c)}
    \label{fig:vertex_split}
\end{figure}


\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/fusion_decomposition.jpg}
    \caption{Synthesize a high degree vertex in (a) by a basic fusion pattern in (b). Represent the fusion pattern by a fusion graph in (c), with each node representing a resource state, each edge representing a fusion operation}
    \label{fig:fusion_decomp}
\end{figure}

In order to decompose a general pattern into fusion operations adaptively, we introduce some primitive patterns which serve as basic blocks in our algorithm. First, we can \textit{add a leg} $l_{Vu}$ to a vertex $V$ by a fusion pattern as shown in Fig.~\ref{fig:primitive}(a), where $u$ can represent either $V$ itself or a different computational qubit $W$. The choice of its representation will be explained when we introduce the algorithm. Second, two computational qubits $V,W$ can be connected by a \textit{leg contraction} between $l_{Vw}$ and $l_{vW}$ as shown in Fig.~\ref{fig:primitive}(b). Third, the degree of a vertex $V$ can be increased by 1 with a \textit{vertex contraction} as shown in Fig.~\ref{fig:primitive}(c), which fuses two auxiliary qubits that represent the same computational qubit. %Fourth, same computational qubits can be merged by a \textit{vertex merge} as shown in Fig.~\ref{fig:primitive}(d), which also leads to an increase in the degree of vertex $V$. Note that a vertex merge can be implemented by adding a leg and then doing a vertex contraction. But we still list it here because it is a small enough pattern that is frequently used in our algorithm.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{fig/primitive.pdf}
    \caption{Primitive Pattern}
    \label{fig:primitive}
\end{figure}


One-way quantum computing behaves differently with circuit model in its dependency among commands. As an example, all Clifford gates can be executed simultaneously regardless of its position in the corresponding circuit. One type of dependency, which has been well studied, arises from the non-determinism of single-qubit measurements. The other type, which is specific for our setting, comes from the non-determinism of fusion measurements. In the following paragraphs, we rephrase the first type of dependency, specify the second type of dependency, and show how to resolve both types of dependencies jointly.

As introduced in [introsection], 
%a measurement $M_i^\alpha$ on qubit $i$ under $\ket{\pm_\alpha}$ basis induces an operator $X^m J(\alpha)$ with $m$ being the measurement outcome, and any single qubit gate $U$ can be decomposed as $U = e^{i\alpha}J(0)J(\beta)J(\gamma)J(\delta)$.
a dependent measurement \[
_t[M_i^\alpha]^s=M_i^\alpha X_i^s Z_i^t = M_i^{(-1)^s\alpha+t\pi}
\] on qubit $i$ under $\ket{\pm_\alpha}$ basis can be implemented by adjusting the measurement angle from $\alpha$ to $(-1)^s\alpha+t\pi$, where we refer to $s$ as $X$-dependency and $t$ as $Z$-dependency. Note that changing the angle from $\alpha$ to $\alpha+\pi$ only changes $\ket{\pm_\alpha}$ to $\ket{\mp_\alpha}$, i.e., the eigenvalues are interchanged, but the eigenbasis they form remains unchanged. Therefore we do not really need to change the angle but only need to flip the measurement outcome, i.e. interchanging 0 with 1. Namely, the $Z$-dependency only affects the interpretation of the outcome, but does not necessarily leads to an adjustment of measurement basis. We rephrase the rule as following.

\begin{lemma}
\textit{A measurement on a qubit in the graph is executable if all its $X$-dependent qubits are measured and all the $Z$-dependent qubits of each of its $X$-dependent qubits are measured}
\label{lemma:executable_rule}
\end{lemma}

In our fusion-based setting, similar dependency exists due to the non-determinism in fusion operations. 

\begin{lemma}
Let $\ket{\phi},\ket{\psi}$ be arbitrary states. Suppose the original state of $q_1,q_2$ is $E_{12}(\ket{\phi}_1\otimes\ket{+}_2)$, and the original state of $q_3,q_4$ is $E_{12}(\ket{+}_3\otimes\ket{\psi}_4)$. If upon applying a fusion operator on $q_3,q_4$, the outcome is $Z_2X_3=m_{1},X_2Z_3=m_{2}$, then the state of $q_1,q_4$ collapses to\[
\ket{\Psi}=Z_1^{m_{1}}Z_4^{m_{2}}E_{ij}(\ket{\phi}_1\otimes\ket{\psi}_4)
\]
\label{lemma:fusion_Z_correction}
\end{lemma}

Namely, a fusion operator on two qubits induces possible $Z$-corrections on their neighbors, which is illustrated with Fig.~\ref{fig:fusion_Z_correction}. Suppose that in the measurement pattern, $q_4$ is $X$-dependent on $q_1$, then according to Lemma~\ref{lemma:executable_rule}, $q_4$ is executable only after the measurement on $q_1$ and the fusion on $q_2,q_3$ are both completed in the past time cycles.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.3\linewidth]{fig/fusion_Z_correction.pdf}
    \caption{Fusion Z-correction}
    \label{fig:fusion_Z_correction}
\end{figure} 


==> 05_algorithm_module2.tex <==
\subsection{2D-Lattice Mapping and Routing}
\label{sect:module2}
This step is to map each resource state to a RSG location of a certain physical layer while satisfying the spatial and temporal constraints on connectivity.

%\subsection{Planarity-Aware Heuristic Mapping}
The final step is to map the fusion graph onto physical device. Our goal is to minimize the depth (or volume) while taking consideration of the limited size of each physical layer and the spatial and temporal constraints on connectivity. We emphasize the importance of planarity awareness when tackling the mapping problem because it significantly reduces conflicts between the paths of different edges. In general, optimizing the compactness of a planar layout on a grid is a NP-hard problem[?]. Our problem is at least the same hard because it can reduce to the general problem by lifting the boundary constraints. Therefore, we adopt a planar-awareness heuristic method for finding a compact layout under the hardware constraints.

\paragraph{Mapping Order of Edges}
In a planar graph, we observe that only the planar order (clockwise or counter-clockwise) among edges involved in cycles matter for the planarity, while the planar order of non-cycle edges are permutable, both permutable among themselves and permutable with the cycle edges. Therefore we prioritize the mapping of cycle edges by adding all cycle edges of a vertex before its non-cycle edges. In specific, the mapping order the edges is determined by a depth-first order along with cycle priority as follows: 1) We first find a subgraph containing all the cycles by pruning the trees, and push the cycle edges into a queue in the order of a depth-first search of the subgraph. 2) After pushing each cycle edge, we check whether the cycle edges of a certain vertex are all added. 3) If so, we then push the edges of the tree rooted at that vertex. 

\paragraph{Planar Mapping}
During the mapping stage, we first find a planar embedding of the cycle involved subgraph. For a cycle edge, we search for its mapping while keeping consistent with the planar embedding, while for a tree edge, that is not required. A viable layout of edge $(s,e)$ in each step of the heuristic search should satisfy the following constraints: 1) If $(s,e)$ is a non-cycle edge, we need to make sure that $s$ the adjacent grid positions available is no less than its remaining degrees so as to accommodate all its neighbors; if not, then we extend $s$ until we find an open area with enough adjacent availability. 2) If $(s,e)$ is a cycle edge, this adjacent availability should also take the planar order into consideration, i.e. the layout of the edge should not only be consistent with the planar order with existing edges, but should also leave enough adjacent positions for all its clockwise neighbors and counter-clockwise neighbors. Under those
constraints, we propose the following heuristic.

\todo{pseduocode}

However, besides synthesizing necessary computational qubits, we also need to take care of the qubits delayed from previous physical layers considering there is a limit in the delay time. That is, if the formation time of a computational qubit is too much earlier than its execution time, the qubit may have exceeded the delay limit by the time it is executable. We address that by introducing an \textit{aging mechanism}, i.e., a qubit ages with the time it is stored in the delay line, and should be \textit{refreshed}, as shown in Fig.~\ref{fig:refresh}, once it is too old. In Fig.~\ref{fig:refresh}(a), $V$ is a synthesized vertex. We refresh it by synthesizing a pattern in Fig.~\ref{fig:refresh}(b) and fusing it with the original vertex as shown in Fig.~\ref{fig:refresh}(c), with the qubits in red is assigned an $X$-measurement and qubits in blue assigned a $Z$-measurement. \textcolor{red}{(explain?)}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/refresh.pdf}
    \caption{Qubit Refreshing}
    \label{fig:refresh}
\end{figure}

 Note that if a qubit needs to be refreshed before its execution, then it is unnecessary to add its legs because they will be removed in the refresh. Thus we optimize the algorithm of vertex synthesis by check the $O_\mathrm{form}$ and $O_\mathrm{exec}$ of a qubit before synthesizing it. If $O_\mathrm{exec} - O_\mathrm{form} > \tau$ where $\tau$ is the delay time limit, then we add only one leg \textcolor{red}{(more precise)} to the vertex, which we refer to as a \textit{partial synthesis}. After that, we update its $O_\mathrm{form}$ by the current time. If we still have $O_\mathrm{exec} - O_\mathrm{form} > \tau$, then similarly we add only one leg when synthesize the new vertex in Fig.~\ref{fig:refresh}(b), which we refer to as a \textit{partial refresh}.


==> 05_algorithm_module3.tex <==
\subsection{Graph Partition and Scheduling}
\label{sect:module3}


In this section, we construct a scheduler by analyzing the dependency among operations and taking care of the hardware constraints. Given a measurement pattern in form of a graph, the scheduler finds the executable operations as well as the necessary operations to execute in order to comply with the constraint on delay time.


Let $H$ be a subgraph of $G$, let $H'$ be the graph formed by adding to $H$ all the edges of $G$ with one end in $H$ and the other end in $G-H$. Those edges are called \textit{virtual edges}, and their ends in $G-H$ are called virtual vertices. The virtual vertices are labeled as their counterparts in $G$ but kept separable, i.e. there may be many virtual vertices with the same label, each with exactly one entering edge. We say a vertex is \textit{synthesized} if all its virtual edges, if exist, are added to the subgraph with the help of fusion. The virtual vertices are then stored into delay lines for use of synthesizing future vertices. For example, suppose we have a measurement pattern as shown in Fig.~\ref{fig:graph_synthesis}(a), then Fig.~\ref{fig:graph_synthesis}(b) shows the process of synthesizing $\{A,B,C\}$ in $t=0$, synthesizing $\{D\}$ in $t=1$, $\{E\}$ in $t=2$, etc., with filled dots standing for synthesized vertices, hollow dots standing for the virtual vertices. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/graph_synthesis.pdf}
    \caption{Graph Synthesis}
    \label{fig:graph_synthesis}
\end{figure} From Lemma~\ref{lemma:executable_rule} and Lemma~\ref{lemma:fusion_Z_correction}, each vertex has to be synthesized at least one clock cycle prior to its execution so that is has time to adjust the measurement basis accordingly. In Fig.~\ref{fig:graph_synthesis}, measurable vertices are marked by yellow dots. However, synthesizing the vertices too early bring a risk of qubit expiration due to the limit in delay time, as a result we adopt the one-step lookahead for synthesizing vertices. That is, we find the vertices that can be unblocked by the measurements of this cycle, and synthesize them in this time cycle so that they can be measured in the next time cycle.

Note that in Fig.~\ref{fig:graph_synthesis}, qubit $A$ is born in $t=0$ but need to wait for fusion in the delay line until $t=3$. In a more complex pattern, this waiting period can exceed the limit of delay time. Therefore we need to introduce a refresh mechanism to prevent it from being expired. (more details...)


\begin{lemma}
The scheduler follows the following rules to schedule operations in each round
\begin{itemize}
    \item `measure' to the qubits in the front layer
    \item `synthesize' to the qubits in the next layer
    \item `delay' to all virtual qubits
    \item `refresh' the qubits whose...
\end{itemize}
\end{lemma}

The output of the scheduler is a subgraph with virtual vertices, with some vertices assigned a `measurement' operation, some vertices assigned a `synthesis' operation, all the newly created virtual vertices assigned a `delay' operation, and some of the old vertices assigned a `refresh' operation.

==> 05_hezi_module1.tex <==
\vspace{0.3em}
\section{Fusion Graph Generation}
\label{sect:module1}

We start introducing \frameworkname~from a planar graph component that has been partitioned and scheduled from the input program.
% small cases where the graph state of the input program has already been  partitioned and scheduled to planar sub-graphs. 
The key challenge at this step is to synthesize the high-degree nodes in the planar graphs from low-degree nodes that are directly supported by the hardware.

%This section focuses on generating the fusion graph from a graph state which has been partitioned and scheduled to planar sub-graphs. Details about partitioning and scheduling will be discussed in section \ref{sect:module3}.
%\newline
\vspace{0.3em}
\subsection{Basic Patterns}
We start by defining a set of basic patterns, which will lay a foundation for supporting arbitrary graph states via small resource states. As shown in Fig.~\ref{fig:basic_fusion_patterns}, the degree of a node $V$ in a sub-graph can be incremented by applying a fusion between $V$ and a \fix{multi-degree node (those of degree $>1$)} of a resource state (Fig.~\ref{fig:basic_fusion_patterns}(a)); the length of an edge from $V$ can be extended by applying a fusion between $V$ and a \fix{leaf node (those of degree 1)} of a resource states (Fig.~\ref{fig:basic_fusion_patterns}(b)). Hence an arbitrary graph can be synthesized by alternating those two basic patterns dynamically. Moreover, two synthesized graphs can be connected by applying a fusion between two leaf nodes of them (Fig.~\ref{fig:basic_fusion_patterns}(c)). This plays the key role of connecting the sub-graphs scheduled in different rounds.

\begin{figure}[h!]
    \centering
    %  \vspace{-5pt}
    \includegraphics[width=0.65\linewidth]{fig/three_basic_patterns.pdf}
    \caption{(a) Increment the degree of a node. (b) Extend the length of a line. (c) Connecting two sub-graphs into a graph.} 
    % \vspace{-5pt}
    \label{fig:basic_fusion_patterns}
\end{figure}


% \vspace{0.2em}
\subsection{Graph synthesis}
High degree nodes are prevalent in graph states of MBQC. For example, a logical qubit (G in Fig.~\ref{fig:procedure}(a)) involved in multiple CNOT gates in a circuit can result in a high degree node (G in Fig.~\ref{fig:procedure}(b)) in the corresponding graph state. Our framework supports such high degree nodes on small resource states via the basic pattern of degree increment (Fig.~\ref{fig:basic_fusion_patterns}(a)). As shown in Fig.\ref{fig:linear_fusion}(a)(b), we can synthesize a node of arbitrarily high degree by repeatedly fusing a lower degree node with the multi-degree node of a resource state until enough degree is obtained. In this way, a node of degree $n$ can be synthesized from $n-1$ resource states. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.65\linewidth]{fig/linear_fuse.pdf}\\
    (a)\hspace{50pt}(b)\hspace{50pt}(c)
    \caption{Synthesize a high degree node in (a) by a basic fusion pattern in (b). Represent the fusion pattern by a fusion graph in (c), with each `$\otimes$' node representing a resource state, each edge representing a fusion operation.}
    % \vspace{-15pt}
    \label{fig:linear_fusion}
\end{figure}

To synthesize a graph, we can first synthesize the high degree nodes in the above way and synthesize the low degree lines by the basic pattern of line extension (Fig.~\ref{fig:basic_fusion_patterns}(b)). Then, the high degree nodes and lines can be connected via the basic pattern of sub-graph connection (Fig.~\ref{fig:basic_fusion_patterns}(c)). We demonstrate it with an example of synthesizing a graph in Fig.~\ref{fig:vertex_split}(a). In Fig.~\ref{fig:vertex_split}(b), we break down the graph into high degree nodes $A,B,C,D,O$ and lines $PQ,RS$. Each node high degree node or each line is connected with some nodes in hollowed dots, which represent its neighbors in Fig.~\ref{fig:vertex_split}(a). Those nodes are referred to as \emph{virtual nodes}. Note that multiple virtual nodes are allowed to represent the same node, such as $A,B,C,D,O$. In Fig.~\ref{fig:vertex_split}(c), we pair up the virtual nodes according to the original graph Fig.~\ref{fig:vertex_split}(a) and synthesize the graph by applying the basic pattern of sub-graph connection (Fig.~\ref{fig:basic_fusion_patterns}(c)) on the paired virtual nodes. \label{subsect:graph_synthesis}


% We can represent a fusion pattern with a \textit{fusion graph} representation, where each node stands for a resource state, and each edge stands for a fusion operation between qubits on two nodes. In this way our basic fusion pattern can be represented by Fig.~\ref{fig:linear_fusion}(c).

% To make our framework able to support graph states with arbitrarily high-degree nodes through small resource states, we define a pattern that synthesizes high degree nodes from resource states as small as 3-qubit GHZ states, whose qubits are all of degree $\le 2$.

% We define a basic fusion pattern to synthesize high degree nodes in a graph state from a bunch of GHZ resource states whose qubits are of degree $\le 2$. As shown in Fig.\ref{fig:basic_fusion_patterns}, the degree of a node can be incremented by fusing it with the root node in a GHZ state (Fig.\ref{fig:basic_fusion_patterns}(b)), where a leaf node, if not exist, can be added to a graph by fusing the graph with a leaf node in a GHZ state (Fig.\ref{fig:basic_fusion_patterns}(a)), which also increments the degree of the original node. 

% Based on this observation, we adopt a  linear pattern to synthesize high degree nodes. As shown in Fig.\ref{fig:linear_fusion}(a)(b), we can synthesize a high degree node by repeatedly fusing a lower degree node with the root of a GHZ resource state until enough degree is obtained. In this way, a node of degree $n$ can be synthesized from $n-1$ GHZ resource states. We can represent a fusion pattern with a \textit{fusion graph} representation, where each node stands for a resource state, and each edge stands for a fusion operation between qubits on two nodes. In this way our basic fusion pattern can be represented by Fig.~\ref{fig:linear_fusion}(c).

%Note that there exist multiple options. The optimization of the choice of basic patterns can be left to future work. 

% \input{05_algorithm_module0.tex}

% \begin{figure}[h!]
%     \centering
%      \vspace{-5pt}
%     \includegraphics[width=\linewidth]{fig/basic_fusion_paterns.pdf}
%      \vspace{-10pt}
%     \caption{Synthesize a high degree vertex in (a) by a basic fusion pattern in (b). Represent the fusion pattern by a fusion graph in (c), with each node representing a resource state, each edge representing a fusion operation}
%     \label{fig:basic_fusion_patterns}
% \end{figure}

\vspace{0.3em}
\subsection{Optimized Fusion Graph}
The fusion relations between small resource states in a synthesis pattern can be abstracted to a \emph{fusion graph} by considering each resource state as a whole. For example, the synthesis pattern of a high degree node in Fig.~\ref{fig:linear_fusion}(b) can be represented by a fusion graph in Fig.~\ref{fig:linear_fusion}(c), with each node `$\otimes$' representing a resource state, and each edge representing a fusion between certain qubits of the resource states. With a breakdown (Fig.~\ref{fig:vertex_split}(b)) of the graph state (Fig.~\ref{fig:vertex_split}(a)), a fusion graph can be generated by replacing the high degree nodes with their corresponding fusion graphs 
% (`$\otimes$'s in the same grey circle)
(Fig.~\ref{fig:vertex_split}(c)) and joining them together (Fig.~\ref{fig:vertex_split}(d)).

Yet, not every fusion graph is equally good. We hope that the fusion graph generation does not break the planarity of the original graph due to a hardware constraint that will be introduced in Section~\ref{subsect:hardware_constraint}. Namely, the generated fusion graph of a planar graph should still be a planar graph, meaning that the graph can be drawn on a plane with edges not crossing each other. This can be achieved by first finding a planar embedding (Fig.~\ref{fig:vertex_split}(a)) of the original graph, i.e. a way of drawing it on the plane with no crossing edges, and then
% then replacing each high degree node with their linear fusion graphs while 
keeping the clockwise (counter-clockwise) orders among the edges when connecting the fusion graphs of the high degree nodes (Fig.~\ref{fig:vertex_split}(d)). 

For example, in the planar graph in Fig.~\ref{fig:vertex_split}(a), the 4-degree node $O$ has neighbors $A,B,D,C$ in the clockwise order. So we replace it with a fusion graph component of 3 nodes (component $O$ in the grey circle at the center of Fig.~\ref{fig:vertex_split}(c)), and connect it with fusion graph components of $A,B,D,C$ clockwisely (Fig.~\ref{fig:vertex_split}(d)). Note that one of the nodes in component $O$ connects with both components $C$ and $D$. For the 3-degree node $A$ (and $B,C,D$ similarly) which has clockwise neighbors $B,O,P$, we replace it with a fusion graph component of 2 nodes (component $A$ in Fig.~\ref{fig:vertex_split}(c)) and connect it with components $B,O,P$ clockwisely. As a comparison, Fig.~\ref{fig:vertex_split}(e) shows a fusion graph that breaks the planarity if not keeping the clockwise (counter-clockwise) edge orders.

% $B,A,C,D$ in a counter clockwise order, so we replace $O$ with the corresponding fusion graph component of 3 nodes (the grey circle in the center of Fig.~\ref{fig:vertex_split}(c)), and join the nodes with $B,A,C,D$ in a counter clockwise order (Fig.~\ref{fig:vertex_split}(d)). Note that the last node joins with both $D$ and $C$. For the 3-degree node $A$ (similarly for $B,C,D$) with counter clockwise neighbors $B,C,O$, we replace it with a component of 2 nodes, and join the nodes with $B,C,O$ in an counter clockwise order (Fig.~\ref{fig:vertex_split}(c)). As a comparison, Fig.~\ref{fig:vertex_split}(d) shows a fusion graph that breaks the planarity if not keeping the clockwise (counter-clockwise) orders.

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/planar_graph_synthesis-4.pdf}\\
    \vspace{-10pt}
    (a)\hspace{85pt}(b)\hspace{85pt}(c)\hspace{85pt}(d)\hspace{110pt}(e)
    \caption{Fusion graph generation. (a) A planar embedding of the graph state geometry. (b) Split the edges. (c) Replace each high-degree node with a piece of fusion graph, with each `$\otimes$' node representing a resource state. (d) Connect the pieces of fusion graphs while keeping the clockwise (counter-clockwise) edge orders in the planar embedding so as to obtain a planar fusion graph. (e) The planarity may be broken if not keeping the clockwise (counter-clockwise) edge orders.}
    
    % A graph state (a) can be synthesized by first synthesizing high degree nodes with the basic pattern of degree increment and synthesizing lines with the basic pattern of line extension (obtaining (b)), then connecting them with the basic pattern of sub-graph connection as in (c). An optimized fusion graph of a planar graph (a) should still be planar, e.g. (d), while a random fusion graph may break the planarity, e.g. (e). \todo{todo}}
    \vspace{-10pt}
    \label{fig:vertex_split}
\end{figure*}



==> 05_hezi_module2.tex <==
\vspace{0.3em}
\section{Fusion Mapping and Routing}
\label{sect:module2}
% After resolving the high-degree nodes, t
The next step is to map each resource state in the fusion graph to a RSG location of a (extended) physical layer. The main challenge is to fit the irregular structure of fusion graphs into the orthogonal structure of the spatial and temporal connectivity on the hardware.
%\newline

\vspace{0.3em}
\subsection{Routing}
\emph{Routing} plays an important role in finding a 2D lattice mapping as it resolves the conflicts between the geometry of fusion graphs and the 2D lattice connections between the RSGs. In particular, it allows fusions between non-neighboring resources states by finding a path between them on the 2D lattice. For example, a triangular fusion graph as shown in the shaded area of Fig.~\ref{fig:procedure}(c) does not have a direct mapping onto the grid because when $P,Q$ are mapped adjacently on the grid, $R$ can be adjacent to at most one of them. However as shown in the shaded area of Fig.~\ref{fig:procedure}(d), when mapping $R$ adjacent to $P$, $R$ can reach $Q$ by routing via a path of consecutive fusions through $S$ at the cost of consuming an extra resource state. In resource state $S$, two qubits participate in the fusions along the path, while the blue qubit is removed by a Z-measurement.

Specifically, routing resolves two types of conflicts in finding a 2D-lattice mapping. The fist type occurs when mapping a new node onto the 2D-lattice if the neighboring locations of existing nodes cannot provide enough degrees. For example, in Fig.~\ref{fig:case_study}(a), if we want to map a node that connects to a mapped node $B$ and two not-yet-mapped nodes $E,F$, then we should map it to location $B'$ via a routing path through $R_2$. Otherwise there would not be enough adjacent locations to accommodate both $E$ and $F$ since there is only one location left around $B$. The second type of conflicts occurs when mapping an edge between two nodes already mapped to the 2D-lattice, shown as the pink paths in Fig.~\ref{fig:case_study}(b). Such cases arise from the cyclic structure of a graph. For example, to form a cycle as shown in the shaded area of Fig.~\ref{fig:case_study}(b), we need to connect the nodes by finding a shortest routing path $A,B,C$.

A hardware constraint for routing is that each resource state can be used by only one path due to its limited size, because each routing path consumes two qubits of every resource state along the path. This means that all routing paths should not cross each other in a 2D-lattice mapping. Namely, the fusion graph mapped to the 2D-lattice should be a planar graph.
\label{subsect:hardware_constraint}

% The first case is that when a node in the crowd does not have enough space around it to grow all its branches, we would route it to an open area with enough available RSGs around it. For example, in Fig.~\ref{fig:case_study}(a), the pink nodes $R_1,R_2$ route $A,B$ to $A',B'$ respectively, so that they can grow edges $A'C,A'D$ and $B'E,B'F$. The second case is that when we need to map an edge between two nodes already on the grid, such as cycle edges, we would use routing to find a shortest path between the two nodes. For example, in Fig.~\ref{fig:case_study}(b), the pink nodes $A,B,C$ form a path to connect $D$ and $E$ so that the shaded cycle can be mapped onto the grid.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.75\linewidth]{fig/detour.pdf}
%     \caption{Routing: delete the middle fig}
%     \label{fig:detour}
% \end{figure}

\vspace{0.3em}
\subsection{Planar Mapping}
We are now ready to introduce the algorithm that finds a mapping from a scheduled planar fusion graph to the 2D-lattice. 
% The scheduling of planar sub-graphs of a general graph will be introduced in Section~\ref{sect:module3}. 
We propose a heuristic search algorithm with a goal of finding a compact layout on the 2D-lattice.

We map the edges in a cycle-prioritized breadth-first order. That is, we map all the edges involved in cycles in a breadth-first order, along the way adding tree edges of each node once its cycle edges are all traversed. The insight behind it is that only the \emph{planar orders} (i.e. clockwise or counter-clockwise orders) between cycle edges matter for a planar embedding, while the permutation among tree edges does not break the planarity. Every time when a new edge is mapped, a heuristic cost function $H$ is used to rate the candidate layout. Then the layout with the lowest cost is selected and used to update the current layout. We design the heuristic cost function as
\[
H = - \alpha\cdot \#\mathrm{mapped\_edges} +\beta \cdot \mathrm{routing\_length} + B
\] where \#$\mathrm{mapped\_edges}$ is the number of edges mapped onto the lattice and $\mathrm{routing\_length}$ is the total number of extra resource states consumed by all the routing paths, with $\alpha,\beta$ being two hyper parameters. These two terms ranks the compactness of a candidate layout by rewarding the accommodation of more edges and penalizing the use of long routing paths. $B$ is a look-ahead cost function that penalizes the congestion among nodes by comparing the number of remaining unmapped neighbors of each node and the number of its available adjacent locations that may accommodate those neighbors in a correct planar order.

There are two key optimizations for the heuristic search: planarity awareness and physical layer extension. First, the mapping of individual edges follows a planar embedding of the fusion graph found before the heuristic search so that it prevents routing paths from crossing each other and naturally increases the number of edges that can be accommodated by a physical layer. Second, the searching area can be adjusted dynamically by allowing an \emph{extended physical layer} consisting of multiple physical layers. As shown in Fig.~\ref{fig:archoverview}, a 3-layer extended physical layer can be obtained by ignoring the temporal connections among layer $t_0,t_1,t_2$ except those between the resource states on the m-th column of layer $t_0$ and layer $t_1$, and those between the resource states on the 0-th column of layer $t_1$ and layer $t_2$. This extension enables a more global optimization by allowing the mapping of a larger planar graph without being interrupted by the narrow boundaries.

% There are two key components in mapping an individual edge: boundary recognition and planar order recognition. First, the layout searching in our framework should be restricted within the boundaries of a physical layer or an \emph{extended physical layer}, and the nodes whose edges are not all mapped should be reserved to the next physical layer if the current physical layer is not enough. An extended physical layer is ... Second, 

% with $B$ being a look-ahead blocking cost which penalizes the case of not having enough degree around a node (i.e., $< \#(\mathrm{remaining\_neighbors})$), where the cost of a complete blockage (i.e. having no available adjacent locations) is larger than that of a partial blockage (i.e., the number of available adjacent locations $>0$ but $ < \#(\mathrm{remaining\_neighbors})$). When calculating the number of available adjacent locations, we also take the planar embedding into consideration. That is, we only look for adjacent locations that satisfy the clockwise (counter-clockwise) orders among edges.
%\newline

\vspace{0.3em}
\subsection{Non-Planar Shuffling}
The overall philosophy of mapping is that each planar sub-graph of a fusion graph is mapped to a separate (extended) physical layer, and the connections between those planar components are addressed by a re-arrangement of the connecting nodes via routing paths on intermediate layers in between, called \emph{shuffling}. For example, the two planar sub-graphs in Fig.~\ref{fig:program_non-planarity}(c) of the non-planar graph in Fig.~\ref{fig:program_non-planarity}(b) can be connected by joining their virtual nodes in pair.

To implement shuffling between the layouts of two planar sub-graphs, we first pair up their connecting nodes according to the original fusion graph, and sort the node pairs by their distances. Then we allocate one (or more) extra physical layers between the (extended) physical layers of those two layouts and find a shortest routing path between each pair of nodes in an ascending order of their distances.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.65\linewidth]{fig/shuffling_bold.pdf}\\
%     (a)\hspace{40pt}(b)\hspace{40pt}(c)
%     \caption{Mappings on extened physical layers (red `QUANTUM' on (a) and purple `COMPUTING' on (c)) connected by a layer of shuffling in between (green lines on (b)). Green dots on (a) represent the incomplete nodes whose edges are not all mapped yet, with the other ends of those edges falling to purple dots on (c). Corresponding nodes are connected through an intermediate layer (b).}
%     \label{fig:linear_fusion}
% \end{figure}



% After finding mappings for each planar fusion graphs, we now assemble the mapped sub-graphs to reconstruct the entire input program.
% This can be done by connecting the virtual nodes by a shuffling of their positions, with an overhead of consuming one or multiple physical layers between the planar mappings. We first match the virtual nodes in pair according to the virtual edges in the fusion graphs. Then, in ascending order of the Manhattan distances of those pairs, we connect the paired nodes by finding a shortest path between their locations on the physical layers. 

% Shuffling can be triggered in two cases. The first is between different partitions scheduled to different rounds. The second is when the heuristic search for a planar graph halts because no more edges can be added to the mapping, which is often due to the constraints of boundaries. In this case, we need to restart the heuristic search for the incomplete sub-graph on a new (extended) physical layer and connect the new mapping with the halted mapping by a shuffling.
%\newline

%Due to length limit of the delay lined, 
% One critical constraint on phonics devices is that
% the qubits stored in the delay lines have a limited lifetime and may have expired when they are needed to fuse with later qubits. To address this issue, we propose a mechanism to refresh the qubits on demand, with a new type of measurement dependency we recognize. 

% The refreshing operation utilize the fact that two consecutive X-measurements can be considered as a wire, and a Z-measurement can remove a qubit from the graph, as introduced in Section~\ref{sect:background}. In Fig.~\ref{fig:refresh}(a), $A$ is a node connected with virtual nodes $B$. In Fig.~\ref{fig:refresh}(a), we can fuse it with two other GHZ resource states, measuring $A,C$ in X-basis, and let $A',B'$ play the role of $A,B$ respectively. For a high degree node with virtual nodes $C,D$ in Fig.~\ref{fig:refresh}(b), we can fuse it with other GHZ resource states in the same pattern, measuring $A,E,F,G$ in X-basis, then let $A',C',D'$ play the role of $A,C,D$ respectively. Note that $A$ is not measurable before its connected virtual nodes are fused with their correspondence because the non-determinism in the fusion as a joint measurement induces a dependency of the measurement on a node on the fusion outcomes of its neighbors. Details about the dependency will be discussed in Section~\ref{sect:module3}.


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.55\linewidth]{fig/refreshing.pdf}
%     \caption{Qubit Refreshing}
%     \vspace{-10pt}
%     \label{fig:refresh}
% \end{figure}




==> 05_hezi_module2_rebuttal.tex <==
\section{Fusion Mapping and Routing}
\label{sect:module2}
% After resolving the high-degree nodes, t
The next step is to map each resource state in the fusion graph to a RSG location of a (extended) physical layer. The main challenge is to fit the flexible structure of fusion graphs into the rigid structure of the spatial and temporal connectivity on the hardware.
%\newline

\subsection{Routing}
\emph{Routing} plays an important role in finding a 2D lattice mapping as it resolves the conflicts between the geometry of fusion graphs and the 2D lattice connections between the RSGs. In particular, it allows fusions between non-neighboring resource states by finding a path between them on the 2D lattice. For example, a triangular fusion graph as shown in the shaded area of Fig.~\ref{fig:procedure}(c) does not have a direct mapping onto the grid because when $P,Q$ are mapped adjacently on the grid, $R$ can be adjacent to at most one of them. However as shown in the shaded area of Fig.~\ref{fig:procedure}(d), when mapping $R$ adjacent to $P$, $R$ can reach $Q$ by routing via a path of consecutive fusions through $S$ at the cost of consuming an extra resource state. In resource state $S$, two qubits participate in the fusions along the path, while the blue qubit is removed by a Z-measurement.

Specifically, routing resolves two types of conflicts in finding a 2D-lattice mapping. The first type occurs when mapping a new node onto the 2D-lattice if the neighboring locations of existing nodes cannot provide enough degrees. For example, in Fig.~\ref{fig:case_study}(a), if we want to map a node that connects to a mapped node $B$ and two not-yet-mapped nodes $E,F$, then we should map it to location $B'$ via a routing path through $R_2$. Otherwise there would not be enough adjacent locations to accommodate both $E$ and $F$ since there is only one location left around $B$. The second type of conflicts occurs when mapping an edge between two nodes already mapped to the 2D-lattice, shown as the pink paths in Fig.~\ref{fig:case_study}(b). Such cases arise from the cyclic structure of a graph. For example, to form a cycle as shown in the shaded area of Fig.~\ref{fig:case_study}(b), we need to connect the nodes by finding a shortest routing path $A,B,C$.

A hardware constraint for routing is that each resource state can be used by only one path due to its limited size, because each routing path consumes two qubits of every resource state along the path. This means that all routing paths should not cross each other in a 2D-lattice mapping. Namely, the fusion graph mapped to the 2D-lattice should be a planar graph.
\label{subsect:hardware_constraint}

% The first case is that when a node in the crowd does not have enough space around it to grow all its branches, we would route it to an open area with enough available RSGs around it. For example, in Fig.~\ref{fig:case_study}(a), the pink nodes $R_1,R_2$ route $A,B$ to $A',B'$ respectively, so that they can grow edges $A'C,A'D$ and $B'E,B'F$. The second case is that when we need to map an edge between two nodes already on the grid, such as cycle edges, we would use routing to find a shortest path between the two nodes. For example, in Fig.~\ref{fig:case_study}(b), the pink nodes $A,B,C$ form a path to connect $D$ and $E$ so that the shaded cycle can be mapped onto the grid.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.75\linewidth]{fig/detour.pdf}
%     \caption{Routing: delete the middle fig}
%     \label{fig:detour}
% \end{figure}

\subsection{Planar Mapping}
We are now ready to introduce the algorithm that finds a mapping from a scheduled planar fusion graph to the 2D-lattice. 
% The scheduling of planar sub-graphs of a general graph will be introduced in Section~\ref{sect:module3}. 
We propose a heuristic search algorithm with a goal of finding a compact layout on the 2D-lattice.

We map the edges in a cycle-prioritized breadth-first order. That is, we map all the edges involved in cycles in a breadth-first order, along the way adding tree edges of each node once its cycle edges are all traversed. The insight behind it is that only the \emph{planar orders} (i.e. clockwise or counter-clockwise orders) between cycle edges matter for a planar embedding, while the permutation among tree edges does not break the planarity. \fix{Edges connecting existing nodes are mapping by finding their shortest paths, while edges introducing new nodes are mapped by picking a layout that minimizes the heuristic cost
\begin{align*}
    H = \#&\mathrm{partially\_blocked\_nodes}\\
&+ \alpha\cdot\#\mathrm{totally\_blocked\_nodes}
\end{align*}
where \emph{partially} blocked nodes
refer to the nodes that have less available adjacent locations than the number of its unmapped edges, while \emph{totally} blocked nodes refer to those whose adjacent locations are all occupied. $\alpha$ should be larger than 1 because a total blockage is more severe than a partial blockage, which can be addressed by extending the routing paths (Fig.\ref{fig:case_study}(a)). Typically, $\alpha$ can be set as the maximum degree of each physical layer, which is 4 when each physical layer is a squared lattice.}

There are two key optimizations for the heuristic search: planarity awareness and physical layer extension. First, the mapping of individual edges follows a planar embedding of the fusion graph found before the heuristic search so that it prevents routing paths from crossing each other and naturally increases the number of edges that can be accommodated by a physical layer. Second, the searching area can be adjusted dynamically by allowing an \emph{extended physical layer} consisting of multiple physical layers. As shown in Fig.~\ref{fig:archoverview}, a 3-layer extended physical layer can be obtained by ignoring the temporal connections among layer $t_0,t_1,t_2$ except those between the resource states on the m-th column of layer $t_0$ and layer $t_1$, and those between the resource states on the 0-th column of layer $t_1$ and layer $t_2$. This extension enables a more global optimization by allowing the mapping of a larger planar graph without being interrupted by the narrow boundaries.

% There are two key components in mapping an individual edge: boundary recognition and planar order recognition. First, the layout searching in our framework should be restricted within the boundaries of a physical layer or an \emph{extended physical layer}, and the nodes whose edges are not all mapped should be reserved to the next physical layer if the current physical layer is not enough. An extended physical layer is ... Second, 

% with $B$ being a look-ahead blocking cost which penalizes the case of not having enough degree around a node (i.e., $< \#(\mathrm{remaining\_neighbors})$), where the cost of a complete blockage (i.e. having no available adjacent locations) is larger than that of a partial blockage (i.e., the number of available adjacent locations $>0$ but $ < \#(\mathrm{remaining\_neighbors})$). When calculating the number of available adjacent locations, we also take the planar embedding into consideration. That is, we only look for adjacent locations that satisfy the clockwise (counter-clockwise) orders among edges.
%\newline

\subsection{Non-Planar Shuffling}
The overall philosophy of mapping is that each planar sub-graph of a fusion graph is mapped to a separate (extended) physical layer, and the connections between those planar components are addressed by a re-arrangement of the connecting nodes via routing paths on intermediate layers in between, called \emph{shuffling}. For example, the two planar sub-graphs in Fig.~\ref{fig:program_non-planarity}(c) of the non-planar graph in Fig.~\ref{fig:program_non-planarity}(b) can be connected by joining their virtual nodes in pair.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/planar_decomp.png}\\
    \hspace{-10pt}(a)\hspace{70pt}(b)\hspace{100pt}(c)
    \caption{A non-planar graph state (b) translated from a circuit (a), with the measurement basis omitted. The non-planar graph (b) can be broken into two planar sub-graphs in (c).}
    % \vspace{-5pt}
    \label{fig:program_non-planarity}
\end{figure}

To implement shuffling between the layouts of two planar sub-graphs, we first pair up their connecting nodes according to the original fusion graph, and sort the node pairs by their distances. Then we allocate one (or more) extra physical layers between the (extended) physical layers of those two layouts and find a shortest routing path between each pair of nodes in an ascending order of their distances.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/flipped_shuffling.pdf}\\
    (a)\hspace{40pt}(b)\hspace{40pt}(c)
    \caption{Mappings of `QUANTUM' (red) and `COMPUTING' (purple) connected by a layer of shuffling in between (green lines on). Red dots on (c) represent the incomplete nodes whose edges are not all mapped yet, with the other ends of those edges falling to purple dots on (a). Corresponding nodes are connected through an intermediate layer (b).}
    \label{fig:linear_fusion}
\end{figure}



% After finding mappings for each planar fusion graphs, we now assemble the mapped sub-graphs to reconstruct the entire input program.
% This can be done by connecting the virtual nodes by a shuffling of their positions, with an overhead of consuming one or multiple physical layers between the planar mappings. We first match the virtual nodes in pair according to the virtual edges in the fusion graphs. Then, in ascending order of the Manhattan distances of those pairs, we connect the paired nodes by finding a shortest path between their locations on the physical layers. 

% Shuffling can be triggered in two cases. The first is between different partitions scheduled to different rounds. The second is when the heuristic search for a planar graph halts because no more edges can be added to the mapping, which is often due to the constraints of boundaries. In this case, we need to restart the heuristic search for the incomplete sub-graph on a new (extended) physical layer and connect the new mapping with the halted mapping by a shuffling.
%\newline

%Due to length limit of the delay lined, 
% One critical constraint on phonics devices is that
% the qubits stored in the delay lines have a limited lifetime and may have expired when they are needed to fuse with later qubits. To address this issue, we propose a mechanism to refresh the qubits on demand, with a new type of measurement dependency we recognize. 

% The refreshing operation utilize the fact that two consecutive X-measurements can be considered as a wire, and a Z-measurement can remove a qubit from the graph, as introduced in Section~\ref{sect:background}. In Fig.~\ref{fig:refresh}(a), $A$ is a node connected with virtual nodes $B$. In Fig.~\ref{fig:refresh}(a), we can fuse it with two other GHZ resource states, measuring $A,C$ in X-basis, and let $A',B'$ play the role of $A,B$ respectively. For a high degree node with virtual nodes $C,D$ in Fig.~\ref{fig:refresh}(b), we can fuse it with other GHZ resource states in the same pattern, measuring $A,E,F,G$ in X-basis, then let $A',C',D'$ play the role of $A,C,D$ respectively. Note that $A$ is not measurable before its connected virtual nodes are fused with their correspondence because the non-determinism in the fusion as a joint measurement induces a dependency of the measurement on a node on the fusion outcomes of its neighbors. Details about the dependency will be discussed in Section~\ref{sect:module3}.


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.55\linewidth]{fig/refreshing.pdf}
%     \caption{Qubit Refreshing}
%     \vspace{-10pt}
%     \label{fig:refresh}
% \end{figure}




==> 05_hezi_module3.tex <==
% \vspace{0.3em}
\section{Graph Partition and Scheduling}
\label{sect:module3}
In this section, we complete the entire compilation flow by introducing how our framework partitions and schedules a general graph state.
%
This module is the first stage in the compilation flow, with the partitioned graph being the input for fusion state generation.

% \vspace{0.3em}
% \subsection{Program Dependency}
\subsection{Temporal-Spatial Co-optimization}
The non-deterministic nature of quantum measurements requires a classical feed-forward that induces dependencies between measurements.
%
The partial order between measurements can be described by a causal flow~\cite{translation}, which is determined by two types of dependencies.
%
Specifically, according to the measurement outcome of a certain qubit, the measurement angles of its neighboring qubits may be adjusted from $\alpha$ to $(-1)^s\alpha+t\pi$, with the dependency on $s$ called $X$-dependency and that on $t$ called $Z$-dependency.
%
Note that changing the angle from $\alpha$ to $\alpha+\pi$ only interchanges $\ket{\pm_\alpha}$ and $\ket{\mp_\alpha}$, which means the $Z$-dependency is equivalent to a re-interpretation of the measurement outcome of the affected qubit, we can find the condition when a measurement becomes executable, as stated in Lemma~\ref{lemma:executable_rule}.
%

\begin{lemma}
\textit{A measurement on a qubit in the graph state is executable if all its $X$-dependent qubits are measured and all the $Z$-dependent qubits of all its $X$-dependent qubits are measured.}
\label{lemma:executable_rule}
\end{lemma}

According to the order of executablity, nodes in a graph state can be partitioned to multiple \emph{dependency layers}, with the lower layers being executable earlier than the higher layers.
%
We use a backward-determined dependency order to minimize the wait time of photons in the delay line, thus enhancing the fidelity.
%
This is defined by the dependency layers determined backward from the output qubits, so that measurements are not executed until its processors can be scheduled in the next round.

% To prevent qubits from waiting in delay lines for too long, a principle of scheduling is that the qubits in higher dependency layers should be scheduled later than those in lower dependency layers.



However, there is a tradeoff between the reduction of the delay time of each qubit and the reduction of resource state consumption.
%
The insight is that while a scheduling strictly according to the dependency layers can minimize the delay times of qubits, it may lead to more demand of shuffling by losing the information of the global structure in each layer.
%
This can be addressed by a co-consideration of both the dependency order and the graph geometry.
%
In particular, the graph state is partitioned in a coarse-grained manner, with multiple dependency layers included in each subgraph. 
%
Then, the dependency layers in the same subgraph are scheduled together on an extended physical layer.
%
This is shown in Algorithm~\ref{alg:planarize_and_merge}, where the planarity related steps are explained in the next subsection.

\subsection{Graph Planarization}
To further address the planarity constraint for resource states of small size, we impose a planarization process to Algorithm~\ref{alg:planarize_and_merge}.
%
In particular, a general non-planar graph is \emph{planarized} into several components such that each component is a planar graph.
%
For example, a graph state as shown in Fig.~\ref{fig:program_non-planarity}(b) cannot be scheduled onto a physical layer since the fusion graph of such a non-planar graph is non-planar too. At least two physical layers are needed by decomposing the graph into two planar graphs as shown in Fig.~\ref{fig:program_non-planarity}(c), with hollowed dots being the virtual nodes introduced in Section~\ref{subsect:graph_synthesis}. 
%
In Algorithm~\ref{alg:planarize_and_merge}, this is achieved by examining the planarity in the process of adding dependency layers to each partition, breaking the process when the partition is no more planar.
%
If the graph of a certain single dependency layer is already non-planar, we take its maximal planar sub-graph, defined as a subgraph such that the addition of any edge $e\in G-G_i$ breaks the planarity of $G_i$.
%
This can be achieved by traversing the edges, adding them to the partition until the planarity is broken.


\begin{algorithm}[h]
% \scriptsize
% \small
% \footnotesize
\SetAlgoLined

\KwIn{A graph state $G$}
\KwOut{A list of sub-graphs $R=[]$ }
$planar\_graph\_list=[], r=[], R=[]$\;
\While{there are nodes in G not visited}{
    $L\leftarrow$ sub-graph of  $G$ consisting all executable nodes\;
    \While{there are nodes in L not visited}{
        $l\leftarrow$ maximal planar graph of $L$\;
        $planar\_graph\_list.append(l)$ \; 
    }
}
\For{each $l$ in $planar\_graph\_list$}{
    \uIf{$r\cup l$ is planar}{
        $r\leftarrow r\cup l$
    }
    \uElse{
        Add virtual nodes to $r$ according to $G$\;
        $R.append(r)$\;
        $r\leftarrow[]$\;
    }
}

\caption{Temporal-Spatial Co-optimization}
\label{alg:planarize_and_merge}
\end{algorithm}








%Now we put the two types of dependencies 
% Our program graph partitioning and scheduling will consider the two types of dependencies and the planar graph property.
% Combining Lemma~\ref{lemma:fusion_Z_correction} with the fusion-induced dependency, we can find
%According to dependency relations among qubit measurements by Lemma~\ref{lemma:executable_rule}, 
% We first find all executable qubits in each round without considering the fusion-induced dependency and divide them into \emph{dependency layers} $\left\{l_1,l_2,\dots\right\}$ accordingly. Then the fusion graphs can be generated and mapped to the RSG locations in the ascending order of the dependency layers, with the attention being paid that the mapped qubits should not be measured before their neighboring nodes in the graph are mapped as well due to the fusion-induced dependency.

% To taking advantage of the delay lines, we do a multi-physical-layer optimization
% by padding small dependency layers toward the volume of the active physical layers. That is, when the sizes of some dependency layers are small, we schedule multiple consecutive dependency layers $L_i = \left\{l_j,l_{j+1},\dots l_{j+m}\right\}$ in the same round and store the qubits in the delay lines until the measurements are executable.

% Within each round, we partition the sub-graph by a planarization. Namely, we divide the sub-graph into partitions by iteratively finding its maximal planar sub-graphs. When a round $L_i$ contains multiple dependency layers, we find the maximal planar sub-graph by adding dependency layers one by one in the ascending order until the combined sub-graph becomes non-planar.


% \begin{figure}[h!]
%     \centering
%     \vspace{-10pt}
%     \includegraphics[width=\linewidth]{fig/fusion_decomposition.pdf}
%     \caption{Synthesize a high degree vertex in (a) by a basic fusion pattern in (b). Represent the fusion pattern by a fusion graph in (c), with each node representing a resource state, each edge representing a fusion operation}
%     \vspace{-10pt}
%     \label{fig:fusion_decomp}
% \end{figure}

==> 05_module1_camera_ready.tex <==
\vspace{0.3em}
\section{Fusion Graph Generation}
\label{sect:module1}

We start introducing the key modules of \frameworkname\ from \emph{fusion graph generation}. 
%
This is the second stage in the compilation flow (Figure~\ref{fig:designoverview}), which takes a partitioned and scheduled graph as the input. 
%
We start from this module because it lays the foundation of understanding the other modules.
%
In this module, we give an algorithm to synthesis a graph state from resource states of limited qubit degrees.
%
We first state the algorithm when the resource state is a 3-qubit GHZ state, then modify it to accommodate more generic resource states.
%
As mentioned in Section~\ref{sect:intro}, there is an additional constraint related to graph planarity from resource states of small size.
%
As a result, we discuss about it in the end of this subsection, whose motivation will more clear in ~\ref{sect:module2}.

\subsection{Synthesis From 3-qubit GHZ states}
A graph state can be synthesized from resource states as small as 3-qubit GHZ states by first synthesizing its high-degree nodes and (low-degree) lines, then connecting them according to the graph geometry.


\begin{figure}[h!]
    \centering
    %  \vspace{-5pt}
    \includegraphics[width=0.6\linewidth]{fig/three_basic_patterns.pdf}
    \caption{Basic fusion patterns.} 
    % \vspace{-5pt}
    \label{fig:basic_fusion_patterns}
\end{figure}

High-degree nodes are synthesized by the basic fusion pattern in Fig.~\ref{fig:basic_fusion_patterns}(a), which increments the node degree by fusing a leaf qubit $u_1$ (qubit of degree 1) with a qubit $u_2$ of degree $> 1$. 
%
Specifically, if $u_1$ is connected to an m-degree qubit $V$ while $u_2$ is an n-qubit degree, then the fusion between $u_1,u_2$ increments the degree of $V$ by n-1, generating an (m+n-1)-degree node, with m and n being 2 in the case of 3-qubit GHZ states.
%
This degree increment continues until a node of high enough degree is obtained, which is shown as 
Figure \ref{fig:linear_fusion}(a)(b). 
%
The resulted fusion pattern can be represented by a \emph{fusion graph} in \ref{fig:linear_fusion}(c), with each node representing a resource state, and each edge representing a fusion operation.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.65\linewidth]{fig/linear_fuse.pdf}\\
    (a)\hspace{50pt}(b)\hspace{50pt}(c)
    \caption{Synthesize a high degree node in (a) by a basic fusion pattern in (b). Represent the fusion pattern by a fusion graph in (c), with each `$\otimes$' node representing a resource state, each edge representing a fusion operation.}
    % \vspace{-15pt}
    \label{fig:linear_fusion}
\end{figure}

Lines are synthesized by the basic pattern of line extension (Fig.~\ref{fig:basic_fusion_patterns}(b)). Then, the high degree nodes and (low-degree) lines can be connected via the basic pattern of sub-graph connection (Fig.~\ref{fig:basic_fusion_patterns}(c)). We demonstrate it with an example of synthesizing a graph in Fig.~\ref{fig:vertex_split}(a). In Fig.~\ref{fig:vertex_split}(b), we break down the graph into high degree nodes $A,B,C,D,O$ and lines $PQ,RS$. Each node high degree node or each line is connected with some nodes in hollowed dots, which represent its neighbors in Fig.~\ref{fig:vertex_split}(a). Those nodes are referred to as \emph{virtual nodes}. Note that multiple virtual nodes are allowed to represent the same node, such as $A,B,C,D,O$. In Fig.~\ref{fig:vertex_split}(c), we pair up the virtual nodes according to the original graph Fig.~\ref{fig:vertex_split}(a) and synthesize the graph by applying the basic pattern of sub-graph connection (Fig.~\ref{fig:basic_fusion_patterns}(c)) on the paired virtual nodes. \label{subsect:graph_synthesis}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig/planar_graph_synthesis-4.pdf}\\
    \vspace{-10pt}
    (a)\hspace{85pt}(b)\hspace{85pt}(c)\hspace{85pt}(d)\hspace{110pt}(e)
    \caption{Fusion graph generation. (a) A planar embedding of the graph state geometry. (b) Split the edges. (c) Replace each high-degree node with a piece of fusion graph, with each `$\otimes$' node representing a resource state. (d) Connect the pieces of fusion graphs while keeping the clockwise (counter-clockwise) edge orders in the planar embedding so as to obtain a planar fusion graph. (e) The planarity may be broken if not keeping the clockwise (counter-clockwise) edge orders.}
\label{fig:vertex_split}
\end{figure*}

\subsection{Synthesis From Generic Resource States}
The fusion graph for 3-qubit GHZ states has a simplicity that its nodes and edges match with those in the graph states except for the leaf nodes.
%
For generic resource states, this synthesis algorithm can be made applicable by a modification containing two steps.


First, nodes of the fusion pattern in Figure~\ref{fig:linear_fusion}(c) can be reduced by utilizing qubits of degree $> 2$.
%
% If the resource states contain qubits of degree $>2$, then the high-degree nodes can be synthesized with less resource states.
%
In particular, for resource states with max degree $m$, an $n$-degree node can be synthesized by $n // m + 1$ resource states, where the extra $(n$ mod $m)$ qubits would be removed by Z-measurements.
%
Therefore, the fusion graph in Figure~\ref{fig:linear_fusion}(c) becomes a linear graph containing $n // m + 1$ nodes, instead of $n-1$ nodes for the 3-qubit GHZ states.
%
Second, edges in the fusion graph for 3-qubit GHZ states can be contracted by utilizing the connections between qubits within the resource states.
%
This can be achieved a pattern matching process that traverses the graph searching lines or cycles that matches the intrinsic geometry of the resource states.
%
For example, the line $B_1 O_3 O_2$ in Figure~\ref{fig:vertex_split}(d) can be contracted to $B_1 O_2$ if the resource state $B_1$ or $O_2$ contains remaining line structures after synthesizing the high-degree nodes.

In this process, qubits in resource states can be removed by Z-measurements when necessary. For example, a $n$-qubit ring-like resource state can be tailored to a ($n-1$)-qubit linear resource state by removing one qubit, if line structures instead of rings need to be synthesized. Moreover, we create a dict to keep track of the unfused qubits, as now there can be multiple unfused qubits in each node of the fusion graph. Unfused qubits that do not contribute to the graph state geometry should be marked as redundant and removed by Z-measurements.


\subsection{Planarity Preservation}
To address the additional planarity constrain which will become more clear in Section~\ref{sect:module2}, the fusion graph generation provides the ability to preserve the planarity if the input graph is planar.
%
Namely, the generated fusion graph of a planar graph is still a planar graph, meaning that the graph can be drawn on a plane with edges not crossing each other. 
%
This can be achieved by first finding a planar embedding (Fig.~\ref{fig:vertex_split}(a)) of the original graph, i.e. a way of drawing it on the plane with no crossing edges, and then
keeping the clockwise (counter-clockwise) orders among the edges when connecting the fusion graphs of the high degree nodes (Fig.~\ref{fig:vertex_split}(d)). 
%
The search for the planar embedding can be efficiently done by existing tools such as Networkx[??] in a $O(|V|)$ complexity where $|V|$ is the number of nodes in the graph state geometry.


For example, in the planar graph in Fig.~\ref{fig:vertex_split}(a), the 4-degree node $O$ has neighbors $A,B,D,C$ in the clockwise order. So we replace it with a fusion graph component of 3 nodes (component $O$ in the grey circle at the center of Fig.~\ref{fig:vertex_split}(c)), and connect it with fusion graph components of $A,B,D,C$ clockwisely (Fig.~\ref{fig:vertex_split}(d)). Note that one of the nodes in component $O$ connects with both components $C$ and $D$. For the 3-degree node $A$ (and $B,C,D$ similarly) which has clockwise neighbors $B,O,P$, we replace it with a fusion graph component of 2 nodes (component $A$ in Fig.~\ref{fig:vertex_split}(c)) and connect it with components $B,O,P$ clockwisely. As a comparison, Fig.~\ref{fig:vertex_split}(e) shows a fusion graph that breaks the planarity if not keeping the clockwise (counter-clockwise) edge orders.

==> 07_evaluation.tex <==
\vspace{0.3em}
\section{Evaluation}\label{sect:eval}

% \todo{Rephrase for more insights!}
\vspace{0.3em}
\subsection{Experiment Setup}\label{sect:expset}

\textbf{Platform} We perform all experiments on a Manjaro Linux laptop with a 4$\times$Intel Core i7-7500U CPU and 8GB RAM.
Other software includes Python 3.10.2 and Qiskit 0.36.1~\cite{Qiskit}.

\noindent \textbf{Baseline} 
Our baseline is based on the naive MBQC interpreter introduced in Section~\ref{sect:background}. 
%
There are two steps in the baseline implementation. The first step is generating a 3D cluster state by fusions from small resource states generated by the RSGs. 
%
Instead of adopting a specific generation algorithm, we calculate the minimum number of RSGs and the minimum number of fusions required to generate a large enough cluster state and use these lower bounds in the baseline data. 
%
The second step is compiling the circuit with state-of-the-art compiler in the circuit model \cite{sabre} and then converting the compiled circuit into a measurement pattern on the 3D cluster state via the naive MBQC interpreter.


\noindent \textbf{Benchmark programs} We select Quantum Fourier transform (QFT), quantum approximate optimization algorithm (QAOA), Ripple-Carry Adder (RCA)~\cite{RCA} and Bernstein-Vazirani (BV) algorithm as our benchmarks, which include both building blocks of quantum programs (QFT and RCA) and application driven programs targeting at solving real-world problems (QAOA and BV).
For QAOA,
we choose the graph maxcut problem on randomly generated graphs. For BV, we select the secret strings randomly. In Table~\ref{tab:benchmark}, we list the number of qubits and gates  for each benchmark. We also list the minimum area of each layer of the cluster state required by the baseline as `cluster area' and the minimum area of each physical layer required by the baseline as `physical area'.  We use the same physical area in the evaluation of \frameworkname~in order to compare with the baseline. The number of qubits we select are of the form $n^2$ because that is the maximum number of logical qubits that can be accommodated by the area (qubit number between $(n-1)^2+1$ and $n^2$ all require the same area).

\begin{table}[t]
    \centering
      \caption{Benchmark programs.}
      \vspace{-5pt}
      
    \resizebox{0.43\textwidth}{!}{
    \renewcommand*{\arraystretch}{1.4}
    \begin{tabular}{|p{1.5cm}|p{1.0cm}|p{1.0cm}|p{1.5cm}|p{1.5cm}|}  \hline
    Name & \# qubit & \# gate & cluster area & physical area  \\ \hline

  \multirow{3}{1.5cm}{Quantum Fourier Transform (QFT)} & 9 & 320 & \qnineGrid & \qnineRSG \\ \cline{2-5} 
 & 16 & 1000 & \qsixteenGrid & \qsixteenRSG\\ \cline{2-5}
  & 25 & 2400 & \qtwentyfiveGrid & \qtwentyfiveRSG  \\ \hline %\cline{2-5}
  
  \multirow{3}{1.5cm}{Quantum Approximate Optimization Alg (QAOA)} & 9 & 130 & \qnineGrid & \qnineRSG\\\cline{2-5}
 & 16 & 400 & \qsixteenGrid & \qsixteenRSG  \\ \cline{2-5}
 & 25 & 700 & \qtwentyfiveGrid & \qtwentyfiveRSG \\\hline % \cline{2-5}
 
 \multirow{3}{1.5cm}{Ripple-Carry Adder (RCA)} 
 & 16 & 500 & \qsixteenGrid & \qsixteenRSG\\ \cline{2-5}
  & 25 & 840 & \qtwentyfiveGrid & \qtwentyfiveRSG  \\ \cline{2-5}
  & 49 & 1750 & \qfortynineGrid & \qfortynineRSG \\ \hline %\cline{2-5}
  
 \multirow{3}{1.5cm}{Bernstein Vazirani (BV)} & 100 & 300 & \qhundrGrid & \qhundrRSG \\ \cline{2-5}
 & 196 & 600 & \qtwohundrGrid & \qtwohundrRSG \\ \cline{2-5}
 & 324 & 1000 & \qthreehundrGrid & \qthreehundrRSG  \\ \hline
\end{tabular}
}
 \vspace{-10pt}
    \label{tab:benchmark}
\end{table}


% \begin{figure}[t]
%     \newcommand{\fhe}{0.2}
%     \hspace{15pt}
%         \includegraphics[height=\fhe\textwidth]{imgs/8-degree-vertex-mapping.pdf} \hfill \includegraphics[height=\fhe\textwidth]{imgs/3-qubit-QFT_8x8_large_node.pdf} \hspace{15pt}
%         \\
%         \hphantom{} \hspace{58pt}(a) \hspace{105pt} (b) 
%         % \vspace{-5pt}
%         \caption{(a) Slices of mapping for 8-qubit BV with secret string '11111111'. (b) Mapping of 3-qubit QFT. Blue dots correspond to nodes `$\otimes$' existing in the fusion graph, pink dots represents auxiliary vertices to help form high degree vertices and cycles.\todo{need to label ABCD}
%         }
        
%         \vspace{-10pt}
%         \label{fig:case_study}
% \end{figure}


\begin{figure}[t]
    \newcommand{\fhe}{0.23}
        \includegraphics[height=\fhe\textwidth]{fig/labeled_left.pdf} \hfill \includegraphics[height=\fhe\textwidth]{fig/labeled_right.pdf}
        \\
        \hphantom{} \hspace{58pt}(a) \hspace{105pt} (b) 
        % \vspace{-5pt}
        \caption{(a) Mapping of fusion graph for 8-qubit BV with secret string '11111111'. (b) Mapping of fusion graph for 3-qubit QFT. Blue dots correspond to nodes `$\otimes$' existing in the fusion graph, pink dots represent auxiliary resource states used for routing.
        }
        \vspace{-15pt}
        \label{fig:case_study}
\end{figure}


\noindent\textbf{Metric} As discussed in Section~\ref{sect:overview}, the first metric we consider is the physical depth, i.e., the number of physical layers that are consumed by the compiled program. To make it comparable with the baseline, we assume that the number of RSGs on the hardware is the same as that is required by the implementing baseline.
The second metric is the number of fusion operations executed by the compiled program, which is denoted as `\# fusion'. A better compiler should compile a quantum program into a smaller depth which indicates a shorter execution time, and a smaller `\# fusion' which indicates less consumption of resources and being less error-prone. For comparison, we define an improvement factor of physical depth as the ratio of the depth in the baseline and the depth in \frameworkname, and an improvement factor of `\#fusion' as the ratio of the number of fusions consumed in the baseline and the that consumed by \frameworkname.
%\newline


\begin{table*}[t!]
\centering
    \caption{The results of \frameworkname~and its relative performance to the baseline. }
  %  The name column are acronyms of test programs in Table~\ref{tab:benchmark}.}
\resizebox{\textwidth}{!}{
\renewcommand*{\arraystretch}{1.2}
\begin{tabular}{|p{2cm}|p{2cm}|p{2.5cm}|p{2cm}|p{2.4cm}|p{2.9cm}|p{2cm}|}  \hline
{Name-\#qubits} &  {Baseline Depth} & {\frameworkname~Depth} & Improv. Factor & Baseline \#Fusions   & \frameworkname~\#Fusions & Improv. Factor \\ \hline

% QFT-4 & 5x5 && 11x6 & 6(old) & - & - & 85 & -\\\hline
%RCA-7 & - & 22 & - & - & 976 & - \\\hline

QFT-9 & 462 & 29 & 16 & 66,528 & 1,158 & 57\\\hline
QFT-16  & 1,392 & 82 & 17 & 356,352 & 4,821 & 74\\\hline
QFT-25 & 3,678 & 214 & 17 & 1,621,998 & 18,143 & 89\\\hline
% QFT-9-fast & 462 & 42 & 11 & 66,528 & 1,365 & 49\\\hline
% QFT-16-fast  & 1,272 & 73 / 91 & 17 / 14 & 356,352 & 6,656 / 5,763 & 54 / 62\\\hline
% QFT-25-fast & 2,352 & 157 & 15 & 1,621,998 & 23,974 & 68\\\hline
% QFT-36-fast & 3,846 & 320 & 12 &  & 62,444 & \\\hline
% QFT-49-fast & 7,032 & 529 & 13 &  & 145,740 & \\\hline
% QFT-9-4star & 462 & 31 &  & 66,528 & 1,029 & \\\hline
% QFT-16-4star  & 1,272 & 82 / 78 / 77 &  & 356,352 & 5,552 / 5,088 / 4,941 & \\\hline
% QFT-25-4star & 2,352 & 187 &  & 1,621,998 & 17,844 & \\\hline

% QFT-36 & 21x21 & 1355x6 & - & - & - & - & -\\\hline
%QFT-49 & 25x25 & 2532x6 & - & - & - & - & -\\\hline
QAOA-9  & 426 & 23 & 19 & 61,344 & 911 & 67\\\hline
QAOA-16  & 1,050 & 60 & 18 & 268,800 & 2,979 & 90\\\hline
QAOA-25  & 1,584 & 99 & 16 & 698,544 & 7,336 & 95\\\hline

% RCA-16 & 930 & 57 & 16.3 & 238,080 & 3,158 & 75.4\\\hline

RCA-25 & 1572 & 87 & 18 & 693,252 & 5,834 & 119 \\\hline
RCA-36 & 2,418 & 136 & 18 & 1,511,250 & 8,763 & 172 \\\hline
RCA-49 & 3,471 & 206 & 17 & 3,123,900 & 13,372 & 234 \\\hline
% RCA-16-fast &  & 41 &  &  & 5,249 &  \\\hline
% RCA-49-fast & 3,471 & 138 / 125 & 25 & 3,123,900 & 20,673 / 21,287 & 151 \\\hline
% RCA-64-fast &  & 165 &  &  & 31,613 &  \\\hline
% RCA-81-fast &  & 221 &  &  & 41,347 &  \\\hline

BV-100 & 1,290 & 4 & 323 & 2,385,210 & 437 & 5458\\\hline
BV-196  & 2,142 & 5 & 428 & 7,970,382 & 801 & 9951\\\hline
BV-324 & 4,500 & 7 & 643 & 28,084,500 & 1,358 & 20681\\\hline
\end{tabular}
    }

    \label{tab:evaluation}
\end{table*}


% \begin{table*}[t!]
% \centering
%     \caption{The results of \frameworkname~and its relative performance to the baseline. }
%   %  The name column are acronyms of test programs in Table~\ref{tab:benchmark}.}
% \resizebox{\textwidth}{!}{
% \renewcommand*{\arraystretch}{1.2}
% \begin{tabular}{|p{2cm}|p{2cm}|p{2.5cm}|p{2cm}|p{2.4cm}|p{2.9cm}|p{2cm}|}  \hline
% {Name-\#qubits} &  {Baseline Depth} & {\frameworkname~Depth} & Improv. Factor & Baseline \#Fusions   & \frameworkname~\#Fusions & Improv. Factor \\ \hline

% % QFT-4 & 5x5 && 11x6 & 6(old) & - & - & 85 & -\\\hline
% %RCA-7 & - & 22 & - & - & 976 & - \\\hline

% QFT-9 & 462 & 29 & 15.9 & 66,528 & 1,158 & 57.4\\\hline
% QFT-16  & 1,392 & 82 & 17.0 & 356,352 & 4,821 & 73.9\\\hline

% QFT-25 & 3,678 & 214 & 17.2 & 1,621,998 & 18,143 & 89.4\\\hline
% % QFT-36 & 21x21 & 1355x6 & - & - & - & - & -\\\hline
% %QFT-49 & 25x25 & 2532x6 & - & - & - & - & -\\\hline
% QAOA-9  & 426 & 23 & 18.5 & 61,344 & 911 & 67.3\\\hline
% QAOA-16  & 1,050 & 60 & 17.5 & 268,800 & 2,979 & 90.2\\\hline
% QAOA-25  & 1,584 & 99 & 16.0 & 698,544 & 7,336 & 95.2\\\hline

% % RCA-16 & 930 & 57 & 16.3 & 238,080 & 3,158 & 75.4\\\hline
% RCA-25 & 1572 & 87 & 18.1 & 693,252 & 5,834 & 118.8 \\\hline
% RCA-36 & 2,418 & 136 & 17.8 & 1,511,250 & 8,763 & 172.5 \\\hline
% RCA-49 & 3294 & 206 & 16.0 & 2,964,600 & 13,372 & 221.7 \\\hline

% BV-100 & 1,290 & 4 & 322.5 & 2,385,210 & 437 & 5458.1\\\hline
% BV-196  & 2,142 & 5 & 428.4 & 7,970,382 & 801 & 9950.5\\\hline
% BV-324 & 4,500 & 7 & 642.9 & 28,084,500 & 1,358 & 20680.8\\\hline
% \end{tabular}
%     }

%     \label{tab:evaluation}
% \end{table*}
\begin{figure*}[t]
    \centering    
    % \vspace{-5pt}
    \includegraphics[height=0.2\linewidth,width=0.8\linewidth]{fig/QFT_16qbt_3lyr.png}
    \caption{Mapping of the fusion graph of a 16-qubit QFT program with a more global optimization by considering an extended physical layer consisting of 3 successive physical layers of size $13\times13$. Blue and green dots correspond to the nodes `$\otimes$' existing in the fusion graph, with the green ones being the incomplete nodes whose edges are not all mapped yet. Pink dots represent the auxiliary resource states used for routing.}
    \vspace{-10pt}
    \label{fig:global_optimization}
\end{figure*}


\vspace{0.3em}
\subsection{Experiment Result}

% As shown in Table~\ref{tab:evaluation}, \frameworkname~achieves a significant reduction in both physical depth and `\# fusion' compared to the baseline. In specific, \frameworkname~reduces the physical depth on by a factor of 39 on average (geomean), up to 643. \frameworkname~also reduces the number of fusions by a factor of 320 on average (geomean), up to 20681.

\fix{Table~\ref{tab:evaluation} shows the results of the baseline and \frameworkname as the number of qubits varies when the resource states are 3-qubit GHZ states.}
It can be seen that \frameworkname~achieves a significant reduction in both physical depth and `\# fusion' compared to the baseline. In specific, \frameworkname~reduces the physical depth on by a factor of 39 on average (geomean), up to 643. \frameworkname~also reduces the number of fusions by a factor of 320 on average (geomean), up to 20681.

Among the benchmarks, \frameworkname~has the most significant improvement for BV. The reasons are two folds. First, the graph state representation of BV in the one-way model contains no cycles and is thus completely planar. This naturally fits the planar-centric design of \frameworkname. Second, the graph representation of BV contains a very high-degree node, i.e., as high as half of the number of qubits on average. In the simulation approach adopted by the baseline, that requires a huge number of inserted SWAP gates and thus waste a lot of physical layers. However, in \frameworkname, it can be suppressed to a few of physical layers by a heuristic planar search that fully utilizes the resource states in those physical layers. 
In contrast, the graph representations of QFT, RCA and QAOA contain a lot of short-range and long-range cycles, which not only makes the heuristic search much harder than that of BV, but also breaks the planarity of the graph. However, \frameworkname~still achieves a reduction on the physical depth by a factor of 17 (geomean), and a reduction on the number of fusions by a factor of 100 (geomean).
%\newline

\fix{For generalization, Fig.\ref{fig:different_resource_states} shows the improvement factor of depth (\ref{fig:different_resource_states}(a)) and the improvement factor of \#fusions (\ref{fig:different_resource_states}(b)) for various resource states, including 3-qubit line-shaped cluster state (GHZ state), 4-qubit line-shaped cluster state, 4-qubit star-shaped cluster state and 4-qubit ring-shaped cluster states, respectively. The results for BV are omitted, as they exhibit exceptional improvement due to their graph states being planary and acyclic. It can be seen that the significant improvements brought by \frameworkname is applicable to different resource states.}

\vspace{0.3em}
\subsection{Optimization Analysis}
\textbf{Increase resource utilization}
The significant improvements by \frameworkname~come from the increased utilization of resource states on each physical layer.
To demonstrate, Fig.~\ref{fig:case_study} shows the mappings of fusion graphs generated by \frameworkname.
Fig.~\ref{fig:case_study}(a) is a 8-qubit BV program mapped onto a $8\times 8$ RSG grid while Fig.~\ref{fig:case_study}(b) is a 3-qubit QFT program mapped onto a $8\times 8$ RSG grid. 
These two programs are two typical cases of acyclic structure and 
cyclic structure. In the figure, each dot represents a resource state. Dots in blue correspond to the nodes `$\otimes$' existing in the fusion graph, and the pink dots represent the auxiliary resource states used for routing. \frameworkname~enables a dense mapping that increases the utilization of each physical layer, in contrast to the sparse mapping in the baseline caused by the rigid pattern of mapping and the large amount of preserved Z-measurement qubits. 






\noindent \textbf{Flexible Physical Area}
Besides the improvement in performance, \frameworkname~also enables a lower constraint and more flexibility to the varying size of physical layers. In comparison with the fixed sizes of physical layers required by the baseline approach caused by the fixed locations of logical qubits, \frameworkname~does not put a strict constraint on the size of physical layers. \FrameworkName~can compile the program onto a much smaller physical hardware than the baseline, with a trade-off of more physical layers. For example, Fig.~\ref{fig:global_optimization} shows a slice of fusion graph mapping of a 16-qubit QFT program on three physical layers each with 169 resource states, which is much smaller than the physical layers of 256 resource states required by the baseline. Moreover, when the physical layers are larger than required by the baseline, the simulation approach has no way to utilize the extra resource, while \frameworkname~allows an optimization by spanning the mapping all over the physical layers.
% rigid pattern used by the baseline with a fixed occupation pattern and lots of unoccupied locations preserved to assist non-neighboring multi-qubit gates, our framework enables the mapping onto small physical layers and take more advantage of the large physical layers when they are available.

% \begin{figure*}[h]
%     % \newcommand{\fhe}{0.114}
%     \newcommand{\fhe}{0.114}
%         \includegraphics[height=\fhe\textwidth]{imgs/BVz=0.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BVz=1.pdf} 
%         \includegraphics[height=\fhe\textwidth]{imgs/BVz=2.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BVz=3.pdf}
%         \includegraphics[height=\fhe\textwidth]{imgs/BVz=4.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BVz=5.pdf} 
%         \includegraphics[height=\fhe\textwidth]{imgs/BVz=6.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BVz=7.pdf}  
%         \\
%         % \vspace{-5pt}
%         \caption{(a) The effect of planarity awareness during adaptive fusion on depth. (b) The effect of planarity awareness during adaptive fusion on `\# fusion'.
%         }
%         \label{fig:case_study}
% \end{figure*}






\noindent \textbf{More Global Optimization}
With the \archName~proposed in Section~\ref{sect:hardware_model} (Fig.~\ref{fig:archoverview}), \frameworkname~also enables a more global optimization in the mapping by searching through an extended physical layer composed by multiple physical layers. As a demonstration, Fig.~\ref{fig:global_optimization} shows a slice of mapping generated by \frameworkname~for a 16-qubit QFT program. The whole rectangular $13\times39$ plane is composed of 3 layers of $13\times 13$ resource state grid (much smaller than the $16\times 16$ physical layers required by the baseline). The first physical layer ranges from column 1 to column 13, the second ranges from column 14 to column 26, and the third from column 27 to column 39 respectively. In the figure, blue and green dots correspond to the nodes `$\otimes$' existing in the fusion graph, with the green ones representing the incomplete nodes, which means that some of edges connected to them have not been mapped onto the grid. Again, pink dots represent the auxiliary resource states used for routing.

As can be seen, the mapping onto extended physical layers enables an optimization by allowing long-range structures (e.g., long-range cycles crossing the boundaries of individual physical layers, i.e., column 13,14 and column 26,27) in the mapping, at a cost of sacrificing some inter-layer connections not on the boundaries. Moreover, this mapping strategy onto extended physical layers also reduces the searching space from a 3D grid to a large 2D grid, which significantly improves the compilation efficiency without much loss of performance.


% \textbf{The effect of dynamic scheduling:} 
% We study the effect of dynamic scheduling by comparing the Clifford-eager scheduling with a non-eager one. Fig~\ref{fig:opt1}(a) shows the comparison of the improvement factors of depth and `\# fusion' between the Clifford-eager scheduling and the non-eager scheduling.

\begin{figure*}[t]
        \includegraphics[width=0.33\linewidth]{fig/depth_with_shape.pdf} \includegraphics[width=0.33\linewidth]{fig/fusion_with_shape.pdf}
        \includegraphics[width=0.33\linewidth]{fig/improv_large_cluster_states.pdf}
    
        \hspace{85pt}(a)\hspace{160pt}(b) \hspace{160pt}(c)
        \caption{Improvement factors of (a) depth and (b) \#fusions for different resource states. (c) The depth improvement against cluster size when a large cluster state is available.
        }
        \vspace{-15pt}
        \label{fig:different_resource_states}
\end{figure*}



==> 07_evaluation_0801.tex <==

\section{Evaluation}\label{sect:eval}

% \todo{Rephrase for more insights!}

\subsection{Experiment Setup}\label{sect:expset}

\textbf{Platform} We perform all experiments on a Manjaro Linux laptop with a 4$\times$Intel Core i7-7500U CPU and 8GB RAM.
Other software includes Python 3.10.2 and Qiskit 0.18.3 ~\cite{Qiskit}.

\noindent \textbf{Baseline} 
We implement the baseline by simulating quantum circuits in the one-way model using the `mapping onto regular lattice first' approach as introduced in Section~\ref{sect:baseline}. There are two steps in the simulation. The first step is synthesizing a 3D cluster state with fusions from small resource states generated by the RSGs. For this step we use a lower bound by calculating the minimum number of resource states required to synthesize the large cluster state. The second step is simulating the state-of-the-art compiler \cite{sabre} on the cluster state, with gates implemented with the measurement patterns introduced in Section~\ref{sect:baseline}.

% the state-of-the-art compiler in circuit based model[?] using one-way model with the , with each gate implemented as in [?]. 

\noindent \textbf{Benchmark programs} We consider two categories of benchmark programs, building blocks and real world applications. As listed in Table~\ref{tab:benchmark}, the first category focuses on implementing specific elementary functions, eg. multi-controlled gate and ripple-carry adder, which are often used as the building blocks of large quantum applications. The second category includes quantum Fourier transform (QFT), quantum approximate optimization algorithm (QAOA) and Bernstein-Vazirani (BV) algorithm, which are application driven programs targeting at solving real-world problems. For QAOA,
we choose the graph maxcut problem. For BV, we choose the secret strings randomly. In Table~\ref{tab:benchmark}, we list the number of qubits, gates and CX for each benchmark as well as the minimum area of each layer of the 3D cluster state required by implementing the baseline. The number of qubits we select are of the form $n^2$ because that is the maximum number of logical qubits that can be accommadated by the area (qubit number between $(n-1)^2+1$ and $n^2$ all require the same area).

\begin{table}[t]
    \centering
      \caption{Benchmark programs. \todo{revise}}
      \vspace{-5pt}
      
    \resizebox{0.47\textwidth}{!}{
    \renewcommand*{\arraystretch}{1.4}
    \begin{tabular}{|p{1.0cm}|p{1.5cm}|p{1.0cm}|p{1.3cm}|p{1.0cm}|p{1.5cm}|}  \hline
    Type & Name & \# qubit & \# gate & \# CX & cluster area  \\ \hline
\multirow{6}{1.0cm}{Build-ing Blocks} & \multirow{3}{1.5cm}{Multi-Controlled Gate (MCTR)} & 100 & 10 & 10640 & 4560 \\ \cline{3-6} 
 &  & 200 & 20 & 21840 & 9360  \\ \cline{3-6} 
 &  & 300 & 30 & 33040 & 14160 \\ \cline{2-6} 
 & \multirow{3}{1.5cm}{Ripple-Carry Adder (RCA)} & 100 & 10 & 1569 & 785 \\ \cline{3-6} 
 &  & 200 & 20 & 3169 & 1585  \\ \cline{3-6}
 &  & 300 & 30 & 4769 & 2385 \\ 
 \hline
\multirow{9}{1.0cm}{Real World Appli-cations} & \multirow{3}{1.5cm}{Quantum Fourier Transform (QFT)} & 9 & g & 265 & \qnineGrid \\ \cline{3-6} 
 &  & 16 & g & cx & \qsixteenGrid\\ \cline{3-6} 
 &  & 25 & g & cx & \qtwentyfiveGrid  \\ \cline{2-6} 
 & \multirow{3}{1.5cm}{QAOA} & 9 & g & cx & \qnineGrid\\ \cline{3-6} 
 &  & 16 & g & cx & \qsixteenGrid  \\ \cline{3-6} 
 &  & 25 & g & cx & \qtwentyfiveGrid \\ \cline{2-6} 
 & \multirow{3}{1.5cm}{Bernstein Vazirani (BV)} & 100 & g & cx & \qhundrGrid \\ \cline{3-6} 
 &  & 196 & g & cx & \qtwohundrGrid \\ \cline{3-6} 
 &  & 324 & g & cx & \qthreehundrGrid  \\ \hline
\end{tabular}
}
 \vspace{-10pt}
    \label{tab:benchmark}
\end{table}


\begin{figure}[t]
    \newcommand{\fhe}{0.18}
        \includegraphics[height=\fhe\textwidth]{imgs/8-degree-vertex-mapping.pdf} \hfill \includegraphics[height=\fhe\textwidth]{imgs/3-qubit-QFT_8x8_large_node.pdf} 
        \\
        \hphantom{} \hspace{58pt}(a) \hspace{105pt} (b) 
        % \vspace{-5pt}
        \caption{(a) Slices of mapping for 8-qubit BV with secret string '11111111'. (b) Mapping of 3-qubit QFT. Blue dots correspond to nodes `$\otimes$' existing in the fusion graph, pink dots represents auxiliary vertices to help form high degree vertices and cycles.\todo{need to label ABCD}
        }
        
        \vspace{-10pt}
        \label{fig:case_study}
\end{figure}


\noindent\textbf{Metric} As discussed in Section~\ref{sect:overview}, the first metric we consider is the physical depth, i.e. the number of physical layers that are consumed by the program. To make it comparable with the baseline, we assume that the number of RSG on the hardware is the same as that is required by the implementing baseline.
The second metric is the number of fusion operations executed by the compiled program, which is denoted as `\# fusion'. A better compiler should have a smaller depth which indicates a shorter runtime, and less `\# fusion' which indicates less consumption of resources and being less error-prone. For comparison, we define a improvement factor of physical depth as the ratio of the depth in the baseline and the depth in \frameworkname, and a improvement factor of `\#fusion' as the ratio of the number of fusions consumed in the baseline and the that consumed by \frameworkname.
%\newline





\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}{
\renewcommand*{\arraystretch}{1.2}
\begin{tabular}{|p{2.2cm}|p{2.2cm}|p{2.2cm}|p{2.2cm}|p{2.4cm}|p{2.2cm}|p{2.4cm}|p{2.6cm}|p{2cm}|}  \hline
{Name-\#qubits} & {\#RSG per layer} & {\# gates} &  {baseline depth} & {framework depth} & Improv. factor & baseline \#fusion   & framework \#fusions & Improv. factor \\ \hline
MCTR-100 & - & & - & - & - & - & - & - \\\hline
MCTR-200 & - & & - & - & - & - & - & -\\\hline
MCTR-300 & - & & - & - & - & - & - & -\\\hline
RCA-100 & - & & - & - & - & - & - & -\\\hline
RCA-200 & - & & - & - & - & - & - & -\\\hline
RCA-300 & - & & - & - & - & - & - & -\\\hline

% QFT-4 & 5x5 && 11x6 & 6(old) & - & - & 85 & -\\\hline
QFT-9 & 9x9 && 77x6 & 25(old) & - & - & - & -\\\hline
QFT-16 & 13x13 && 232x6 & 97(new) & - & 200,448 & 6,753 & -\\\hline
QFT-16 & 23x23 (13x1.73) && 232x6 & 97(new) & - & 673,728 & 6,753 & -\\\hline
QFT-25 & 30x30 &2400& 613x6 & 179 (latest) & - & 3,093,198 & 20,180 & -\\\hline
% QFT-36 & 21x21 & 1355x6 & - & - & - & - & -\\\hline
%QFT-49 & 25x25 & 2532x6 & - & - & - & - & -\\\hline
QAOA-9 & 12x12 && - & 23 & - & - & 911 & -\\\hline
QAOA-16 & 23x23 && - & 60 & - & - & 2979 & -\\\hline
QAOA-25 & 30x30 &800& - & 99 & - & - & 7336 & -\\\hline
BV-100 & 28x28 &300& 215x6 & 4 & 54 & 156735x6 & 437 & 359\\\hline
BV-196 & 40x40 &600& 357x6 & 5 & 71 & 542997x6 & 801 & 678\\\hline
BV-324 & 52x52 &1000& 750x6 & 7 & 107 & 1950750x6 & 1358 & 1436\\\hline
\end{tabular}
    }
    \caption{The results of {\frameworkname} and its relative performance to the baseline. \todo{revise}
    The name column are acronyms of test programs in Table~\ref{tab:benchmark}.}
    \label{tab:evaluation}
\end{table*}
\begin{figure*}[t]
    \centering    
    \vspace{-5pt}
    \includegraphics[width=0.85\linewidth]{fig/QFT_16qbt_3lyr.png}
    \caption{Mapping of the fusion graph of a 16-qubit QFT program with a more global optimization by considering 3 layers of $13\times13$ RSG grid together. Blue and green dots correspond to the nodes `$\otimes$' existing in the fusion graph, with the green ones being the incomplete nodes whose neighbors are not all mapped yet. Pink dots represent the auxiliary resource states used for routing.}
    \vspace{-10pt}
    \label{fig:global_optimization}
\end{figure*}



\subsection{Experiment Result}

As shown in Table~\ref{tab:evaluation}, {\frameworkname} achieves significant reduction in both physical depth and `\# fusion' compared to the baseline. In specific, \frameworkname reduces the physical depth on by a factor of xxx on average, up to xxx. \frameworkname also reduces the number of fusions by a factor of xxx on average, up to xxx.

Among the benchmarks, \frameworkname has the most significant improvement for BV. The reasons are folds. First, the graph state representation of BV in the one-way model contains no cycles, and is thus completely planar. This naturally fits the planar-centric design of \frameworkname. Second, the graph representation of BV contains a very high-degree node, i.e. as high as half of the number of qubits on average. In the simulation approach adopted by the baseline, that requires a huge number of inserted SWAP gates and thus waste a lot of physical layers. However, in \frameworkname, it can be suppressed to a few of physical layers by a heuristic planar search that fully utilizes the resource states in those physical layers. 

In contrast, the graph representations of QFT and QAOA contain a lot of short-range and long-range cycles, which not only makes the heuristic search much harder than that of BV, but also breaks the planarity of the graph. However \frameworkname still achieves a reduction on the physical depth by a factor of xxx, xxx, and a reduction on the number of fusions by a factor of xxx,xxx for QFT and QAQA respectively.
%\newline


\subsection{Optimization Analysis}
\textbf{Increase resource utilization}
The significant improvements by \frameworkname come from the increased utilization of resource states on each physical layer.
To demonstrate, Fig.~\ref{fig:case_study} shows the mappings of fusion graphs generated by \frameworkname.
Fig.~\ref{fig:case_study}(a) is a 9-qubit BV program mapped onto a $8\times 8$ RSG grid while Fig.~\ref{fig:case_study}(b) is a 3-qubit QFT program mapped onto a $8\times 8$ RSG grid. 
These two program are two typical cases of acyclic structure and 
cyclic structure. In the figure, each dot represents a resource state. Dots in blue corresponds to the nodes existing in the fusion graph, and pink dots represents the auxiliary resource states used for routing. In compared with the sparse mapping (Fig.~\ref{fig:3d_simulation}) in the baseline caused by the rigid pattern of mapping and the large amount of preserved Z-measurement qubits, \frameworkname enables a possibly dense mapping by increasing the utilization of each physical layer. 






\noindent \textbf{Flexible Physical Area}
Besides the improvement in performace, \frameworkname also enables a lower constraint and a more flexible adaptivity to the varied size of physical layers. In comparison with the fixed size of physical layers required by the baseline approach caused by the fixed locations of logical qubits in the baseline, \frameworkname does not put a strict constraint on the size of physical layers. \frameworkname can compile the program onto a much smaller physical hardware than the baseline, with a trade-off of more physical layers. For example, Fig.~\ref{fig:global_optimization} shows a slice of fusion graph mapping of a 16-qubit QFT program on three layers of $13\times 13$ RSG grid, which is much smaller than the $23\times 23$ RSG grid required by the baseline. Moreover, when the physical layers are larger than required by the baseline, the simulation approach has no way to utilize the extra resource, while \frameworkname allows an optimization by spanning the mapping all over the physical layers.
% rigid pattern used by the baseline with a fixed occupation pattern and lots of unoccupied locations preserved to assist non-neighboring multi-qubit gates, our framework enables the mapping onto small physical layers and take more advantage of the large physical layers when they are available.

% \begin{figure*}[h]
%     % \newcommand{\fhe}{0.114}
%     \newcommand{\fhe}{0.114}
%         \includegraphics[height=\fhe\textwidth]{imgs/BVz=0.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BVz=1.pdf} 
%         \includegraphics[height=\fhe\textwidth]{imgs/BVz=2.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BVz=3.pdf}
%         \includegraphics[height=\fhe\textwidth]{imgs/BVz=4.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BVz=5.pdf} 
%         \includegraphics[height=\fhe\textwidth]{imgs/BVz=6.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BVz=7.pdf}  
%         \\
%         % \vspace{-5pt}
%         \caption{(a) The effect of planarity awareness during adaptive fusion on depth. (b) The effect of planarity awareness during adaptive fusion on `\# fusion'.
%         }
%         \label{fig:case_study}
% \end{figure*}






\noindent \textbf{More Global Optimization}
With the \archName proposed in Section~\ref{sect:hardware_model} (Fig.~\ref{fig:archoverview}), \frameworkname also enables a more global optimization in the mapping by searching through the extended plane composed by multiple active layers. As a demonstration, Fig.~\ref{fig:global_optimization} shows a slice of mapping generated by \frameworkname for a 16-qubit QFT program. The whole rectangular plane is composed of 3 layers of $13\times 13$ RSG grid (much less than the $23\times 23$ physical layers required by the baseline). In the figure, blue and green dots correspond to the nodes `$\otimes$' existing in the fusion graph, with the green ones representing the incomplete nodes, which means that some of their neighbors have not been mapped onto the grid. Again, pink dots represent the auxiliary resource states used for routing.

As can be seen, ... at a cost of sacrificing the inter-layer connectivity except for those at boundaries. Moreover, suppress the search space


% \textbf{The effect of dynamic scheduling:} 
% We study the effect of dynamic scheduling by comparing the Clifford-eager scheduling with a non-eager one. Fig~\ref{fig:opt1}(a) shows the comparison of the improvement factors of depth and `\# fusion' between the Clifford-eager scheduling and the non-eager scheduling.




==> 07_evaluation_rebuttal.tex <==
\vspace{0.3em}
\section{Evaluation}\label{sect:eval}

% \todo{Rephrase for more insights!}
\vspace{0.3em}
\subsection{Experiment Setup}\label{sect:expset}

% \textbf{Platform} We perform all experiments on a Manjaro Linux laptop with a 4$\times$Intel Core i7-7500U CPU and 8GB RAM. Other software includes Python 3.10.2 and Qiskit 0.36.1~\cite{Qiskit}.
\noindent\textbf{Metric} As discussed in Section~\ref{sect:overview}, the first metric we consider is the physical depth, i.e., the number of physical layers consumed in the execution of the program. 
% To make it comparable with the baseline, we assume that the number of RSGs on the hardware is the same as that is required by the implementing baseline.
The second metric is the number of fusion operations performed in the execution of the program, which is denoted as `\#~fusion'. A better compiler should compile a quantum program into a smaller depth which indicates a shorter execution time and less consumption of resources, and a smaller `\#~fusion' which indicates less overhead and being less error-prone. For comparison with the baseline, we define an improvement factor of physical depth as the ratio of the depth in the baseline to the depth in \frameworkname, and an improvement factor of `\#~fusion' as the ratio of the number of fusions consumed in the baseline to the that consumed in \frameworkname.
%\newline

\noindent \textbf{Baseline} 
Our optimized baseline is based on the basic MBQC interpreter introduced in Section~\ref{sect:background} but with two preprocessing steps.
The first step is synthesizing a sufficiently large 3D cluster state by fusions from small resource states generated by the RSGs. The sufficient size of each 2D layer of the cluster state is referred to as \emph{cluster area}, while the number of RSGs required to form a cluster state of that size is referred to as \emph{physical area}. The second step is finding a layout for the circuit so that measurement patterns of all gates in the circuit can be joined in a way shown as Figure~\ref{fig:circuit_simulation}. 

For the first step, instead of relying on any specific synthesis strategy, we adopt a lower bound of the physical area, which indicates the least number of required resource states when ignoring the spatial constraints for fusion routing.
For the second step, to ensure an efficient implementation of a two-qubit gate with MBQC, it is necessary to place the strips of the involved qubits close to each other in the cluster state, similar to that in the circuit model with solid-state-qubit quantum computing. As a result, we utilize the qubit mapping and routing functions of Qiskit~\cite{Qiskit} to address the issues related to far-apart 2-qubit gates prior to mapping the circuit onto the cluster state.
Specifically, this is achieved by using a 2D coupling graph that shares the same structure with each 2D layer of the cluster state as the hardware coupling graph to Qiskit. 

In the implementation of this baseline approach, 2-qubit gates such as controlled phase gates and SWAP gates are decomposed to CNOT gates along with 1-qubit gates due to the lack of available measurement patterns for them. Thus future work that finds more efficient measurement patterns for these 2-qubit gates can be used to improve this baseline.


% As result, the depth of the baseline is calculated as 6 times that of the depth given by the Qiskit compiled circuit, assuming that each one-qubit and two-qubit can be implemented by a measurements pattern of length 6, as shown in Figure~\ref{fig:circuit_simulation}. This assumption makes the calculated depth also a lower bound, in the sense that it is not known yet know how a controlled phase gate or a SWAP gate can be implemented within a pattern of length 6. The number of fusion required by the baseline approach is calculated by the number of required fusions to form the cluster state, that is, the required fusions to form each layer of cluster state multiplying the baseline depth calculated above.




% The first step is generating a large enough 3D cluster state by fusions from small resource states generated by the RSGs, with the required size of each 2D layer of the cluster state defined as \emph{cluster area}, and the number of RSGs required to form a cluster state of that size as \emph{physical area}. Lacking an existing efficient fusion algorithm, we instead estimate a lower bound for the physical area.} 
%
% \fix{The second step is to optimize the input circuit so that it better matches the naive MBQC interpreter. The key insight is that an efficient implementation of a two-qubit gate with MBQC also requires the strips of these two qubits to be placed close to each other in the cluster state, similar to that with the circuit model on solid-state-qubit quantum computing. Thus we use the qubit mapping and routing functions of Qiskit~\cite{Qiskit} to resolve far-apart 2-qubit gate issues before mapping the circuit to the cluster state. This is achieved by using a 2D coupling graph that shares the same structure with each 2D layer of the cluster state as the hardware coupling graph to Qiskit. }

\noindent \textbf{Benchmark programs} We select Quantum Fourier transform (QFT), quantum approximate optimization algorithm (QAOA), Ripple-Carry Adder (RCA)~\cite{RCA} and Bernstein-Vazirani (BV) algorithm as our benchmarks, which include both building blocks of quantum programs (QFT and RCA) and application driven programs targeting at solving real-world problems (QAOA and BV).
For QAOA,
we choose the graph maxcut problem on randomly generated graphs. Specifically, the graphs are generated by randomly selecting half of its all possible edges.
% Specifically, among all the possible edges among the given nodes, half of them are selected randomly to generate the graphs.
For BV, we select the secret strings randomly, with approximately half of the digits being 0 and half being 1. In table~\ref{tab:benchmark}, we list the number of qubits and the number of gates  for each benchmark, as well as the cluster area and physical area required by the baseline approach. For each benchmark, our framework is evaluated on the same physical area with the baseline to make them more comparable.
%\fix{We also list the number of qubits in each layer of the cluster state required by the baseline approach, referred to as \emph{cluster area}, and the minimum size of the RSG array required to form the cluster state of that size, referred to as \emph{physical area}.} 
% We also list the cluster area and physical area require by the baseline approach.
% Our framework are evaluated on the same physical areas with the baseline for the sake of comparison.
%We also list the minimum area of each layer of the cluster state required by the baseline as \todo{`cluster area'} and the minimum area of each physical layer required by the baseline as `physical area'. We use the same physical area in the evaluation of \frameworkname~in order to compare with the baseline. 
%The number of qubits we select are of the form $n^2$ because that is the maximum number of logical qubits that can be accommodated by the area (qubit number between $(n-1)^2+1$ and $n^2$ all require the same area).

\begin{table}[h]
    \centering
      \caption{Benchmark programs.}
      % \vspace{-5pt}
      
    \resizebox{0.43\textwidth}{!}{
    \renewcommand*{\arraystretch}{1.4}
    \begin{tabular}{|p{1.8cm}|p{1.0cm}|p{1.5cm}|p{1.8cm}|}  \hline
    Name & \#qubit & cluster area & physical area  \\ \hline

  \multirow{3}{1.8cm}{Quantum Fourier Transform (QFT)} 
 & 16  & \qsixteenGrid & \qsixteenRSG\\ \cline{2-4}
  & 25 & \qtwentyfiveGrid & \qtwentyfiveRSG  \\ \cline{2-4}
  & 36 & 11x11  & 25x25  \\ \hline%\cline{2-5}
  
  \multirow{3}{1.8cm}{Quantum Approximate Optimization Alg (QAOA)} & 16  & \qsixteenGrid & \qsixteenRSG\\ \cline{2-4}
  & 25 & \qtwentyfiveGrid & \qtwentyfiveRSG  \\ \cline{2-4}
  & 36 & 11x11  & 25x25  \\ \hline%\cline{2-5}
 
 \multirow{3}{1.8cm}{Ripple-Carry Adder (RCA)} 
 & 16  & \qsixteenGrid & \qsixteenRSG\\ \cline{2-4}
  & 25 & \qtwentyfiveGrid & \qtwentyfiveRSG  \\ \cline{2-4}
  & 36 & 11x11  & 25x25  \\ \hline%\cline{2-5}
 \multirow{3}{1.8cm}{Bernstein Vazirani (BV)} 
 & 16  & \qsixteenGrid & \qsixteenRSG\\ \cline{2-4}
  & 25 & \qtwentyfiveGrid & \qtwentyfiveRSG  \\ \cline{2-4}
 & 100 & 19x19 & 43x43 \\ \hline
\end{tabular}
}
 % \vspace{-10pt}
    \label{tab:benchmark}
\end{table}

% \begin{table}[h]
%     \centering
%       \caption{Benchmark programs.}
%       % \vspace{-5pt}
      
%     \resizebox{0.43\textwidth}{!}{
%     \renewcommand*{\arraystretch}{1.4}
%     \begin{tabular}{|p{1.8cm}|p{1.0cm}|p{1.0cm}|p{1.5cm}|p{1.8cm}|}  \hline
%     Name & \#qubit & \#gate & cluster area & physical area  \\ \hline

%   \multirow{4}{1.8cm}{Quantum Fourier Transform (QFT)} & 9 & 320 & \qnineGrid & \qnineRSG \\ \cline{2-5} 
%  & 16 & 1000 & \qsixteenGrid & \qsixteenRSG\\ \cline{2-5}
%   & 25 & 2400 & \qtwentyfiveGrid & \qtwentyfiveRSG  \\ \cline{2-5}
%   & 36 &  & 11x11 & 25x25  \\ \hline%\cline{2-5}
  
%   \multirow{3}{1.8cm}{Quantum Approximate Optimization Alg (QAOA)} & 9 & 130 & \qnineGrid & \qnineRSG\\\cline{2-5}
%  & 16 & 400 & \qsixteenGrid & \qsixteenRSG  \\ \cline{2-5}
%  & 25 & 700 & \qtwentyfiveGrid & \qtwentyfiveRSG \\\hline % \cline{2-5}
 
%  \multirow{3}{1.8cm}{Ripple-Carry Adder (RCA)} 
%  & 16 & 500 & \qsixteenGrid & \qsixteenRSG\\ \cline{2-5}
%   & 25 & 840 & \qtwentyfiveGrid & \qtwentyfiveRSG  \\ \cline{2-5}
%   & 49 & 1750 & \qfortynineGrid & \qfortynineRSG \\ \hline %\cline{2-5}
  
%  \multirow{3}{1.8cm}{Bernstein Vazirani (BV)} 
%  & 16 & 50 & 7x7 & 16x16 \\ \cline{2-5}
%  & 100 & 300 & \qhundrGrid & \qhundrRSG \\ \cline{2-5}
%  & 196 & 600 & \qtwohundrGrid & \qtwohundrRSG \\ \hline
% \end{tabular}
% }
%  % \vspace{-10pt}
%     \label{tab:benchmark}
% \end{table}


% \begin{figure}[t]
%     \newcommand{\fhe}{0.2}
%     \hspace{15pt}
%         \includegraphics[height=\fhe\textwidth]{imgs/8-degree-vertex-mapping.pdf} \hfill \includegraphics[height=\fhe\textwidth]{imgs/3-qubit-QFT_8x8_large_node.pdf} \hspace{15pt}
%         \\
%         \hphantom{} \hspace{58pt}(a) \hspace{105pt} (b) 
%         % \vspace{-5pt}
%         \caption{(a) Slices of mapping for 8-qubit BV with secret string '11111111'. (b) Mapping of 3-qubit QFT. Blue dots correspond to nodes `$\otimes$' existing in the fusion graph, pink dots represents auxiliary vertices to help form high degree vertices and cycles.\todo{need to label ABCD}
%         }
        
%         \vspace{-10pt}
%         \label{fig:case_study}
% \end{figure}

%%%%%%% original version graph
% \begin{figure}[t]
%     \newcommand{\fhe}{0.23}
%         \includegraphics[height=\fhe\textwidth]{fig/labeled_left.pdf} \hfill \includegraphics[height=\fhe\textwidth]{fig/labeled_right.pdf}
%         \\
%         \hphantom{} \hspace{58pt}(a) \hspace{105pt} (b) 
%         % \vspace{-5pt}
%         \caption{(a) Mapping of fusion graph for 8-qubit BV with secret string '11111111'. (b) Mapping of fusion graph for 3-qubit QFT. Blue dots correspond to nodes `$\otimes$' existing in the fusion graph, pink dots represent auxiliary resource states used for routing.
%         }
%         \vspace{-15pt}
%         \label{fig:case_study}
% \end{figure}


% \begin{figure*}[t]
%     \newcommand{\fhe}{0.16}
%         \includegraphics[height=\fhe\textwidth]{fig/labeled_left.pdf}  \includegraphics[height=\fhe\textwidth]{fig/labeled_right.pdf}
%         \hspace{5pt}
%         \includegraphics[height=0.16\linewidth,width=0.63\linewidth]{fig/QFT_16qbt_3lyr.png}
%         \\
%         \hphantom{}(a) \hspace{70pt} (b) \hspace{200pt} (c) \hspace{100pt}
%         % \vspace{-5pt}
%         \caption{(a) Mapping of fusion graph for 8-qubit BV with secret string `11111111'. (b) Mapping of fusion graph for 3-qubit QFT. (c) Mapping of the fusion graph of a 16-qubit QFT program with a more global optimization by considering an extended physical layer consisting of 3 successive physical layers of size $13\times13$. Blue and green dots correspond to the nodes `$\otimes$' existing in the fusion graph, with the green ones being the incomplete nodes whose edges are not all mapped yet. Pink dots represent the auxiliary resource states used for routing.
%         }
%         % \vspace{-15pt}
%         \label{fig:case_study}
% \end{figure*}



% \begin{table*}[h]
% \centering
%     \caption{The results of \frameworkname~and its relative performance to the baseline. }
%   %  The name column are acronyms of test programs in Table~\ref{tab:benchmark}.}
% \resizebox{\textwidth}{!}{
% \renewcommand*{\arraystretch}{1.2}
% \begin{tabular}{|p{2cm}|p{2cm}|p{2.5cm}|p{2cm}|p{2.4cm}|p{2.9cm}|p{2cm}|}  \hline
% {Name-\#qubits} &  {Baseline Depth} & {Our Depth} & Improv. Factor & Baseline \#Fusions   & Our \#Fusions & Improv. Factor \\ \hline

% QFT-9 & 372 & 29 & 13 & 53,568 & 1,747 & 31\\\hline
% QFT-16  & 1,206 & 73 & 17 & 308,736 & 7,752 & 40 \\\hline
% QFT-25 & 3,002 & 162 & 19 & 1,323,882 & 26,921 & 49\\\hline
% QFT-36 & 6,436 & 324 & 20 & 4,022,500 & 66,830 & 60 \\\hline
% QFT-49 & 12,158 & 214 & 17 &  & 18,143 & \\\hline

% QAOA-9  & 86 & 11 & 8 & 12,384 & 696 & 18\\\hline
% QAOA-16  & 283 & 35 & 8 & 72,448 & 3,019 & 24 \\\hline
% QAOA-25  & 633 & 65 & 10 & 279,153 & 9,016 & 31\\\hline
% QAOA-36  & 1,322 & 151 & 9 & 826,250 & 20,268 & 41\\\hline

% RCA-16 & 730 & 49 & 15 & 186,880 & 2,930 &  \\\hline
% RCA-25 & 1,278 & 69 & 18 & 563,598 & 5,849 & \\\hline
% RCA-49 & 2,738 & 143 & 19 & 2,464,200 & 13,962 &  \\\hline

% BV-16 & 93 & 1 & 93 & 23,808 & 63 & 378\\\hline
% BV-49 & 415 & 4 & 104 & 373,500 & 309 & 1,209\\\hline
% BV-100 & 797 & 4 & 199 & 1,473,653 & 644 & 2,288\\\hline
% % BV-196  & 2,142 & 5 & 428 & 7,970,382 & 801 & 9951\\\hline
% % BV-324 & 4,500 & 7 & 643 & 28,084,500 & 1,358 & 20681\\\hline
% \end{tabular}
%     }

%     \label{tab:evaluation}
% \end{table*}


\begin{table*}[h]
\centering
    \caption{The results of \frameworkname~and its relative performance to the baseline. }
  %  The name column are acronyms of test programs in Table~\ref{tab:benchmark}.}
\resizebox{\textwidth}{!}{
\renewcommand*{\arraystretch}{1.4}
\begin{tabular}{|p{2cm}|p{2cm}|p{2.5cm}|p{2cm}|p{2.4cm}|p{2.9cm}|p{2cm}|}  \hline
{Name-\#qubits} &  {Baseline Depth} & {Our Depth} & Improv. Factor & Baseline \#Fusions   & Our \#Fusions & Improv. Factor \\ \hline

QFT-16  & 1,916 & 82 & 23 & 490,296 & 8,167 & 60 \\\hline
QFT-25 & 3,584 & 162 & 22 & 1,580,544 & 26,921 & 59\\\hline
QFT-36 & 6,108 & 324 & 19 & 3,817,500 & 66,830 & 57 \\\hline

QAOA-16  & 809 & 29 & 28 & 207,104 & 2,578 & 80 \\\hline
QAOA-25  & 1,963 & 63 & 31 & 865,683 & 8,343 & 104\\\hline
QAOA-36  & 4,292 & 122 & 35 & 2,682,500 & 21,302 & 126\\\hline

RCA-16 & 1,020 & 46 & 22 & 261,120 & 4,568 & 57 \\\hline
RCA-25 & 1,877 & 65 & 29 & 827,757 & 8,915 & 93 \\\hline
RCA-36 & 2,863 & 85 & 34 & 1,789,375 & 14,115 & 127 \\\hline

BV-16 & 132 & 1 & 132 & 33,792 & 63 & 536\\\hline
BV-25 & 284 & 1 & 284 & 125,244 & 114 & 1,099\\\hline
BV-100 & 1,371 & 4 & 343 & 2,534,979 & 644 & 3,936\\\hline
% BV-49 & 415 & 4 & 104 & 373,500 & 309 & 1,209\\\hline
% BV-100 & 797 & 4 & 199 & 1,473,653 & 644 & 2,288\\\hline
% BV-196  & 2,142 & 5 & 428 & 7,970,382 & 801 & 9951\\\hline
% BV-324 & 4,500 & 7 & 643 & 28,084,500 & 1,358 & 20681\\\hline
\end{tabular}
    }

    \label{tab:evaluation}
\end{table*}


% \begin{table*}[h]
% \centering
%     \caption{The results of \frameworkname~and its relative performance to the baseline. }
%   %  The name column are acronyms of test programs in Table~\ref{tab:benchmark}.}
% \resizebox{\textwidth}{!}{
% \renewcommand*{\arraystretch}{1.2}
% \begin{tabular}{|p{2cm}|p{2cm}|p{2.5cm}|p{2cm}|p{2.4cm}|p{2.9cm}|p{2cm}|}  \hline
% {Name-\#qubits} &  {Baseline Depth} & {Our Depth} & Improv. Factor & Baseline \#Fusions   & Our \#Fusions & Improv. Factor \\ \hline

% QFT-9 & 462 & 29 & 16 & 66,528 & 1,158 & 57\\\hline
% QFT-16  & 1,392 & 82 & 17 & 356,352 & 4,821 & 74\\\hline
% QFT-25 & 3,678 & 214 & 17 & 1,621,998 & 18,143 & 89\\\hline

% QAOA-9  & 426 & 23 & 19 & 61,344 & 911 & 67\\\hline
% QAOA-16  & 1,050 & 60 & 18 & 268,800 & 2,979 & 90\\\hline
% QAOA-25  & 1,584 & 99 & 16 & 698,544 & 7,336 & 95\\\hline

% RCA-16 & 730 & 49 & 15 & 186,880 & 2,930 & 64 \\\hline
% RCA-25 & 1,278 & 69 & 18 & 563,598 & 5,849 & 96\\\hline
% RCA-49 & 2,738 & 143 & 19 & 2,464,200 & 13,962 & 177 \\\hline

% BV-16 & 96 & 4 & 24 & 24,576 & 220 & 112\\\hline
% BV-100 & 1,290 & 4 & 323 & 2,385,210 & 437 & 5458\\\hline
% BV-196  & 2,142 & 5 & 428 & 7,970,382 & 801 & 9951\\\hline
% BV-324 & 4,500 & 7 & 643 & 28,084,500 & 1,358 & 20681\\\hline
% \end{tabular}
%     }

%     \label{tab:evaluation}
% \end{table*}


% \begin{table*}[t!]
% \centering
%     \caption{The results of \frameworkname~and its relative performance to the baseline. }
%   %  The name column are acronyms of test programs in Table~\ref{tab:benchmark}.}
% \resizebox{\textwidth}{!}{
% \renewcommand*{\arraystretch}{1.2}
% \begin{tabular}{|p{2cm}|p{2cm}|p{2.5cm}|p{2cm}|p{2.4cm}|p{2.9cm}|p{2cm}|}  \hline
% {Name-\#qubits} &  {Baseline Depth} & {\frameworkname~Depth} & Improv. Factor & Baseline \#Fusions   & \frameworkname~\#Fusions & Improv. Factor \\ \hline

% % QFT-4 & 5x5 && 11x6 & 6(old) & - & - & 85 & -\\\hline
% %RCA-7 & - & 22 & - & - & 976 & - \\\hline

% QFT-9 & 462 & 29 & 15.9 & 66,528 & 1,158 & 57.4\\\hline
% QFT-16  & 1,392 & 82 & 17.0 & 356,352 & 4,821 & 73.9\\\hline

% QFT-25 & 3,678 & 214 & 17.2 & 1,621,998 & 18,143 & 89.4\\\hline
% % QFT-36 & 21x21 & 1355x6 & - & - & - & - & -\\\hline
% %QFT-49 & 25x25 & 2532x6 & - & - & - & - & -\\\hline
% QAOA-9  & 426 & 23 & 18.5 & 61,344 & 911 & 67.3\\\hline
% QAOA-16  & 1,050 & 60 & 17.5 & 268,800 & 2,979 & 90.2\\\hline
% QAOA-25  & 1,584 & 99 & 16.0 & 698,544 & 7,336 & 95.2\\\hline

% % RCA-16 & 930 & 57 & 16.3 & 238,080 & 3,158 & 75.4\\\hline
% RCA-25 & 1572 & 87 & 18.1 & 693,252 & 5,834 & 118.8 \\\hline
% RCA-36 & 2,418 & 136 & 17.8 & 1,511,250 & 8,763 & 172.5 \\\hline
% RCA-49 & 3294 & 206 & 16.0 & 2,964,600 & 13,372 & 221.7 \\\hline

% BV-100 & 1,290 & 4 & 322.5 & 2,385,210 & 437 & 5458.1\\\hline
% BV-196  & 2,142 & 5 & 428.4 & 7,970,382 & 801 & 9950.5\\\hline
% BV-324 & 4,500 & 7 & 642.9 & 28,084,500 & 1,358 & 20680.8\\\hline
% \end{tabular}
%     }

%     \label{tab:evaluation}
% \end{table*}

%%%%%%%%%%%%% first version graph
% \begin{figure}[t]
%     \centering    
%     % \vspace{-5pt}
%     \includegraphics[height=0.25\linewidth,width=\linewidth]{fig/QFT_16qbt_3lyr.png}
%     \caption{Mapping of the fusion graph of a 16-qubit QFT program with a more global optimization by considering an extended physical layer consisting of 3 successive physical layers of size $13\times13$. Blue and green dots correspond to the nodes `$\otimes$' existing in the fusion graph, with the green ones being the incomplete nodes whose edges are not all mapped yet. Pink dots represent the auxiliary resource states used for routing.}
%     \vspace{-10pt}
%     \label{fig:global_optimization}
% \end{figure}


% \vspace{0.3em}
\subsection{Experiment Result}

We first show the results of  the baseline and \frameworkname\ for 3-qubit resource states in Table~\ref{tab:evaluation}, as the number of qubits increases for each benchmark. It can be seen that \frameworkname\ outperforms the baseline by orders of magnitude in both physical depth and the number of fusions. As the number of qubits increases, this improvement of performance stays stable or slightly increases.

Among the benchmarks, \frameworkname\ has the most significant improvement for BV. This is because the graph state of BV is acyclic and planar, making it easier the heuristic search in \frameworkname\ to find a compact layout for the graph and map it to only a few physical layers. In contrast, the graph states of the QFT, QAOA and RCA contain a lot of short-range and long-range cycles, which makes the structure more complex and increases the demand for routing. However, for these benchmarks, \frameworkname\ still achieves a reduction on the physical depth by a factor of over 20, and a reduction on the number of fusions by a factor of over 50.

\noindent\textbf{General resource states}
To achieve greater generality, our optimization modules are designed to be extendable to a wide range of resource states. 
This is made possible by accommodating flexible fusion strategies for synthesizing graph states and representing each strategy with a fusion graph.
Fig.\ref{fig:different_resource_states} shows the results when the resource states are 3-qubit line-shaped graph state, 4-qubit line-shaped, star-shaped and ring-shaped graphs states, respectively. The improvements in physical depth and the number of fusions are shown in (a) and (b), respectively. It can be seen that \frameworkname\ achieves similar levels of improvement in performance for these various resource states. 

\begin{figure}[h!]
        \centering
        \hspace{-15pt}\includegraphics[width=0.7\linewidth]{fig/depth_with_shape.pdf} \\
        (a)\\
        \vspace{5pt}
        \hspace{-15pt}\includegraphics[width=0.7\linewidth]{fig/fusion_with_shape.pdf}\\
        (b)
    
        % \hspace{30pt}(a)\hspace{160pt}(b) 
        \caption{\fix{Improvement factors of physical depth (a) and \#~fusions (b)  of 16-qubit QFT, QAOA, RAC and BV for different basic resource states.}
        }
        % \vspace{-15pt}
        \label{fig:different_resource_states}
\end{figure}

\begin{figure}[h!]
        \centering
        \hspace{-15pt}\includegraphics[width=0.7\linewidth]{fig/depth_with_layer_shape.pdf} \\
        (a)\\
        \vspace{5pt}
        \hspace{-15pt}\includegraphics[width=0.7\linewidth]{fig/fusion_with_layer_shape.pdf}\\
        (b)
    
        % \hspace{30pt}(a)\hspace{160pt}(b) 
        \caption{Normalized improvement factors of physical depth (a) and \#~fusions (b) of 16-qubit QFT, QAOA, RCA and BV on different shapes of physical layers. Improvement factors on rectangular physical layers (ratio $>1$) are normalized by those on square physical layers (ratio $= 1$). 
        % Horizontal axis indicates the ratio of length and width for the physical layers.
        }
        % \vspace{-15pt}
        \label{fig:different_layer_shapes}
\end{figure}

\begin{figure*}[t]
    % \newcommand{\fhe}{0.16}
    % \includegraphics[height=0.16\linewidth,width=0.63\linewidth]{fig/QFT_16qbt_3lyr.png}
    \includegraphics[height=0.2\linewidth,width=0.7\linewidth]{fig/QFT_16qbt_3lyr.png}
        \\
        % \vspace{-5pt}
        \caption{ Mapping of the fusion graph of a 16-qubit QFT program with a more global optimization by considering an extended physical layer consisting of 3 successive physical layers of size $13\times13$. Blue and green dots correspond to the nodes `$\otimes$' existing in the fusion graph, with the green ones being the incomplete nodes whose edges are not all mapped yet. Pink dots represent the auxiliary resource states used for routing.
        }
        % \vspace{-15pt}
        \label{fig:extended_case_study}
\end{figure*}






\noindent \textbf{Flexible coupling structure} While the results in Table~\ref{tab:evaluation} are on physical layers of $N\times N$ square coupling structure, \frameworkname\ is applicable to more general coupling structures. Figure~\ref{fig:different_layer_shapes} shows the physical depth (\ref{fig:different_layer_shapes}(a)) and the number of fusions (\ref{fig:different_layer_shapes}(b)) when the ratio of each physical layer is 16x16  (ratio = 1), 20x13 (ratio = 1.5), 23x11  (ratio = 2.1) and 26x10 (ratio = 2.6) respectively. For comparison, the results are normalized by that on the 16x16 physical layer. It can be seen that \frameworkname\ achieves similar levels of performance on these various shapes of physical layers. Moreover, the area of physical layers is adjustable by regarding multiple consecutive physical layers as an extended physical layer, which can be used to accommodate more global structure of the graph. As a demonstration, Fig.~\ref{fig:extended_case_study} shows a slice of mapping generated by \frameworkname~for a 16-qubit QFT program. The whole rectangular $13\times39$ extended physical layer is composed of 3 layers of $13\times 13$ grid. The first physical layer ranges from column 1 to column 13, the second ranges from column 14 to column 26, and the third from column 27 to column 39 respectively. In the figure, blue and green dots correspond to the nodes `$\otimes$' existing in the fusion graph, with the green ones representing the incomplete nodes, which means that some of edges connected to them have not been mapped onto the grid. Pink dots represent the auxiliary resource states used for routing. In principle, the optimization techniques in \frameworkname\ is also applicable when the coupling structure between RSGs are not orthogonal (e.g., triangular, hexagonal) since none of our optimization modules has explicit dependency on a specific coupling architecture.



\textbf{Effect of physical area}
In contrast to the fixed size of physical layers required by the baseline approach, \frameworkname\ does not impose strict constraints on the size of physical layers, allowing programs to be compiled onto hardware of different sizes. Specifically, the physical depth can be decreased by allowing longer routing paths on larger physical layers, with a cost of more fusions. Figure~\ref{fig:depth_with_physical_area} shows the improvement factors of physical depth and the number of fusions when compiling onto different sizes of physical layers. When the physical area increases, the improvement factor of physical depth initially increases rapidly, but eventually reaches a plateau when the physical area becomes sufficiently large. On the other hand, the improvement factor of the number of fusions shows a reverse trend, decreasing as the physical area increases. Note that if physical layers are larger than necessary, they can be truncated by restricting compilation to a portion of the physical layers.

% As the physical area increases, the improvement factor of physical depth increases rapidly, and then begins to plateau when the physical area becomes sufficiently large, while the improvement factor of the number of fusions shows a reverse trend. Certainly, physical layers can always be truncated by restricting the compilation within part of the physical layers when they are larger than necessary.


\begin{figure}[h!]
        \centering
        \hspace{-15pt}\includegraphics[width=0.7\linewidth]{fig/area_effect_on_depth.pdf} \\
        (a)\\
        \vspace{5pt}
        \hspace{-15pt}\includegraphics[width=0.7\linewidth]{fig/area_effect_on_fusion.pdf}\\
        (b)
        \caption{\fix{Improvement factors of (a) depth and (b) \#~fusions of 16-qubit QFT, QAOA, RAC and BV for different physical areas.}
        }
        % \vspace{-15pt}
        \label{fig:depth_with_physical_area}
\end{figure}

% The significant improvements by \frameworkname\ come from the increased utilization of resource states on each physical layer.
% To demonstrate, Fig.~\ref{fig:case_study} shows the mappings of fusion graphs generated by \frameworkname.
% Fig.~\ref{fig:case_study}(a) is a 8-qubit BV program mapped onto a $8\times 8$ RSG grid while Fig.~\ref{fig:case_study}(b) is a 3-qubit QFT program mapped onto a $8\times 8$ RSG grid. 
% These two programs are two typical cases of acyclic structure and 
% cyclic structure. In the figure, each dot represents a resource state. Dots in blue correspond to the nodes `$\otimes$' existing in the fusion graph, and the pink dots represent the auxiliary resource states used for routing. \frameworkname~enables a dense mapping that increases the utilization of each physical layer, in contrast to the sparse mapping in the baseline caused by the rigid pattern of mapping and the large amount of preserved Z-measurement qubits. 




% \noindent \textbf{Flexible to Number of RSGs.}
% In contrast to the baseline approach, \frameworkname~does not impose strict constraints on the size of physical layers, allowing programs to be compiled onto hardware with different sizes, either smaller with the trade-off of using more physical layers, or larger with the benefit of utilizing the extra resources. For instance, Fig.\ref{fig:case_study}(c) shows a subgraph of the fusion graph of 16-qubit QFT mapped onto three physical layers, each with 169 resource states, despite the baseline requires each physical layer with 256 resource states.


% % rigid pattern used by the baseline with a fixed occupation pattern and lots of unoccupied locations preserved to assist non-neighboring multi-qubit gates, our framework enables the mapping onto small physical layers and take more advantage of the large physical layers when they are available.

% \noindent 
% \fix{\textbf{Scaling with Large Cluster States.} Fig.\ref{fig:different_resource_states}(c) shows the depth improvement for applying our compiler to quantum hardware (Fig.~\ref{fig:archoverview}), for which each layer is directly built by a large native cluster state without the help of fusion. 
% %Our framework can still provide considerable improvement of #depth even if large cluster states are directly available without the help of fusion. 
% Indeed, the improvement of #depth is still significant, 
% %comparable to that in Table II, 
% as our routing and scheduling modules remain essential to address the discrepancy between the fixed hardware cluster states and varying graph states that represent different input circuits.  However, the fusion graph generation module is simplified to a straightforward high-degree node decomposition module as we do not need the optimizations for fusing a set of small cluster states anymore.
% Generally speaking, more advanced hardware will make software design easier, but software solutions are often more cost-effective and can help achieve similar levels of performance even without more advanced hardware.  
% }
%It can be seen that the improvement of depth becomes more significant as the size of cluster states increases, but eventually levels off when the size becomes too large. This is because our framework provides flexibility to leverage the increasing size of the physical layer, while the baseline is limited to using a constant physical area regardless of its size.

% \begin{figure*}[h]
%     % \newcommand{\fhe}{0.114}
%     \newcommand{\fhe}{0.114}
%         \includegraphics[height=\fhe\textwidth]{imgs/BVz=0.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BVz=1.pdf} 
%         \includegraphics[height=\fhe\textwidth]{imgs/BVz=2.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BVz=3.pdf}
%         \includegraphics[height=\fhe\textwidth]{imgs/BVz=4.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BVz=5.pdf} 
%         \includegraphics[height=\fhe\textwidth]{imgs/BVz=6.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BVz=7.pdf}  
%         \\
%         % \vspace{-5pt}
%         \caption{(a) The effect of planarity awareness during adaptive fusion on depth. (b) The effect of planarity awareness during adaptive fusion on `\# fusion'.
%         }
%         \label{fig:case_study}
% \end{figure*}



% \noindent \textbf{More Global Optimization.}
% With the \archName~proposed in Section~\ref{sect:hardware_model}, \frameworkname~enables a more global optimization in the mapping by searching through an extended physical layer composed by multiple physical layers. As a demonstration, Fig.~\ref{fig:case_study}(c) shows a slice of mapping generated by \frameworkname~for a 16-qubit QFT program. The whole rectangular $13\times39$ plane is composed of 3 layers of $13\times 13$ resource state grid (much smaller than the $16\times 16$ physical layers required by the baseline). The first physical layer ranges from column 1 to column 13, the second ranges from column 14 to column 26, and the third from column 27 to column 39 respectively. In the figure, blue and green dots correspond to the nodes `$\otimes$' existing in the fusion graph, with the green ones representing the incomplete nodes, which means that some of edges connected to them have not been mapped onto the grid. Again, pink dots represent the auxiliary resource states used for routing.

% As can be seen, the mapping onto extended physical layers enables an optimization by allowing long-range structures (e.g., long-range cycles crossing the boundaries of individual physical layers, i.e., column 13,14 and column 26,27) in the mapping, at a cost of sacrificing some inter-layer connections not on the boundaries. Moreover, this mapping strategy onto extended physical layers also reduces the searching space from a 3D grid to a large 2D grid, which significantly improves the compilation efficiency without much loss of performance.

% \noindent 
% \fix{\textbf{Correctness of Our Compiler.} Our compiler is verified manually for each proposed compilation rule. For example, in the routing process, we leverage the rule that two consecutive X-measurements (or three consecutive Y-measurements) form a pattern of an identity gate, which has no impact on the computation result. Our routing process inserts these identity patterns between necessary nodes to address the hardware constraints while minimizing the lengths of routing paths. This is similar to how a compiler in the circuit model compiles the program by finding optimal insertions of the semantic-preserving Swap gates. }

%At a small scale, we also use a classical simulator~\cite{} for MBQC to run the vanilla~\cite{} and our optimized versions and check their final results.}

% \textbf{The effect of dynamic scheduling:} 
% We study the effect of dynamic scheduling by comparing the Clifford-eager scheduling with a non-eager one. Fig~\ref{fig:opt1}(a) shows the comparison of the improvement factors of depth and `\# fusion' between the Clifford-eager scheduling and the non-eager scheduling.





==> 07_experiments.tex <==
\section{Evaluation}

% TODO: map overhead; error estimation; other metrics.

\subsection{Metrics}

1. time estimation: how many time steps are needed;

2. CNOT number estimation: relates to error estimation;



In this section, we will give an extensive evaluation of our design under different settings of application and hardware.

\subsection{Experiment Setup}
\paragraph{Benchmarks \& Datasets}
We choose two representative GNN models for node classification tasks to cover different types of operations in aggregation:
\textbf{1) Graph Convolutional Network (GCN)}~\cite{GCNConv} is one of the most popular GNN architectures. 
%It has been widely adopted in node classification, graph classification, and link prediction tasks. Besides,
It is also the key backbone network for many other GNNs, such as GraphSage~\cite{SageConv}, and differentiable pooling (Diffpool)~\cite{diffpool}. Therefore, improving the performance of GCN will also benefit a broad range of GNNs. Note that for GCN evaluation, we use the setting: \textit{2 layers with 16 hidden dimensions}, which is also the setting from the original paper~\cite{GCNConv};
% The computation of a standard 2-layer GCN can be expressed as
% \begin{equation} \small
%     Z = softmax(\hat{A}\ ReLU(\hat{A}XW^1)W^2).
% \end{equation}
% where $\hat{A}$ is the adjacent matrix of the input graph with self-loop, and $X$ is the input node embedding matrix $\in R^{N\times D}$ ($N $: \#nodes in a graph, $D$: node embedding dimension). $W^1$ and $W^2$ are the weight matrix in layer-1 and layer-2, respectively. 
%\vspace{2pt}
\textbf{2) Graph Isomorphism Network (GIN)}~\cite{GINConv}.
%another typical type of GNN, aims to distinguish the graph-structure that cannot be identified by GCN.
%is , another typical type of GNNs. It aims to distinguish the graph-structure that cannot be identified by GCN. %, and 
% One of its major tasks is graph classification. Each layer of GIN uses the following formula: % as follows:  
% \begin{equation} \small
% h_{v}^{l+1} = MLP^{l}((1+\epsilon^{l})\dot h^{l} + \sum_{u\in N_{(v)}}h_{u}^{l}).    
% \end{equation}
% where $l$ is the layer ID, $MLP$ is a fully-connected neural network, $h_{v}$ is the node embedding for node $v$, and $N_{(v)}$ stands for the neighbors of node $v$. 
GIN differs from GCN in its aggregation function, which weights the node embedding values from the node itself. In addition, GIN is also the reference architecture for many other advanced GNNs with more edge properties, such as Graph Attention Network (GAT)~\cite{GATConv}. Note that for GIN evaluation, we use the setting: \textit{5 layers with 64 hidden dimensions}, which is also the setting used in the original paper~\cite{GINConv}. Graphs used in our evaluation~\cite{snapnets, GCNConv} are large in their number of nodes and edges that demand multi-GPU computation power for effective GNN computation. These graphs demonstrate high irregularity in its structures, which are challenging for most of the existing GNN frameworks. Details of the above datasets are listed in Table~\ref{table: Evaluation Dataset}. 
Note that $\#Class$ is used for node classification task.
% \paragraph{GraphSage}
% While sharing some similarity with GCN, GraphSage~\cite{SageConv} distinguishes itself in inductive learning, which is mostly useful for many real-world setting that requires learning on a small part of the graph and apply the model on the "unknown" part of the graph, even on a totally-new graph that has never seen before. Graphsage aggregation kernel has the following format.
% \begin{edqua}
% \end{edqua}{}

% \vspace{-7pt}

\paragraph{Baselines} 
\label{sect: Baseline Implementations}
% We aim to compare \Mname~with all existing GNN multi-GPU designs. 
% However, ROC~\cite{sysMLROC} and NeuGraph~\cite{ma2019neugraph} does not publicly open-source their designs. 
\underline{1) \textbf{UVM-based Design}} has been highlighted in the recent work~\cite{kim2020batch} in handling irregular graph computations (such as Breadth-First Search and PageRank) on out-of-GPU-memory graphs. 
%
Note that~\cite{kim2020batch} is not open-sourced, we implement the UVM-based kernel design by following the design strategies from \cite{kim2020batch} and incorporating all kernel optimizations from MGG ($\S$\ref{sect: NVSHMEM-based Kernel}) except the hybrid GNN data placement, which is specific to NVSHMEM-based design. Also, hierarchical workload management ($\S$\ref{sect: Hierarchical Workload Management}) is not applicable to UVM-based design, since all graph structural data (\textit{e.g.}, edge lists) and node embeddings are maintained at the same unified virtual memory space regardless of their physical location;
% is one of the most common practice adopted in many state-of-the-art multi-GPU GNN framework on GPUs, including the Neugraph~\cite{ma2019neugraph}, ROC~\cite{sysMLROC}. 
% The UVM-based design leverages the large host memory as the main storage for holding the GNN inputs that cannot be fully accommodated on the GPU device memory. Therefore, we make an in-depth comparison with UVM-based design in our evaluation;
%
\underline{2) \textbf{DGCL}}~\cite{cai2021dgcl} is the state-of-the-art work in addressing the GNN communication bottleneck in the multi-GPU settings.  
%
The core of DGCL is its GCCL~\cite{cai2021dgcl} library, a distributed graph communication library, which can be seen as an improved version of NCCL~\cite{nccl} with optimizations tailored for GNN computation. 
%
DGCL stores the partitioned subgraphs with their node embeddings on the device memory of different GPUs. 
%
During the computation, DGCL will first apply the $\mathit{Allgather}$ function for fetching the remote node embedding to local GPU global memory and then apply a local neighbor aggregation by leveraging the single-GPU GNN kernel from deep graph library~\cite{wang2019dgl}.
%
Additional multi-GPU designs, ROC~\cite{sysMLROC} and NeuGraph~\cite{ma2019neugraph} are not the state-of-the-art~\cite{cai2021dgcl, sysMLROC} and are not open-sourced. Therefore, we exclude the comparison with these two designs.
% \vspace{-2pt}
% \paragraph{Datasets}
% We choose three different types of datasets
% to cover the vast majority of the GNN inputs. 
% \textbf{Type I} graphs are the typical datasets used by many previous GNN algorithm papers~\cite{GCNConv, GINConv, SageConv}. 
% They are usually small in the number of nodes and edges, but rich in node embedding information with high dimensionality. These graphs can validate pure algorithm performance (\textit{e.g.}, the accuracy of link prediction). 
% \textbf{Type II} graphs~\cite{KKMMN2016} are the popular benchmark datasets for graph kernels and have been selected as the built-in datasets for DGL~\cite{wang2019dgl} and PyG~\cite{pyG}. Each dataset consists of a set of small graphs, which only have intra-graph edge connections without inter-graph edge connections. These graphs are generally used for batched training or inference. 
% \textbf{Type III and Type IV} 

% \begin{table}[t] \small
% \centering
% \caption{Datasets for Evaluation.}
% \vspace{-6pt}
% \scalebox{0.89}{
%  \begin{tabular}{|| l r r r r ||}
%  \hline 
%  \hline
% \textbf{Dataset} & \textbf{\#Vertex} & \textbf{\#Edge} & \textbf{\#Dim} & \textbf{{\#Class}}\\
% \hline
% \multicolumn{5}{||c||}{\textbf{Type (I)}} \\
% \hline
% Citeseer    & 3,327	    & 9,464	    & 3,703 & 6      \\
% Cora	    & 2,708     & 10,858	& 1,433 & 7      \\
% Pubmed	    & 19,717	& 88,676	& 500  & 3      \\
% PPI	        & 56,944	& 818,716	& 50   & 121    \\
% % NELL	    & 75,492	& 263,986	& 5414 & 210    \\
% \hline
% \multicolumn{5}{||c||}{\textbf{Type (II)}} \\
% \hline
% % ENZYMES	        &   19,327	       & 74,564	    &   18	    & 6 \\
% PROTEINS\_full	&   43,471	       & 162,088	&   29	    & 2 \\
% OVCAR-8H	    &   1,890,931	   & 3,946,402	&   66	    & 2 \\
% Yeast	        &   1,714,644	   & 3,636,546	&   74	    & 2 \\
% DD	            &   334,925	       & 1,686,092	&   89	    & 2 \\
% TWITTER-Partial	&   580,768	       & 1,435,116	&   1,323    & 2 \\
% SW-620H	        &   1,889,971	   & 3,944,206	&   66	    & 2 \\
% \hline
% \multicolumn{5}{||c||}{\textbf{Type (III)}} \\
% \hline
% % Reddit	        & 232,965	& 114,615,892	& 602 & 41 \\
% amazon0505	    & 410,236	& 4,878,875	    & 96  & 22 \\
% artist	        & 50,515	& 1,638,396	    & 100 & 12 \\
% com-amazon	    & 334,863	& 1,851,744	    & 96  & 22 \\
% % web-BerkStan	& 685,230	& 13,298,940	&100  & 12\\
% % wiki-topcats	& 1,791,489	& 50,892,080	& 300 & 22 \\
% soc-BlogCatalog	& 88,784	& 2,093,195	    & 128 & 39 \\
% amazon0601	    & 403,394	& 3,387,388	    & 96 & 22 \\
% % \hline
% % \multicolumn{5}{||c||}{\textbf{Type (IV)}} \\
% % \hline
% Reddit & 232,965 & 114,615,892 & 649 & 41 \\ 
% enwiki-2013 & 4,203,323 & 202,623,226 & 96 & 128 \\ 
% ogbn-products & 1,511,819,904 & 917,156,352 & 100 & 64 \\ 
% ogbn-proteins & 1,286,363,072 & 175,742,400 & 128 & 112 \\
% Com-Orkut & 3,072,441 & 117,185,083 & 128 & 32 \\ 
% Web-Google & 916,428 & 5,105,039 & 256 & 64 \\ 
% wiki-Talk & 2,394,385 & 5,021,410 & 256 & 96 \\ 
% \hline
% \end{tabular}}
% \label{table: Evaluation Dataset}
% \end{table}


\begin{table}[t] \small
\centering
\caption{Datasets for Evaluation.}
\vspace{-6pt}
\scalebox{0.84}{
 \begin{tabular}{ l | r r r r }
\specialrule{.1em}{.05em}{.05em} 
\textbf{Dataset} & \textbf{\#Vertex} & \textbf{\#Edge} & \textbf{\#Dim} & \textbf{{\#Class}}\\
\hline\hline
% amazon0505	    & 410,236	& 4,878,875	    & 96  & 22 \\
% artist	        & 50,515	& 1,638,396	    & 100 & 12 \\
% soc-blogCatalog	& 88,784	& 2,093,195	    & 128 & 39 \\
% com-amazon	    & 334,863	& 1,851,744	    & 96  & 22 \\
% amazon0601	    & 403,394	& 3,387,388	    & 96 & 22 \\
reddit(\textbf{RDD})          & 232,965   & 114,615,892 & 602 & 41 \\ 
enwiki-2013(\textbf{ENWIKI})     & 4,203,323 & 202,623,226 & 96 & 128 \\ 
ogbn-products(\textbf{PROD})   & 1,511,819,904 & 917,156,352 & 100 & 64 \\ 
ogbn-proteins(\textbf{PROT})   & 1,286,363,072 & 175,742,400 & 128 & 112 \\
com-orkut(\textbf{ORKT})       & 3,072,441 & 117,185,083 & 128 & 32 \\ 
% web-google      & 916,428   & 5,105,039 & 256 & 64 \\ 
% wiki-talk       & 2,394,385 & 5,021,410 & 256 & 96 \\ 
\specialrule{.1em}{.05em}{.05em} 
\end{tabular}}
\label{table: Evaluation Dataset}
\end{table}



% \vspace{-5pt}
\paragraph{Platforms \& Tools} 
\label{sect: Platforms and Metrics }
Our major evaluation platform is an NVIDIA DGX-A100 system with a Dual AMD Rome 7742 processor (128 cores total, 2.25 GHz base clock), 1TB host memory, and 8 NVIDIA Ampere A100 GPUs (each with 40 GB device memory) connected via NVSwitch. 
%
For comparative study in our modeling, we also leverage the NVIDIA DGX-1 platform with 4$\times$NVIDIA Tesla V100 GPUs connected via NVLINK.
%
This system comes with 600 GB/s GPU-to-GPU bi-directional bandwidth. 
%
We use CUDA (v11.3.1) and NVSHMEM (v2.0.3) for building our \Mname~design. 
For other NN operators (such as the dense linear, pooling, and softmax layer) outside the sparse neighbor aggregation, we incorporate cuBLAS~\cite{cublas} and cuDNN (v8.2)~\cite{cuDNN} for implementation. 
For kernel-level profiling, we use NVIDIA NSight Compute (v2021.1.1) to get the detailed performance metrics.
To measure the performance improvement, we calculate the averaged speedup of 100 rounds under the same setting. 

\subsection{Compared with UVM-based Design}
\label{sect: compared with UMD}
\begin{figure*}[h] \small
    \centering
    \subfloat{\includegraphics[width=0.5\textwidth]{imgs/gcn-A100.pdf}}
    \subfloat{\includegraphics[width=0.5\textwidth]{imgs/gin-A100.pdf} }
    % \vspace{-5pt}
    \caption{Performance comparison with UVM-based design on GCN and GIN on DGX-A100.}
    % \vspace{-15pt}
    \label{fig: Comparisons with Other GNN Frameworks.}
\end{figure*}
In this experiment, we comprehensively compare MGG with UVM-based design on the DGX-A100 platform. For UVM-based design, we put graph and embedding data in a global virtual memory space spanning across CPUs and GPUs without knowing its underlying layout and management strategy. 
% \vspace{2pt}
% \noindent \underline{\textbf{Type I Graphs:}} 
% The performance improvements against UMD are significantly higher for GCN (on average $10.16\times$).
% %The major reason is their different GNN computation patterns.
% The major reason is that UMD leverages the on-demand page-faulting strategy to fetch the node embedding that is not presented in the GPU devices. In the setting of small graphs, each memory page size would have lots of wasted payloads to be transferred, while the cost of migrating each memory page across the host and device memory could not be reduced even with the small payload. 
% % We also notice that with the increase of the number of G
% % \vspace{2pt}
% \noindent \underline{\textbf{Type II Graphs:}} \Mname~ achieves higher average performance (average $14.57\times$ speedup) improvements compared with UMD. There are two major reasons. First, Type II datasets are larger compared with Type I datasets, therefore, our effective workload partitioning would help to fully utilize the available GPU resources to improve the neighbor-aggregation parallelism and the memory access efficiency. However, UMD design could not enjoy such benefits due to a lack of effective workload partitioning and memory optimizations. Second, compared with the Type I graphs, the across-device communication is lower because the edge connections of the Type II graphs are condensed into a set of subgraphs. Cross-device communication is required for those subgraphs (called boundary subgraphs) that are split and placed into different GPU devices. In the case of UMD, those boundary subgraphs trigger more frequent memory page-faulting on different GPUs, leading to lots of low-efficient memory pages migration between GPU and CPU host. In contrast, \Mname~fetches the neighbor embedding at finer granularity instead of bulk-size memory pages. Moreover, the data communication in \Mname~would only requires the interconnections among GPUs via NVLink, which usually offer much higher data transferring efficiency compared with GPU-to-CPU connections via PCIe.
% \vspace{2pt}
% \noindent \underline{\textbf{Type III Graphs:}} 
% \textbf{Overall Speedup:} 
As shown in Figure~\ref{fig: Comparisons with Other GNN Frameworks.}, \Mname~achieves $7.14\times$ speedup on average compared to UVM-based design on GCN, respectively. It is mainly because \Mname~can fetch the non-local node embedding in fine-grained remote access via NVSHMEM. And such remote access can also fully overlap with the local aggregation computation to fully utilize the GPU resources.
% The speedup is also evident (average $3.04\times$ speedup) for GCN on graphs with a large number of nodes and edges with highly irregular connections. 
% Compared with the above two types of graphs, \Mname~'s speedup is relatively lower because, for those large graphs, more non-local data fetching from the unified are more likely to hit the same memory pages, considering that nodes of the real-world graphs tend to share neighbors. Therefore, each page-faulting becomes more cost-effective which can serve more vertices for aggregation computation. 
Comparing among different datasets, we can notice that for graphs with a larger number of edges our \Mname~would demonstrate more speedup under the same number of GPUs, such as \textit{ogbn-products}. This is because of our hierarchical workload management that can manage to create an appropriate size of workload to each warp meanwhile achieving sufficient computation parallelism among different warps. Comparing among the settings of different number of GPUs,  
we can observe an overall trend that with the increasing of the number of GPUs, \Mname~would achieve higher speedup. 
This is because of our effective usage of fine-grained data transfer in NVSHMEM. 
In contrast, UVM-based design leverages the page-faulting-based remote data access that is more coarse-grained (around 64 KB) in comparison with a single node embedding size (less than 5KB), which leads to higher overhead and lower effective bandwidth usage. 
This would also make UVM-based design challenging for GPU SM schedule to effectively dispatch instructions for the next available warps since most of the warps are waiting for the long-cycle page-faulting and page-migration routine to complete.

To gain more insights from the performance strength of \Mname, we further measure two performance-critical (computation and memory) GPU kernel metrics via Nightsight Compute profiling tool: \textit{Achieved Occupancy} and \textit{SM utilization}, 
%
where the former is the utilization of all available SMs on a single GPU while the latter is the ratio of the average active warps per active cycle to the maximum number of warps supported on an individual SM.
\Mname~achieves an average of 21.15\% better SM utilization and an average of $39.20\%$ higher achieved occupancy and compared with UVM-based design, which indicates that neighbor partitioning and workload interleaving can 1) effectively distribute workload to SMs as many as possible to improve the overall SM utilization of a GPU, and 2) overlap the execution of non-local memory access and local neighbor aggregation computation from different warps that are running on the same SMs to maximize the SM utilization.

% \vspace{-10pt}
\subsection{Compared with DGCL}
\label{sect: Compared with DGCL}
In this section, we compare our design with the state-of-the-art DGCL~\cite{cai2021dgcl} design. 
DGCL can be seen as a GNN-tailored NCCL design. And it mainly accelerates the neighbor embedding communication in the conventional multi-GPU GNN design, which has non-overlapped communication and aggregation phase. For this evaluation, we compile and build DGCL from their source file. And we select the 8-GPU settings (which is also the major experimental setting in their paper) on the DGX-A100 server and choose 1-layer GCN with 16 hidden dimensions for comparison.
\begin{table}[t] \small
\caption{Performance comparison with DGCL on 1-layer GCN on DGX-A100 with 8 GPUs. 
% Note that ``GP'' is for graph preprocessing, such as partitioning, ``GCN'' is for running 1-layer GCN.
}
\scalebox{0.9}{
\begin{tabular}{l| r r | r r}
\specialrule{.1em}{.05em}{.05em}
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Settings}}} & \multicolumn{2}{c|}{\textbf{Graph Preprocessing}} & \multicolumn{2}{c}{\textbf{GCN}} \\ 
\cline{2-5} 
\multicolumn{1}{c|}{} & \multicolumn{1}{r}{\textbf{DGCL(ms)}} & \textbf{MGG(ms)} & \multicolumn{1}{r}{\textbf{DGCL(ms)}} & \multicolumn{1}{r}{\textbf{MGG(ms)}} \\ \hline
\textbf{RDD} & 82.82$\times10^3$ & 0.59$\times10^3$ & 12.74 & 6.95 \\ 
\textbf{ENWIKI} & 401.56$\times10^3$ & 1.22$\times10^3$ & 153.06 & 12.79 \\ 
\textbf{PROD} & 134.35$\times10^3$ & 1.41$\times10^3$ & 35.64 & 3.35 \\ 
\textbf{PROT} & 59.15$\times10^3$ & 0.54$\times10^3$ & 11.36 & 2.66 \\ 
\textbf{ORKT} & 274.41$\times10^3$ & 1.60$\times10^3$ & 140.99 & 17.20 \\  \specialrule{.1em}{.05em}{.05em}
\end{tabular}}
\label{tbl: Performance Comparison with DGCL.}
\end{table}
% \begin{table}[h] \small
% \centering
% \vspace{-10pt}
% \caption{\todo{Performance comparison with DGCL on DGX-A100.}}
% \vspace{-5pt}
% \scalebox{0.88}{
% \begin{tabular}{|l|r|r|r|r|r|r|}
% \specialrule{.1em}{.05em}{.05em} \multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Settings}}} & \multicolumn{2}{c|}{\textbf{2-GPU}} & \multicolumn{2}{c|}{\textbf{4-GPU}} & \multicolumn{2}{c|}{\textbf{8-GPU}} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & DGCL & MGG & DGCL & MGG & DGCL & MGG \\ \hline
% RDD & 12.17 & 26.76 & 17.92 & 7.42 & 15.30 & 2.20 \\ 
% ENWIKI & 82.60 & 45.37 & 230.76 & 26.84 & 202.76 & 15.85 \\ 
% PROD & 50.37 & 40.04 & 64.00 & 25.24 & 52.87 & 15.79 \\ 
% PROT & 7.88 & 13.24 & 14.65 & 8.92 & 13.04 & 4.90 \\ 
% ORKT & 61.93 & 22.52 & 326.08 & 15.98 & 218.93 & 12.73 \\ \specialrule{.1em}{.05em}{.05em} 
% \end{tabular}}
% \label{tbl: Performance Comparison with DGCL.}
% \vspace{-5pt}
% \end{table}
As shown in Table~\ref{tbl: Performance Comparison with DGCL.}, we can see that \Mname~can outperform DGCL with an average $7.38\times$ speedup on GCN computation. This is mainly because \Mname~can 1) effectively overlaps the computation and the fine-grained remote memory access, whereas DGCL has to fully complete the communication for fetching the remote neighbor embeddings before its neighbor aggregation computation can start. And 2) our hierarchical workload management strategy can maximize the utilization of the available GPU resources, whereas DGCL relies on the fixed single-GPU kernel design that cannot adapt towards different GNN inputs. 
%
% Another observation from this comparison is that with the increase of the number of GPUs, our \Mname~design would demonstrate more advantages, while on the smaller number of GPUs DGCL would show more benefits. Because with more GPUs, the graph would likely be partitioned and placed to more different GPUs, Therefore, DGCL would spend more time fetching node neighbors that could reside on different GPUs leading to higher waiting latency for all inter-GPU communication to complete before the local aggregation can start. 

Another evident drawback of the DGCL is its extremely long data prepossessing time which limits its practical usage in many real-world settings. 
%
This is because DGCL requires applying their dedicated STSP algorithm to generate communication-optimized partitioning and device mapping for each input graph. This algorithm comes with high overhead, making their design scales poorly when the incoming graph is large. 
In contrast, the graph partition and workload balancing in our \Mname~design is lightweight, which is much faster (more than 100$\times$ speedup) compared with DGCL during the graph prepossessing phase. Such a huge improvement in the end-to-end execution time would also demonstrate the advantage of our \Mname~design to effectively adapt toward different inputs while achieving high performance.

\subsection{Optimization Analysis}
In this experiment, we will break down our optimization to demonstrate the effectiveness of our optimizations.
\paragraph{Workload Interleaving} 
To show the importance of workload interleaving, we compare \Mname~with the baseline design without the workload interleaving (i.e., non-local neighbor aggregation and local neighbor aggregation are mapped separately to the GPU warps. For example, in the case of 6 total aggregation workloads, the \{0,1,2\} will be local neighbor aggregation and the \{3,4,5\} will be non-local neighbor aggregation. While \Mname~will choose \{0,2,4\} warp for local aggregation and \{1,3,5\} warp for non-local aggregation). For all other configurations, we fix the size of the neighbor partition to 16 and the warp-per-block size to 2.
\begin{figure} [t] \small
    \centering
    % \vspace{-10pt}
    \includegraphics[width=\columnwidth, height=2.6cm]{imgs/opt_workload_interleave.pdf}
    \vspace{-10pt}
    \caption{Optimization analysis of Workload Interleaving.}
    % \vspace{-5pt}
    \label{fig: Workload Interleaving analysis}
\end{figure}
As shown in Figure~\ref{fig: Workload Interleaving analysis}, we can observe that \Mname~consistently outperforms the non-interleaved based with $1.38\times$ speedup. The major reason is that without interleaving the local/non-local workload, the workload distribution would be highly skewed, where the heavy/intensive non-local aggregation would be gathered on certain warps close to each other while the lightweight local aggregation would be gathered on some other warps close to each other. Therefore, it leads to inflexible low-efficient warp scheduling and higher latency.

\paragraph{Neighbor Partitioning}
To show the importance of workload interleaving, we compare \Mname~with the baseline design without applying the neighbor partitioning technique (\textit{i.e.}, each aggregation workload consists of all local/non-local neighbors). 
We apply the workload interleaving for both implementations and fix the warp-per-block size to 2 to eliminate the impact from other performance-related factors. And we evaluate on 2 and 4 GPUs settings. 
\begin{figure} [t] \small
    \centering
    \includegraphics[width=\columnwidth]{imgs/opt_neighbor_partition.pdf}
    \vspace{-10pt}
    \caption{Optimization analysis of Neighbor Partitioning.}
    % \vspace{-5pt}
    \label{fig: neighbor partitioning analysis}
\end{figure}
As shown in Figure~\ref{fig: neighbor partitioning analysis}, we can observe higher latency for designs without applying neighbor partitioning. Because the workload imbalance becomes more severe across different warps without neighbor partitioning. Especially for those graphs with lots of non-local aggregation workload, leading to limited computing parallelism and underutilization of the GPU resources (\textit{e.g.}, SMs). 

\paragraph{Shared Memory Optimization}
To show the benefits of our block-level shared memory design, we compare MGG with the baseline design without applying such GNN-tailored shared memory optimization. Specifically, we fix the hidden dimension to 16, the neighbor partition size to 2, the distance of workload interleaving to 2, and the warp-per-block size to 2.
As shown in Figure~\ref{fig: optimization analysis of shared memory design}, we can observe that tailoring the shared memory layout for GNN computation can bring the $3.25\times$ speedup on average. Whereas the design without such shared memory optimization can lead to much more atomic operations due to the final aggregation result synchronization and frequent high-overhead
global memory access.
\begin{figure} [t] \small
    \centering
    \includegraphics[width=\columnwidth,height=3cm]{imgs/shared_memory_optimization.pdf}
    \vspace{-10pt}
    \caption{Optimization analysis of shared memory design.}
    % \vspace{-5pt}
    \label{fig: optimization analysis of shared memory design}
\end{figure}

\subsection{Additional Studies}
\label{sect: Additional Studies}
% \paragraph{Distance of Workload Interleaving}
% \vspace{-5pt}
% We evaluate our design for workload interleaving (discussed in Section~\ref{sect: Workload Interleaving and Warp-based Mapping}). We consider several different settings of the interleaved distance ($\mathit{dist}$). Specifically, the $\mathit{dist}$=1 means that we will put one local aggregation and one remote aggregation on the same warp, such that the distance between two local/remote aggregations would be one aggregation workload. Note that here we refer to the aggregation workload as the aggregation on a neighbor partitioning, which may only involve the local memory access or all require remote access for fetching neighbors' embeddings. By configuring this variable, we can control how we overlap the local/remote workload such that the schedule of these workloads can maximize the GPU utilization.  As shown in Figure~\ref{fig: Interleaved distance.}, we can observe that the overall trend is that the initial increase of the interleaved distance would decrease the overall execution latency. Because at this phase, we are essentially adding more work on the same warp, which can help to improve the underutilized GPU SMs. Meanwhile, at this phase, we can more warps (each consists of local/remote aggregation workload) that could facilitate latency hiding for that high-cost remote access. In the second phase, however, when we further increase the interleaved distance, we are likely to observe a latency increase. This is because more aggregation workloads are gathered to a fewer number of warps such that the overall all computation parallelism would decrease. Meanwhile, the scheduling of each warp on SMs becomes inefficient due to more workload per warp.
% \begin{figure} [t] \small
%     \centering
%     \includegraphics[width=\columnwidth]{imgs/dist_type3.pdf}
%     \vspace{-10pt}
%     \caption{\todo{Normalized latency when interleaved distance ($\mathit{dist}$) grows. Note that the we use the setting at $dist=1$ as the base (=1) for normalization. (Change Dataset)}}
%     % \vspace{-5pt}
%     \label{fig: Interleaved distance.}
% \end{figure}

\paragraph{Size of Neighbor Partition}
% \vspace{-5pt}
\label{sect: Size of Neighbor Partition}
We further analyze the importance of configuring neighbor partition for workload management. In this study, we fix the size of interleaved distance to 1 and warp-per-block size to 2 and the hidden dimension of the GCN model is 16. And we use A100 GPUs connected via bi-directional NVlink. As shown in Figure~\ref{fig: neighbor partition size}, we can observe that the overall pattern for partition size on the design latency is similar to the above interleaved distance. The difference is that in adjusting the size of the neighbor partition, such performance impact on latency is relatively smaller compared with the interleaved distance. This is because partition size would change the workload at a finer granularity. By adding one more neighbor to each neighbor partition, we could increase the workload of the original warp by accommodating 2$\times \mathit{dist}$ for aggregation. In contrast, when by increasing the interleaved distance by one, we will introduce $2\times ps$ neighbors for aggregation. Considering that $dist$ << $ps$ in general, the latency performance would change less drastically when we adjust neighbor partition size.
\begin{figure} [t] \small
    \centering
    \includegraphics[width=\columnwidth]{imgs/neighbor_partition_analysis.pdf}
    \vspace{-5pt}
    \caption{Normalized latency when neighbor partition size ($ps$) grows. Note that the we use the setting at $ps=1$ as the base (=1) for normalization.}
    % \vspace{-5pt}
    \label{fig: neighbor partition size}
\end{figure}

\paragraph{Size of Hidden Dimensions} 
We also analyse the dimension size impact on our aggregation performance across different number of GPUs. In this study, we fix the size of interleaved distance to 1 and warp-per-block size to 2 and the hidden dimension of GCN model is 16. 
% Each pair of two A100 GPUs connected via bi-directional NVlink. 
\begin{figure} [t] \small
    \centering
    \includegraphics[width=\columnwidth]{imgs/hidden_dimension.pdf}
    \vspace{-5pt}
    \caption{Normalized latency when hidden dimension grows. Note that the we use the setting at $D=16$ as the base (=1) for normalization.}
    % \vspace{-5pt}
    \label{fig: hidden dimension}
\end{figure}
As shown in Figure~\ref{fig: hidden dimension}, we can see that with the increase of the hidden dimension, the overall latency increases as well. This is because of the pronounced overhead in remote access. In the relatively lower dimension, the latency increase is slower because the time spent on computation and the remote memory access has smaller differences which make the overlapping computation and memory access more effective. Under the high-dimensional cases, the overall execution time of each warp would largely be dominated by remote access.

\paragraph{Modeling and Optimization}
We further analyze the effectiveness of our lightweight analytical model for design space search. Specifically, two key parameters are studied, the size of neighbor partitioning, the interleave distance, and the warp-per-block.
%
Specifically, we consider three different settings: 
I: \textit{Reddit} GCN on 4$\times$A100 GPUs as the basic setting.
II: \textit{Reddit} GCN on 8$\times$A100 GPUs to demonstrate the adaptability towards the different number of GPUs.
III: \textit{Reddit} GCN on 4$\times$V100~\cite{tesla-v100} GPUs for demonstrate the adaptability towards different type of GPUs.
As shown in Figure~\ref{fig: Parameter Selection for Four Settings}, we decompose and show the searching results in two separate steps: 1) searching for the meta-optimal combination of partition size ($ps$) and interleaved distance ($dist$). In this step, we will initialize the value of $ps$, $dist$, and $wpb$ with all ones; and 2) searching for the optimal value of warp-per-block and based on the $ps$ and $dist$ determined in the last step. 
From the result, we can observe that our performance modeling and parameter selection strategy can pinpoint the low-latency design for the above three settings. And the overall searching process only requires less than 10 iterations to reach final optimal settings. 
Note that here we show latency results for all possible settings for comparison against our searched design points. Whereas in the actual cross-iteration optimization phase, we only traverse a small part of the whole design space.

\begin{figure} [t] \small
    \centering
    \includegraphics[width=\columnwidth]{imgs/analytical-modeling.pdf}
    \vspace{-5pt}
    \caption{Parameter selection for three settings. (a) is for setting I; (b) is for setting II; (c) is for setting III. Note that the figures on the left side show the runtime latency for different combination of $ps$ and $dist$, while figures on the right side figure show the latency for different combinations of $wpb$ and $dist$. black triangle is the meta-optimal combination for $ps$ and $dist$, while block star is the optimal for $wpb$ given the $dist$ and $ps$ in the last step.}
    % \vspace{-5pt}
    \label{fig: Parameter Selection for Four Settings}
\end{figure}
By comparing the final optimal runtime configuration setting and the initial configuration, we can see that modeling and cross-iteration optimization can decrease the execution time up to 70\%. 
In the end-to-end GNN training which usually consists of more than 100 iterations, such a saving in the later iterations would also be significant.
This demonstrates the effectiveness of our analytical modeling in assisting parameter selection to optimize the performance of GNN computation for the NVSHMEM-based multi-GPU platform.

==> 07_sensitive_analysis.tex <==
\begin{figure*}[h]
    % \newcommand{\fhe}{0.114}
    \newcommand{\fhe}{0.15}
        \includegraphics[height=\fhe\textwidth]{imgs/BV10x10_z=0.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BV10x10_z=1.pdf} 
        \includegraphics[height=\fhe\textwidth]{imgs/BV10x10_z=2.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BV10x10_z=3.pdf}
        \includegraphics[height=\fhe\textwidth]{imgs/BV10x10_z=4.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BV10x10_z=5.pdf} 
        % \includegraphics[height=\fhe\textwidth]{imgs/BV10x10_z=6.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BV10x10_z=7.pdf}  
        \\
        \includegraphics[height=\fhe\textwidth]{imgs/QFT4_z=0.pdf} \includegraphics[height=\fhe\textwidth]{imgs/QFT4_z=1.pdf} 
        \includegraphics[height=\fhe\textwidth]{imgs/QFT4_z=2.pdf} \includegraphics[height=\fhe\textwidth]{imgs/QFT4_z=3.pdf}
        \includegraphics[height=\fhe\textwidth]{imgs/QFT4_z=4.pdf} \includegraphics[height=\fhe\textwidth]{imgs/QFT4_z=5.pdf} 
        % \includegraphics[height=\fhe\textwidth]{imgs/BV10x10_z=6.pdf} \includegraphics[height=\fhe\textwidth]{imgs/BV10x10_z=7.pdf}  
        \\
        % \vspace{-5pt}
        \caption{Mapping of 100-qubit BV on multi layers of 10x10 grid. Blue and green dots represents vertices in the fusion graph, with blue dots being the complete vertices and green dots being the incomplete ones which needs to fuse with the next physical layer. Pink dots represents the auxiliary vertices to help form the structure.
        }
        \label{fig:case_study}
\end{figure*}


\subsection{Sensitivity Analysis}\label{sect:senstivity}
\paragraph{The effect of planarity:} The cycles contained by a measurement pattern can bring difficulties in finding an efficient implementation on the hardware because they often lead to crossing edges. We demonstrate the importance of planarity awareness as the key to overcome the difficulty. Fig~\ref{fig:opt2} compares the depth and `\# fusion' between four strategies: randomized fusion + regular mapping, planar fusion + regular mapping, randomized fusion + planar mapping, and planar fusion + planar mapping. In randomized fusion, we stick to the same pattern of synthesizing high degree nodes, but choose of random leg when assigning a vertex to the synthesized high-degree node, instead of an optimized one to maintain planarity. In regular mapping, we do the same heuristic search but without considering the planar order of the edges. It can be seen that...

\begin{figure}[h]
    \newcommand{\fhe}{0.159}
        \includegraphics[height=\fhe\textwidth]{imgs/oblation_planarity_on_depth.pdf} \hfill \includegraphics[height=\fhe\textwidth]{imgs/oblation_planarity_on_fusion_num.pdf} 
        \\
        \hphantom{} \hspace{58pt}(a) \hspace{105pt} (b) 
        % \vspace{-5pt}
        \caption{(a) The effect of planarity awareness during adaptive fusion on depth. (b) The effect of planarity awareness during adaptive fusion on `\# fusion'.
        }
        \label{fig:opt2}
\end{figure}


\paragraph{The effect of physical area:} The limited area (or width) of each physical layer can affect the depth and `\# fusion' because the boundaries put a constraint on the heuristic search. The dense layout enabled by our framework can implement the measurement patterns on a much smaller, while it also take advantage of the larger physical device when it is available. Fig.\ref{fig:area_effect} shows the depth and `\# fusion' when the size of the physical layers vary. It can be seen that when the area is very small, the depth and `\#fusion' are both large because the crowd space results in higher demand of auxiliary resource states. As the physical device scales up, the depth drops fast and eventually converges, while the `\# fusion' drops first, and then slightly increases as a tradeoff of the decreased depth.

\begin{figure}[h]
    \newcommand{\fhe}{0.159}
        \includegraphics[height=\fhe\textwidth]{imgs/area_effect_on_depth.pdf} \hfill \includegraphics[height=\fhe\textwidth]{imgs/area_effect_on_fusion_num.pdf} 
        \\
        \hphantom{} \hspace{58pt}(a) \hspace{105pt} (b) 
        % \vspace{-5pt}
        \caption{(a) Effect of the area of physical layers on depth. (b) Effect of the area of physical layers on `\# fusion'.
        }
        \label{fig:area_effect}
\end{figure}


% \begin{figure*}[tb]
% \newcommand{\fhe}{0.22}
%     \includegraphics[height=\fhe\textwidth]{imgs/oblation_planarity.pdf} \hfill \includegraphics[height=\fhe\textwidth]{imgs/oblation_planarity.pdf} \hfill \includegraphics[height=\fhe\textwidth]{imgs/oblation_planarity.pdf} \\
%     %\hspace{3pt}\hphantom{}\\
%     \hphantom{} \hspace{80pt}(a) \hspace{155pt} (b) \hspace{150pt} (c)
%     \caption{(a)-(c) The effects of the proposed optimizations. Bars with different colors denote different configurations of (\#qubit, \#node). %: (100,10), (200,20) and (300,30), respectively from left to right. 
%     For (a)(b), the y-axis is the ratio of \# remote communications. For (c), the y-axis is the ratio of program latency. (d)(e) The effects of \#\,qubit and \#\,node on the improv. factor of \frameworkName. The test program in (d)(e) is MCTR.}
%     \label{fig:opti}
% \end{figure*}





\paragraph{The effect of delay line limit:}
The performance of the implementation can also be affected by the limit of delay lines. When the delay line is short, qubits can be stored for only a short time, and needs to be refreshed from time to time. Fig.~\ref{fig:delay_effect} shows the effect of delay line limit on depth and `\# fusion'. It can be seen that increasing the limit of delay line leads to a smaller depth, and a slight improvement on `\# fusion' especially for... When the limit of delay lines is long enough, it no longer has significant effect and the performance would converge.


\begin{figure}[h]
    \newcommand{\fhe}{0.159}
        \includegraphics[height=\fhe\textwidth]{imgs/delay_effect_on_depth.pdf} \hfill \includegraphics[height=\fhe\textwidth]{imgs/delay_effect_on_fusion_num.pdf} 
        \\
        \hphantom{} \hspace{58pt}(a) \hspace{105pt} (b) 
        % \vspace{-5pt}
        \caption{(a) Effect of the limit of delay lines on depth. (b) Effect of the limit of delay lines on `\# fusion'.
        }
        \label{fig:delay_effect}
\end{figure}



% \paragraph{The effect of resource state structure:} 


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> old/05_workload_management.tex <==
\section{Hierarchical Workload Management}
\label{sect: Hierarchical Workload Management}
% In this section, we will detail our novel hierarchical workload management (HWM) from two major aspects, the categorization of the workload and the workload mapping on GPU programming primitives. Figure~\ref{fig: Workflow of Hierarchical Workload Management.} shows the overall workflow of our hierarchical workload management and we will provide details in the following sections.
% We will also discuss the design parameterization and performance-resource tradeoffs.

% \subsection{Multi-level Workload Balancing}
While the NVSHMEM offers efficient fine-grained GPU-initiated data communication, the irregular nature of GNN computation would still largely offset such benefits due to unbalanced workloads among different GPUs and computing units (GPU SMs).
To systematically improve the GPU performance in handling irregular GNN workloads on multi-GPU platforms, we propose a novel multi-level workload balancing technique based on three key metrics, \textit{the number of devices}, \textit{the types of workload}, and \textit{the number of neighbors}. Correspondingly, we introduce three following techniques.

\textbf{Edge-balanced Node Split:} This step is to balance the workload among different GPU devices. Specifically, we cut the whole graphs by selecting $n$ node-split points, where $n$ is the number of GPUs. 
%
To determine these points, we will first get the total number of edges of the whole graph and divide this number by the number of GPUs to get the approximate number of edges processed for each GPU. 
%
Then we leverage a \textit{range-constrained binary search} to determine the node-split points such that each GPU would process an almost equal number of edges.
%
% \begin{algorithm}[t]
% \SetAlgoLined
% \KwResult{Node-split Points ($S_0, S_i, ..., S_{n-1}$).}
% $\mathit{edgesPerGPU} = \mathit{numEdges/numGPUs}$\;
% $\mathit{iter} = 0$\;
% $last = 0$\;
%  \While{$\mathit{iter}$ < $\mathit{numGPUs} - 1$}{
%   $S_{iter}=$\;
%   $\mathbf{BinarySearch}(\mathit{last}+\mathit{edgesPerGPU}, [\mathit{last}, \mathit{numNodes - 1}])$ \;
%   $\mathit{last} = S_{iter}$ \;
%   $\mathit{iter++}$ \;
%  }
%  \caption{Edge-balanced Node Partitioning.}
% \end{algorithm}
% Algorithm~\ref{} describes the workflow of node-split algorithms, and
Here we give a short example for illustration. For an input graph with 10,000 nodes and 20,000 edges to be processed on 4 GPUs, 1) we will get the approximate number of edges for each GPUs as $\frac{20,000}{4} = 5,000$; 2) For 4 GPUs, we will have 3 node-split points, for the first node-split point, we will employ the binary search on the range between $[0, \#nodes - 1]$ for a nodes $S_0$ whose $\mathit{nodePtr}[S_0]$ is the minimum value that is right larger than $5,000$, where $\mathit{nodePtr}$ is the node pointer array for graph CSR. Then all nodes with IDs in the range $[0, S_0-1]$ will be assigned to the GPU-0 for processing. For determining the second and third node-split point, we would follow the similar procedure by repeating the above step 2, and we only need to limit the binary search space as $[S_{i-1}, \#nodes - 1]$ and maintain $S_i - S_{i-1} \geq 5000$, where $i\in \{1,2\}$.
\begin{figure} [t] \small
    \centering
    \includegraphics[width=0.98\linewidth]{imgs/graph_split.pdf}
    \vspace{-5pt}
    \caption{Multi-level Workload Balancing for Edge Split and Neighbor Partitioning. Note that ``LNP'' refers the local neighbor partitions; ``RNP'' refers the remote neighbor partitions.}
    \label{fig: Multi-level Workload Balancing.}
    % \vspace{-5pt}
\end{figure}

\textbf{Locality-aware Edge Split:} 
This step is to split the workload on each GPU based on its type after the completion of the above step. We categorize the sparse multi-GPU GNN computation into two categories. The first type of aggregation involves only the local memory on the current GPU device memory. The key character of processing these types of neighbors is the low-cost neighbor access, leading to shorter execution latency. The second type of aggregation triggers remote access for non-local neighbors, which features high latency and overhead. To delicately handle these two types of workloads, we group the same types of neighbors together (as illustrated in Figure~\ref{fig: Multi-level Workload Balancing.}(\circled{1})) to build two separate CSR for local and remote virtual graphs, respectively. The aggregation will be conducted on local and remote virtual graphs in parallel, and the partial aggregation result of the same node in both local and remote virtual graphs will be merged to generate the final output embedding.
% To this end, we employ a fine-grained node-level workload balancing technique to amortize such irregularity. As shown in Figure~\ref{fig: Workload Partitioning and Interleaving}, neighbors of different nodes are further partitioned by equal-sized partitions. 
% For example, the neighbors of Node-2 will span across three different partitions, where each partition will contain two neighbors. 
% Moreover, our design offers another layer of flexibility to allow users to set the size of the different partitions for local and remote access neighbors.

\textbf{Workload-aware Neighbor Split:} 
This step is to handle the workload imbalance among nodes within each virtual graph. Because different nodes would have a different number of neighbors from each other in virtual local and remote graphs, therefore, the aggregation workload among different nodes would also be largely diverse. This makes it challenging for massively parallel GPU devices to harvest the real performance gains due to the imbalance workload and diverged execution flow. Our neighbor partitioning strategy is to further divide the neighbors of each local/remote node into fixed-sized partitions such that the workload irregularity and imbalance across nodes can be amortized. As exemplified in Figure~\ref{fig: Multi-level Workload Balancing.}(\circled{2}), by limiting the size of each neighbor partitioning as 2, we can get a more balanced workload among different nodes in their local and remote virtual graph aggregation.
% The key design insight behind is that fetching neighbors from the remote address would lead to high cost in comparison with the locally-fetched neighbor, which can be easily fetched through a global memory address. Therefore, the workload for the equal-sized local neighbor partition and the remote neighbor partition would be largely different even though the size of neighbors is the same. To address such an issue, we make our design partition size locality-aware for local and remote access. For instance, we can set the local neighbor partition size as 4, while allowing the size for remote partition neighbor as 2 to accommodate the overhead for remote access.

==> old/06_cross_iteration_optimization.tex <==
\section{Modeling and Design Optimization}
\label{sect: Modeling and Design Optimization}
We will discuss performance modeling and design optimization to improve the runtime performance of \Mname.

\textbf{Analytical Modeling:}
The performance/resource analytical model of \Mname~has two variables: workload per warp ($\mathit{WPW}$) and shared memory usage per block ($\mathit{SMEM}$).
\begin{equation} \small
\label{equ: workload per threads}
\begin{split}
    \mathit{WPW} &= 2\cdot\mathit{ps}\cdot{D}\cdot\mathit{dist}, \\
    \mathit{SMEM} &=\mathit{ps}\cdot\mathit{wpb}\cdot{IntS} + 2\cdot\mathit{wpb}\cdot{D}\cdot\mathit{FloatS}
\end{split}
\end{equation}
where $\mathit{ps}$, $\mathit{wpb}$, and $D$ is the size of neighbor partition, warp per block, and embedding dimension, respectively; 
$\mathit{dist}$ is the interleaved distance of local/remote workloads ($\S$\ref{sect: Workload Interleaving and Warp-based Mapping});
$\mathit{Dim}$ is the node embedding dimension; 
$\mathit{IntS}$ and $\mathit{FloatS}$ are both 4 bytes on GPUs.

\textbf{Parameter Auto Selection:}
To determine the value of the $\mathit{ps}$, $\mathit{wpb}$, and $\mathit{dist}$, we follow two steps iteratively.
First, given an input graph, we compute its local/remote workload units based on the initially selected $\mathit{ps}$ as shown in
\begin{equation} \small
\label{equ: numWarps}
\begin{split}
    \mathit{numWarps} &= \frac{\max\{local, remote\}}{dist}
\end{split}
\end{equation}
then we compute the total number blocks and the estimated block per SMs by using
\begin{equation} \small
\label{equ: numBlocks}
\begin{split}
    \mathit{numBlocks} &= \frac{\mathit{numWarps}}{\mathit{wpb}}, \\
    \mathit{blockPerSMs} &= \frac{\mathit{numBlocks}}{\mathit{numSMs}}
\end{split}
\end{equation}

Second, based on our micro-benchmarking on diverse datasets, we define our parameter search space and constraints: 
%
1) $ps\in[1\dots32]$ to balance the computation parallelism and synchronization overhead;
%
2) $\mathit{dist}\in[1\dots16]$ to effectively overlap the computation and remote memory access;
%
3) $\mathit{wpb}\in [1\dots16]$ to maintain SM warp scheduling flexibility for high occupancy and throughput; 
%
4) $SMEM\leq{c}$, where $c$ is the hardware constraints related to the GPU micro-architecture~\cite{GPU-micro-arch}. For example, NVIDIA A100 GPU has the maximum of 164KB shared memory per SM.
We further demonstrate the effectiveness of our analytical model in Section~\ref{sect: Additional Studies} of our evaluation.

\subsection{Cross Iteration Optimization}
We start with all ones parameters for $\mathit{ps}$, $\mathit{dist}$, and $\mathit{dist}$ at the initial iteration. And then we optimize one parameter in each of the following iterations. 
First, we start by increasing the $\mathit{ps}$ to maximize the warp utilization. When further increasing the $ps$ would also increase the latency, we would stop the search on $\mathit{ps}$ and switch to $dist$.
%
Second, we apply the similar strategy to locate the value for $\mathit{dist}$ for locating the point that can maximize the overlap of local computation and remote access.
%
Third, we increase $\mathit{wbp}$ to maximize the utilization of the entire SM. If any increase of $\mathit{wpb}$ would increase the latency, we can know that there may be too large block or too heavy workload on individual warps that lower SM warp scheduling efficiency or computation parallelism. 
We would ``retreat'' (\textit{i.e.}, decrease) $\mathit{ps}$ to its second highest value and restart the increasing of $\mathit{wpb}$.
%
This optimization algorithm will stop when any decrease of $\mathit{ps}$ and increase of $\mathit{wpb}$ would lead to higher latency than the top-3 lowest latency.
%
Latency for each iteration during the optimization will be recorded by a configuration lookup table, after the optimization phase, the configuration with the lowest latency will be recovered for all the following iterations. 
%
Our experimental study shows that optimization phase would take no more than 10 iterations, which is low in overhead compared with the hundreds of iterations of the GNN training.

==> old/06_memory_optimization.tex <==
% \section{Multi-Layer Memory Optimization}
\section{NVSHMEM-based Kernel}
\label{sect: NVSHMEM-based Kernel}
In this section, we will detail our NVSHMEM-based kernel design, including the hybrid GNN data placement for leveraging different types of global memory, warp-based mapping and workload interleaving for improving GPU execution efficiency, and shared memory layout and pipeline loading optimization. 
\begin{figure} [t] \small
    \centering
    \includegraphics[width=\linewidth]{imgs/nvshmem_pattern.pdf}
    \caption{NVSHMEM Design and Communication Pattern. Note that ``NE-i'' is the node embedding partition stored on the i-th GPU. ``GP-i'' is the graph edges partition processed by the i-th GPU. ``GPU-i [lb, ub]'' is the node-id range [lowerbound, upperbound] of the node embeddings on the i-th GPU.}
    \label{fig: NVSHMEM Design and Communication Pattern.}
\end{figure}

\subsection{Hybrid GNN Data Placement} 
For managing the data of GNNs, we enforce two types of strategies, as exemplified in the left side of Figure~\ref{fig: NVSHMEM Design and Communication Pattern.}. 
For node embeddings (\textbf{NE}) that are too large to fit into a single GPU memory. we leverage NVSHMEM ``shared'' global memory to maintain the whole graph embeddings, which essentially distributes node embeddings to different GPUs' global memory addresses. 
We first partition the input graphs into $n$ partitions (where $n$ is the number of GPUs) and each partition is placed on one GPU's ``shared'' global memory space, created by \texttt{nvshmem\_malloc} API. 
Note that compared with the traditional \texttt{cudaMalloc} that allocates the ``private'' global memory address dedicated for the current GPU, global memory space allocated by \texttt{nvshmem\_malloc} can be accessed all GPUs involved in the current NVSHMEM context via the GPU id and the memory address offset.

On the other hand, for storing partitioned graph structure (\textbf{GP}) data (\textit{e.g.}, the edge list), we use \texttt{cudaMalloc} to allocate the ``private'' global memory space that is only visible to current GPU. Considering that NVSHMEM ``shared'' global memory offset would start from zero for each GPU, the original global node id in the edge list should be converted to a GPU-local memory index for accessing the correct neighbor embeddings according to the node-id range on different GPUs, as illustrated in the right side of Figure~\ref{fig: NVSHMEM Design and Communication Pattern.}.

\subsection{Warp-based Mapping and Workload Interleaving}
\label{sect: Workload Interleaving and Warp-based Mapping}
In collaborating with our hierarchical workload management, we will explore how to map such logically balanced workload to the underlying programmable GPU computing units (threads/warps/threadblocks) for better overall performance.
Firstly, we choose the warp as the basic working unit for handling the workload of each partition. 
Because a warp of threads can effectively collaborate to work on the aggregation across different node embedding dimensions. Whereas using a single or a number of threads (less than a warp) would hardly explore the computation parallelism and would cause warp-level divergence. 
Besides, NVSHMEM remote access imitated by a warp would merge the requests into one remote memory transaction to reduce the overhead.
The method we choose for remote access is GET, which is initiated by the GPU kernel that demands certain neighbor embeddings for aggregation. Compared with PUT method, using GET will simplify the overall design. Because using PUT, we have to employ a complex receiver-side synchronization mechanism to consistently check the local memory buffer to make sure that the required node embedding arrives before the its aggregation begins. This would also lead to extract computation cost that would degrade the overall GNN computation performance.
% To fetch the embeddings on the remote GPU, we leverage the \texttt{nvshmem\_float\_get\_warp} API which is tailored for warp-based execution. It is a synchronized function call that will be returned until all data has been received at the target local memory address, which could be the private global memory address or the block-level shared memory. For faster and low-overhead access, we choose the shared memory and we detail its design in the next section.

In the second step, we will decide how we map each workload to the underlying warp.
The most straightforward way is to continuously map the neighbor partitions from the local and remote workload list to GPU warps with continuous IDs, as shown in Figure~\ref{fig: Workload Interleaving and Warp-based Mapping.}.
However, this strategy would easily suffer from the workload imbalance of GPU SMs. Because warps with continuous ids are more likely to be placed in the same thread block, which is assigned to one SMs for processing. Therefore, SMs assigned with warps for handling remote neighbor partitions would much longer latency than SMs assigned with warps for processing local neighbor partitions. Such a workload imbalance would lead to an execution critical path with poor GPU utilization and execution performance. 
\begin{figure} [t] \small
    \centering
    \includegraphics[width=\linewidth]{imgs/workload_interleaving.pdf}
    % \vspace{-5pt}
    \caption{Workload Interleaving and Warp-based Mapping. Note that ``LNP'' refers the local neighbor partitions; ``RNP'' refers the remote neighbor partitions.}
    \label{fig: Workload Interleaving and Warp-based Mapping.}
    % \vspace{-5pt}
\end{figure}

To this end, we introduce our novel workload interleaving strategy to balance the workload among SMs on GPUs. 
Each warp of threads running on GPU would handle one or more pairs of local/remote workload partitions. 
We introduce a new metric -- \textit{interleaving distance} to more precisely adjust the way of mixing different types of workloads. We give the examples with the interleaving distance equal 1 and 2 in Figure~\ref{fig: Workload Interleaving and Warp-based Mapping.} for illustration,
% When we have two pairs of local and remote workload, the interleave distance would be two. 
The major design insight is that by mixing different types (local/remote) of workload together, we can achieve better GPU utilization. Because when one warp is blocked for high-cost remote access, other warps that are working on local computation can still be served by the SMs warp scheduler for filling up these idle GPU cycles. 
Such a design would also improve the design flexibility: 
given an input graph with a selected neighbor partition size, we can adjust the interleaving distance and the workload per warp such that the waiting cycles of the remote access can be amortized by the computation cycles of the neighbor aggregation. Therefore, each warp can be fully utilized while the overall design can achieve sufficient parallelism.
% For different size of local and remote neighbor partition, such a interleave distance would be different. 
% The selection of its value would be aimed to maximize the SM utilization and minimize the runtime latency, 
We discuss such parameter selection in Section~\ref{sect: Modeling and Design Optimization}. 


% Whereas all other solutions require the termination of the current computing kernel and switching the execution to the host program 
% for a host-side inter-GPU data communication, resulting in additional overhead and low execution performance. The basic design pattern of NVSHMEM is illustrated in Figure~\ref{fig: NVSHMEM Design and Communication Pattern.}, where a part of the memory from each GPU is ``gathered'' to build an NVSHMEM memory space that can be accessed by all GPUs. And there is also private device-memory space that can only be accessed by individual GPUs. Note that both the private and NVSHMEM memory can be seen as two different types of global memory in conventional GPU computing.

% \begin{figure}[t] \small
% \vspace{-5pt}
% \begin{lstlisting}[caption=CUDA NVSHMEM APIs.,style=tt1,label={code: wmma API interface.}]
% // Initialize the NVSHMEM context.
% nvshmem_init();
% // Get the current PE ID.
% int mype_node = nvshmem_team_my_pe(NVSHMEMX_TEAM_NODE);
% // Set the GPU based on the PE ID.
% cudaSetDevice(mype_node);

% // Define NVSHMEM memory visible for all PEs.
% d_shared_mem = (void*) nvshmem_malloc (num_bytes); 

% // NVSHMEM APIs for fetching data from remote PEs.
% __device__ nvshmem_TYPE_get(void *dest, const void *source, size_t  nelems, int pe);
% __device__ nvshmem_TYPE_get_warp(void *dest, const void *source, size_t nelems, int pe);
% __device__ nvshmem_TYPE_get_block(void *dest, const void *source, size_t  nelems, int pe);

% // Sync all PEs within current NVSHMEM context.
% nvshmem_barrier_all();
% // Release NVSHMEM objects.
% nvshmem_free(d_shared_mem);
% // Terminate the current NVSHMEM context.
% nvshmem_finalize();
% \end{lstlisting} 
% % \vspace{-10pt}
% \end{figure}
% NVSHMEM offers several APIs to support inter-GPU communication. As shown in Listing~\ref{code: wmma API interface.}, to enable the multi-GPU computing context, we start with the \texttt{nvshmem\_init} followed by get the current GPU (PE) ID and set the target GPU device (Line 1 to Line 6). 
% Note that launching a NVSHMEM program is similar to running a MPI program, where numbers of concurrent host threads are created for managing each GPU device.
% %
% We can create the shared memory by using \texttt{nvshmem\_malloc} that is visible to all engaged PEs. 
% %
% One of the major type of operation in the sparse GNN computation is the kernel-level API \texttt{nvshmem\_TYPE\_get}, where the \texttt{TYPE} can be replaced with \texttt{float}, \texttt{int}, and etc. 
% Depending on the caller's type, there are several variants of such API, where can either call from a single thread or via the collaboration from a warp and a block of threads.
% %
% To wait for all participated PEs to finish, we will use \texttt{nvshmem\_barrier\_all}. 
% Finally, we can release the allocated shared NVSHMEM memory via \texttt{nvshmem\_free} and clean up the context of NVSHMEM via \texttt{nvshmem\_finalize}.



% To exploit the performance benefits of MGG hierarchical workload, we introduce GNN-specialized memory optimizations, 
% including \textit{Locality-aware Node2Device mapping} and \textit{Block-level Shared Memory Orchestration} to systematically improve the memory performance at different levels of granularity.

% \subsection{Adjacency-aware Node Remapping} 
% \label{sect: Node Renumbering}
% To explore the performance benefits of neighbor locality in GNN sparse computation, we incorporate a lightweight node remapping technique by reordering node IDs to improve the temporal/spatial locality during GNN aggregation without compromising output correctness.
% The major insight behind this is that nodes with the same neighbor nodes processed on the same device can bring the memory performance benefits at the GPU device level from several aspects. 
% First, at the GPU device level, putting the nodes and their common neighbors on the same GPU device can largely reduce the remote memory access overhead. 
% Second, at the GPU kernel level, an adjacent neighbor with more number of the shared neighbors would likely benefit from the L1 cache on the GPU block. 
% %
% For handling such a node mapping in a lightweight manner, we incorporate the BFS-based Reverse Cuthill-McKee (RCM)~\cite{RCM-Algorithm}) in a fully parallel computing setting. RCM algorithm has also been proved to outperform other graph clustering approaches for node id remapping such as~\cite{METIS, boldi2011layered, raghavan2007near, karantasis2014parallelization, RCM-Algorithm}, including Community-based methods, such as METIS~\cite{METIS}.
% %
% As shown in Algorithm~\ref{algo: graph-bandwidth reduction.}, it first selects the min-degree vertex from the graph and adds this vertex to a visited list. It will traverse all vertices of the graph by 1) getting the all unvisited neighbors of all nodes in the current frontier, 2) sorting these neighbors by their degrees (note that all edges are undirected), and 3) adding these ordered neighbors to a globally ordered list of the graph.
% %
% Note that this step is only need to be conducted once at the beginning of the GNN computation. We will further quantitatively discuss its optimization benefits and the runtime overhead in our evaluation section~\ref{}.
\begin{figure}[t] \small
\vspace{-10pt}
\begin{lstlisting}[caption=Shared Memory Design.,label={code: shared memory design.}, style=tt3]
__global__ MGG_kernel (param1, param2, ...)
{
    // Get the global thread-id
    int tid =  blockIdx.x * blockDim.x + threadIdx.x;  
    // Get the global warp-id
    int warpId = tid / WARP_SIZE; 
    // Get the block-level warp-id
    int block_warpId = threadIdx.x / WARP_SIZE;
    // Get the warp-level thread-id, namely laneid.
    int laneid = threadIdx.x % WARP_SIZE;                
    
    // Define the dynamic shared memory.
    extern __shared__ int part_meta[];                      
    // Starting address for node neighbors IDs.
    int *partial_ids = part_meta;
    // Starting address for partial aggregation result.
    float *partial_results = (float*)&part_meta[partSize*warpPerBlock];     
    // Starting address for remotely-fetched embeddings.
    float *tmp_local = (float*)&partial_results[partSize*warpPerBlock*dim];   
    
    // Calculate the offset for each warp.
    int ids_offset = warpId*partSize;
    int partial_offset = warpId*partSize*dim;
    int tmp_offset = warpId*partSize*dim;
    
    // Warp-level aggregation computation ...
}

// ----------launching the kernel on HOST-------------
__global__ MGG_host (param1, param2, ...)
{
    // Calculate the kernel configuration.
    int n_parts = max(lc_parts, re_parts);
    int block = warpPerBlock * WARP_SIZE;
    int grid = (n_parts * WARP_SIZE + block  - 1) / block; 
    int shared_memory = partSize*warpPerBlock*sizeof(int) + 2*partSize*warpPerBlock*dim*sizeof(float); 
    
    // Launch the kernel.
    MGG_kernel <<<grid, block, shared_memory>>> (param1, param2, ...);
    // other following operations ...
}
\end{lstlisting}
\vspace{-10pt}
\end{figure}

\subsection{Specialized Memory Design and Optimization} 
\hspace{5pt} \textbf{Shared memory layout:} Based on our MGG's warp-based workload design, we further propose a block-level shared memory orchestration to maximize the performance gains. The key insight for such a design is several folds. 
First, our neighbor partition-based workload will generate the intermediate results that can be cached at the high-speed shared memory for reducing the frequent low-speed global memory access.
Second, NVSHMEM-based remote data access demands a local scratch-pad memory for holding the remote data for local operation. There are several steps for us to utilize the block-level shared memory.
For the local neighbor aggregation, we reserve a shared memory space ($4\times \mathit{Dim}$ bytes for floating-point embeddings) for the target node of each neighbor partition, such that the threads from a warp can cache the intermediate results of reduction in shared memory.
For the remote neighbor aggregation, the shared memory space is doubled ($2\times \mathit{nps} \times \mathit{D}$). Because we need the first half ($nps \times D$) for caching the partial aggregation results of each warp but also the second half ($\mathit{nps}\times \mathit{D}$) for the remotely accessed neighbor embeddings. The detailed customization procedure is described in Listing~\ref{code: shared memory design.}. For each MGG kernel design, we will first identify the warp-level information, such as the warp ids (as illustrated from Line 3 to Line 10). Then within each thread block, we define the customized shared memory layout by splitting the contiguous shared memory address into three different parts for neighbor ids (\texttt{partial\_ids}), partial aggregation results (\texttt{partial\_results}), and the remotely-fetched node embeddings (\texttt{tmp\_local}), at Line 12 to 19. 
%
We also need to calculate the relative address for each warp within each part of shared memory space, at Line 21 to 24. 
%
Note that the we use the dynamic shared memory design in MGG for better design flexibility considering that parameters (\textit{e.g.}, the \texttt{partSize}, \texttt{warpPerBlock}, and \texttt{dim} can only be determined at runtime). We will first calculate the size of shared memory (Line 36) and then pass it as one of the kernel launching parameters (Line 39) at the runtime. 


\textbf{Pipelined Memory Operation:}
In the above section~\ref{sect: Workload Interleaving and Warp-based Mapping}, we have discussed about the assigning local (LNP) and remote (RNP) neighbor aggregation workload to warps, such that different warps can overlap their computation and communication to fully saturate the active cycles of the GPU SM scheduler. However, only exploiting the inter-warp communication-computation is not enough to maximize the utilization of GPU resources, we further explore the overlapping of the computation and communication at the intra-warp level by carefully scheduling the memory operations. 
\begin{figure} [t] \small
    \centering
    \includegraphics[width=\linewidth]{imgs/memory-overlaping.pdf}
    % \vspace{-5pt}
    \caption{Pipeling memory operations for overlapping computation and communication of an individual warp.}
    \label{fig: pipeline memory operations}
    % \vspace{-5pt}
\end{figure}
As shown in Figure~\ref{fig: pipeline memory operations}(a) for the case with two LNP and two RNP, the basic design by using the synchronized remote access design can just sequentially process the LNP and RNP, where the long latency remote access can happen only after the completion of its preceding LNP. This could lead to longer GPU stall for memory operations and low GPU SM utilization. To amortize the cost of remote access for each warp, we introduce the asynchronized remote memory operations, as illustrated in Figure~\ref{fig: pipeline memory operations}(b). This improved design consists of three major steps. First, we can simultaneously launch the local memory access while initializing the remote memory access for fetching the node embedding (\circled{1}), therefore, the time for remote access can be amortized by the processing of LNP. Second, once the remote access finished, the current warp will start to aggregation on the remotely-fetched node embedding data (\circled{2}). The last step will start the new iteration of the previous two steps, which will process a new pair of LNP and RNP.
% \todo{We further introduce our shared memory optimizations for latency hiding on the latest Ampere GPU. The key of our design is to overlap the operations of the high-overhead remote access with the local low-cost aggregation computation. Instead of waiting for all the previous aggregation to complete, our design based on the asynchronized memory copying can issue another remote access request for the following neighbor embeddings.}
% \todo{Another benefit of our design is the register-bypassing, in the previous design, memory access from the ``shared'' global memory has to go through the L1 cache and registers before it can reach the shared memory, which introducing additional overhead. In contrast, our design can directly skip the registers by directly transferring data from the L1 cache to shared memory, with less register pressure and better occupancy.}

==> old/ext_01_motivation.tex <==
\section{Motivation}
Over the most recent years, graph-based deep learning attracts lots of attentions from the research and industry. Among these techniques, graph neural networks (GNN) get highlighted most due to its success in many graph-based deep learning tasks (\textit{e.g.,} node embedding generation for node classification~\cite{kaspar2010graph, gibert2012graph, duran2017learning} and link prediction~\cite{chen2005link, kunegis2009learning, tylenda2009towards}).  
\begin{figure*} [h] \small
    \centering
    \includegraphics[width=0.9\textwidth]{imgs/overall.pdf}
    \caption{Overview of \Mname.}
    \label{fig: Overview}
    % \vspace{-5pt}
\end{figure*}
GNN computation on large graphs with millions of nodes and edges is a huge challenge because of the high memory consumption and computation demands. 
{One type of efforts~\cite{chen2018fastgcn,clusterGCN,Zeng2020GraphSAINT}
adapt the existing single-GPU GNN algorithm for multi-GPU platforms by leveraging neighbor sampling and data-parallel mini-batch processing.} 
However, research~\cite{sysMLROC, chen2018fastgcn} shows that such algorithmic modifications would compromise the accuracy of GNN models compared with full-batch GNNs that consider all neighbors. 
%
The second type of efforts~\cite{sysMLROC, ma2019neugraph, cai2021dgcl} keep the GNN algorithm intact (using full-batch GNN) and tailor optimizations (\textit{e.g.}, communication) of multi-GPU systems for GNN-specific operations (\textit{e.g.}, scatter and gather). 
%
This is also the most preferred solution, which can achieve better performance without hurting the GNN model predictability. However, this type of solutions is still preliminary and could suffer from 1) the imbalance workload resulting in poorly utilization of available hardware resources; 2) the decoupled communication and computation leading to severe communication bottleneck and inefficient execution; 3) the non-configurable design causing limited input adaptability.
% For instance, ROC~\cite{sysMLROC} and NeuGraph~\cite{ma2019neugraph}  mainly count on the large CPU main memory for handling the large GNN input graphs that cannot fit into a single GPU device memory. Their design can be summarized as a typical unified memory design where the computation-related data of GNNs is fetched from host memory to GPU memory on demand before the corresponding computation is carried on GPUs. DGCL~\cite{cai2021dgcl} is the state-of-the-art multi-GPU GNN design that relies on different GPU device memory to store a subset of graph node embeddings. DGCL incorporates a highly optimized communication library GCCL as a drop-in replacement of NCCL~\cite{nccl} for efficient remote embedding access before the neighbor aggregation in each layer of GNNs.
% However, the performance of GNN is unsatisfiable in comparison with conventional deep neural networks (DNNs), such as convolutional neural networks, on the modern hardware platforms, such as GPUs. 
% %
% This is because the computation of the DNNs is largely \textit{data independent}, which leads to low ratio of communication and computation. 
% %
% The only process demands the multi-device collaboration is at the end of each forward propagation during the training, where the loss from each GPU device is collectively gathered and reduced, and the backward gradient is collectively scattered. 
% %
% In contrast, the computation of the GNN is highly \textit{data dependent}. 
% % The major bottleneck of GNN is at the sparse aggregation process, where each vertex has to gather information from all of its neighbor nodes. 
% Considering the modern GNN models usually comes with high dimensional node embedding feature, this aggregation step would trigger excessive data movements. In the setting of multi-GPU, where node embedding cannot fit into one GPU devices, the access overhead for fetching the remote node embedding would be non-trivial (100$\times$ higher latency when using PCIe 3.0 in comparison with the global memory access on a single GPU). 
% %
% % Some previous efforts~\cite{clusterGCN,Zeng2020GraphSAINT} try to circumvent such high overhead remote access by changing the algorithm design, such as partitioning the large input graph into a set of small subgraphs and only do subgraph aggregation. However, the research evidence~\cite{sysMLROC} shows that such modifications would hurt the accuracy of GNN models. 

% To tackle the challenge of multi-GPU computation, previous work can be classified into two categories. 
% The first type~\cite{wang2016gunrock, ma2019neugraph, sysMLROC} leverages the host memory for maintaining all node embedding and communicates GPU device memory on demand.
% The second type~\cite{pyG, wang2019dgl}, maintain the node embedding data on GPU devices and transfer the node embedding data among GPUs directly.

==> old/ext_02_limitation_of_SOTA.tex <==
\section{Limitations of the State of the Art}

\paragraph{NCCL-based Design}
To support the multi-GPU deep learning, NVIDIA has announced its high-performance communication library -- NCCL~\cite{nccl} for handling the inter-GPU communication. 
%
Compared with MPI~\cite{cudaMPI}, NCCL demonstrates its strength in collective operations (\textit{e.g.}, gather, reduce, and scatter) for DNN training.
% Such an improvement is most significant in the context of low-communication settings, such as training deep neural networks via data parallelism, where each batch of input data (such as a set of images) is well partitioned and organized to be feed into the neural network models, which have been duplicated on different GPU devices. The communication only happens at 1) all-reduce for forwarding propagation loss reduction; 2) all-scatter for output layer backward propagation. 
However, in the communication-intensive GNNs, NCCL could hardly demonstrate its strength. There are several reasons. 
%
First, NCCL's major APIs are mainly optimized for inter-GPU communication based on scalar numbers (\textit{e.g.}, loss). Whereas GNNs require communication support for vector-like node embeddings.
%
Second, NCCL is designed for regular communication patterns, which can hardly find their place in irregular sparse GNN computation. For instance, one of the well-known NCCL's collective operations all-reduce follows the ring-based reduction across GPUs. While in GNNs, the remote access among different GPUs largely relies on irregular point-to-point data transferring without following any existing communication patterns. 
%
Third, NCCL can only be used outside the GPU kernel by calling from the host CPU. Therefore, it suffers low GPU utilization because of the non-overlapped computation and memory operations in GNN computations.
%
% To show the performance of NCCL in multi-GPU GNN computation, we build a basic NCCL GNNs, where each GPU maintain a fixed-size subset of node embeddings in its device memory, and it will forward its current node embedding subset to the next GPU (a ring-based node embedding forwarding) once it finishes its aggregation.
% As we can see from Figure~\ref{fig: NCCL profiling for 1 GCN layer.}, the data transferring via NCCL could take more than $5\times$ of the sparse computation at a single graph convolutional layer. This is mainly because of NCCL's inefficiency in transferring vector-based node embeddings and the huge bandwidth gap between the high-speed global memory (around 1TB/s) and inter-GPU connections, like NVLink (around 100GB/s).
% Meanwhile, this part of communication cannot be overlapped with the sparse computation, leading to higher overall execution latency.
%
While the recent work DGCL~\cite{cai2021dgcl} improves NCCL by introducing GNN-tailored $\mathit{Allgather}$ function, we still find several of its drawbacks: 1) it still could not overlap the computation and remote memory access to amortize the communication costs; 2) it has high latency costs for graph partitioning and communication schedule generation (400$\times$ \textit{w.r.t.} per-epoch running time) that limits it practical usability in real-world settings; 3) it has to cache all of the remote neighbor embeddings before the local aggregation, leading to non-trivial extra memory overhead. 
% With the recent surge of the multi-GPU deep learning, NVIDIA has announced its own high-performance communication library -- NCCL~\cite{nccl} for handling the inter-GPU communication. 
% %
% Despite such a great success in the conventional deep neural networks, in the communication-intensive sparse graph neural networks, NCCL could hardly demonstrate its strength. There are several reasons. 
% %
% First, NCCL's major APIs are optimized for inter-GPU communication based on scalar numbers (\textit{e.g.}, loss). In contrast, in the GNNs, the communication among GPUs require the support and optimizations for vector-like node embeddings.
% %
% Second, NCCL is designed for regular communication pattern, which can hardly find its place in irregular sparse GNN computation. For instance, one of well-known NCCL's collective operations all-reduce follows the tree-like reduction among different GPUs, while in GNNs, the remote access among different GPUs largely relies on point-to-point data transferring instead of following any existing distributed communication algorithm. 
% %
% Third, NCCL can only be used outside GPU kernel by calling from the host CPU. Therefore, it suffers low GPU utilization because of the non-overlapped computation and memory operations in the GNN computation settings.


\paragraph{Mixed Compute-Communication Design}
Another type of work would rely on the unified virtual memory (UVM)~\cite{unifiedMemory} to build a layer of global memory across different devices. UVM maintains a global ``virtual'' view of single address space among different devices (CPUs and GPUs) with the automatic memory page migration during the runtime, which is transparent to the programmer.
When the GPU kernel wants to access the data that are not presented on GPU-device memory, a GPU-side memory page fault would happen and a host-to-GPU page migration would be triggered to fetch the corresponding data from remote memory to local device memory. 
%
Even though UVM offers the easiest way for handling GNN inputs that cannot be fit into a single GPU device, the performance of such a design could hardly satisfiable. There are several major challenges. First, GNN computation is highly irregular in-memory access. Therefore, using the unified memory would trigger lots of GPU-side page-fault for fetching the non-local data in fine granularity. The page size is fixed (around 64KB) while the node embedding size (less than 4KB) of an individual neighbor node is relatively small. Thus, each high-cost page-faulting and migration operation is largely under-utilized. 
%
Second, UVM mainly has to count on the slow CPU processor and low-bandwidth PCIe connection for communication, which could easily stall the high-performance GPU.

==> old/ext_03_key_insight.tex <==
\section{Key Insights}
% \paragraph{Customizing the compute-friendly cross-device data layout.}
% The computation of GNNs demands the frequent irregular memory access for neighbor embedding features. In the setting of multi-GPU, such a memory access overhead would be escalated due to the fact that inter-GPU data communication is intrinsically high-cost in comparison with the intr-GPU data access. Therefore, a carefully maintained ``global view'' of the graph structural and embedding data among multiple inter-connected GPUs would be essential for overall GNN computing performance. The design should consider the propertities of GNNs and the topology of the GPU hardware-level inter-connections.

\paragraph{Balancing workload at different levels of granularities}
Existing mutli-GPU GNN frameworks~\cite{cai2021dgcl, ma2019neugraph} rely on METIS~\cite{METIS} or the basic 2D edge partitioning~\cite{ma2019neugraph}. The former splits the input graph by nodes for a more balanced node size within each partition, while the latter divides the input graph by edges, based on the source and destination node IDs of each edge. However, neither of these strategies is well-suited for GNNs. While METIS can maintain balanced node size among different partitions, it could not guarantee balanced neighbor size for aggregation workload. While 2D edge partitioning would guarantee workload balance among different GPUs, it would distribute edges of the same nodes to different GPUs, leading to non-trivial costs for synchronization of final results. 
Therefore, we need to comprehensively balance the workload among different GPU devices and the different processing units on the same GPU.

\paragraph{Overlapping the communication and computation} 
Existing frameworks~\cite{cai2021dgcl, sysMLROC, ma2019neugraph} are built with different kernels for managing computation and communication separately. For example, the popular multi-GPU communication libraries (\textit{e.g.}, NCCL~\cite{nccl} and MPI~\cite{cudaMPI}) only allow initiating the communication routine on the host CPU program after all GPU kernel computation exit. This would 1) induce high overhead for context switching between CPU host and GPU kernel for communication, and 2) idle GPU resources (e.g., SMs) during the kernel computation could not be leveraged for communication purposes, leading to GPU underutilization. Therefore, effective overlapping the communication and computation can largely amortize the overhead and achieve high performance.

\paragraph{Improving the input adaptability of design.}
Existing multi-GPU GNN frameworks~\cite{wang2019dgl,ma2019neugraph} employ static optimizations through a compiler or optimized libraries (\textit{e.g.}, NCCL for communication and cuSPARSE~\cite{cusparse} for computation). However, GNNs input would demonstrate wide diversity in terms of nodes, edges, and embedding sizes, which exposes great opportunities for 1) input-aware workload partition that can well balance the among devices and computing units for better overall utilization, and 2) scheduling the communication and computation by considering the ratio of high-overhead remote neighbor access and low-cost neighbor aggregation for different input graphs.

==> old/ext_04_key_exp_results.tex <==
\section{Key Experimental Results}
% \vspace{-3pt}
% Comprehensive evaluations on the mainstream GNN model architectures across a diverse range of datasets show that 
\Mname~outperforms the state-of-the-art unified virtual memory design (average $3.65\times$ faster) and DGCL design (average $7.38\times$ faster) on multi-GPU platform across different settings. 
%
Our benefits breakdown studies also show that our MGG achieves an average of 21.15\% better SM utilization and an average of 39.20\% higher achieved occupancy and compared with UVM-based design. 
%
Besides, our workload interleaving and shared memory optimization can offer 1.38$\times$ and $3.24\times$ compared with the baseline implementation w/o such an optimization. 
%
In addition, our design analytical modeling and cross-iteration optimization can decrease the execution time up to 70\%. 
% which can improve our design adaptability to confidently and efficiently handle different inputs.

==> old/ext_04_main_artifacts.tex <==
\section{Main Artifacts}
% To this end, we propose, \textbf{\Mname}, an optimization framework for accelerating GNNs on GPU platforms. As shown in Figure~\ref{fig: Overview}, \Mname~integrates PyTorch~\cite{pytorch} as the front-end to improve programmability and ease user implementation. Behind such a  user-friendly programming interface, \Mname~consists of several key components to facilitate GNN optimization and execution on GPUs. First, \Mname~incorporates an input extractor to explore the input-level information that can guide our system-level optimizations. Second, \Mname~utilizes a kernel \& runtime crafter to customize the our parameterized GNN kernel design and CUDA runtime through effective 2D workload management and GNN-specialized memory optimizations.
% We summarize our key contributions as follows.

% \paragraph{Input Analysis of GNN Applications} 
% We explore several types of performance-critical GNN input-level information, (\textit{e.g.}, GNN model architectures and  graph properties), and give in-depth analysis of their importance in guiding our system-level optimizations for GPU-based GNN computing.

% \paragraph{2D Workload Management}
% We propose the first GNN workload abstraction by projecting GNN workload to 2D space with node neighbor and node embedding dimensionality as the base vector. We also introduce a coarse-grained neighbor partitioning strategy to reduce computing imbalance and a fine-grained dimension partitioning approach to improve computing parallelism.

% \paragraph{Specialized Memory Optimization}
% We leverage a set of GPU-based specialized memory optimizations for GNNs to further improve memory performance in two aspects: 1) data locality improvement through community-aware node renumbering, and 2) memory access reduction through block-level memory customization.
In this paper,  we introduce, \textbf{\Mname}, a holistic system design for GNN acceleration on multi-GPU platforms via NVSHMEM~\cite{nvshmem}, as illustrated in Figure~\ref{fig: Overview}. 
%
{NVSHMEM is the latest programmatic communication library for universal inter-GPU communication and synchronization patterns, independent from
the hardware-level interconnects and topologies.
The appearance of NVSHMEM draws much attentions~\cite{wilczek2000qcd,LBANN}, but its current exploration is still preliminary. 
%
We are the first to demonstrate the potential of NVSHMEM in the irregular multi-GPU GNN computation.}
%
The highlight of \Mname~is our novel NVSHMEM-based kernel design, which incorporates an effective pipelining of the high-cost remote neighbor embedding access with the low-overhead local neighbor aggregation in GNN computation. 
%
To further maximize the performance gains, we introduce hierarchical workload management featured with an efficient workload interleaving and warp-based mapping for maximizing GPU utilization while reducing latency. 
%
Furthermore, we introduce a set of tunable design parameters (\textit{e.g.}, the interleaving distance) that make our design highly configurable for achieving better performance.
% To this end, we introduce, \textbf{\Mname}, an efficient and systematic design for GNN acceleration on GPUs.
% %
% As shown in Figure~\ref{fig: Overview}, \Mname~consists of several key components to facilitate the GNN optimization and execution on multi-GPU platform.
% %
% First, \Mname~introduces an input \textit{Data Layout Planner (DLP)} based on the graph input propertities and the GPU inter-connecting topology.
% %
% Second, \Mname~incorporates a \textit{Workload Partitioner (WP)} equipped with a hierarchical GNN workload partitioning scheme for amortizing the computation irregularity at the device and vertex level. WP will first do a coarse-grained categorization of multi-GPU GNN workload, based on whether it will trigger local or remote GPU memory access. 
% Then, within each type of ``raw'' workload, WP will further carry out a fine-grained workload partitioning by grouping neighbors of each vertex. 
% %
% Third, \Mname~integrates a \textit{Kernel Crafter (KC)} with a GNN-tailored share-memory design to improve memory performance, and a highly-efficient warp-based workload mapping strategy based on overlapping the high-overhead memory access and low-cost aggregation computation, to maximize the GPU Stream-Multiprocessor utilization.
% %
% Fourth, \Mname~equips a \textit{Runtime Configuration Tunner (RCT)} to dynamically adjust the configuration parameters during the training of GNNs to optimize its performance based on those collected input and workload propertities during the runtime.





==> old/ext_05_relevance_to_asplos.tex <==
\section{Relevance to ASPLOS Community}
We propose and implement MGG, a novel multi-GPU system design for accelerating GNNs by leveraging NVSHMEM with multi-GPU shared memory and fine-grained communication support. Our work is related to ASPLOS because 1) our key technical contributions, such as hierarchical GNN workload management and NVSHMEM-based GNN kernel design, are system-level innovations to support the emerging multi-GPU GNN computation, and 2) our novel analytical modeling and cross-iteration optimization strategy can comprehensively improve system performance and generality.
